Testing Firm Conduct

Evaluating policy in imperfectly competitive markets requires understanding firm behavior. While researchers test conduct via model selection and assessment, we present advantages of Rivers and Vuong (2002) (RV) model selection under misspecification. However, degeneracy of RV invalidates inference. With a novel definition of weak instruments for testing, we connect degeneracy to instrument strength, derive weak instrument properties of RV, and provide a diagnostic for weak instruments by extending the framework of Stock and Yogo (2005) to model selection. We test vertical conduct (Villas-Boas, 2007) using common instrument sets. Some are weak, providing no power. Strong instruments support manufacturers setting retail prices.

==> Appendices/old/Emipirical.tex <==
\subsection{Data}\label{sec:data}

Our main source of data is the IRI Academic Dataset (see \cite{bkm08} for a description).  This dataset contains weekly price and quantity data for upcs sold in a sample of stores in the United States.  While this is the same data source as in \cite{v07}, it is not the same dataset as it covers a later time period and significantly more geographic markets.  Thus, our aim is not to replicate her findings; instead we seek to use this important empirical setting to illustrate our approach to testing. In cleaning the data, we try to mimic her choices as closely as possible.

Our data is for the year of 2010.\footnote{We choose to use only one year because the IRI dataset does not provide cross-reference for supermarket chains' identity across years and for computational reasons.} We define a market as a retail store-quarter.  We drop data coming from two geographic markets (``EAU CLAIRE'' and ``PITTSFIELD'') for which IRI does not provide geographical location information. We approximate the market size with a measure of the traffic in each store,  derived from the store-level revenue information from IRI. For approximately 5\% of stores, this approximation is poor resulting in an outside share below 50\%.  We drop these from our sample.  

In defining a product, we restrict attention to upcs labelled as ``yogurt'' in the IRI data and focus on the most commonly purchased sizes: 6, 16, 24 and 32oz.\footnote{For example, we drop products labelled ``soy yogurt'' and ``goat yogurt''}  Similar to \cite{v07}, we define a product as a brand-fat content-flavor-size, where flavor takes the value ``Plain'' or ``Other'' and fat content is either light (less than 4.5\% fat content) or whole.\footnote{Given that we lack detailed information for private label products,  we do not add other nutritional information.}  We further standardize package sizes to 6oz serving sizes.

Based on market shares, we exclude niche firms and products from the analysis. In particular, any firm which have less than a 5\% inside share  in all markets is dropped. We also drop products from a market which have an inside share lower than 0.1\% in that market and for which their cumulative inside share is not bigger than 1\%. After cleaning, our dataset has  205,123 observations for 5,034 markets corresponding to  1,309 stores.

We supplement our main dataset with county level demographics obtained from the Census Bureau's PUMS database which we match to the DMAs in the IRI data.  In particular, we draw 1000 households and record household income and age of the head of the household. We exclude households with income lower than \$12k or bigger than \$1 million. The demographic variables are adjusted to reflect their deviation from the mean.

We also measure transportation costs from manufacturer to retailer using average fuel cost times distance.  To do so, we use data on average regional on-highway diesel prices in dollars per gallon by quarter from the US Energy Information Administration.\footnote{https://www.eia.gov/dnav/pet/pet\_pri\_gnd\_dcus\_nus\_w.htm} Manufacturer plant locations were collected by hand.\footnote{We thank Xinrong Zhu for generously sharing this data with us.}
 
 Table \ref{Tab:summarystats} contains summary statistics for the main variables of interest in the paper.  
\begin{table}[!h]\footnotesize\caption{Summary Statistics}\label{Tab:summarystats}\centering
\input{Empirical/Tables/summary_stat}
%\input{Tables/summary_stat_count}
\end{table}    

\subsection{Demand Model, Identification, and Estimation}

\noindent \textbf{Demand Model:}
We begin by describing our model of demand which follows a standard framework from  \cite{blp95}, as in \cite{v07}.  Each consumer $i$ receives utility from purchasing product $j$ in market $t$ according to the following utility index:
\begin{align}\label{eq:utility}
    u_{ijt} = \beta_i x_j + \alpha_i p_{jt} + \xi_{t} + \xi_{s} + \xi_{b(j)} + \xi_{jt} + \epsilon_{ijt} 
\end{align}
where $x_j$ includes a set of product characteristics: package size and dummy variables for whether the yogurt is low fat and for whether it is plain flavored. We also include the log of the number of flavors offered in the market, following \cite{ar05}. $p_{jt}$ represents the price charged for product $j$ in market $t$.   
All specifications have fixed effects for quarter, store and brand producing product $j$, denoted $\xi_{t}$, $\xi_{s}$, and $\xi_{b(j)}$ respectively.  $\xi_{jt}$ and $\epsilon_{ijt}$ denotes unobservable shocks at the product-market and the individual product market level, respectively.  Finally, we allow consumer preferences for characteristics $\beta_i$ and price $\alpha_i$ to vary across individuals. As in \cite{v07}, we do so by interacting their mean with individual level demographics for income and age of the head of household so that
\begin{align}
    \alpha_i &= \bar\alpha + \tilde\alpha\times D_i\\
    \beta_i &= \bar\beta + \tilde\beta\times D_i
\end{align}    
where $\bar\alpha$ and $\bar\beta$ represent the mean taste across consumers and $D_i$ denotes demographics.


To close the model of demand, we make additional assumptions which are standard in the literature.  In particular, we normalize the utility consumer $i$ receives from consuming the outside option as $u_{i0t} = \epsilon_{i0t}$.  The idiosyncratic errors $\epsilon_{jt}$ and $\epsilon_{i0t}$ are assumed to be distributed i.i.d. Type I extreme value. Under the assumption that each consumer purchases one unit of the good that gives her the highest utility, including the outside good, the market share of product $j$ in market $t$ takes the following form:      
\begin{equation}\label{eq:shares}
s_{jt} = \int \frac{\exp({\beta_{i}x_{j}  + \alpha_i p_{jt} +\xi_{t} + \xi_{s} + \xi_{b(j)}  + \xi_{jt}})}{1 +\sum_{l\in{\mathcal{J}_{t}}} \exp({\beta_{i}x_{l}  + \alpha_i p_{lt} +\xi_{t} + \xi_{s} + \xi_{b(l)}  + \xi_{lt}})}f(\alpha_i,\beta_i) \text{d}\alpha_i\text{d}\beta_i
\end{equation}

\noindent \textbf{Identification and Estimation:}   Demand estimation and testing can either be performed \textit{sequentially}, in which demand estimation is a preliminary step, or \textit{simultaneously} by stacking the demand and supply moments.  Following \cite{v07}, we adopt a sequential approach.  For the purposes of illustrating the empirical relevance of the findings in Sections 4 and 5, the computationally simpler simultaneous approach is sufficient.  We estimate demand following the approach developed in \cite{blp95}.  Including brand, store, and quarter fixed effects in (\ref{eq:utility}) controls for all unobservables that are constant either within a brand, a store, or a quarter. Thus, the source of endogeneity which threatens identification is limited to the set of unobservables that vary across these dimensions, denoted as $\xi_{jt}$.  
As prices and shares may be correlated with  $\xi_{jt}$, instruments are then required to identify the coefficient on price $\alpha_i$ and parameters for the individual specific components of utility, $\tilde\alpha$ and $\tilde\beta$, as these latter parameters enter the model non-linearly.    

We use a standard set of instruments.  For each brand in each market, we interact the average highway fuel cost for the region of the country where that market is located with the distance from the store to the brand's nearest manufacturing plant.  As we lack information on plant location for some products, including private labels, we interact the unobserved vector of fuel costs for all observations with a dummy indicating that plant location is observed.  This cost shifter provides exogenous variation to identify the coefficient on price, $\alpha$. 

The non-linear parameters are identified using instrumental variables proposed in \cite{gh19}.  For the nonlinear price parameters on demographics $\tilde\alpha$, we interact the fuel cost instrument with the mean of the demographics for the DMA in which the market is located. For $\tilde\beta$, we interact the observed characteristics with the mean of the demographics for the DMA in which the market is located.  Under the timing assumptions of the model, \cite{gh19} demonstrate that this interaction provides exogenous cross-sectional variation to identify the parameters of interest.  

Estimation proceeds via GMM.     For each guess of the non-linear parameters, we employ the contraction presented in \cite{blp95} to recover the mean utility of each product in each market.  We then regress the mean utilities on price and a set of dummy variables for the fixed effects via two-stage least squares and recover the unobserved product market unobservables as residuals.  We then interact these residuals with the instruments to form the sample moments which enter the GMM objective function. The GMM procedure recovers estimates of the nonlinear parameters, $\tilde\alpha$ and $\tilde\beta$, as well as the price coefficient, $\alpha$, and the fixed effects.  We compute demand estimates using the PyBLP package developed in \cite{cg19}.\footnote{We refer to PyBLP documentation website https://pyblp.readthedocs.io/en/stable/index.html# for detailed information of the methods used.}.


\noindent \textbf{Results:} Results for demand estimation are reported in Table \ref{Tab:demand}.  As a reference, we report estimates of a standard logit model of demand in Columns 1 and 2.  In Column 1, the logit model is estimated via OLS while in Column 2, we use fuel cost as an instrument for price and estimate the model via 2SLS.  We see a large reduction in the price coefficient, indicative of endogenity not controlled for by the fixed effects.  Columns 3 and 4 report estimates of the full demand model.  Our full demand model generates reasonable elasticities which are comparable to those obtained in \cite{v07} who finds a mean own price elasticity of -5.64.      

\begin{table}[H]\footnotesize
\caption{Demand Estimates}\centering
    \input{Tables/demand_models}\label{Tab:demand}
\end{table}
 \begin{tablenotes}
 \item[] \footnotesize{In the table, we report demand estimates for a logit model of demand obtained from OLS estimation in column 1 and 2SLS  estimation in column 2. Column 3 corresponds to the full BLP model. All specifications have fixed effects for quarter, store and brand and are estimated with 205,123 observations.} 
\end{tablenotes}


%\begin{table}[!h]\footnotesize
%    \centering\caption{Markups Summary Stat}
%    \input{MarkupDescTable}
%\end{table}

%\begin{figure}[!h]
%    \centering\caption{Markups Distribution}
%    \subfloat[IV1]{\includegraphics[scale=0.5]{MarkupFig1.png}}
%    \subfloat[Mixed 2]{\includegraphics[scale=0.5]{MarkupFig2.png}}
    
%    \label{fig:my_label}
%\end{figure}

==> Appendices/old/ManyInstruments.tex <==
\subsection{Many Instruments for Testing: Bias of RV}\label{sec:manyinstr} 

The RV test fundamentally depends on predicting markups from the instruments.  When the first stage is viewed in this light, one may consider adding a large number of instruments in order to improve the predictions.  In light of Proposition \ref{prop:degen}, there may be benefits to doing so in the context of RV.  However, this comes at a cost.  The econometrics literature has discussed the problem of many instruments in an estimation context.  Specifically  \cite{b94} and \cite{cs05} show that the 2SLS estimator is inconsistent under a many instruments asymptotic.  More troubling, this asymptotic has been found to approximate well the finite sample distribution of the estimator, thus revealing substantial bias towards the OLS estimator.  The intuition, discussed in \cite{ad09} is that increasing the number of instruments overfits the endogenous variable.  In the extreme, one predicts the endogenous variable perfectly and thus reverts to OLS in the second stage.  

We show that the use of many instruments has a similar impact on the RV test that it does in 2SLS.  We first establish the analogue of OLS in testing.  Consider alternative moments
$g^{OLS}_m = \frac{\Delta'\hat\omega_m}{n}$,
which are the moments one would use to estimate Equation (\ref{eq:test}) by OLS. We define a measure of fit using these moments as $Q_m^{OLS} = g^{OLS\prime}_m(\frac{\Delta'\Delta}{n})^{-1} g^{OLS}_m$. Now we can define a version of the RV test statistic with the OLS moments: $T^{OLS} = \frac{\sqrt{n}}{\hat  \sigma_{RSS}} (Q_1^{OLS} - Q_2^{OLS}).$
As shown in Appendix XX, this test is inconsistent and has a plim given by:
$$\frac{T^{OLS}}{\sqrt{n}} &\rightarrow_p  \frac{E[(\Delta^{OLS}_i -\Delta_{1i})^2 - (\Delta^{OLS}_i -\Delta_{2i})^2]	}{\sigma_{OLS}}$$
This shows that OLS-based tests asymptotically reject in favor of the model for which the implied markups are closer to the OLS markups. Since $\Delta$ is generally correlated with $\omega$, $\Delta^{OLS}$ may be very far from $\Delta_0$.  While $T^{OLS}$ may seem artificial, we show in Appendix XX that it is equivalent to an implementation of the RV test based on residual sum of squares (RSS) which has been popular in the applied IO literature.\footnote{For example, \cite{b87}, \cite{glv92}, \cite{bd10} and \cite{bdvk13} use RSS-based procedures to test hypotheses on conduct.} 



Now, to formalize the bias of many instruments, 
we consider a many instrument asymptotic, following \cite{b94} and \cite{cs05}.   Specifically, letting $\Gamma = [\Gamma_1, \Gamma_2]$, we assume the following:

\begin{assumption}\label{as:manyinstr} Let the number of instruments grow at rate $n$ so that $\frac{d_z}{n} \rightarrow_p \delta_z > 0$.  Moreover, suppose:
(i) $\frac{\hat\Gamma'z'z\hat\Gamma}{n}\rightarrow H_1 + o_p(1)$ and (ii) $\frac{\hat\Gamma'z'z\hat\Gamma_0}{n}\rightarrow H_2 + o_p(1)$ for some matrices $H_1,H_2>0$.
\end{assumption}
The above assumption maintains that  the concentration parameters $\frac{\Gamma'z'z\Gamma}{n}$ and $\frac{\Gamma'z'z\Gamma_0}{n}$ are non-diverging as the number of instruments grows.  Thus, the variance of the predicted markups remains finite. One way to interpret this assumption is that additional instruments are eventually uninformative in predicting markups. Regardless of the interpretation, the econometrics literature has found that the asymptotic distribution obtained with this assumption is a good approximation of the finite sample performance even if $d_z$ is small (see \cite{b94} and \cite{ak95}).\looseness=-1


Under Assumption \ref{as:manyinstr}, we can characterize the behavior of the RV test statistic in a many instrument setting.  Specifically, we derive the following result:
\begin{proposition}\label{prop:biasmany} Suppose that Assumptions \ref{as:momcond}, \ref{as:regcond}, and \ref{as:manyinstr} are satisfied. Then:
\begin{align*}
    \frac{T^{RV}}{\sqrt{n}} \rightarrow_p 
    & \frac{1-\delta_z}{\sigma_{RV}}
    \bigg(E[(\Delta^z_{1i}-\Delta^z_{0i})^2] - E[(\Delta^z_{2i}-\Delta^z_{0i})^2]\bigg)
    \\&\qquad +\frac{\delta_z}{\sigma_{RV}}\bigg(E[(\Delta_{1i}-\Delta^{OLS}_i)^2] - E[(\Delta_{2i}-\Delta^{OLS}_i)^2]\bigg)
\end{align*}

\end{proposition}

Proposition \ref{prop:biasmany} sheds light on important aspects of testing with many instruments. In estimation, the presence of many instruments biases 2SLS estimates to their OLS counterpart.  Likewise, we see that the RV test is biased towards the RSS test discussed in Section \ref{sec:RSS}, which forms the moments with the endogenous markups.  The extent of the bias depends on the magnitude of $\delta_z$.  \cite{h20} states that although there is no set rule of thumb, many instruments are a serious concern whenever the number of instruments exceeds 5\% of the sample size. However, many instruments can still create significant bias below that threshold.  In fact, \cite{ak95} find severe bias in a setting where  $\frac{d_z}{n}$ is as small as 0.005.  


Thus, a researcher should be concerned when using many instruments \textit{even if they are valid}.  While valid instruments implement the condition in Lemma 1, there is no guarantee that using them to form the RV test will allow one to  achieving correct inference either in finite sample or asymptotically.  We return to the problem of many instruments in Section \ref{sec:sieveIJIVE} and propose a modification of the RV test statistic which removes the finite sample bias that they cause.

==> Appendices/old/SimSeqDemand.tex <==

Consider a setting where testing is performed in a GMM environment and the supply moments for a model of conduct $m$ are $g_m\left(\theta^{D}\right) = \frac{1}{n}z'(p-\Delta_m(\theta^{D}))$.  The supply moments depend on demand parameters $\theta^D$ through markups $\Delta_m=\Delta_m(\theta^D)$. Demand moments are $
 h\left(\theta^{D}\right) = \frac{1}{n}\textbf{z}^{D\prime}\boldsymbol{\xi}(\theta^{D})$,
where $\boldsymbol{\xi}(\theta^{D})$ is the value of the demand unobservable implied by $\theta^D$, and $\textbf{z}^{D}$ is a vector of demand instruments.\footnote{Demand moments could include micro-moments; our discussion in this section would still apply.} We assume that the dimension of $\textbf{z}^D$ is sufficient to identify $\theta^{D}$ from demand moments alone. \looseness=-1  

We define plim of the demand parameters obtained from sequential estimation as:
\begin{align*}
    \theta^{Dseq} = \arg\min_{\theta^D} \mathcal{Q}^D(\theta^D),
\end{align*}
where $\mathcal{Q}^D=plim(h(\theta^{D})'W^{D}h(\theta^{D}))$ and $W^{D} = (\frac{\textbf{z}^{D\prime}\textbf{z}^D}{n})^{-1}$. We construct the RV test statistic  in a second step  from a measure of fit based on supply moments.   The asymptotic value of the measure of fit for each model $m$ is:
\[
\mathcal{Q}_{m}(\theta^{Dseq})=\mathcal{g}_m(\theta^{Dseq})'W\mathcal{g}_m(\theta^{Dseq}).
\]



Alternatively, we could use the supply moments to estimate demand. Stacking the demand and supply moments, the simultaneous GMM objective function is:
\begin{align*}
Q_m^{sim}(\theta^D) = (g_m(\theta^D)',h(\theta^D)')W^{sim}(g_m(\theta^D)',h(\theta^D)')'
\end{align*}
%\begin{align*}
%Q_m^{sim}(\theta^D) & =\left[\begin{array}{c}
%g_m(\theta^D)\\
%h(\theta^D)
%\end{array}\right]^{\prime}W^{sim}\left[\begin{array}{c}
%g_m(\theta^D)\\
%h(\theta^D)
%\end{array}\right].
%\end{align*}
We maintain the following assumption on $W^{sim}$ for tractability:
\begin{assumption}\label{as:blockdiag}
    $W^{sim}$ is block diagonal, so that $W^{sim}=diag(W, W^D)$.  
\end{assumption}
\noindent The plim of the demand parameters obtained from simultaneous estimation are: $$\theta_m^{Dsim} = \arg\min_{\theta^{D}} \mathcal{Q}_m(\Delta(\theta^{D})) + \mathcal{Q}^{D}(\theta^{D}).$$ 
\noindent While the value of $\theta_m^{Dsim}$ is model specific, $\theta^{Dseq}$ is not. We now establish the following:
\begin{proposition}\label{prop:demand}
Let Assumption \ref{as:blockdiag} hold, $\textbf{w}$ be correctly specified, $\theta_m^{Dsim}$ be unique, and $\theta^{Dseq}\neq\theta_m^{Dsim}$ for model $m$. Then, $E[(\tilde \Delta_0 - \tilde \Delta_m(\theta_m^{Dsim}))^2] <         E[(\tilde \Delta_0 - \tilde \Delta_m(\theta^{Dseq}))^2]$.\footnote{ If cost shifters $\textbf{w}_a$ are not correctly specified but  Assumption \ref{as:misspmc} holds, then 
        $E[(\tilde \Delta^\textbf{a}_0 - \tilde \Delta_m(\theta_m^{Dsim}))^2] <         E[(\tilde \Delta^\textbf{a}_0 - \tilde \Delta_m(\theta^{Dseq}))^2]
    $
    where $\Delta^\textbf{a}_0=M_{\textbf{w}_a}(\boldsymbol{\Delta}_0+\textbf{w}\tau-\textbf{w}_a\tau_a)$.}
\end{proposition}    
    

The consequences of the proposition  depend on the model of conduct $m$ and the testing environment. Suppose $m=1$ is the true model and there is no misspecification.  Then $\theta^{Dseq}=\theta_1^{Dsim}$, and $ E[(\tilde \Delta_0 - \tilde \Delta_1(\theta_1^{Dsim}))^2] =         E[(\tilde \Delta_0 - \tilde \Delta_1(\theta^{Dseq}))^2] = 0.$   It follows that  $\mathcal{Q}_1 - \mathcal{Q}_2$ is smaller in magnitude under simultaneous estimation.  Instead, when demand is misspecified, the proposition implies that $B$ is smaller with a simultaneous approach. However, predicted markups for $m=2$ also get closer to the true ones.
Thus, a simultaneous approach provides a (weakly) better fit for both models. If the researcher assumes that the testing environment has low misspecification  and has a large dataset, a simultaneous approach may change the sign for the RV statistic and cause the researcher to conclude for a wrong model. However, if misspecification is severe or if the dataset is small, a simultaneous approach may offer advantages by improving the fit of a true model. We summarize these findings as follows:
\begin{corollary}\label{cor:demand}
Let Assumption \ref{as:blockdiag} hold, $\theta_m^{Dsim}$ be unique, and $\theta^{Dseq}\neq\theta_m^{Dsim}$ for model $m$. 
\begin{itemize}
    \item[(i)] Without misspecification, the plim of the RV numerator is smaller in magnitude under simultaneous estimation, but has the same sign as under sequential estimation.
    \item[(ii)]  With misspecification, the sign and magnitude of plim of the RV numerator could differ under simultaneous and sequential estimation.
\end{itemize}
\end{corollary}

\noindent While we focus on the numerator, the mode of demand estimation will also effect the denominator of $T^{RV}$. This effect on the power of RV is ambiguous even under our simplifying assumptions and we leave it to future research.
 

The demand estimation literature (see \cite{cg19}) has discussed how simultaneous and sequential estimation affect estimates and standard errors for the demand parameters. Our results show that simultaneous estimation does not guarantee demand parameter estimates closer to the true demand parameters. Instead, the supply moments pull the demand parameters towards values which improve the fit of the predicted markups under the assumed conduct model. Moreover, efficiency considerations that apply to estimation do not immediately apply to our setup as one of the models we consider is not correctly specified. \looseness=-1   


==> Appendices/pyRV.tex <==
\begin{figure}[H]
    \centering
    \caption{Code for Demand Estimation and Testing}
    \hspace{-2.5cm}\begin{subfigure}[b]{0.5\textwidth}
          \caption*{\hspace{-1.5cm}Panel A. Demand Estimation Code}
         \includegraphics[scale=0.3, trim={.1cm 0 0 0}, clip]{Figures/pyBLP_problem1.png}\\
\includegraphics[scale=0.3, trim={.1cm 0 0 0}, clip]{Figures/pyBLP_problem2.png}\\
\vspace{1.75cm}
     \end{subfigure}
     \hspace{-1cm}\begin{subfigure}[b]{0.4\textwidth}
        
         \caption*{\hspace{1.5cm}Panel B. Testing Code}
         \includegraphics[scale=0.3]{Figures/pyRV_problem.png}
     \end{subfigure}
    
\subcaption*{Panel A and B respectively report the definition of the demand estimation problem in \texttt{PyBLP} and the testing problem in \texttt{pyRV}. }
\end{figure}

==> Empirical/Robustness/TablesGraphs/ARStat_logit.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
\cline{2-5}1. Zero wholesale margin&1392.5, 1173.7&1392.5, 1432.8&1392.5, 1432.7&1392.5, 1363.4\\
2.Zero retail margin&&1173.7, 1432.8&1173.7, 1432.7&1173.7, 1363.4\\
3.Simple linear pricing&&&1432.8, 1432.7&1432.8, 1363.4\\
4.Hybrid model&&&&1432.7, 1363.4\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/ARStat_nestedlogit.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
\cline{2-5}1. Zero wholesale margin&396.4, 1218.1&396.4, 1124.7&396.4, 1122.5&396.4, 351.4\\
2.Zero retail margin&&1218.1, 1124.7&1218.1, 1122.5&1218.1, 351.4\\
3.Simple linear pricing&&&1124.7, 1122.5&1124.7, 351.4\\
4.Hybrid model&&&&1122.5, 351.4\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/CostTable.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lccccccc}
\toprule
& Median& S.D.& Min& q10& q90& Max& \%$<0$ \\
\cline{2-8}Zero wholesale margin&0.4201&0.2312&-0.2602&2.1317&0.2309&0.7728&0.0400\\
Zero retail margin&0.5460&0.2605&0.0856&2.4372&0.3549&0.9569&0.0000\\
Simple linear pricing&0.3050&0.2150&-0.4023&1.9102&0.1241&0.6353&0.8600\\
Hybrid model&0.3102&0.2088&-0.2602&1.9102&0.1460&0.6361&0.5000\\
Wholesale collusion&0.1053&0.2546&-2.1383&1.5322&-0.1956&0.4335&31.6900\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/Fstat_logit_blp.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&906.3&427.1&428.3&174.6\\
2.Zero retail margin&&422.6&422.6&348.5\\
3.Simple linear pricing&&&556.8&534.1\\
4.Hybrid model&&&&534.1\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/Fstat_logit_diff.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&6.2&7.4&7.4&4.3\\
2.Zero retail margin&&5.7&5.7&4.5\\
3.Simple linear pricing&&&5.6&3.8\\
4.Hybrid model&&&&3.8\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/Fstat_nestedlogit_blp.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&281.2&263.3&271.2&16.2\\
2.Zero retail margin&&186.7&192.3&69.3\\
3.Simple linear pricing&&&248.4&99.5\\
4.Hybrid model&&&&98.7\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/Fstat_nestedlogit_diff.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&5.3&6.7&6.7&2.8\\
2.Zero retail margin&&4.6&4.6&3.0\\
3.Simple linear pricing&&&4.7&2.4\\
4.Hybrid model&&&&2.4\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/MkupTable.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccccc}
\toprule
& Median& S.D.& Min& q10& q90& Max \\
\cline{2-7}Zero wholesale margin&37.6&10.7&13.6&27.4&53.3&169.9\\
Zero retail margin&19.7&4.3&8.3&14.7&25.7&53.9\\
Simple linear pricing&54.3&13.8&14.1&41.2&74.7&208.0\\
Hybrid model&52.7&13.0&14.1&40.1&71.9&178.2\\
Wholesale collusion&84.4&34.1&20.3&56.2&134.8&674.0\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/RVstat_logit_blp.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1.Zero wholesale margin&14.76&-17.16&-17.15&-18.04&0.00\\
2.Zero retail margin&&-18.32&-18.32&-18.16&1.00\\
3.Simple linear pricing&&&7.33&-17.94&0.00\\
4.Hybrid model&&&&-17.94&0.00\\
5.Wholesale collusion&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/RVstat_logit_diff.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1.Zero wholesale margin&2.28&2.41&2.41&-1.75&0.06\\
2.Zero retail margin&&-0.76&-0.77&-1.87&1.00\\
3.Simple linear pricing&&&-0.10&-2.13&0.46\\
4.Hybrid model&&&&-2.13&0.45\\
5.Wholesale collusion&&&&&0.06\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/RVstat_nestedlogit_blp.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1.Zero wholesale margin&3.10&-17.12&-17.15&-9.26&0.00\\
2.Zero retail margin&&-11.41&-11.42&-8.58&1.00\\
3.Simple linear pricing&&&3.65&-7.97&0.00\\
4.Hybrid model&&&&-7.97&0.00\\
5.Wholesale collusion&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/RVstat_nestedlogit_diff.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1.Zero wholesale margin&1.93&2.33&2.28&-1.41&0.12\\
2.Zero retail margin&&-0.62&-0.64&-1.52&1.00\\
3.Simple linear pricing&&&-0.25&-1.68&0.54\\
4.Hybrid model&&&&-1.68&0.53\\
5.Wholesale collusion&&&&&0.12\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/VarPredDelta.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lccccc}
\toprule
Instrument& $\Delta^z_1$& $\Delta^z_2$& $\Delta^z_3$& $\Delta^z_4$& $\Delta^z_5$ \\
\cline{1-6}BLP&2.02e-04&6.26e-05&2.84e-04&2.85e-04&2.51e-03\\
DIFF&2.79e-07&2.00e-07&7.01e-07&6.90e-07&1.61e-06\\
pcaBLP&1.15e-04&5.68e-05&1.84e-04&1.85e-04&1.53e-03\\
pcaDIFF&1.52e-07&1.29e-07&4.38e-07&4.29e-07&1.02e-06\\
blpcs&1.42e-04&1.81e-05&1.61e-04&1.64e-04&1.87e-03\\
diffcs&2.08e-07&1.98e-08&1.71e-07&1.66e-07&8.53e-07\\
blpcsavg&5.76e-05&5.04e-07&6.27e-05&6.42e-05&7.41e-04\\
M&4.57e-05&2.15e-06&3.67e-05&3.73e-05&9.14e-04\\
blp\_const&1.11e-04&5.36e-05&1.94e-04&1.94e-04&1.51e-03\\
Xiblp&1.23e-04&2.48e-05&1.54e-04&1.54e-04&1.89e-03\\
nfirms\_mkt&8.06e-05&1.57e-06&7.21e-05&7.40e-05&8.69e-04\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_BLP.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&76.5&18.1&18.0&79.5\\
2&&26.8&26.8&76.4\\
3&&&23.3&44.9\\
4&&&&45.0\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_DIFF.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&4.0&1.8&1.8&2.7\\
2&&1.7&1.7&3.0\\
3&&&0.9&1.8\\
4&&&&1.8\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_M.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&13.2&31.8&32.4&61.1\\
2&&66.2&66.2&40.9\\
3&&&47.0&32.8\\
4&&&&32.8\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_Xiblp.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&33.3&12.5&12.5&105.3\\
2&&10.1&10.4&82.4\\
3&&&10.0&33.9\\
4&&&&33.1\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_blp_const.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&63.6&28.0&28.0&91.3\\
2&&37.8&37.9&78.5\\
3&&&50.1&29.3\\
4&&&&29.1\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_blpcs.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&63.3&17.0&17.0&103.0\\
2&&40.2&40.9&85.1\\
3&&&33.8&26.2\\
4&&&&26.2\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_blpcs1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&105.7&0.2&0.2&118.6\\
2&&12.1&13.0&123.5\\
3&&&8.8&21.8\\
4&&&&22.4\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_blpcs2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&69.1&24.2&24.1&97.1\\
2&&35.1&35.2&84.8\\
3&&&45.7&31.1\\
4&&&&30.9\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_blpcs3.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&100.9&0.6&0.6&107.0\\
2&&10.3&10.9&113.0\\
3&&&8.8&26.9\\
4&&&&27.3\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_blpcs4.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&67.7&21.9&21.8&92.2\\
2&&30.6&30.7&81.3\\
3&&&37.6&34.3\\
4&&&&34.1\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_blpcsavg.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&68.6&1.1&1.3&131.6\\
2&&44.8&47.0&112.9\\
3&&&5.2&33.7\\
4&&&&34.6\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_blpcsavg1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&68.6&1.1&1.3&131.6\\
2&&44.8&47.0&112.9\\
3&&&5.2&33.7\\
4&&&&34.6\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_blpcsavg2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&67.0&23.9&23.8&96.4\\
2&&34.7&34.9&83.4\\
3&&&44.4&29.7\\
4&&&&29.5\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_blpcsavg3.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&63.6&1.0&1.1&109.7\\
2&&18.4&19.0&96.6\\
3&&&5.2&34.2\\
4&&&&34.7\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_blpcsavg4.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&65.7&21.5&21.5&91.7\\
2&&30.1&30.2&80.1\\
3&&&36.3&33.1\\
4&&&&33.0\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_blpdiff.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&65.0&23.6&23.5&85.8\\
2&&31.2&31.3&75.5\\
3&&&40.1&31.6\\
4&&&&31.4\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_diffcs.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&12.1&3.8&3.8&4.8\\
2&&7.1&7.0&8.1\\
3&&&1.8&2.8\\
4&&&&2.8\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_diffcs1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&20.2&3.8&3.8&6.9\\
2&&9.2&9.1&13.0\\
3&&&1.3&2.1\\
4&&&&2.1\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_diffcs2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&66.2&25.9&25.8&89.7\\
2&&35.7&35.8&78.3\\
3&&&49.4&27.8\\
4&&&&27.6\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_diffcs3.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&8.4&2.7&2.6&4.2\\
2&&3.2&3.2&5.8\\
3&&&1.2&2.3\\
4&&&&2.3\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_diffcs4.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&64.8&23.2&23.1&84.9\\
2&&30.5&30.6&74.9\\
3&&&39.0&32.2\\
4&&&&32.0\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_nfirms_mkt.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&127.5&0.0&0.0&175.9\\
2&&30.2&31.8&166.9\\
3&&&17.8&35.4\\
4&&&&35.9\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_pcaBLP.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&66.4&26.3&26.2&90.7\\
2&&36.4&36.6&79.0\\
3&&&50.8&27.2\\
4&&&&26.9\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_pcaBLPpcaDIFF.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&65.0&23.6&23.5&85.8\\
2&&31.2&31.3&75.5\\
3&&&40.1&31.6\\
4&&&&31.4\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robFstat_pcaDIFF.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1&5.7&2.5&2.5&3.7\\
2&&2.2&2.2&4.3\\
3&&&1.0&2.5\\
4&&&&2.5\\
5&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_BLP.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&-0.25&-3.30&-3.35&-4.81&1.00\\
2&&-1.22&-1.22&-3.66&0.81\\
3&&&-1.07&-4.19&0.26\\
4&&&&-4.20&0.26\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_DIFF.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&0.56&0.37&0.36&-1.04&0.76\\
2&&0.29&0.28&-0.95&0.77\\
3&&&-1.42&-0.74&1.00\\
4&&&&-0.74&0.77\\
5&&&&&0.59\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_M.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&4.13&0.96&0.90&-6.27&0.00\\
2&&-5.94&-5.94&-5.98&1.00\\
3&&&-5.62&-5.96&0.00\\
4&&&&-5.96&0.00\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_Xiblp.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&1.64&0.38&0.37&-5.29&0.23\\
2&&-1.78&-1.83&-4.50&1.00\\
3&&&-0.91&-4.26&0.23\\
4&&&&-4.27&0.23\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_blp_const.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&0.52&-5.33&-5.36&-5.40&0.61\\
2&&-3.11&-3.10&-4.23&1.00\\
3&&&-0.25&-4.49&0.02\\
4&&&&-4.50&0.02\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_blpcs.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&0.46&-3.60&-3.69&-4.97&0.65\\
2&&-1.61&-1.60&-3.96&1.00\\
3&&&-0.73&-4.49&0.20\\
4&&&&-4.49&0.20\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_blpcs1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&-0.60&0.65&0.63&-4.28&0.52\\
2&&1.24&1.21&-2.95&0.42\\
3&&&-1.10&-3.90&1.00\\
4&&&&-3.91&0.52\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_blpcs2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&0.31&-3.53&-3.54&-5.12&0.76\\
2&&-2.37&-2.36&-3.99&1.00\\
3&&&0.94&-4.34&0.10\\
4&&&&-4.35&0.10\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_blpcs3.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&-0.59&0.63&0.62&-4.28&0.53\\
2&&1.29&1.26&-2.95&0.41\\
3&&&-1.12&-3.88&1.00\\
4&&&&-3.89&0.53\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_blpcs4.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&0.31&-3.39&-3.40&-5.12&0.76\\
2&&-2.40&-2.38&-3.98&1.00\\
3&&&0.90&-4.33&0.10\\
4&&&&-4.34&0.10\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_blpcsavg.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&-0.76&-0.33&-0.46&-4.06&1.00\\
2&&0.82&0.80&-3.01&0.45\\
3&&&-1.33&-3.94&0.75\\
4&&&&-3.95&0.67\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_blpcsavg1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&-0.76&-0.33&-0.46&-4.06&1.00\\
2&&0.82&0.80&-3.01&0.45\\
3&&&-1.33&-3.94&0.75\\
4&&&&-3.95&0.67\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_blpcsavg2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&0.37&-3.63&-3.64&-5.14&0.71\\
2&&-2.47&-2.46&-4.02&1.00\\
3&&&0.29&-4.36&0.09\\
4&&&&-4.37&0.09\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_blpcsavg3.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&-0.75&-0.11&-0.20&-4.06&1.00\\
2&&0.89&0.86&-3.01&0.45\\
3&&&-1.38&-3.90&0.91\\
4&&&&-3.91&0.86\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_blpcsavg4.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&0.37&-3.48&-3.49&-5.14&0.71\\
2&&-2.50&-2.48&-4.02&1.00\\
3&&&0.24&-4.35&0.09\\
4&&&&-4.36&0.09\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_blpdiff.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&0.65&-3.33&-3.33&-5.37&0.51\\
2&&-3.21&-3.20&-4.24&1.00\\
3&&&0.11&-4.46&0.04\\
4&&&&-4.47&0.04\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_diffcs.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&-2.90&-0.05&-0.07&1.07&0.72\\
2&&1.13&1.09&1.99&0.19\\
3&&&-1.11&0.56&0.72\\
4&&&&0.57&0.70\\
5&&&&&1.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_diffcs1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&-3.18&-0.22&-0.24&2.33&0.37\\
2&&1.12&1.09&2.87&0.06\\
3&&&-0.97&1.01&0.37\\
4&&&&1.01&0.37\\
5&&&&&1.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_diffcs2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&0.64&-3.42&-3.43&-5.37&0.52\\
2&&-3.18&-3.17&-4.24&1.00\\
3&&&0.14&-4.47&0.04\\
4&&&&-4.47&0.04\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_diffcs3.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&-1.48&0.22&0.21&-0.50&0.82\\
2&&0.45&0.44&0.11&0.82\\
3&&&-1.28&-0.38&1.00\\
4&&&&-0.37&0.82\\
5&&&&&0.82\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_diffcs4.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&0.64&-3.29&-3.29&-5.37&0.52\\
2&&-3.22&-3.21&-4.24&1.00\\
3&&&0.08&-4.46&0.04\\
4&&&&-4.46&0.04\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_nfirms_mkt.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&-1.94&0.14&0.13&-3.45&0.90\\
2&&2.10&2.09&-2.09&0.05\\
3&&&-0.19&-3.37&1.00\\
4&&&&-3.38&0.90\\
5&&&&&0.01\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_pcaBLP.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&0.65&-3.46&-3.47&-5.37&0.51\\
2&&-3.17&-3.16&-4.25&1.00\\
3&&&0.17&-4.48&0.04\\
4&&&&-4.48&0.04\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_pcaBLPpcaDIFF.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&0.65&-3.33&-3.33&-5.37&0.51\\
2&&-3.21&-3.20&-4.24&1.00\\
3&&&0.11&-4.46&0.04\\
4&&&&-4.47&0.04\\
5&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Robustness/TablesGraphs/robRVstat_pcaDIFF.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1&0.77&0.40&0.39&-1.05&0.74\\
2&&0.28&0.28&-1.02&0.78\\
3&&&-1.19&-0.81&1.00\\
4&&&&-0.81&0.78\\
5&&&&&0.55\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Tables/ARstat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&3407.22, 5324.48&3407.22, 5825.49&3407.22, 5813.52&3407.22, 650.2\\
2.Zero retail margin&&5324.48, 5825.49&5324.48, 5813.52&5324.48, 650.2\\
3.Simple linear pricing&&&5825.49, 5813.52&5825.49, 650.2\\
4.Hybrid model&&&&5813.52, 650.2\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Tables/ARstat2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&9.4, 18.11&9.4, 64.1&9.4, 65.74&9.4, 18.94\\
2.Zero retail margin&&18.11, 64.1&18.11, 65.74&18.11, 18.94\\
3.Simple linear pricing&&&64.1, 65.74&64.1, 18.94\\
4.Hybrid model&&&&65.74, 18.94\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Tables/CostTable.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccccc}
\toprule
& Mean& Median& S.D.& Min& Max& \%$<0$ \\
\cline{2-7}Zero wholesale margin&0.47&0.42&0.23&-0.26&2.13&0.04\\
Zero retail margin&0.61&0.55&0.26&0.09&2.44&0.00\\
Linear pricing&0.35&0.31&0.21&-0.40&1.91&0.86\\
Hybrid model&0.36&0.31&0.21&-0.26&1.91&0.50\\
Wholesale collusion&0.11&0.11&0.25&-2.14&1.53&31.69\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Tables/Coxstat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&-1.37, -2.74&1.32, -7.13&1.39, -7.02&2.54, -5.92\\
2.Zero retail margin&&-0.92, -3.31&-0.93, -3.31&-1.42, -5.38\\
3.Simple linear pricing&&&1.05, -1.09&2.38, -4.92\\
4.Hybrid model&&&&2.4, -4.92\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Tables/Coxstat2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&-0.43, -1.51&0.8, -4.48&0.84, -4.39&0.88, -2.53\\
2.Zero retail margin&&-0.74, -1.2&-0.74, -1.2&-0.99, -2.28\\
3.Simple linear pricing&&&0.16, -0.18&0.82, -2.09\\
4.Hybrid model&&&&0.83, -2.09\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Tables/EBstat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&386.32, 1516.42&378.29, 1819&374.15, 1772.99&89.12, 40.51\\
2.Zero retail margin&&707.84, 1960.33&712.64, 1940.86&1018.38, 3455.57\\
3.Simple linear pricing&&&2365.9, 2351.24&2284.54, 24725.95\\
4.Hybrid model&&&&2225.96, 24319.23\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Tables/EBstat2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&8.68, 79.02&2.58, 12.77&2.53, 12.31&0.42, 0.06\\
2.Zero retail margin&&6.02, 29.45&6.12, 29.51&34.27, 152.76\\
3.Simple linear pricing&&&40.08, 39.14&20.17, 156.71\\
4.Hybrid model&&&&18.82, 156.14\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Tables/Fblp1stat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&3962.3, 739.9&6309, 1042&6173.3, 1043.5&3064.5, 1622.4\\
2.Zero retail margin&&3038.3, 969.4&3070.9, 968.4&3302.8, 1346.3\\
3.Simple linear pricing&&&202, 1305.5&3188.3, 1776.6\\
4.Hybrid model&&&&3169.2, 1779.7\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Tables/Fblp2stat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&12506.2, 1709.6&26318, 3326&25683.1, 3329.2&8299.1, 5660.6\\
2.Zero retail margin&&7859.1, 2805.7&7962.6, 2799.5&9079, 4682.1\\
3.Simple linear pricing&&&660.4, 4568.9&9058.5, 6329\\
4.Hybrid model&&&&8984.8, 6338.6\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Tables/Fdiff1stat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&1.8, 6.7&12, 5.9&11.8, 5.9&1.8, 5.1\\
2.Zero retail margin&&3.2, 5.7&3.1, 5.7&1.8, 5.4\\
3.Simple linear pricing&&&1.5, 5&2, 4.5\\
4.Hybrid model&&&&2, 4.5\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Tables/Fdiff2stat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&1.8, 6.7&12, 5.9&11.8, 5.9&1.8, 5.1\\
2.Zero retail margin&&3.2, 5.7&3.1, 5.7&1.8, 5.4\\
3.Simple linear pricing&&&1.5, 5&2, 4.5\\
4.Hybrid model&&&&2, 4.5\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Tables/MarkupDescTable.tex <==
\begin{tabular}{lrr}
\hline
       &           IV1 &        Mixed 2 \\
\hline
 count & 205123        & 205123         \\
 mean  &      0.250668 &      0.222563  \\
 std   &      0.084924 &      0.0509135 \\
 min   &      0.057056 &      0.0939126 \\
 25\%   &      0.184493 &      0.184744  \\
 50\%   &      0.247817 &      0.217921  \\
 75\%   &      0.308962 &      0.255025  \\
 max   &      0.87463  &      0.621748  \\
\hline
\end{tabular}


==> Empirical/Tables/MixedFstat.tex <==
\begin{tabular}{llr}
\hline
                & Mixed 1   &   Mixed 2 \\
\hline
 prices         & 1295.4    &     656.3 \\
                & 175.3     &     249.6 \\
 income x price & 1849.8    &    1031.6 \\
                & 250.4     &     371.6 \\
 income x light &           &    6749   \\
                &           &   15784.5 \\
 age x light    &           &     967.6 \\
                &           &    2355.2 \\
 age x size     &           &     849.2 \\
                &           &    1303.1 \\
\hline
\end{tabular}


==> Empirical/Tables/MkupTable.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lccccc}
\toprule
& Mean& Median& S.D.& Min& Max \\
\cline{2-6}Zero wholesale margin&39.4&37.6&10.7&13.6&169.9\\
Zero retail margin&20.0&19.7&4.3&8.3&53.9\\
Linear pricing&56.6&54.3&13.8&14.1&208.0\\
Hybrid model&54.8&52.7&13.0&14.1&178.2\\
Wholesale collusion&91.3&84.4&34.1&20.3&674.0\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Tables/RSSstat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&-0.57&1.19&1.19&-5.39\\
2.Zero retail margin&&1.02&0.97&-4.40\\
3.Simple linear pricing&&&-7.17&-3.08\\
4.Hybrid model&&&&-3.08\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Tables/RVstat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1.Zero wholesale margin&-0.25&-3.29&-3.34&-4.80&1.00\\
2.Zero retail margin&&-1.22&-1.22&-3.66&0.81\\
3.Simple linear pricing&&&-1.07&-4.19&0.26\\
4.Hybrid model&&&&-4.19&0.26\\
5.Wholesale collusion&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Tables/RVstat2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1.Zero wholesale margin&0.56&0.37&0.36&-1.04&0.76\\
2.Zero retail margin&&0.29&0.28&-0.96&0.77\\
3.Simple linear pricing&&&-1.41&-0.74&1.00\\
4.Hybrid model&&&&-0.73&0.77\\
5.Wholesale collusion&&&&&0.59\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Tables/RVstat3.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1.Zero wholesale margin&0.65&-3.45&-3.45&-5.37&0.52\\
2.Zero retail margin&&-3.18&-3.17&-4.25&1.00\\
3.Simple linear pricing&&&0.17&-4.47&0.04\\
4.Hybrid model&&&&-4.48&0.04\\
5.Wholesale collusion&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Tables/RVstat4.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc|c}
\toprule
& 2& 3& 4& 5& MCS \\
1.Zero wholesale margin&0.65&-3.44&-3.45&-5.36&0.51\\
2.Zero retail margin&&-3.18&-3.17&-4.24&1.00\\
3.Simple linear pricing&&&0.16&-4.47&0.04\\
4.Hybrid model&&&&-4.47&0.04\\
5.Wholesale collusion&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Empirical/Tables/demand_models.tex <==
\begin{tabular}{lcccc}
\hline
                &  Logit-OLS  &  Logit-2SLS  &   ML1   &   ML2   \\
\hline
 prices         &    -1.75    &    -6.519    & -13.301 & -12.001 \\
                &   (0.019)   &   (0.209)    & (0.94)  & (0.777) \\
 size           &    0.037    &    0.018     &  0.009  &  -0.06  \\
                &    (0.0)    &   (0.001)    & (0.002) & (0.013) \\
 light          &    0.259    &    0.413     &  0.477  &  -0.27  \\
                &   (0.01)    &   (0.014)    & (0.019) & (0.144) \\
 flavor\_Plain   &    0.508    &    0.423     &  0.391  &  0.439  \\
                &   (0.007)   &   (0.009)    & (0.012) & (0.012) \\
 log\_nflavors   &    1.127    &    1.106     &  1.111  &  1.135  \\
                &   (0.004)   &   (0.005)    & (0.006) & (0.007) \\
 income x price &             &              &  4.889  &  4.333  \\
                &             &              & (0.459) & (0.378) \\
 income x light &             &              &         &  0.215  \\
                &             &              &         & (0.069) \\
 age x light    &             &              &         & -0.565  \\
                &             &              &         & (0.113) \\
 age x size     &             &              &         & -0.067  \\
                &             &              &         & (0.008) \\
 Elast mean     &    -1.32    &    -4.917    &  -6.46  & -6.306  \\
 Elast median   &   -1.177    &    -4.384    & -6.307  & -6.187  \\
 J stat         &   2.0e-23   &   1.9e-21    & 1.2e+01 & 2.5e-01 \\
\hline
\end{tabular}


==> Empirical/Tables/summary_stat_count.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Mar 12, 2021 - 03:58:36 PM
\begin{tabular}{@{\extracolsep{5pt}} ccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & N & mean & sd & median & max & min \\ 
\hline \\[-1.8ex] 
Obs & $205,123$ & $$ & $$ & $$ & $$ & $$ \\ 
Stores & $1,309$ & $$ & $$ & $$ & $$ & $$ \\ 
Chains & $93$ & $$ & $$ & $$ & $$ & $$ \\ 
Cities & $48$ & $$ & $$ & $$ & $$ & $$ \\ 
Markets & $5,034$ & $$ & $$ & $$ & $$ & $$ \\ 
Firms & $105$ & $$ & $$ & $$ & $$ & $$ \\ 
Brands (per firm) & $171$ & $2$ & $3$ & $1$ & $20$ & $1$ \\ 
Products (per firm) & $530$ & $5$ & $5$ & $4$ & $52$ & $1$ \\ 
PUMs (per market) & $446,969$ & $9,312$ & $7,695$ & $7,224$ & $42,258$ & $1,747$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 


==> Notes/MonteCarlos.tex <==
%\begin{comment}
\section{Monte Carlo Evidence}\label{sec:montecarlo}

We present in this section Monte Carlo evidence meant to illustrate the performance of the testing procedures discussed previously. We start by describing the setup for the simulation.

\subsection{Setup}

\textbf{Simulation Model - } We generate data from a static model of demand and supply in the class described in Section 2. The demand side follows the standard mixed logit formulation. In market $t$, consumer $i$ chooses among $\mathcal{J}_t=\{1,...,J_t\}$ products with characteristics $(\mathbf{x}_t,\mathbf{p}_t)$ and for which consumer $i$ has an indirect utility of the form
\begin{equation}
U_{ijt}=\mathbf{x}_{jt}\beta+\mathbf{p}_{jt}\alpha +\boldsymbol{\xi}_{jt}+\boldsymbol{\mu}_{ijt}+ \boldsymbol{\varepsilon}_{ijt}
\end{equation}
where $\boldsymbol{\xi}_{jt}$ is an unobserved product-market specific shock to utility common to all consumers and $\boldsymbol{\mu}_{ijt}$ is an individual-specific taste for product attributes given as:
\begin{equation}
\mathbf{\mu}_{ijt} = \mathbf{x}_{jt}\mathbf{\upsilon}_{itx}\sigma_x+\mathbf{p}_{jt}\mathbf{\upsilon}_{itp}\sigma_p \nonumber.
\end{equation}
where $\upsilon_{itx},\upsilon_{itp}\sim N(0,1)$.  Finally, utility depends on an idiosyncratic shock $\mathbf{\varepsilon}_{ijt}$ which is distributed iid $ T1EV$. The parameters governing consumer preferences are $\alpha $, $\beta$ and $\sigma$. For a given value of these parameters, the model implies a matrix $D_{\mathbf{p}_t}\equiv[\partial \mathbf{s}_j/\partial \mathbf{p}_t]$ of partial derivatives of product $j'$s market share with respect to prices. 

On the supply side we consider two candidate models of firm conduct that imply markups $\mathbf{\Delta}_m$: Nash-Bertrand price setting $(B)$ and a collusive model in which firms maximize joint profits $(C)$. As in Section 2, costs are assumed to be the sum of a linear index of the observed cost shifters $\mathbf{w}$ and an unobserved component $\boldsymbol{\omega}$. For the two models we consider, markups are respectively:
\begin{align}
    \mathbf{\Delta}_{Bt} & = (\Omega_{Bt}\odot D_{\mathbf{p}_t})^{-1}\mathbf{s}_{Bt} \\ 
    \mathbf{\Delta}_{Ct} & = (\Omega_{Ct}\odot D_{\mathbf{p}_t})^{-1}\mathbf{s}_{Ct}, 
\end{align}
where $\Omega_{Bt}$ is the ownership matrix in market $t$ where element $(i,j)$ is an indicator that the same firm produces products $i$ and $j$, and $\Omega_{Ct}$ is a $\mathcal{J}_t \times \mathcal{J}_t$ matrix of ones.\\

\noindent \textbf{Parametrization - }  In our baseline, we have $N_m=200$ markets, $N_f=10$ firms and $N_p=40$ products. We first allocate all products to all markets, and then randomly remove 40\% of them, setting a higher probability of removing products from lower market indices. Firm-product pairs are randomly drawn to create an unbalanced ownership structure, where each firm can have at least 2 and at most 22 products. These allocation methods for product-market and firm-product create significant variation in market structure, which is important given the instruments that we use. The vector of product characteristics $\mathbf{x}$ contains a constant and a scalar $\mathbf{x}^{(1)}$. The vector of cost shifters $\mathbf{w}$ includes  $\mathbf{x}$ and a scalar $\mathbf{w}^{(1)}$. Both $\mathbf{x}^{(1)}$ and $\mathbf{w}^{(1)}$ are independently drawn from a standard uniform distribution. In our baseline specification we set the following parameter values:
\begin{align*}
    \text{Preference parameters:}  & \qquad \sigma_x=3, \quad \sigma_p=0.25, \quad \alpha=-1.5, \quad \beta=(-6, 6) \\
    \text{Cost parameters:} & \qquad \tau=(2, 1, 0.2)\\    
    \text{Unobserved shocks:} & \qquad (\boldsymbol{\xi}_{jt},\boldsymbol{\omega}_{jt})\sim N(0,\Sigma), \quad \sigma^2_{\boldsymbol{\xi}}=\sigma^2_{\boldsymbol{\omega}}=0.2\text{ and } \sigma_{\boldsymbol{\xi}\boldsymbol{\omega}}=0.
\end{align*}
Given parameter values, we draw observed $\mathbf{x}^{(1)}$, $\mathbf{w}^{(1)}$, and unobserved shocks for each of the $N_S=100$ simulations and compute endogenous prices and quantities as the solution of the market share equations and first order conditions for each model $m$. The choice of parameter values and distributions create realistic outside shares for the Bertrand DGP, around 0.9.\\

\noindent \textbf{Instruments - } We construct two types of instruments for the Monte Carlo exercise: BLP instruments and differentiation instruments. For product-market $jt$, let $O_{jt}$ be the set of products other than $j$ sold by the firm that produces $j$ and let $R_{jt}$ be the set of products produced by rival firms. The instruments are:
\[\mathbf{z}^{BLP}_{jt}=\left[\begin{matrix} \sum\limits_{k\in O_{jt}} 1[k\in O_{jt}] & \sum\limits_{k\in R_{jt}} 1[k\in R_{jt}] &\sum\limits_{k\in O_{jt}} \mathbf{x}_k & \sum\limits_{k\in R_{jt}} \mathbf{x}_k \end{matrix}\right]\]
\[\mathbf{z}^{Diff}_{jt}=\left[\begin{matrix}\sum\limits_{k\in O_{jt}} \mathbf{d}_{jkt}^2 & \sum\limits_{k\in R_{jt}} \mathbf{d}_{jkt}^2 &\sum\limits_{k\in O_{jt}} 1[|\mathbf{d}_{jkt}|<sd(\mathbf{d})] & \sum\limits_{k\in R_{jt}} 1[|\mathbf{d}_{jkt}|<sd(\mathbf{d})] \end{matrix}\right]\]
where, following \cite{gh19}, $\mathbf{d}_{jkt}\equiv \mathbf{x}^{(1)}_{kt}-  \mathbf{x}^{(1)}_{jt}$ and $sd(\mathbf{d})$ is the standard deviation across the distance vector. In most of the exercises, we use differentiation instruments and exogenous cost-shifters to estimate demand, and BLP instruments to perform supply side estimations.\footnote{In the environment of our simulations, we found that while differentiation instruments work better for the demand side, BLP instruments seem to perform better for supply side estimation. We compare instruments using Angrist-Pischke test statistic for weak instruments.}\\

\noindent \textbf{Implementation - } We construct simulated data and compute demand estimates using the PyBLP package developed in \cite{cg19}. To solve for the equilibrium prices and shares as a fixed point, PyBLP uses the decomposition of the first order conditions in \cite{ms11}. To compute demand estimates, PyBLP uses a nested fixed point algorithm and concentrates out the linear parameters from the two-step GMM minimization process. We use the default method in PyBLP for the fixed point (\textit{simple}) and for the optimization (\textit{l-bfgs-b}) routines, with stopping conditions \textit{1e-12} and \textit{gtol: 1e-5} respectively.\footnote{We refer to PyBLP documentation website https://pyblp.readthedocs.io/en/stable/index.html\# for detailed information of the methods used.} Integration is performed according to a level-9 Gauss Hermite product rule. Testing is performed using MATLAB. We account for the two-step estimation error in the computation of standard errors for all the testing procedures - see Appendix \ref{sect:TwoStep} for details.

\subsection{Comparison between RV Test and RSS Test}

In this subsection we illustrate the importance of constructing moments with valid instruments for testing. In particular, we show that endogeneity leads RSS-based tests to generate misleading conclusions. To emphasize this point, we abstract from demand estimation and use the true demand parameters to form markups for two models of firm behavior: Nash Bertrand and full collusion/joint profit maximization. In turn,  we consider each of these two models as the DGP (in Panels A and B, respectively), and use both as candidate models for testing given the DGP.  We choose different parameters (found in Table \ref{tab:RV_RSS}) to create simulation environments characterized by different amounts of endogeneity. Results for simulation environment (1) in Table \ref{tab:RV_RSS} describe a case where endogeneity is small. For both DGPs, the RSS test and the RV test reject the null in favor of better fit of the correct model in every simulation. 

\begin{table}[h]\centering\caption{Test of Bertrand vs Joint Profit Maximization}
\input{Output/Tab_Comp_rss}\label{tab:RV_RSS}
\begin{tablenotes}
\item[] \footnotesize{This table reports, for each simulation environment and for each hypothesis, the fraction of simulations in which the test either did not reject the null (for $H_0$) or concluded in favor of one alternative (for either $H_m$).}  Panels A and B correspond to Bertrand and joint profit maximization DGPs, respectively. Rows (1), (3) and (4) augment the baseline in the described way.  Unless specified, parameters remain the same as in baseline.
\end{tablenotes}
\end{table}

Next we show that, RSS performs poorly as endogeneity increases. In statistical environment (2) we increase the amount of endogeneity by increasing the value of the demand parameter $\alpha$, which determines consumers price sensitivity. The RV test still concludes in favor of the correct model in almost all simulations for both DGPs.  Instead, in Panel A, the RSS test now concludes in favor of the correct Bertrand model in only 17 percent of simulations. In simulation environment (3), the problems with the RSS test become even more evident. Here we increase the endogeneity of markups by increasing the variance of $\boldsymbol\omega$, and observe that RSS rejects the null in favor of superior fit for joint profit maximization, the wrong model, in 79 percent of simulations. Simulation environment (4) adds additional endogeneity by increasing $\sigma_{\boldsymbol\omega\boldsymbol\xi}$, the covariance of the unobserved demand and cost shocks. While the performance of the RV test is largely unchanged, RSS now rejects the null in favor of the wrong model in 90 percent of the simulations, while never rejecting the null in favor of the correctly specified model. Taken together Panel A shows that in a simple simulation setting, the RSS test is highly susceptible to the degree of endogeneity of markups, and one cannot perform testing without valid instruments.

We then turn to analyze Panel B of Table \ref{tab:RV_RSS}, where the DGP is joint profit maximization. We can see that in all simulation environments, with either strong or weak endogeneity, the RSS test always rejects the null in favor of the correct model of joint profit maximization. It becomes apparent that in this setup, the nature of the bias resulting from endogeneity pushes the RSS test statistic, regardless of the DGP, towards rejecting in favor of joint profit maximization. Thus, while RSS superficially seems to perform well in Panel B, it does so for a reason that undermines the credibility of the test.  

Proposition \ref{prop:RSS} allows us to rationalize the results in Table \ref{tab:RV_RSS}. RSS concludes in favor of the model whose implied markups are asymptotically closer to the markups implied by the OLS estimate of $\theta$. In Figure \ref{fig:markupdistributionOLS} we plot the distribution of markups implied by the OLS estimate of $\theta$. In both the low and high endogeneity simulation environments, the distributions of markups implied by the OLS estimate of the model are quite different from the distributions of markups implied by either the Bertrand or collusive models. In the low endogeneity environment (Panel A of Figure \ref{fig:markupdistributionOLS}), markups implied by the OLS estimate happen to be closer to markups for the true rather than the wrong model.  Thus, the RSS test is able to conclude in favor of the true model.  As endogeneity increases (Panel B of Figure \ref{fig:markupdistributionOLS}), the differences between the distribution of markups implied by the OLS estimate and either candidate model become large in an absolute sense. However, for both DGPs, the nature of the bias in this example is such that the distribution of markups implied by the OLS estimates is closer to the distribution for the collusive model, so the RSS test concludes in favor of the model of collusion.     

\begin{figure}[H]
\captionsetup[subfigure]{labelformat=empty}
\centering \caption{Distribution of Markups implied by $\theta_{OLS}$} \label{fig:markupdistributionOLS}
\footnotesize{Panel A. Table 1 Environment (1) - Low Endogeneity}\\
\subfloat[DGP = Bertrand]{\includegraphics[scale = 0.51]{Graphs/Margins1_table1_model1_B.png}}\qquad
\subfloat[DGP = Collusion]{\includegraphics[scale = 0.51]{Graphs/Margins1_table1_model1_M.png}}\\
\footnotesize{Panel B. Table 1 Environment (4) - High Endogeneity}\\
\subfloat[DGP = Bertrand]{\includegraphics[scale = 0.51]{Graphs/Margins2_table1_model4_B.png}}\qquad
\subfloat[DGP = Collusion]{\includegraphics[scale = 0.51]{Graphs/Margins2_table1_model4_M.png}}\\
\caption*{\footnotesize{This figure compares the distribution of predicted markups at the OLS estimate of $\theta$ to the predicted markups for the Bertrand and Collusive models. Panel A plots the predicted markups for simulation environment (1) in Table \ref{tab:RV_RSS}, a low endogeneity environment, whereas Panel B plots the distribution of predicted markups for simulation environment (4) in Table \ref{tab:RV_RSS}, a high endogeneity environment.  In each panel, the left plot represents the distributions of markups when the true model is Bertrand and the right plot represents the distribution of markups when the true model is joint profit maximization. 
}}
\end{figure}

\subsection{Comparing performance between EB, AR, Cox and RV without misspecification}

Given that we have shown that testing needs to be done with valid moments, we now turn to compare the four testing procedures when the tests are based on such moments. For a realistic comparison of the tests as they would be used in practice, we estimate demand in a first step to compute the markups implied by the two candidate models.\footnote{Hence, all the test statistics need to account for the error coming from the demand estimation. The details on how to compute standard errors in this two-step approach are in Appendix \ref{sect:TwoStep}.} In Table \ref{tab:Tab_Comp_base}, we present the results from comparing the performance of the four testing procedures in the baseline environment. We report in the table the fraction of simulations for which a specific test concludes in favor of an outcome.\footnote{Notice that this statement has different meanings for different testing approaches.  For instance, when RV concludes in favor of $B$ only, it is rejecting the null of equal fit in favor of an alternative of better fit of $B$.  Meanwhile for AR, EB and Cox concluding for $B$ only means not rejecting the null that $B$ is the true model while rejecting the null that $C$ is the true model, pitted against all possible alternatives.} Since all four approaches are designed to account for endogeneity, they perform well in a setting without any misspecification of demand. As we increase the sample size EB, AR, and Cox approach the correct size and RV always rejects the null in favor of the true model.

\begin{table}[H]\centering\caption{Test Comparison - No Misspecification}\label{tab:Tab_Comp_base}
\input{Output/Tab_Comp_base}
  \begin{tablenotes}
 \item[] \footnotesize{This table compares the performance of the four testing procedures: our RV procedure, the auxiliary regression based approach (AR), the estimation based approach (EB), and the Cox approach (Cox), for two models of conduct: Bertrand (DGP $B$) and joint profit maximization (DGP $C$).  Rows correspond to all possible outcomes across these tests. Columns correspond to a particular testing environment applied to data generated by a specific DGP. Panels A and B report results for simulations where the number of markets $N_m$ is set to 200 and 2000 respectively. We report in the table the fraction of simulations for which a specific test concludes in favor of a specific outcome. }
\end{tablenotes}
\end{table}

In Figure \ref{fig:markupdistributionnomis} we plot the distribution of predicted markups implied by the 2SLS estimate of $\theta$ in the setting with no misspecification.  This figure illustrates why all four testing procedures work well in Table \ref{tab:Tab_Comp_base}.  When demand and costs are correctly specified, the predicted markups implied by the 2SLS estimates of $\theta$ very closely match the distribution of predicted markups for the true model.  This approximation improves as the number of markets increases.  As such, all four tests are consistent and have power against the wrong model of conduct.  Thus, without misspecification, tests designed for model selection or model assessment conclude in favor of the true model in almost all simulations with either 200 (Panel A of Figure \ref{fig:markupdistributionnomis}) or 2000 markets (Panel B of Figure \ref{fig:markupdistributionnomis}).      

\begin{figure}[H]
 \captionsetup[subfigure]{labelformat=empty}
 \centering \caption{Distribution of Markups implied by $\hat \theta_{2SLS}$ with No Misspecification of Demand} \label{fig:markupdistributionnomis}
 \footnotesize{Panel A. $N_m = 200$}\\
 \subfloat[DGP = Bertrand]{\includegraphics[scale = 0.51]{Graphs/Margins3_table2_Nm200_B.png}}\qquad
 \subfloat[DGP = Collusion]{\includegraphics[scale = 0.51]{Graphs/Margins3_table2_Nm200_M.png}}\\
 \footnotesize{Panel B. $N_m = 2000$}\\
 \subfloat[DGP = Bertrand]{\includegraphics[scale = 0.51]{Graphs/Margins4_table2_Nm2000_B.png}}\qquad
 \subfloat[DGP = Collusion]{
  \includegraphics[scale = 0.51]{Graphs/Margins4_table2_Nm2000_M.png}}\\
 \caption*{\footnotesize{This figure compares the distribution of predicted markups at the 2SLS estimate of $\theta$ to the predicted markups for the Bertrand and Collusive models. Panel A plots the predicted markups estimated across 200 markets, whereas Panel B plots the distribution of predicted markups estimated across 2000 markets.  In estimating demand and markups, the functional form of demand and cost are correctly specified.  For each panel, the left plot represents the distributions of markups when the true model is Bertrand and the right plot represents the distribution of markups when the true model is joint profit maximization. 
 }}
 \end{figure}

\subsection{Comparing performance between EB, AR, Cox and RV with misspecification}



%We first explore the distinct forces of bias and noise illustrated in Figure \ref{fig:effect_noise} for the four tests. We construct a simple setup under a Bertrand DGP where demand (and hence markups under each model of supply) is not estimated, but bias is generated by altering one specific demand parameter value while holding others fixed at their true values.\footnote{In particular, while the true constant term in the indirect utility of consumers is -6, we alter it to -4.3.} This misspecification of the demand system generates incorrect markups, and hence biases the estimates of the supply-side parameter $\theta$.  For this given level of bias, we also vary the noise.\footnote{We do so by changing at the same time the number of markets $N_m$ and the level of noise in the instruments. We alter the number of markets from 20 to 200 and alter the instruments so that $\mathbf{z} = \mathbf{z}^{BLP} + ((2-n/50)^{1.6})\epsilon$ where $n$ is the number of observations and $\epsilon$ is standard normal noise.} Figure \ref{fig:Tests_MonteC} shows the results of our simulation.   

%\begin{landscape}
%\begin{figure}[H]
%\centering \caption{Effect of Noise on Test Performance in Simulations} \label{fig:Tests_MonteC}
%\includegraphics[scale = 0.55]{Graphs/NB_theta.png}\includegraphics[scale = 0.55]{Graphs/NB_comp.png}\\
%\caption*{\footnotesize{This figure illustrates how the relative performance of the RV, AR, EB and Cox tests depends on noise and bias in Monte Carlo simulations.  The left graph shows estimates of the parameter $\theta_{1}$ - the solid line plots the median estimate in 100 simulations, while the dashed lines plot the respective confidence intervals. Since we draw the figure under the assumption that model 1 is the true model, the true value of $\theta_{1}$ is 1. The right graph plots the seven test statistics associated with the four tests against the critical values. Test statistics are normalized so that all share the same critical values.  
%}}
%\end{figure}

%In the left panel we plot the median estimate of the $\theta$ parameter that multiplies the joint profit maximization markups ($\hat\theta_{1}$) in the EB test setting. We also plot the median value of the confidence interval implied by each estimate. The bias created by the misspecification of demand is evident, and in a low noise environment it causes the true value of 1 to lie outside of the confidence interval for most of the simulations. As we add more noise to the estimation, confidence intervals become wider and eventually the true parameter lies inside the boundaries. However, if noise is large enough, then the value corresponding to the wrong hypothesis also lies inside the confidence interval. Thus noise has different implications for tests based model selection and tests based on hypotheses testing.

%In the right panel, as in Figure \ref{fig:Tests_LowB}, we plot the seven test statistics - these are the test statistic for RV, and statistics for the two different nulls of AR, EB, and Cox - as a function of increasing noise. All seven test statistics decline in absolute value as noise increases. For low noise, RV concludes in favor of the correct hypothesis while AR, EB and Cox reject both. As noise increases, RV becomes inconclusive, while AR, EB and Cox initially conclude for the correct hypothesis, but eventually do not reject either hypothesis. The conclusions one draws from the four tests under bias and noise are qualitatively the same as what was depicted in Figure \ref{fig:Tests_LowB}. Thus, this simulation shows the empirical relevance of Proposition 4.

%While Figure \ref{fig:Tests_MonteC} illustrates the results proved in Section 7, it considers an environment where demand is not estimated and misspecification is introduced by directly choosing parameters of the demand system that depart from true values. To get closer to the challenges encountered by researchers, we conduct Monte Carlo simulations of test performance in a more realistic environments, where demand needs to be estimated and misspecification comes from a wrong choice of functional form for demand. 
We now consider the consequences of demand misspecification by estimating a logit demand system instead of a mixed logit. The misspecification of demand affects the markups used in the implementation of the tests. In Table \ref{tab:Tab_Comp_logit} we see that RV performs better than AR, EB and Cox for both DGPs and for both sample sizes. Compared with the results from Table \ref{tab:Tab_Comp_base}, we see the differential impact of misspecification on the model selection versus the model assessment procedures. 



\begin{table}[H]\centering\caption{Test Comparison - Misspecification}
\input{Output/Tab_Comp_logit}\label{tab:Tab_Comp_logit}
  \begin{tablenotes}
 \item[] \footnotesize{This table compares the performance of the four testing procedures in an environment where demand is misspecified as logit. The true demand model in the DGP is a random coefficient model as in the baseline.  Rows correspond to all possible outcomes across these tests. Columns correspond to a particular testing environment applied to data generated by a specific DGP. Panels A and B report results for simulations where the number of markets $N_m$ is set to 200 and 2000 respectively. We report in the table the fraction of simulations for which a specific test concludes in favor of a specific outcome.}
\end{tablenotes}
\end{table}


For a small sample size as in Panel A, the presence of noise leads the model assessment approaches to conclude in favor of the correct model in a quarter to a half of the simulations. However, if we increase the number of markets, as in Panel B, then EB, AR and Cox reject both alternatives in all simulations. In contrast, in a small number of markets RV rejects in favor of the true model in a vast majority of simulations, and as the number of markets increases, it does so in all simulations.

 

\begin{figure}[H]
\captionsetup[subfigure]{labelformat=empty}
\centering \caption{Distribution of Markups implied by $\hat \theta_{2SLS}$ with Misspecification of Demand} \label{fig:markupdistributionmis}
\footnotesize{Panel A. $N_m = 200$}\\
\subfloat[DGP = Bertrand]{\includegraphics[scale = 0.51]{Graphs/Margins5_table3_Nm200_B.png}}\qquad
\subfloat[DGP = Collusion]{\includegraphics[scale = 0.51]{Graphs/Margins5_table3_Nm200_M.png}}\\
\footnotesize{Panel B. $N_m = 2000$}\\
\subfloat[DGP = Bertrand]{\includegraphics[scale = 0.51]{Graphs/Margins6_table3_Nm2000_B.png}}\qquad
\subfloat[DGP = Collusion]{\includegraphics[scale = 0.51]{Graphs/Margins6_table3_Nm2000_M.png}}
\caption*{\footnotesize{This figure compares the distribution of predicted markups at the 2SLS estimate of $\theta$ to the predicted markups for the Bertrand and Collusive models. Panel A plots the predicted markups for estimation across 200 markets, whereas Panel B plots the distribution of predicted markups for 2000 markets.  In estimating demand and markups, demand has been misspecified as logit.  For each panel, the left plot represents the distributions of markups when the true model is Bertrand and the right plot represents the distribution of markups when the true model is joint profit maximization. 
}}
\end{figure}


To better understand the source of these results, we plot, in Figure \ref{fig:markupdistributionmis}, the distribution of predicted markups implied by the 2SLS estimate of $\theta$ for one simulation.  First, the figure shows that the distributions of predicted markups implied by the estimated model do not exactly fit the distribution of predicted markups implied by either candidate model. Further, this discrepancy is not reduced as the sample size increases.  Thus, the tests designed for model assessment (EB, AR, and Cox) reject both models, as we see in the vast majority of simulations in Table \ref{tab:Tab_Comp_logit}.  However, in this low misspecification environment, visual inspection suggests that the distribution of predicted markups implied by the estimated model is closer to the true model than the wrong model. As such, the RV test designed for model selection is able to conclude in favor of the correct model in every simulation for 2000 markets. 


==> Notes/Todo_AER.tex <==
* Abstract must be down to 100 words
* Change the title? Testing Firm Conduct: Misspecification, Model Selection, and Weak Instruments
* In abstract, include an Andrews reference?
* Any other reference can be added to IA's work on structural models?
* "General Interest" effort in fist paragraph of intro
* Anything else to be done to intro?
* Appendices - finish putting in text
* Section 7 - clean up the text in case it doesn't match the new numbers 

* put in text references to the appendix tables
* comment on log(Flavors) in text



Testing Firm Conduct with Weak Instruments
Testing Firm Conduct: Weak Instruments and Misspecification
Testing Firm Conduct: Misspecification, Model Selection, and Weak Instruments
Testing Firm Conduct in the presence of Weak Instruments and Misspecification

==> OldIntro.tex <==
\section{Introduction}\label{sec:intro}


In order to understand the impact of policy on markets with imperfect competition, it is necessary to have a model of how firms behave. Additionally, studying firm conduct can be of primary interest in itself. However, the true model of conduct is often not known and researchers may therefore test a set of candidate models supported by theory. Recent examples include detecting the competitive effect of common ownership \citep[][]{bcs20}, labor market monopsony power \citep[][]{rs21}, and the US government's market power in issuing safe assets \citep[][]{ckp22}. \looseness=-1


In an ideal testing setting, the researcher compares markups implied by a model of conduct to the true markups.  As true markups are rarely observed, \cite{bh14} provide a falsifiable restriction for a  model of conduct which requires instruments.  In the standard parametric differentiated products environment, we show that  a model is falsified by the instruments if its predicted markups (markups projected on instruments) are different from the predicted markups for the true model.  This intuition connects testing  with unobserved true markups to the ideal setting while also highlighting the role of instruments in distinguishing conduct. In practice, a researcher must  implement a test by encoding the falsifiable restriction into statistical hypotheses.  In this paper, we elucidate how the form of the hypotheses and the strength of the instruments affect inference.
Based on our findings, we provide methods to ensure valid testing of conduct.\looseness=-1 


The industrial organization (IO) literature uses both model selection and model assessment procedures to test conduct.  These differ in the hypotheses they formulate  from  the falsifiable restriction.  Model selection compares the relative fit of two competing models.  Model assessment checks the absolute fit of a given model. We show that this distinction affects inference under misspecification of either demand or cost. Specifically, the model selection test in \cite{rv02} (RV) distinguishes the model for which predicted markups are closer to the truth. Instead, with misspecification, model assessment tests  reject the true model in large samples.  


 
As misspecification is likely, our results establish the importance of using RV to test firm conduct.  However, this test can suffer from degeneracy, defined as zero asymptotic variance of the difference in lack of fit between models \citep[see][]{rv02}.  With degeneracy, the asymptotic null distribution of the RV test statistic is no longer standard normal.  Despite the precise definition above, the economic causes and inferential effects of degeneracy remain opaque.  Thus, researchers often ignore degeneracy when testing firm conduct.  We show that assuming away degeneracy amounts to  imposing that at least one of the models is falsified by the instruments. Degeneracy obtains if either the markups for the true model are indistinguishable from the markups of the candidate models, or the instruments are uncorrelated with markups.  

To shed light on the inferential consequences of degeneracy, we define a novel  \textit{weak instruments for testing} asymptotic framework adapted from \cite{ss97}.  Under this framework, we show that the asymptotic null distribution of the RV test statistic is skewed and has a non-zero mean.  As skewness declines in the number of instruments while the magnitude of the mean increases,  the resulting size distortions are non-monotone in the number of instruments.  With one instrument or many instruments,  large size distortions are possible. With two to nine instruments, we find that size distortions above 2.5\% are impossible.\looseness=-1

Our characterization of degeneracy allows us to develop a novel diagnostic for weak instruments, which aids researchers in drawing proper conclusions when testing conduct with RV.  In the spirit of \cite{sy05} and \cite{olea13}, our diagnostic uses an effective $F$-statistic.  However, the $F$-statistic is formed from two auxiliary regressions as opposed to a single first stage.  Like \cite{sy05}, we show that instruments can be diagnosed as weak based on worst-case size. With one or many instruments, the proposed $F$-statistic needs to be large to conclude that the instruments are strong for size; we provide the appropriate critical values.\looseness = -1

A distinguishing feature of our weak instruments framework is that power is a salient concern.
In fact, the best-case power of the RV test against either model of conduct is strictly less than one, even in large samples.  The attainable power of the test can differ across the competing models and is lowered by misspecification.  Thus,  diagnosing whether the instruments are strong for power is crucial.   The same $F$-statistic used to detect size distortions is also informative about the best-case power of the RV test.  However, the critical values to compare the $F$-statistic against are different.  For power, the critical values are monotonically declining in the number of instruments, making low power the primary concern with two to nine instruments. In sum, researchers no longer need to assume away degeneracy; instead, they can interpret the results of RV through the lens of our $F$-statistic.\looseness=-1  

Up to here, the discussion presumes researchers precommit to one instrument set. \cite{bh14} show that many sources of exogenous variation exist for testing conduct, although -- reflecting the economics of different models -- some may fail to be relevant in specific applications \citep[][]{mqsw22}.  Pooling all sources of variation into one set of instruments may obscure the degree of misspecification while also diluting instrument strength.   Section \ref{sec:accumulate} discusses how
researchers can separately use these sources of variation to test firm conduct
without needing to precommit to any of them. We propose a conservative procedure whereby a researcher concludes for a set of models when all strong instruments support them.\looseness=-1



In an empirical application,  we revisit the setting of \cite{v07} and test five models of vertical conduct in the market for yogurt, including models of double marginalization and  two-part tariffs. The application illustrates the empirical relevance of our results for inference on conduct with misspecification and weak instruments. Inspection of the price-cost margins implied by different models only allows us to rule out one model. To obtain sharper results, we then perform model selection with RV. Commonly used sets of instruments are weak for testing as measured by our diagnostic.   When the RV test is implemented with these weak instruments, it has essentially no power. This illustrates the importance of using our diagnostic to assess instrument strength in terms of both size and power when interpreting the results of the RV test. \looseness=-1  

Using our procedure to accumulate evidence from different sources of variation,  we conclude for a model in which manufacturers set retail prices. All strong instruments reject the other models. This application speaks to an important debate over vertical conduct in consumer packaged goods industries.  Several applied papers assume a model of two-part tariffs  where manufacturers set retail prices \citep[e.g.,][]{n01,mw17}.  Our results support this assumption. \looseness=-1 

This paper develops tools relevant to a broad literature seeking to understand firm conduct in the context of structural models of demand and supply. Focusing on articles that pursue a testing approach, collusion is a prominent application \citep[e.g.,][]{p83,s85,b87,glv92,v96,gm98,n01,s20}.  Other important applications include common ownership \citep{bcs20}, vertical conduct \citep[e.g.,][]{v07,bd10,g13, z21, lwy21}, price discrimination \citep{ddf19}, price versus quantity setting \citep{fl95}, and non-profit behavior \citep{dmr20}. Outside of IO, recent applications include labor market conduct  \citep{rs21} and the market power of the US government in issuing safe assets \citep[][]{ckp22}. \looseness=-1   


%Parallel to the line of research in this paper, which discusses the implementation in finite sample of conduct testing, \cite{mqsw22} investigate the economic determinants of model falsification. Their results may motivate a-priori instrument choice, and provide an economic interpretation to the notion of instrument relevance developed in this paper. While they show, in a stylized environment, that most common models used in IO are falsified with at least one standard instrument, they also discuss examples where standard instrument choices result in lack of falsification. Even if at least one candidate model may be falsified theoretically by the instruments, the $F$-statistic developed in this paper is useful to diagnose inferential issues that occur in finite sample when models are close to the space of degeneracy.

This paper is also related to econometric work on the testing of non-nested hypotheses \citep[e.g., ][]{pw01}.  We build on the insights of the econometrics literature that performs inference under misspecification and highlights the importance of model selection procedures \citep[e.g.,][]{w82,v89, hi03, k03, mo12,ls20}. Two recent contributions, \cite{s15} and \cite{sw17}, modify the likelihood based test in \cite{v89} to correct size distortions under degeneracy.  In our GMM setting, we show that power, not size, is the salient concern. Furthermore, by connecting degeneracy to instrument strength,   our work is related to the econometrics literature on inference under weak instruments \citep[surveyed in][]{ass19}. Contemporaneous work by \cite{bcs20} shares our goal of enhancing inference on firm conduct. They explore the complementary question of which functional form the researcher should use in constructing the instruments, and propose running the RV test with a single instrument formed by pooling all exogenous variation with a random forest.\looseness=-1

The paper proceeds as follows. Section \ref{sec:themodel} describes the environment: a general model of firm conduct. Section \ref{sec:nevo} formalizes our notion of falsifiability when true markups are unobserved. Section \ref{sec:hypo_formulation} explores the effect of hypothesis formulation on inference, contrasting  model selection and assessment approaches under misspecification. Section \ref{sec:instruments} connects  degeneracy of RV to instrument strength, characterizes the effect of weak instruments on inference, and introduces a diagnostic for weak instruments to report alongside the RV test. Section \ref{sec:accumulate} provides a procedure to accumulate evidence across different sets of instruments. Section \ref{sec:empiricaleg} develops our empirical application: testing models of vertical conduct in the retail market for yogurt. Section \ref{sec:conclusion} concludes. Proofs are found in Appendix \ref{sect:Proofs}. \looseness=-1 


==> Output/StockYogo.tex <==
\newcolumntype{d}[1]{D{.}{.}{#1}}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{\extracolsep{25pt}}rccc}
\toprule
& \multicolumn{3}{c}{Desired Minimal Rejection Probability of RV Test}\\ 
\cline{2-4}
$d_z$&	$r = 0.01$&	$r = 0.025$&	$r = 0.04$\\\midrule
1&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &10.61& , &21.57& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &13.10& , &36.05& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &14.54& , &73.50& ]\end{tabular}\\
2&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &5.42& , &11.41& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &6.68& , &19.97& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &7.76& , &42.82& ]\end{tabular}\\
3&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &4.03& , &8.02& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &4.61& , &15.04& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &5.03& , &33.74& ]\end{tabular}\\
4&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.66& , &6.70& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &4.33& , &11.90& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &4.33& , &29.73& ]\end{tabular}\\
5&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.73& , &5.61& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &4.12& , &10.54& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &4.25& , &27.29& ]\end{tabular}\\
6&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.54& , &4.87& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.99& , &9.40& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &4.17& , &23.89& ]\end{tabular}\\
7&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.58& , &4.35& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.91& , &8.59& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &4.10& , &22.12& ]\end{tabular}\\
8&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.50& , &4.14& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.76& , &7.98& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.85& , &20.35& ]\end{tabular}\\
9&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.46& , &3.81& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.77& , &7.50& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.89& , &19.10& ]\end{tabular}\\
10&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.10& , &3.55& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.54& , &7.24& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.83& , &18.10& ]\end{tabular}\\
%11&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.22& , &3.47& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.63& , &6.91& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.90& , &18.00& ]\end{tabular}\\
%12&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.10& , &3.28& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.54& , &6.63& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.73& , &17.25& ]\end{tabular}\\
%13&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &2.54& , &3.12& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.52& , &6.21& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.62& , &16.44& ]\end{tabular}\\
%14&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &2.80& , &2.98& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.47& , &6.02& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.68& , &15.74& ]\end{tabular}\\
15&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &2.71& , &2.95& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.57& , &6.10& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.62& , &16.34& ]\end{tabular}\\
%16&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &2.62& , &2.92& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.43& , &5.86& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.54& , &15.38& ]\end{tabular}\\
%17&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &2.44& , &2.74& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.48& , &5.73& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.54& , &15.26& ]\end{tabular}\\
%18&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &2.46& , &2.73& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.46& , &5.67& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.52& , &14.60& ]\end{tabular}\\
%19&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &2.36& , &2.65& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.29& , &5.49& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.47& , &14.65& ]\end{tabular}\\
20&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &2.28& , &2.64& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.35& , &5.39& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.46& , &14.52& ]\end{tabular}\\
%21&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &2.23& , &2.57& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.36& , &5.25& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.45& , &14.62& ]\end{tabular}\\
%22&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &2.12& , &2.57& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.20& , &5.33& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.42& , &13.95& ]\end{tabular}\\
%23&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &2.12& , &2.50& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.26& , &5.20& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.43& , &13.73& ]\end{tabular}\\
%24&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &2.11& , &2.39& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.27& , &5.22& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.35& , &13.61& ]\end{tabular}\\
25&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &2.11& , &2.45& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.20& , &5.10& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.33& , &13.55& ]\end{tabular}\\
%26&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &2.11& , &2.40& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.25& , &4.99& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.33& , &13.53& ]\end{tabular}\\
%27&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &2.06& , &2.40& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.16& , &5.11& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.27& , &13.48& ]\end{tabular}\\
%28&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &1.97& , &2.36& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.18& , &4.97& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.30& , &12.88& ]\end{tabular}\\
%29&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &2.01& , &2.31& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.19& , &4.87& ]\end{tabular}&	\begin{tabular}{@{\extracolsep{-7pt}}ld{3.2}cd{3.2}r} [ &3.28& , &13.15& ]\end{tabular}\\
\bottomrule
\end{tabular}

==> Output/StockYogo_Combined.tex <==
\newcolumntype{d}[1]{D{.}{.}{#1}}
\renewcommand{\arraystretch}{1.05}
\footnotesize
\begin{tabular}{@{\extracolsep{30pt}}rrrrl|rrr}
\toprule
&  \multicolumn{3}{l}{\textbf{Panel A:} Maximal Size ${cv^s},\,\, r^s = $} &&  \multicolumn{3}{l}{\textbf{Panel B:} Minimal Power ${cv^p},\,\, r^p = $}\\ 
\cline{2-4}\cline{6-8}
$d_z$&	$0.10$&	$0.15$&	$0.20$ &&	$0.25$ & $0.50$ & $0.75$ \\\midrule
1&49.26&5.99&5.99&&24.24&31.16&39.12\\
2&4.74&4.74&4.74&&11.98&15.47&19.46\\
3&4.20&4.20&4.20&&7.89&10.23&12.80\\
4&3.88&3.88&3.88&&5.94&7.62&9.55\\
5&3.66&3.66&3.66&&5.38&6.41&7.60\\
6&3.50&3.50&3.50&&5.12&5.95&6.98\\
7&3.38&3.38&3.38&&4.87&5.67&6.54\\
8&3.29&3.29&3.29&&4.67&5.36&6.16\\
9&3.21&3.21&3.21&&4.51&5.16&5.89\\
10&4.32&3.14&3.14&&4.39&4.99&5.65\\
11&6.43&3.49&3.08&&4.28&4.82&5.44\\
12&8.45&4.79&3.41&&4.18&4.70&5.27\\
13&10.71&5.88&4.29&&4.10&4.58&5.12\\
14&12.75&7.12&5.08&&4.01&4.47&4.99\\
15&14.55&8.24&5.98&&3.95&4.38&4.88\\
16&16.93&9.26&6.74&&3.87&4.29&4.77\\
17&19.25&10.54&7.53&&3.83&4.22&4.68\\
18&21.53&11.66&8.27&&3.77&4.15&4.58\\
19&23.32&12.76&9.11&&3.73&4.09&4.50\\
20&25.72&14.13&9.97&&3.68&4.04&4.42\\
21&28.49&15.14&10.78&&3.63&3.99&4.37\\
22&30.41&16.40&11.62&&3.59&3.93&4.30\\
23&32.98&17.54&12.27&&3.56&3.88&4.24\\
24&34.92&18.67&13.14&&3.52&3.84&4.19\\
25&37.42&19.83&13.85&&3.49&3.80&4.14\\
26&39.60&20.85&14.67&&3.47&3.76&4.09\\
27&41.21&22.22&15.41&&3.44&3.73&4.05\\
28&43.94&23.04&16.26&&3.41&3.69&4.00\\
29&46.04&24.64&17.04&&3.38&3.66&3.96\\
30&48.06&25.69&17.84&&3.36&3.63&3.92\\
\bottomrule

\end{tabular}

==> Output/StockYogo_Combined_new_talk.tex <==

%\newcolumntype{d}[1]{D{.}{.}{#1}}
%\renewcommand{\arraystretch}{1.05}

\begin{widetable}{.98\columnwidth}{r*{3}{>{\raggedleft\arraybackslash}p{4em}}c*{3}{>{\raggedleft\arraybackslash}p{4em}}}
\toprule
&  \multicolumn{3}{c}{\textbf{Panel A:} Maximal Size ${cv^s},\,\, r^s = $} &&  \multicolumn{3}{c}{{\textbf{Panel B:} Maximal Power ${cv^p},\,\, r^p = $}}\\ 
\cmidrule(lr){2-4}\cmidrule(lr){6-8} 
$d_z$  & 0.075 & 0.10 & 0.125 & &  {0.95} & {0.75} & {0.50}\\
\midrule
1&31.4&14.5&8.4&&{31.1}&{22.6}&{18.0}\\
2&0&0&0&&18.9&13.2&10.4\\
3&0&0&0&&14.6&10.2&8.0\\
%4&0&0&0&&12.3&8.8&6.9\\
%5&0&0&0&&10.8&7.8&6.2\\
6&0&0&0&&9.8&7.2&5.8\\
%7&0&0&0&&9.0&6.7&5.4\\
%8&0&0&0&&8.4&6.4&5.2\\
9&0.3&0&0&&8.0&6.1&5.0\\
10&1.7&0.4&0&&7.6&5.8&4.8\\
%%11&3.3&1.3&0.5&&7.2&5.6&4.6\\
%%12&5.0&2.1&1.1&&7.0&5.4&4.5\\
%%13&6.9&3.1&1.8&&6.7&5.3&4.4\\
%%14&8.8&4.0&2.4&&6.5&5.1&4.3\\
15&10.8&5.0&3.1&&6.3&5.0&4.2\\
20&21.1&10.2&6.6&&5.6&4.6&3.9\\
25&31.8&15.7&10.3&&5.1&4.2&3.7\\
30&42.8&21.2&14.1&&4.8&4.0&3.5\\
\bottomrule
\end{widetable}


==> Output/StockYogo_Combined_new_talk_Power1.tex <==

%\newcolumntype{d}[1]{D{.}{.}{#1}}
%\renewcommand{\arraystretch}{1.05}

\begin{widetable}{.98\columnwidth}{r*{3}{>{\raggedleft\arraybackslash}p{4em}}c*{3}{>{\raggedleft\arraybackslash}p{4em}}}
\toprule
&   \multicolumn{3}{c}{{\textbf{Panel B:} Maximal Power ${cv^p},\,\, r^p = $}}\\ 
\cmidrule(lr){2-4} 
$d_z$  &  \tikzmark{top left 1}{0.95} & {0.75} & {0.50}\tikzmark{bottom right 1}\\
\midrule
1&{31.1}&{22.6}&{18.0}\\
2&18.9&13.2&10.4\\
3&14.6&10.2&8.0\\
%4&12.3&8.8&6.9\\
%5&10.8&7.8&6.2\\
6&9.8&7.2&5.8\\
%7&9.0&6.7&5.4\\
%8&8.4&6.4&5.2\\
9&8.0&6.1&5.0\\
10&7.6&5.8&4.8\\
%%11&3.3&1.3&0.5&&7.2&5.6&4.6\\
%%12&5.0&2.1&1.1&&7.0&5.4&4.5\\
%%13&6.9&3.1&1.8&&6.7&5.3&4.4\\
%%14&8.8&4.0&2.4&&6.5&5.1&4.3\\
15&6.3&5.0&4.2\\
20&5.6&4.6&3.9\\
25&5.1&4.2&3.7\\
30&4.8&4.0&3.5\\
\bottomrule
\end{widetable}

{\DrawBox[ultra thick, mycolor]{top left 1}{bottom right 1}}





==> Output/StockYogo_Combined_new_talk_Power2.tex <==

%\newcolumntype{d}[1]{D{.}{.}{#1}}
%\renewcommand{\arraystretch}{1.05}

\begin{widetable}{.98\columnwidth}{r*{3}{>{\raggedleft\arraybackslash}p{4em}}c*{3}{>{\raggedleft\arraybackslash}p{4em}}}
\toprule
&   \multicolumn{3}{c}{{\textbf{Panel B:} Maximal Power ${cv^p},\,\, r^p = $}}\\ 
\cmidrule(lr){2-4} 
$d_z$  &  \tikzmark{top left 1}{0.95} \tikzmark{bottom right 1} & {0.75} & {0.50}\\
\midrule
1&{31.1}&{22.6}&{18.0}\\
2&18.9&13.2&10.4\\
3&14.6&10.2&8.0\\
%4&12.3&8.8&6.9\\
%5&10.8&7.8&6.2\\
6&9.8&7.2&5.8\\
%7&9.0&6.7&5.4\\
%8&8.4&6.4&5.2\\
9&8.0&6.1&5.0\\
10&7.6&5.8&4.8\\
%%11&3.3&1.3&0.5&&7.2&5.6&4.6\\
%%12&5.0&2.1&1.1&&7.0&5.4&4.5\\
%%13&6.9&3.1&1.8&&6.7&5.3&4.4\\
%%14&8.8&4.0&2.4&&6.5&5.1&4.3\\
\tikzmark{top left 2}15\tikzmark{bottom right 2}&\tikzmark{top left 3}6.3 \tikzmark{bottom right 3}&5.0&4.2\\
20&5.6&4.6&3.9\\
25&5.1&4.2&3.7\\
30&4.8&4.0&3.5\\
\bottomrule
\end{widetable}


{\DrawBox[ultra thick, mycolor]{top left 1}{bottom right 1}}
{\DrawBox[ultra thick, mycolor]{top left 2}{bottom right 2}}
{\DrawBox[ultra thick, mycolor]{top left 3}{bottom right 3}}

==> Output/StockYogo_Combined_new_talk_Power3.tex <==

%\newcolumntype{d}[1]{D{.}{.}{#1}}
%\renewcommand{\arraystretch}{1.05}

\begin{widetable}{.98\columnwidth}{r*{3}{>{\raggedleft\arraybackslash}p{4em}}c*{3}{>{\raggedleft\arraybackslash}p{4em}}}
\toprule
&   \multicolumn{3}{c}{{\textbf{Panel B:} Maximal Power ${cv^p},\,\, r^p = $}}\\ 
\cmidrule(lr){2-4} 
$d_z$  &  {0.95} & {0.75} & {0.50}\\
\midrule
 \tikzmark{top arrow} $\,$ 1 &\tikzmark{top left 1}{31.1}&{22.6}&{18.0}\\
2&18.9&13.2&10.4\\
3&14.6&10.2&8.0\\
%4&12.3&8.8&6.9\\
%5&10.8&7.8&6.2\\
6&9.8&7.2&5.8\\
%7&9.0&6.7&5.4\\
%8&8.4&6.4&5.2\\
9&8.0&6.1&5.0\\
\tikzmark{tb}$\,\,\,\,\,$10&7.6&5.8&4.8\\
%%11&3.3&1.3&0.5&&7.2&5.6&4.6\\
%%12&5.0&2.1&1.1&&7.0&5.4&4.5\\
%%13&6.9&3.1&1.8&&6.7&5.3&4.4\\
%%14&8.8&4.0&2.4&&6.5&5.1&4.3\\
15&6.3&5.0&4.2\\
20&5.6&4.6&3.9\\
25&5.1&4.2&3.7\\
\tikzmark{bottom arrow} $\,\,\,\,\,$  30&4.8\tikzmark{bottom right 1}&4.0&3.5\\
\bottomrule
\end{widetable}

\DrawBox[ultra thick, mycolor]{top left 1}{bottom right 1}

\DrawArrow[ultra thick, mycolor]{top arrow}{bottom arrow}

\DrawTextBox[align=left,rotate=90]{tb}{Critical Values Decreasing}

==> Output/StockYogo_Combined_new_talk_Size1.tex <==

%\newcolumntype{d}[1]{D{.}{.}{#1}}
%\renewcommand{\arraystretch}{1.05}

\begin{widetable}{.98\columnwidth}{r*{3}{>{\raggedleft\arraybackslash}p{4em}}c*{3}{>{\raggedleft\arraybackslash}p{4em}}}
\toprule
&  \multicolumn{3}{c}{\textbf{Panel A:} Maximal Size ${cv^s},\,\, r^s = $} \\ 
\cmidrule(lr){2-4}
$d_z$  & \tikzmark{top left 1} $\,\,$0.075 & 0.10 & 0.125 \tikzmark{bottom right 1} \\
\midrule
1&31.4&14.5&8.4\\
2&0&0&0\\
3&0&0&0\\
%4&0&0&0\\
%5&0&0&0\\
6&0&0&0\\
%7&0&0&0\\
%8&0&0&0\\
9&0.3&0&0\\
10&1.7&0.4&0\\
%%11&3.3&1.3&0.5&&7.2&5.6&4.6\\
%%12&5.0&2.1&1.1&&7.0&5.4&4.5\\
%%13&6.9&3.1&1.8&&6.7&5.3&4.4\\
%%14&8.8&4.0&2.4&&6.5&5.1&4.3\\
15&10.8&5.0&3.1\\
20&21.1&10.2&6.6\\
25&31.8&15.7&10.3\\
30&42.8&21.2&14.1\\
\bottomrule
\end{widetable}
{\DrawBox[ultra thick, mycolor]{top left 1}{bottom right 1}}

==> Output/StockYogo_Combined_new_talk_Size2.tex <==

%\newcolumntype{d}[1]{D{.}{.}{#1}}
%\renewcommand{\arraystretch}{1.05}

\begin{widetable}{.98\columnwidth}{r*{3}{>{\raggedleft\arraybackslash}p{4em}}c*{3}{>{\raggedleft\arraybackslash}p{4em}}}
\toprule
&  \multicolumn{3}{c}{\textbf{Panel A:} Maximal Size ${cv^s},\,\, r^s = $} \\ 
\cmidrule(lr){2-4}
$d_z$  & \tikzmark{top left 1} $\,\,$0.075 \tikzmark{bottom right 1} & 0.10 & 0.125 \\
\midrule
1&31.4&14.5&8.4\\
2&0&0&0\\
3&0&0&0\\
%4&0&0&0\\
%5&0&0&0\\
6&0&0&0\\
%7&0&0&0\\
%8&0&0&0\\
9&0.3&0&0\\
10&1.7&0.4&0\\
%%11&3.3&1.3&0.5&&7.2&5.6&4.6\\
%%12&5.0&2.1&1.1&&7.0&5.4&4.5\\
%%13&6.9&3.1&1.8&&6.7&5.3&4.4\\
%%14&8.8&4.0&2.4&&6.5&5.1&4.3\\
\tikzmark{top left 2}15 \tikzmark{bottom right 2}& \tikzmark{top left 3}10.8 \tikzmark{bottom right 3}&5.0&3.1\\
20&21.1&10.2&6.6\\
25&31.8&15.7&10.3\\
30&42.8&21.2&14.1\\
\bottomrule
\end{widetable}
{\DrawBox[ultra thick, mycolor]{top left 1}{bottom right 1}}
{\DrawBox[ultra thick, mycolor]{top left 2}{bottom right 2}}

{\DrawBox[ultra thick, mycolor]{top left 3}{bottom right 3}}

==> Output/StockYogo_Combined_new_talk_Size3.tex <==

%\newcolumntype{d}[1]{D{.}{.}{#1}}
%\renewcommand{\arraystretch}{1.05}

\begin{widetable}{.98\columnwidth}{r*{3}{>{\raggedleft\arraybackslash}p{4em}}c*{3}{>{\raggedleft\arraybackslash}p{4em}}}
\toprule
&  \multicolumn{3}{c}{\textbf{Panel A:} Maximal Size ${cv^s},\,\, r^s = $} \\ 
\cmidrule(lr){2-4}
$d_z$  &  $\,\,$0.075 & 0.10 & 0.125 \\
\midrule
 1&\tikzmark{top left 1}31.4&14.5&8.4\tikzmark{bottom right 1}\\
2&\tikzmark{top left 2}$\,\,$ 0&0&0\\
3&0&0&0\\
%4&0&0&0\\
%5&0&0&0\\
6&0&0&0\\
%7&0&0&0\\
%8&0&0&0\\
9&0.3&0&0\tikzmark{bottom right 2}\\
10&\tikzmark{top left 3}$\,\,$1.7&0.4&0\\
%%11&3.3&1.3&0.5&&7.2&5.6&4.6\\
%%12&5.0&2.1&1.1&&7.0&5.4&4.5\\
%%13&6.9&3.1&1.8&&6.7&5.3&4.4\\
%%14&8.8&4.0&2.4&&6.5&5.1&4.3\\
15& 10.8&5.0&3.1\\
\tikzmark{tb}20&21.1&10.2&6.6\\
25&31.8&15.7&10.3\\
 30&42.8\tikzmark{bottom right 3}&21.2&14.1\\
\bottomrule
\end{widetable}

\only<1>{\DrawBox[ultra thick, mycolor]{top left 1}{bottom right 1}}
\only<2>{\DrawBox[ultra thick, mycolor]{top left 2}{bottom right 2}}

\only<3>{\DrawBox[ultra thick, mycolor]{top left 3}{bottom right 3}}

%\DrawArrow[ultra thick, mycolor]{top arrow}{bottom arrow}

%\only<3>\DrawTextBox[align=left,rotate=90]{tb}{$cv^s \approx 2(d_z-9)$}

==> Output/StockYogo_Power.tex <==
\newcolumntype{d}[1]{D{.}{.}{#1}}
\renewcommand{\arraystretch}{1.05}
\footnotesize
\begin{tabular}{@{\extracolsep{30pt}}rrrr}

\toprule
&  \multicolumn{3}{c}{${cv},\,\, r = $}\\ 
\cline{2-4}
$d_z$&0.25	&$0.50$&	$0.75$ \\\midrule
1&24.24&31.16&39.12\\
2&11.98&15.47&19.46\\
3&7.89&10.23&12.80\\
4&5.94&7.62&9.55\\
5&5.38&6.41&7.60\\
6&5.12&5.95&6.98\\
7&4.87&5.67&6.54\\
8&4.67&5.36&6.16\\
9&4.51&5.16&5.89\\
10&4.39&4.99&5.65\\
11&4.28&4.82&5.44\\
12&4.18&4.70&5.27\\
13&4.10&4.58&5.12\\
14&4.01&4.47&4.99\\
15&3.95&4.38&4.88\\
16&3.87&4.29&4.77\\
17&3.83&4.22&4.68\\
18&3.77&4.15&4.58\\
19&3.73&4.09&4.50\\
20&3.68&4.04&4.42\\
21&3.63&3.99&4.37\\
22&3.59&3.93&4.30\\
23&3.56&3.88&4.24\\
24&3.52&3.84&4.19\\
25&3.49&3.80&4.14\\
26&3.47&3.76&4.09\\
27&3.44&3.73&4.05\\
28&3.41&3.69&4.00\\
29&3.38&3.66&3.96\\
30&3.36&3.63&3.92\\
\bottomrule

\end{tabular}

==> Output/StockYogo_new.tex <==
\newcolumntype{d}[1]{D{.}{.}{#1}}
\renewcommand{\arraystretch}{1.05}
\footnotesize
\begin{tabular}{@{\extracolsep{30pt}}rccccc}

\toprule
& $\underline{cv}$ & \multicolumn{4}{c}{$\overline{cv},\,\, r = $}\\ 
\cline{3-6}
$d_z$&	&$0.10$&	$0.15$&	$0.20$ &	$0.25$ \\\midrule

1&15.41&48.11&3.84&3.84&3.84\\
2&7.93&3.00&3.00&3.00&3.00\\
3&5.44&2.06&2.60&2.60&2.60\\
4&4.50&2.37&2.37&2.37&2.37\\
5&4.51&2.21&2.21&2.21&2.21\\
6&4.30&2.10&2.10&2.10&2.10\\
7&4.20&2.01&2.01&2.01&2.01\\
8&4.12&1.94&1.94&1.94&1.94\\
9&3.99&1.88&1.88&1.88&1.88\\
10&3.85&3.12&1.83&1.83&1.83\\
11&3.77&5.29&2.39&1.79&1.79\\
12&3.92&7.55&3.62&2.17&1.75\\
13&3.74&9.63&4.75&3.12&2.22\\
14&3.75&11.68&6.02&3.94&2.88\\
15&3.57&13.78&7.15&4.86&3.58\\
16&3.64&15.94&8.25&5.63&4.23\\
17&3.46&18.26&9.47&6.43&4.86\\
18&3.58&20.48&10.59&7.19&5.47\\
19&3.47&22.62&11.82&8.04&6.06\\
20&3.51&24.68&13.07&8.90&6.76\\
21&3.48&27.46&14.09&9.72&7.32\\
22&3.45&29.37&15.35&10.56&7.93\\
23&3.48&31.95&16.5&11.22&8.62\\
24&3.44&33.89&17.63&12.09&9.16\\
25&	3.34&36.39&18.79&12.84&9.78\\
26&3.32&38.96&20.10&13.74&10.39\\
27&3.25&40.61&21.19&14.45&10.99\\
28&3.32&42.92&22.38&15.22&11.66\\
29&3.31&45.34&23.60&16.11&12.24\\
30&3.26&47.63&24.66&16.80&12.82\\
\bottomrule

\end{tabular}

==> Output/Tab_Comp_base.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{5pt}}llcccccccc}
\toprule
&& \multicolumn{4}{c}{DGP $B$}& \multicolumn{4}{c}{DGP $C$}\\
\cline{3-6}\cline{7-10}&Models& RV& AR& EB&Cox& RV& AR& EB &Cox\\
\cline{1-10}\textbf{Panel A.} $N_m=200$&$B$ only&1.00&0.94&0.96&0.97&0.00&0.00&0.00&0.00\\
&$C$ only&0.00&0.00&0.00&0.00&0.99&0.94&0.97&0.99\\
&$B=C$&0.00&&&&0.01&&&\\
&Both&&0.00&0.00&0.00&&0.00&0.00&0.00\\
&Neither&&0.06&0.04&0.03&&0.06&0.03&0.01\\

\midrule\textbf{Panel B.} $N_m=2000$&$B$ only&1.00&0.92&0.93&0.97&0.00&0.00&0.00&0.00\\
&$C$ only&0.00&0.00&0.00&0.00&1.00&0.94&0.95&0.96\\
&$B=C$&0.00&&&&0.00&&&\\
&Both&&0.00&0.00&0.00&&0.00&0.00&0.00\\
&Neither&&0.08&0.07&0.03&&0.06&0.05&0.04\\
\bottomrule
\end{tabular}

==> Output/Tab_Comp_base_slides.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{5pt}}lcccccccc}
\toprule
& \multicolumn{4}{c}{DGP $B$}& \multicolumn{4}{c}{DGP $C$}\\
\cline{2-5}\cline{6-9}Models& RV& AR& EB&Cox& RV& AR& EB &Cox\\
\cline{1-9}&\multicolumn{8}{c}{\textbf{Panel I:} $N_m=200$}\\
$B$ only& \only<2>{\cellcolor{yellow}}1.00& \only<2>{\cellcolor{yellow}}0.94& \only<2>{\cellcolor{yellow}}0.96& \only<2>{\cellcolor{yellow}}0.97&0.00&0.00&0.00&0.00\\
$C$ only&0.00&0.00&0.00&0.00& \only<2>{\cellcolor{yellow}}0.99& \only<2>{\cellcolor{yellow}}0.94& \only<2>{\cellcolor{yellow}}0.97& \only<2>{\cellcolor{yellow}}0.99\\
$B=C$&0.00&&&&0.01&&&\\
Both&&0.00&0.00&0.00&&0.00&0.00&0.00\\
Neither&&0.06&0.04&0.03&&0.06&0.03&0.01\\
\midrule&\multicolumn{8}{c}{\textbf{Panel II:} $N_m=2000$}\\
$B$ only& \only<2>{\cellcolor{yellow}}1.00& \only<2>{\cellcolor{yellow}}0.92& \only<2>{\cellcolor{yellow}}0.93& \only<2>{\cellcolor{yellow}}0.97&0.00&0.00&0.00&0.00\\
$C$ only&0.00&0.00&0.00&0.00& \only<2>{\cellcolor{yellow}}1.00& \only<2>{\cellcolor{yellow}}0.94& \only<2>{\cellcolor{yellow}}0.95& \only<2>{\cellcolor{yellow}}0.96\\
$B=C$&0.00&&&&0.00&&&\\
Both&&0.00&0.00&0.00&&0.00&0.00&0.00\\
Neither&&0.08&0.07&0.03&&0.06&0.05&0.04\\
\bottomrule
\end{tabular}

==> Output/Tab_Comp_logit.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{5pt}}llcccccccc}
\toprule
&& \multicolumn{4}{c}{DGP $B$}& \multicolumn{4}{c}{DGP $C$}\\
\cline{3-6}\cline{7-10}&Models& RV& AR& EB&Cox& RV& AR& EB &Cox\\
\cline{1-10}\textbf{Panel A.} $N_m=200$&$B$ only&0.78&0.48&0.41&0.24&0.00&0.00&0.00&0.00\\
&$C$ only&0.00&0.00&0.00&0.07&0.98&0.43&0.39&0.37\\
&$B=C$&0.22&&&&0.02&&&\\
&Both&&0.01&0.00&0.17&&0.00&0.00&0.02\\
&Neither&&0.51&0.59&0.52&&0.57&0.61&0.61\\

\midrule\textbf{Panel B.} $N_m=2000$&$B$ only&1.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&$C$ only&0.00&0.00&0.00&0.00&1.00&0.00&0.00&0.00\\
&$B=C$&0.00&&&&0.00&&&\\
&Both&&0.00&0.00&0.00&&0.00&0.00&0.00\\
&Neither&&1.00&1.00&1.00&&1.00&1.00&1.00\\
\bottomrule
\end{tabular}

==> Output/Tab_Comp_logit_slides.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{5pt}}lcccccccc}
\toprule
& \multicolumn{4}{c}{DGP $B$}& \multicolumn{4}{c}{DGP $C$}\\
\cline{2-5}\cline{6-9}Models& RV& AR& EB&Cox& RV& AR& EB &Cox\\
\cline{1-9} &\multicolumn{8}{c}{\textbf{Panel I:} $N_m=200$}\\
$B$ only& \only<2>{\cellcolor{yellow}}0.78& 0.48& 0.41& 0.24&0.00&0.00&0.00&0.00\\
$C$ only&0.00&0.00&0.00&0.07& \only<2>{\cellcolor{yellow}}0.98& 0.43& 0.39& 0.37\\
$B=C$&0.22&&&&0.02&&&\\
Both&&0.01&0.00&0.17&&0.00&0.00&0.02\\
Neither&&\only<2>{\cellcolor{yellow}}0.51&\only<2>{\cellcolor{yellow}}0.59&\only<2>{\cellcolor{yellow}}0.52&&\only<2>{\cellcolor{yellow}}0.57&\only<2>{\cellcolor{yellow}}0.61&\only<2>{\cellcolor{yellow}}0.61\\

\midrule&\multicolumn{8}{c}{\textbf{Panel II:} $N_m=2000$}\\
$B$ only& \only<3>{\cellcolor{yellow}}1.00&0.00&0.00& 0.00&0.00&0.00&0.00&0.00\\
$C$ only&0.00&0.00&0.00&0.00& \only<3>{\cellcolor{yellow}}1.00&0.00&0.00&0.00\\
$B=C$&0.00&&&&0.00&&&\\
Both&&0.00&0.00&0.00&&0.00&0.00&0.00\\
Neither&& \only<3>{\cellcolor{yellow}}1.00& \only<3>{\cellcolor{yellow}}1.00& \only<3>{\cellcolor{yellow}}1.00&& \only<3>{\cellcolor{yellow}}1.00& \only<3>{\cellcolor{yellow}}1.00& \only<3>{\cellcolor{yellow}}1.00\\
\bottomrule
\end{tabular}

==> Output/Tab_Comp_rss.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{4pt}}llcccccc}
\toprule
&& \multicolumn{3}{c}{RSS Test}& \multicolumn{3}{c}{RV Test}\\
\cline{3-5}\cline{6-8}&Models& $H_I$: $B$& $H_0$& $H_{II}$: $C$& $H_I$: $B$& $H_0$& $H_{II}$: $C$ \\
\cline{1-8}\textbf{Panel A.} DGP B&(1)&1.00&0.00&0.00&1.00&0.00&0.00\\
&(2)&0.17&0.80&0.03&1.00&0.00&0.00\\
&(3)&0.00&0.21&0.79&0.94&0.06&0.00\\
&(4)&0.00&0.10&0.90&0.93&0.07&0.00\\
\cline{1-8}\textbf{Panel B.} DGP C&(1)&0.00&0.00&1.00&0.00&0.00&1.00\\
&(2)&0.00&0.00&1.00&0.00&0.01&0.99\\
&(3)&0.00&0.00&1.00&0.00&0.13&0.87\\
&(4)&0.00&0.00&1.00&0.00&0.13&0.87\\
\hline\multicolumn{7}{l}{\footnotesize{(1) $\sigma^2_\omega=0.2,\:\sigma_{\xi\omega}=0,\:\:\alpha=-1$}} \\
\multicolumn{7}{l}{\footnotesize{(2) $\sigma^2_\omega=0.2,\:\sigma_{\xi\omega}=0,\:\:\alpha=-1.5$ (baseline)}} \\
\multicolumn{7}{l}{\footnotesize{(3) $\sigma^2_\omega=0.5,\:\sigma_{\xi\omega}=0,\:\:\alpha=-1.5$}} \\
\multicolumn{7}{l}{\footnotesize{(4) $\sigma^2_\omega=0.5,\:\sigma_{\xi\omega}=0.3,\:\:\alpha=-1.5$}} \\
\bottomrule\end{tabular}


==> Output/Tab_Comp_rss_slides.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{4pt}}lcccccc}
\toprule
& \multicolumn{3}{c}{RSS Test}& \multicolumn{3}{c}{RV Test}\\
\cline{2-4}\cline{5-7}Models& $H_A^1$: $B$& $H_0$& $H_{A}^2$: $C$& $H_A^1$: $B$& $H_0$& $H_{A}^2$: $C$ \\
\cline{1-7}\multicolumn{7}{c}{\textbf{Panel I:} DGP B}\\
(1)& \only<2>{\cellcolor{yellow}}1.00&0.00&0.00& \only<2-3>{\cellcolor{yellow}}1.00&0.00&0.00\\
(2)&\only<4>{\cellcolor{yellow}}0.17&0.80&\only<4>{\cellcolor{yellow}}0.03&\only<3>{\cellcolor{yellow}}1.00&0.00&0.00\\
(3)&\only<4>{\cellcolor{yellow}}0.00&0.21&\only<4>{\cellcolor{yellow}}0.79&\only<3>{\cellcolor{yellow}}0.94&0.06&0.00\\
(4)&\only<4>{\cellcolor{yellow}}0.00&0.10&\only<4>{\cellcolor{yellow}}0.90&\only<3>{\cellcolor{yellow}}0.93&0.07&0.00\\
\cline{1-7}\multicolumn{7}{c}{\textbf{Panel II:} DGP C}\\ (1)&0.00&0.00& \only<2>{\cellcolor{yellow}}1.00&0.00&0.00& \only<2-3>{\cellcolor{yellow}}1.00\\
(2)&0.00&0.00&\only<5>{\cellcolor{yellow}}1.00&0.00&0.01&\only<3>{\cellcolor{yellow}}0.99\\
(3)&0.00&0.00&\only<5>{\cellcolor{yellow}}1.00&0.00&0.13&\only<3>{\cellcolor{yellow}}0.87\\
(4)&0.00&0.00&\only<5>{\cellcolor{yellow}}1.00&0.00&0.13&\only<3>{\cellcolor{yellow}}0.87\\
\hline\multicolumn{7}{l}{\footnotesize{(1) $\sigma^2_\omega=0.2,\:\sigma_{\xi\omega}=0,\:\:\alpha=-1$}} \\
\multicolumn{7}{l}{\footnotesize{(2) $\sigma^2_\omega=0.2,\:\sigma_{\xi\omega}=0,\:\:\alpha=-1.5$ (baseline)}} \\
\multicolumn{7}{l}{\footnotesize{(3) $\sigma^2_\omega=0.5,\:\sigma_{\xi\omega}=0,\:\:\alpha=-1.5$}} \\
\multicolumn{7}{l}{\footnotesize{(4) $\sigma^2_\omega=0.5,\:\sigma_{\xi\omega}=0.3,\:\:\alpha=-1.5$}} \\
\bottomrule\end{tabular}


==> Output/Table_Sullivan2020.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{4pt}}lcccccc}
\toprule
	&RSS & RV &\multicolumn{2}{c}{AR}&\multicolumn{2}{c}{EB} \\
\cline{2-2}\cline{3-3}\cline{4-5}\cline{6-7}& & & $M_I$& $M_{II}$ &$M_I$& $M_{II}$\\
Statistic  &-18.24 &5.88 & & & &  \\
critical value    & $\pm$1.96 & $\pm$1.96 & 2.10  & 2.10 & $\pm$1.96  & $\pm$1.96\\
\bottomrule\end{tabular}

==> Output/old/TabRV_BM.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{4pt}}llcccccc}
\toprule
&& \multicolumn{3}{c}{RSS Test}& \multicolumn{3}{c}{RV Test}\\
\cline{3-5}\cline{6-8}&Spec& $H_I$: $B$& $H_0$& $H_{II}$: $J$& $H_I$: $B$& $H_0$& $H_{II}$: $J$ \\
\hline\textbf{A.} DGP $B$&(1)&0.99&0.01&0.00&1.00&0.00&0.00\\
&(2)&0.49&0.36&0.15&1.00&0.00&0.00\\
&(3)&0.27&0.40&0.33&0.98&0.02&0.00\\
&(4)&0.00&0.02&0.98&0.91&0.09&0.00\\
\midrule
\textbf{B.} DGP $J$&(1)&0.00&0.00&1.00&0.00&0.03&0.97\\
&(3)&0.00&0.00&1.00&0.00&0.06&0.94\\
\hline\multicolumn{7}{l}{\footnotesize{(1) baseline: $\sigma^2_\omega=0.2,\:\sigma_{\xi\omega}=0,\:\:\sigma_x=3$}} \\
\multicolumn{7}{l}{\footnotesize{(2) $\sigma^2_\omega=1,\:\sigma_{\xi\omega}=0,\:\:\sigma_x=3$}} \\
\multicolumn{7}{l}{\footnotesize{(3) $\sigma^2_\omega=1,\:\sigma_{\xi\omega}=0.4,\:\:\sigma_x=3$}} \\
\multicolumn{7}{l}{\footnotesize{(4) $\sigma^2_\omega=1,\:\sigma_{\xi\omega}=0.4,\:\:\sigma_x=2$}} \\
\bottomrule\end{tabular}


==> Output/old/TabRV_BM_B.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{4pt}}lcccccc}
\toprule
& \multicolumn{3}{c}{RSS Test}& \multicolumn{3}{c}{RV Test}\\
\cline{2-4}\cline{5-7}Version& $H_I$: $B$& $H_0$& $H_{II}$: $J$& $H_I$: $B$& $H_0$& $H_{II}$: $J$ \\
\cline{2-2}\cline{3-3}\cline{4-4}\cline{5-5}\cline{6-6}\cline{7-7}(1)&0.99&0.01&0.00&1.00&0.00&0.00\\
(2)&0.49&0.36&0.15&1.00&0.00&0.00\\
(3)&0.27&0.40&0.33&0.98&0.02&0.00\\
(4)&0.00&0.02&0.98&0.91&0.09&0.00\\
\hline\multicolumn{7}{l}{\footnotesize{(1) baseline: $\sigma^2_\omega=0.2,\:\sigma_{\xi\omega}=0,\:\:\sigma_x=3$}} \\
\multicolumn{7}{l}{\footnotesize{(2) $\sigma^2_\omega=1,\:\sigma_{\xi\omega}=0,\:\:\sigma_x=3$}} \\
\multicolumn{7}{l}{\footnotesize{(3) $\sigma^2_\omega=1,\:\sigma_{\xi\omega}=0.4,\:\:\sigma_x=3$}} \\
\multicolumn{7}{l}{\footnotesize{(4) $\sigma^2_\omega=1,\:\sigma_{\xi\omega}=0.4,\:\:\sigma_x=2$}} \\
\bottomrule\end{tabular}


==> Output/old/TabRV_BM_M.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{4pt}}lcccccc}
\toprule
& \multicolumn{3}{c}{RSS Test}& \multicolumn{3}{c}{RV Test}\\
\cline{2-4}\cline{5-7}Version& $H_I$: $B$& $H_0$& $H_{II}$: $J$& $H_I$: $B$& $H_0$& $H_{II}$: $J$ \\
\cline{2-2}\cline{3-3}\cline{4-4}\cline{5-5}\cline{6-6}\cline{7-7}(1)&0.00&0.00&1.00&0.00&0.03&0.97\\
(3)&0.00&0.00&1.00&0.00&0.06&0.94\\
\hline\multicolumn{7}{l}{\footnotesize{(1) baseline: $\sigma^2_\omega=0.2,\:\sigma_{\xi\omega}=0,\:\:\sigma_x=3$}} \\
\multicolumn{7}{l}{\footnotesize{(3) $\sigma^2_\omega=1,\:\sigma_{\xi\omega}=0.4,\:\:\sigma_x=3$}} \\
\bottomrule\end{tabular}


==> Output/old/Tab_Comp_D_joint_base.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{5pt}}llcccccc}
\toprule
&& \multicolumn{3}{c}{DGP $B$}& \multicolumn{3}{c}{DGP $J$}\\
\cline{3-5}\cline{6-8}&Models& RV& AR& EB& RV& AR& EB \\
\cline{1-8}\textbf{A.} $N_m=200$&$B$ only&0.99&0.96&0.94&0.00&0.00&0.00\\
&$J$ only&0.00&0.00&0.00&1.00&0.98&0.96\\
&$B=J$&0.01&&&0.00&&\\
&Both &&0.00&0.00&&0.00&0.00\\
&Neither &&0.04&0.06&&0.02&0.04\\
\midrule
\textbf{B.} $N_m=2000$&$B$ only&1.00&0.95&0.97&0.00&0.00&0.00\\
&$J$ only&0.00&0.00&0.00&1.00&0.94&0.89\\
&$B=J$&0.00&&&0.00&&\\
&Both &&0.00&0.00&&0.00&0.00\\
&Neither &&0.05&0.03&&0.06&0.11\\
\bottomrule\end{tabular}

==> Output/old/Tab_Comp_D_joint_base_horiz.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{4pt}}lcccccccccccc}
\toprule
& \multicolumn{6}{c}{$N_m=200$}& \multicolumn{6}{c}{$N_m=2000$}\\
\cline{2-7}\cline{8-13}
& \multicolumn{3}{c}{DGP $B$}& \multicolumn{3}{c}{DGP $J$}& \multicolumn{3}{c}{DGP $B$}& \multicolumn{3}{c}{DGP $J$}\\
\cline{2-4}\cline{5-7}\cline{8-10}\cline{11-13}Models& RV& AR& EB& RV& AR& EB& RV& AR& EB& RV& AR& EB \\
\cline{1-13}$B$ only&0.99&0.96&0.99&0.00&0.00&0.00&1.00&0.95&0.95&0.00&0.00&0.00\\
$J$ only&0.00&0.00&0.00&1.00&0.98&0.98&0.00&0.00&0.00&1.00&0.94&0.92\\
$B=J$&0.01&&&0.00&&&0.00&&&0.00&&\\
Both &&0.00&0.00&&0.00&0.00&&0.00&0.00&&0.00&0.00\\
Neither &&0.04&0.01&&0.02&0.02&&0.05&0.05&&0.06&0.08\\
\bottomrule\end{tabular}



==> Output/old/Tab_Comp_D_joint_logit.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{5pt}}llcccccc}
\toprule
&& \multicolumn{3}{c}{DGP $B$}& \multicolumn{3}{c}{DGP $J$}\\
\cline{3-5}\cline{6-8}&Models& RV& AR& EB& RV& AR& EB \\
\cline{1-8}\textbf{A.} $N_m=200$&$B$ only&0.52&0.26&0.06&0.02&0.00&0.00\\
&$J$ only&0.00&0.00&0.00&0.48&0.88&0.49\\
&$B=J$&0.48&&&0.50&&\\
&Both &&0.04&0.00&&0.07&0.00\\
&Neither &&0.70&0.94&&0.05&0.51\\
\midrule
\textbf{B.} $N_m=2000$&$B$ only&0.78&0.02&0.00&0.00&0.00&0.00\\
&$J$ only&0.00&0.00&0.00&0.58&0.80&0.00\\
&$B=J$&0.22&&&0.42&&\\
&Both &&0.03&0.00&&0.02&0.00\\
&Neither &&0.95&1.00&&0.18&1.00\\
\bottomrule\end{tabular}

==> Output/old/Tab_Comp_D_joint_weak.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{5pt}}llcccccc}
\toprule
&& \multicolumn{3}{c}{DGP $B$}& \multicolumn{3}{c}{DGP $J$}\\
\cline{3-5}\cline{6-8}&Models& RV& AR& EB& RV& AR& EB \\
\cline{1-8}\textbf{A.} $N_m=200$&$B$ only&0.50&0.58&0.66&0.00&0.01&0.01\\
&$J$ only&0.00&0.02&0.00&0.34&0.52&0.46\\
&$B=J$&0.50&&&0.66&&\\
&Both &&0.36&0.01&&0.41&0.00\\
&Neither &&0.04&0.33&&0.06&0.53\\
\midrule
\textbf{B.} $N_m=2000$&$B$ only&0.62&0.63&0.50&0.00&0.00&0.00\\
&$J$ only&0.00&0.00&0.00&0.35&0.55&0.12\\
&$B=J$&0.38&&&0.65&&\\
&Both &&0.25&0.06&&0.34&0.00\\
&Neither &&0.12&0.44&&0.11&0.88\\
\bottomrule\end{tabular}

==> Output/old/Tab_Comp_S_2000_base.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{4pt}}lcccccc}
\toprule
& \multicolumn{3}{c}{DGP B}& \multicolumn{3}{c}{DGP J}\\
\cline{2-4}\cline{5-7}Models& RV& AR& EB& RV& AR& EB \\
\cline{1-7}$B$ only&1.00&0.93&&0.00&0.00&\\
$J$ only&0.00&0.00&&1.00&0.98&\\
$B=J$&0.00&&&0.00&&\\
Both $B$ and $J$&&0.00&&&0.00&\\
Neither $B$ nor $J$&&0.07&&&0.02&\\
\bottomrule\end{tabular}


==> Output/old/Tab_Comp_S_2000_logit.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{4pt}}lcccccc}
\toprule
& \multicolumn{3}{c}{DGP B}& \multicolumn{3}{c}{DGP J}\\
\cline{2-4}\cline{5-7}Models& RV& AR& EB& RV& AR& EB \\
\cline{1-7}$B$ only&1.00&0.01&&0.00&0.02&\\
$J$ only&0.00&0.02&&1.00&0.06&\\
$B=J$&0.00&&&0.00&&\\
Both $B$ and $J$&&0.00&&&0.00&\\
Neither $B$ nor $J$&&0.97&&&0.92&\\
\bottomrule\end{tabular}


==> Output/old/Tab_Comp_S_2000_logitweak.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{4pt}}lcccccc}
\toprule
& \multicolumn{3}{c}{DGP B}& \multicolumn{3}{c}{DGP J}\\
\cline{2-4}\cline{5-7}Models& RV& AR& EB& RV& AR& EB \\
\cline{1-7}$B$ only&0.95&0.33&&0.07&0.02&\\
$J$ only&0.00&0.01&&0.82&0.17&\\
$B=J$&0.05&&&0.11&&\\
Both $B$ and $J$&&0.08&&&0.12&\\
Neither $B$ nor $J$&&0.58&&&0.69&\\
\bottomrule\end{tabular}


==> Output/old/Tab_Comp_S_joint_base.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{5pt}}llcccccc}
\toprule
&& \multicolumn{3}{c}{DGP $B$}& \multicolumn{3}{c}{DGP $J$}\\
\cline{3-5}\cline{6-8}&Models& RV& AR& EB& RV& AR& EB \\
\cline{1-8}\textbf{A.} $N_m=200$&$B$ only&0.78&0.96&&0.00&0.00&\\
&$J$ only&0.00&0.00&&1.00&0.96&\\
&$B=J$&0.22&&&0.00&&\\
&Both &&0.00&&&0.00&\\
&Neither &&0.04&&&0.04&\\
\midrule
\textbf{B.} $N_m=2000$&$B$ only&1.00&0.94&&0.00&0.00&\\
&$J$ only&0.00&0.00&&1.00&0.93&\\
&$B=J$&0.00&&&0.00&&\\
&Both &&0.00&&&0.00&\\
&Neither &&0.06&&&0.07&\\
\bottomrule\end{tabular}

==> Output/old/Tab_Comp_S_joint_logit.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{5pt}}llcccccc}
\toprule
&& \multicolumn{3}{c}{DGP $B$}& \multicolumn{3}{c}{DGP $J$}\\
\cline{3-5}\cline{6-8}&Models& RV& AR& EB& RV& AR& EB \\
\cline{1-8}\textbf{A.} $N_m=200$&$B$ only&1.00&0.05&&0.00&0.03&\\
&$J$ only&0.00&0.02&&1.00&0.46&\\
&$B=J$&0.00&&&0.00&&\\
&Both &&0.05&&&0.05&\\
&Neither &&0.88&&&0.46&\\
\midrule
\textbf{B.} $N_m=2000$&$B$ only&1.00&0.03&&0.00&0.00&\\
&$J$ only&0.00&0.01&&1.00&0.02&\\
&$B=J$&0.00&&&0.00&&\\
&Both &&0.00&&&0.00&\\
&Neither &&0.96&&&0.98&\\
\bottomrule\end{tabular}

==> Output/old/Tab_Comp_S_joint_weak.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{5pt}}llcccccc}
\toprule
&& \multicolumn{3}{c}{DGP $B$}& \multicolumn{3}{c}{DGP $J$}\\
\cline{3-5}\cline{6-8}&Models& RV& AR& EB& RV& AR& EB \\
\cline{1-8}\textbf{A.} $N_m=200$&$B$ only&0.79&0.20&&0.03&0.10&\\
&$J$ only&0.00&0.03&&0.72&0.16&\\
&$B=J$&0.21&&&0.25&&\\
&Both &&0.44&&&0.45&\\
&Neither &&0.33&&&0.29&\\
\midrule
\textbf{B.} $N_m=2000$&$B$ only&0.68&0.25&&0.03&0.01&\\
&$J$ only&0.01&0.03&&0.80&0.32&\\
&$B=J$&0.31&&&0.17&&\\
&Both &&0.37&&&0.28&\\
&Neither &&0.35&&&0.39&\\
\bottomrule\end{tabular}

==> Output/old/Tab_Comp_base_slides.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{5pt}}lcccccccc}
\toprule
& \multicolumn{4}{c}{DGP $B$}& \multicolumn{4}{c}{DGP $C$}\\
\cline{2-5}\cline{6-9}Models& RV& AR& EB&Cox& RV& AR& EB &Cox\\
\cline{1-9}&\multicolumn{8}{c}{\textbf{Panel A.} $N_m=200$}\\
$B$ only&1.00&0.94&0.96&0.97&0.00&0.00&0.00&0.00\\
$C$ only&0.00&0.00&0.00&0.00&0.99&0.94&0.97&0.99\\
$B=C$&0.00&&&&0.01&&&\\
Both&&0.00&0.00&0.00&&0.00&0.00&0.00\\
Neither&&0.06&0.04&0.03&&0.06&0.03&0.01\\
\midrule&\multicolumn{8}{c}{\textbf{Panel B.} $N_m=2000$}\\
$B$ only&1.00&0.92&0.93&0.97&0.00&0.00&0.00&0.00\\
$C$ only&0.00&0.00&0.00&0.00&1.00&0.94&0.95&0.96\\
$B=C$&0.00&&&&0.00&&&\\
Both&&0.00&0.00&0.00&&0.00&0.00&0.00\\
Neither&&0.08&0.07&0.03&&0.06&0.05&0.04\\
\bottomrule
\end{tabular}

==> Output/old/Tab_Comp_logit_slides.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{5pt}}lcccccccc}
\toprule
& \multicolumn{4}{c}{DGP $B$}& \multicolumn{4}{c}{DGP $C$}\\
\cline{2-5}\cline{6-9}Models& RV& AR& EB&Cox& RV& AR& EB &Cox\\
\cline{1-9} &\multicolumn{8}{c}{\textbf{Panel A.} $N_m=200$}\\
$B$ only& \only<2>{\cellcolor{yellow}}0.78& 0.48& 0.41& 0.24&0.00&0.00&0.00&0.00\\
$C$ only&0.00&0.00&0.00&0.07& \only<2>{\cellcolor{yellow}}0.98& 0.43& 0.39& 0.37\\
$B=C$&0.22&&&&0.02&&&\\
Both&&0.01&0.00&0.17&&0.00&0.00&0.02\\
Neither&&\only<2>{\cellcolor{yellow}}0.51&\only<2>{\cellcolor{yellow}}0.59&\only<2>{\cellcolor{yellow}}0.52&&\only<2>{\cellcolor{yellow}}0.57&\only<2>{\cellcolor{yellow}}0.61&\only<2>{\cellcolor{yellow}}0.61\\

\midrule&\multicolumn{8}{c}{\textbf{Panel B.} $N_m=2000$}\\
$B$ only& \only<3>{\cellcolor{yellow}}1.00& \only<3>{\cellcolor{yellow}}0.00& \only<3>{\cellcolor{yellow}}0.00& \only<3>{\cellcolor{yellow}}0.00&0.00&0.00&0.00&0.00\\
$C$ only&0.00&0.00&0.00&0.00& \only<3>{\cellcolor{yellow}}1.00&0.00&0.00&0.00\\
$B=C$&0.00&&&&0.00&&&\\
Both&&0.00&0.00&0.00&&0.00&0.00&0.00\\
Neither&& \only<3>{\cellcolor{yellow}}1.00& \only<3>{\cellcolor{yellow}}1.00& \only<3>{\cellcolor{yellow}}1.00&& \only<3>{\cellcolor{yellow}}1.00& \only<3>{\cellcolor{yellow}}1.00& \only<3>{\cellcolor{yellow}}1.00\\
\bottomrule
\end{tabular}

==> Output/old/Tab_Comp_rss_slides.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{4pt}}lcccccc}
\toprule
& \multicolumn{3}{c}{RSS Test}& \multicolumn{3}{c}{RV Test}\\
\cline{2-4}\cline{5-7}Models& $H_I$: $B$& $H_0$& $H_{II}$: $C$& $H_I$: $B$& $H_0$& $H_{II}$: $C$ \\
\cline{1-7}\multicolumn{7}{c}{Panel A. DGP B}\\
(1)&1.00&0.00&0.00&1.00&0.00&0.00\\
(2)&0.17&0.80&0.03&1.00&0.00&0.00\\
(3)&0.00&0.21&0.79&0.94&0.06&0.00\\
(4)&0.00&0.10&0.90&0.93&0.07&0.00\\
\cline{1-7}\multicolumn{7}{c}{Panel B. DGP C}\\ (1)&0.00&0.00&1.00&0.00&0.00&1.00\\
(2)&0.00&0.00&1.00&0.00&0.01&0.99\\
(3)&0.00&0.00&1.00&0.00&0.13&0.87\\
(4)&0.00&0.00&1.00&0.00&0.13&0.87\\
\hline\multicolumn{7}{l}{\footnotesize{(1) $\sigma^2_\omega=0.2,\:\sigma_{\xi\omega}=0,\:\:\alpha=-1$}} \\
\multicolumn{7}{l}{\footnotesize{(2) $\sigma^2_\omega=0.2,\:\sigma_{\xi\omega}=0,\:\:\alpha=-1.5$ (baseline)}} \\
\multicolumn{7}{l}{\footnotesize{(3) $\sigma^2_\omega=0.5,\:\sigma_{\xi\omega}=0,\:\:\alpha=-1.5$}} \\
\multicolumn{7}{l}{\footnotesize{(4) $\sigma^2_\omega=0.5,\:\sigma_{\xi\omega}=0.3,\:\:\alpha=-1.5$}} \\
\bottomrule\end{tabular}


==> Output/tableCoopApp.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{\extracolsep{4pt}}lcccccc}
\toprule
	&RSS & RV &\multicolumn{2}{c}{AR}&\multicolumn{2}{c}{EB} \\
\cline{2-2}\cline{3-3}\cline{4-5}\cline{6-7}& & & $M_I$& $M_{II}$ &$M_I$& $M_{II}$\\
Statistic  &-12.70 &-4.70 &4.73 &23.38 & 0.05 & 3.85 \\
critical value    & $\pm$1.96 & $\pm$1.96 & 2.10  & 2.10 & $\pm$1.96  & $\pm$1.96\\
\bottomrule\end{tabular}

==> Proofs/old/Pf_ConvergDistrib_Misspecification.tex <==
\begin{proof}
%On top of the assumption of Proposition 2 that $\sqrt{n}\hat A_{z\Delta }= \rho + o_p(1),$ we also need a further assumption to define local alternatives, this time involving the true markups $\Delta^*$:
%\begin{align}
%    \sqrt{n}(\hat A_{z\Delta^* } - \hat A_{z\Delta })&= %\rho^* + o_p(1),
%\end{align}
%so that:
%\begin{align}
%\sqrt{n}(\hat A_{ z\Delta^* }\theta_0 -\hat A_{z\Delta}\theta_m)&= A_{zz}^{-1} \rho^*\theta_0 + A_{zz}^{-1}\rho(\theta_0-\theta_m) + o_p(1).
%\end{align}

%We formally state the assumption as:
%\begin{assumption}
%    We assume that the models we consider satisfy the %following local alternatives property:
%    \begin{align}
%    \sqrt{n}(\hat A_{z\Delta^* } - \hat A_{z\Delta })&= \rho^* + o_p(1),
%\end{align}    
%where $\rho^*$ is a finite matrix.
%\end{assumption}

It is useful to note the following:
\begin{align}
\sqrt{n}(\hat A_{ z\Delta^* }\theta_0 -\hat A_{z\Delta}\theta_m)\hat A_{zz}^{-1} \sqrt{n}(\hat A_{ z\Delta^* }\theta_0 -\hat A_{z\Delta}\theta_m)& = E\bigg[\bigg(\theta_0\tilde\Delta^*_{ni} - \theta_m\tilde\Delta_{ni}\bigg)\bigg(\tilde\Delta^*_{ni}\theta_0 - \tilde\Delta_{ni}\theta_m\bigg)\bigg]+ o_p(1)\\
&=E\bigg[\bigg(\tilde\Delta^*_{n,0i} - \tilde\Delta_{n,mi}\bigg)^2\bigg]+ o_p(1)
\end{align}


\begin{itemize}
\item[\textbf{(i) - EB }] To derive the distribution of the test statistic, we first consider:
\begin{align*}
\sqrt{n}(\Delta'P_z\Delta)^{1/2}(\hat\theta - \theta_0)  &= \sqrt{n}(\Delta'P_z\Delta)^{-1/2}\Delta'P_zp - \sqrt{n}(\Delta'P_z\Delta)^{1/2}\theta_0\\
&= \sqrt{n}(\Delta'P_z\Delta)^{-1/2}\Delta'P_z(\Delta^*\theta_0 + \omega_0)- \sqrt{n}(\Delta'P_z\Delta)^{1/2}\theta_0\\
&= \sqrt{n}(\Delta'P_z\Delta)^{-1/2}\Delta'P_z(\Delta^*-\Delta)\theta_0 + \sqrt{n}(\Delta'P_z\Delta)^{-1/2}\Delta'P_z \omega_0\\
&= (\sqrt{n}\hat A_{\Delta z} \hat A_{z z}^{-1} \sqrt{n}\hat A_{z\Delta})^{-1/2}\sqrt{n}\hat A_{\Delta z} \hat A_{z z}^{-1}\sqrt{n}(\hat A_{z\Delta^*}-\hat A_{z\Delta})\theta_0 \\
&\qquad+(\sqrt{n}\hat A_{\Delta z} \hat A_{z z}^{-1} \sqrt{n}\hat A_{z\Delta})^{-1/2}\sqrt{n}\hat A_{\Delta z} \hat A_{z z}^{-1}\frac{z'\omega_0}{\sqrt{n}}\\
&\rightarrow_d{N}\biggl((\rho A_{zz}^{-1}\rho)^{-1/2}\rho A_{zz}^{-1}\rho^*\theta_0,\sigma^2_{\omega_0}\biggr)
\end{align*}
so that 
\begin{align*}
\sqrt{n}\frac{(\Delta'P_z\Delta)^{1/2}}{\hat\sigma_{\omega_0}}(\hat\theta - \theta_m)  &= \sqrt{n}\frac{(\Delta'P_z\Delta)^{1/2}}{\hat\sigma_{\omega_0}}(\hat\theta- \theta_0)  + \sqrt{n}\frac{(\Delta'P_z\Delta)^{1/2}}{\hat\sigma_{\omega_0}}(\theta_0- \theta_m)\\
&= \sqrt{n}\frac{(\sqrt{n}\hat A_{\Delta z} \hat A_{zz}^{-1} \sqrt{n}\hat A_{z\Delta})^{1/2}}{\hat\sigma_{\omega_0}}(\hat\theta- \theta_0)  +\frac{(\sqrt{n}\hat A_{\Delta z} \hat A_{zz}^{-1} \sqrt{n}\hat A_{z\Delta})^{1/2}}{\hat\sigma_{\omega_0}} (\theta_0- \theta_m)\\
&\rightarrow_d{N}\biggl( \frac{(\rho A_{zz}^{-1}\rho)^{-1/2}\rho A_{zz}^{-1}\rho^*\theta_0+(\rho A_{zz}^{-1}\rho)^{1/2}(\theta_0 - \theta_m)}{\hat\sigma_{\omega_0}},1\biggr)\\
&\rightarrow_d{N}\biggl( \frac{(\rho A_{zz}^{-1}\rho)^{1/2}((1+\lambda)\theta_0 - \theta_m)}{\hat\sigma_{\omega_0}},1\biggr)\\
\end{align*}
where $\lambda =(\rho A_{zz}^{-1}\rho)^{-1}\rho A_{zz}^{-1}\rho^*$.  Thus,
\begin{align}
    T^{EB}&\rightarrow_d\chi^2_{2}\bigg(\frac{((1+\lambda)\theta_0 - \theta_m)'(\rho A_{zz}^{-1}\rho)((1+\lambda)\theta_0 - \theta_m)}{\sigma_{\omega_0}^2}\bigg)\\
    &= \chi^2_{2}\bigg(\frac{((1+\lambda)\theta_0 - \theta_m)' E[\tilde\Delta_{ni}\tilde\Delta_{ni}'] ((1+\lambda)\theta_0 - \theta_m)}{\sigma_{\omega_0}^2}\bigg)
\end{align}

\item[\textbf{(ii) - AR }] To derive the distribution of the test statistic, we first consider:
\begin{align*}
\sqrt{n}\hat\pi_m  &= \sqrt{n}(z'z)^{-1}z'(p - \Delta\theta_m)\\
&= \sqrt{n}(z'z)^{-1}z'(\Delta^*\theta_0 + \omega_0 - \Delta\theta_m)\\
&= \hat A_{zz}^{-1}\sqrt{n}(\hat A_{z'\Delta^*}\theta_0-\hat A_{z'\Delta}\theta_m) + \hat A_{zz}^{-1}\frac{z'\omega_0}{\sqrt{n}} \\
&\rightarrow_d \mathcal{N}\biggl(A_{zz}^{-1} \rho^*\theta_0 + A_{zz}^{-1}\rho(\theta_0-\theta_m) ,A_{zz}^{-1}\sigma^2_{\omega_0}\biggr) 
\end{align*}
Thus,
\begin{align}
    T^{AR}&\rightarrow_d\chi^2_{d_z}\bigg(\frac{( \rho^*\theta_0 +\rho(\theta_0-\theta_m))' A_{zz}^{-1}( \rho^*\theta_0 +\rho(\theta_0-\theta_m)) }{\sigma_{\omega_0}^2}\bigg)\\
  &=\chi^2_{d_z}\bigg(\frac{E[(\tilde\Delta^*_{n,0i} - \tilde\Delta_{n,mi})^2]}{\sigma_{\omega_0}^2}\bigg)  
\end{align}

\item[\textbf{(iii) - RV }]
\begin{align*}
\sqrt{n}(Q_1 - Q_2) &= \bigg(\sqrt{n}\bigg(\hat\psi_1-2\hat\psi_0 +  \hat\psi_2 \bigg) +\sqrt{n}(\Gamma_1 + \Gamma_2 - 2\Gamma_0)\bigg)'\frac{z'z}{n}\bigg(\hat\psi_1 -\hat\psi_2+\Gamma_1 - \Gamma_2\bigg)+\\&\qquad 2\bigg(\hat\psi_2-\hat\psi_1 +\Gamma_2-\Gamma_1\bigg)'\frac{z'\omega_0}{\sqrt{n}}
  \end{align*}
Suppose $\hat\Gamma_1 + \hat\Gamma_2 - 2\hat\Gamma_0 = \frac{c}{\sqrt{n}}$. Further suppose that $\hat\Gamma_1-\hat\Gamma_2 =d\neq 0$.  Then we have
\begin{align*}
\sqrt{n}(Q_1 - Q_2) &= \bigg( c\bigg)'\frac{z'z}{n}\bigg(d\bigg)+ 2\bigg(d\bigg)'\frac{z'\omega_0}{\sqrt{n}}\\
&\rightarrow_d \mathcal{N}(c'A_{zz}d,4dA_{zz}d\sigma^2_{\omega_0})\\
&\rightarrow_d \mathcal{N}(\Gamma_0-\Gamma_1+\Gamma_0-\Gamma_2)'E[z_iz_i'](\Gamma_0-\Gamma_1-(\Gamma_0-\Gamma_2)),4dA_{zz}d\sigma^2_{\omega_0})\\
&\rightarrow_d \mathcal{N}E[(\tilde\Delta_{0i}-\tilde\Delta_{1i}+\tilde\Delta_{0i}-\tilde\Delta_{2i})'(\tilde\Delta_{0i}-\tilde\Delta_{1i}-(\tilde\Delta_{0i}-\tilde\Delta_{2i})]),4dA_{zz}d\sigma^2_{\omega_0})\\
&= \mathcal{N}E[(\tilde\Delta_{0i}-\tilde\Delta_{1i})^2+(\tilde\Delta_{0i}-\tilde\Delta_{2i})^2],4E[((\tilde\Delta_{0i}-\tilde\Delta_{1i}- (\tilde\Delta_{0i}-\tilde\Delta_{2i}))^2](\sigma^2_{\omega_0})\\
  \end{align*}
  So we have, under the approximation of the asymptotic variance given in (\ref{eq:avarapprox}):
\begin{align}
 T^{RV} 
&\rightarrow_p \lim_{n\rightarrow\infty} \sqrt{n}\frac{E[(\theta_0 \tilde\Delta^*_{i} -\theta_1 \tilde\Delta_i)^2] - E[(\theta_0 \tilde\Delta^*_{i} -\theta_2 \tilde\Delta_i)^2]}{\sigma_{RV}}\\
&\approx\lim_{n\rightarrow\infty} \sqrt{n}\frac{ E[(\theta_0 \tilde\Delta^*_{i} -\theta_1 \tilde\Delta_i)^2] - E[(\theta_0 \tilde\Delta^*_{i} -\theta_2 \tilde\Delta_i)^2]}{2\sigma_{\omega_0}\sqrt{E[(\tilde\Delta_{1i}-\tilde\Delta_{2i})^2]]}}\\
&=\lim_{n\rightarrow\infty}\sqrt{n} \frac{E\bigg[\bigg((\tilde\Delta^*_{0i}-\tilde\Delta^*_{1i}) +(\tilde\Delta^*_{1i}-\tilde\Delta_{1i}) \bigg)^2-\bigg((\tilde\Delta^*_{0i}-\tilde\Delta^*_{2i}) +(\tilde\Delta^*_{2i}-\tilde\Delta_{2i}) \bigg)^2\bigg]}{2\sigma_{\omega_0} \sqrt{E[(\tilde\Delta_{1i}-\tilde\Delta_{2i})^2]}}.
\end{align} 



Define
$$\hat B = \bigg((\theta_2-\theta_1)'\hat A_{\Delta z} \hat A_{zz}^{-1} \hat A_{z\Delta} (\theta_2-\theta_1)\bigg)^{-1/2}$$
To derive the distribution of the test statistic, we first consider:
\begin{align*}
\sqrt{n}\hat B(Q_1 - Q_2) 
&= \sqrt{n}\hat B\frac{1}{n}(\Delta^*\theta_0 - \Delta\theta_1+ \omega_0)' P_z(\Delta^*\theta_0- \Delta\theta_1+ \sqrt{n}\hat B\omega_0) \\
&\qquad - \sqrt{n}\hat B\frac{1}{n}(\Delta^*\theta_0 - \sqrt{n}\hat B\Delta\theta_2+ \omega_0)'  P_z(\Delta^*\theta_0 - \Delta\theta_2+ \omega_0)\\
&= \bigg((\theta_2-\theta_1)'\sqrt{n}\hat A_{\Delta z} \hat A_{zz}^{-1} \sqrt{n}\hat A_{z\Delta} (\theta_2-\theta_1)\bigg)^{-1/2}\times\\
&\qquad\qquad\sqrt{n}(\theta_0\hat A_{\Delta^*z} -\theta_1\hat A_{\Delta z})' \hat A_{zz}^{-1}\sqrt{n}(\hat A_{\Delta^*z}\theta_0 - \hat A_{\Delta z}\theta_1) \\
&\,\,- \bigg((\theta_2-\theta_1)'\sqrt{n}\hat A_{\Delta z} \hat A_{zz}^{-1} \sqrt{n}\hat A_{z\Delta} (\theta_2-\theta_1)\bigg)^{-1/2}\times \\
&\qquad\qquad\sqrt{n}(\theta_0\hat A_{\Delta^*z} -\theta_2\hat A_{\Delta z})' \hat A_{zz}^{-1}\sqrt{n}(\hat A_{\Delta^*z}\theta_0 - \hat A_{\Delta z}\theta_2) \\
&\,\,+ 2\bigg((\theta_2-\theta_1)'\sqrt{n}\hat A_{\Delta z} \hat A_{zz}^{-1} \sqrt{n}\hat A_{z\Delta} (\theta_2-\theta_1)\bigg)^{-1/2}\times \\
&\qquad\qquad(\theta_2-\theta_1)\sqrt{n}\hat A_{\Delta z} \hat A_{zz}^{-1} \frac{\omega_0'z}{\sqrt{n}}\\
&\rightarrow_d\mathcal{N}\biggl( \bigg((\theta_2-\theta_1)'\rho A_{zz}^{-1} \rho (\theta_2-\theta_1)\bigg)^{-1/2} \mu^{I,II},4\sigma^2_{\omega_0}\biggr)
\end{align*}
where
$$\mu^{I,II}= \bigg(\rho^*\theta_0 + \rho(\theta_0-\theta_1)\bigg)'A_{zz}^{-1}\bigg(\rho^*\theta_0 + \rho(\theta_0-\theta_1)\bigg)-\bigg(\rho^*\theta_0 + \rho(\theta_0-\theta_2)\bigg)'A_{zz}^{-1}\bigg(\rho^*\theta_0 + \rho(\theta_0-\theta_2)\bigg)$$
So that, if we square the RV test statistic, we obtain:
 \begin{align}
 (T^{RV})^2 &\rightarrow_d\chi^2_{1}\bigg(\frac{1}{4\sigma_{\omega_0}^2}\bigg(\frac{E[(\tilde\Delta^*_{n,0i} - \tilde\Delta_{n,1i})^2]}{E[(\tilde\Delta_{n,1i} - \tilde\Delta_{n,2i})^2]^{1/2}}-\frac{E[(\tilde\Delta^*_{n,0i} - \tilde\Delta_{n,2i})^2]}{E[(\tilde\Delta_{n,1i} - \tilde\Delta_{n,2i})^2]^{1/2}}\bigg)^2\bigg).
% &= \chi^2_{1}\bigg(\frac{{c^*_{1}^2}/{c_{1,2}}-{c^*_{2}^2}/{c_{1,2}}}{4\sigma_{\omega_0}^2}\bigg) 
\end{align}

\item[\textbf{(iv) - Cox }] To derive the distribution of the test statistic consider:
\begin{align*}
\sqrt{n}\hat B T^{Cox,m}&= \sqrt{n}\hat B \bigg( Q_{-m}-Q_m -\frac{1}{n}(g_m - g_{-m} )'W(g_m - g_{-m} )\bigg)\\
&=\sqrt{n} \hat B ( Q_{-m}-Q_m)-\sqrt{n} \hat B (\theta_m - \theta_{-m})'\hat A_{\Delta z}\hat A_{zz}^{-1}\hat A_{z\Delta}(\theta_m - \theta_{-m})\\
&=\sqrt{n} \hat B ( Q_{-m}-Q_m) -  \bigg((\theta_2-\theta_1)'\sqrt{n}\hat A_{\Delta z} A_{zz}^{-1}\sqrt{n} \hat A_{z\Delta} (\theta_2-\theta_1)\bigg)^{-1/2}\times \\
&\qquad(\theta_m - \theta_{-m})'\sqrt{n}\hat A_{\Delta z}\hat A_{zz}^{-1}\sqrt{n}\hat A_{z\Delta}(\theta_m - \theta_{-m})\\
&\rightarrow_d\mathcal{N}( \bigg((\theta_m-\theta_{-m})'\rho A_{zz}^{-1} \rho (\theta_m-\theta_{-m})\bigg)^{-1/2} \mu^{cox,m},4\sigma^2_{\omega_0})
\end{align*}
where
\begin{align*}
\mu^{cox,m}&= \bigg(\rho^*\theta_0 + \rho(\theta_0-\theta_{-m})\bigg)'A_{zz}^{-1}\bigg(\rho^*\theta_0 + \rho(\theta_0-\theta_{-m})\bigg)\\
&\qquad-\bigg(\rho^*\theta_0 + \rho(\theta_0-\theta_m)\bigg)'A_{zz}^{-1}\bigg(\rho^*\theta_0 + \rho(\theta_0-\theta_m)\bigg)\\
&\qquad -(\theta_{-m}-\theta_{m})'\rho'A_{zz}^{-1}\rho(\theta_{-m}-\theta_{m})
\end{align*}
%\footnote{If $\theta_{-m} = \theta_0$ and $\Delta^* = \Delta$, then $\rho^* = 0$ and $\mu^{cox,m} = 2\mu^{I,II}$.  Meanwhile if $\theta_m = \theta_0$, $\mu^{cox,m} = 2\mu^{I,II} = 0$}
So that, if we square the Cox test statistic, we obtain:
 \begin{align}
 (T^{cox})^2 &\rightarrow_d\chi^2_{1}\bigg(
 \bigg(\frac{E[(\tilde\Delta^*_{n,0i} - \tilde\Delta_{n,1i})^2] - E[(\tilde\Delta^*_{n,0i} - \tilde\Delta_{n,2i})^2] - E[(\tilde\Delta_{n,1i} - \tilde\Delta_{n,2i})^2]}{2\sigma_{\omega_0}E[(\tilde\Delta_{n,1i} - \tilde\Delta_{n,2i})^2]^{1/2}}\bigg)^2\bigg)\\
 &= \chi^2_{1}\bigg(\frac{{c^{*2}_{1}}/{c_{1,2}}-{c^{*2}_{2}}/{c_{1,2}}-{c_{1,2}}}{4\sigma_{\omega_0}^2}\bigg) 
  \end{align}
  
\end{itemize}
\end{proof}

==> Proofs/old/Pf_ConvergDistrib_NoMisspecification.tex <==
\textbf{Remarks on Local Alternatives} - We start with some preliminary discussion of our definition of local alternatives.
We assume in Proposition 2 that: 
\begin{align}
    \hat A_{z\Delta} = \frac{z'\Delta}{n} = \frac{\rho}{\sqrt{n}} + o_p(n^{-1/2}), \label{eq:localAltI}
\end{align}    
where $\rho$ is a finite matrix, which intuitively means that the covariation between instruments and markups implied by the two models vanishes as the sample size increases. In the spirit of local power analysis, this is not a restriction to take literally, but rather to use as a tool to approximate the finite sample power of the tests we consider in a challenging environment where the two models are hard to tell apart. 

Most standard local power analysis is done by imposing that the parameters that characterize the alternative hypothesis get closer to the truth at a certain rate. In the spirit of the literature on non-nested hypothesis testing and model testing (e.g. Pesaran, 1982; Smith, 1992), we adopt instead a restriction on the joint distribution of the data $(z,\Delta),$ imposing that a certain moment vanishes at a rate that allows to control the asymptotic distribution of the test statistics under the alternative hypothesis. 

It is worth noticing some of the implications of our assumption (\ref{eq:localAltI}). First, notice that our definition of local alternatives implies that:
\begin{align}
g_m=\frac{z'\omega_m}{n} = \frac{g}{\sqrt{n}} + o_p(n^{-1/2}). \label{eq:localAltII}
\end{align}
where $g$ is a finite $d_z-$vector.
In fact consider:
\begin{align}
    g_m &=\frac{z'(\omega_0 + \Delta(\theta_0 - \theta_m))}{n}\\
        &= \frac{z'\Delta}{n} (\theta_0 - \theta_m) + o_p(1)  \label{eq:localAltIII}
\end{align}
Then, if (\ref{eq:localAltI}) holds, it follows immediately that $g_m=\frac{\rho}{\sqrt{n}} (\theta_0 - \theta_m) + o_p(n^{-1/2})$, which implies that (\ref{eq:localAltII}) holds for $g=\rho (\theta_0 - \theta_m)$. The condition (\ref{eq:localAltII}) is similar to the definition of local alternatives adopted in Marmer and Otsu (2012).

Notice moreover that we can write the estimator of the first stage parameter $\hat \Gamma$ as:
\begin{align*}
    \hat \Gamma = (\frac{z'z}{n})^{-1}\frac{z'\Delta}{n},
\end{align*}
so that its population equivalent is 
\begin{align*}
    \Gamma = \Gamma_n = A_{zz}^{-1}\frac{g}{\sqrt{n}},
\end{align*}
where the last equality follows from assumption (\ref{eq:localAltI}). Hence, our assumption, though stronger, implies the condition on $\Gamma$ routinely used to analyze asymptotics with weak instruments (Stock and Staiger, 1997). 

\begin{proof}[Proof of Proposition 2]
We will use in what follows the following facts, which are a consequence of the assumptions of the proposition:
\begin{align}
    \sqrt{n}\hat A_{\Delta z} &= \rho + o_p(1)\\
    \hat A_{z z} &= A_{z z} + o_p(1)\\
    \frac{z'\omega_0}{\sqrt{n}} &\rightarrow_d N(0,A_{z z}\sigma_{\omega_0}^2)\\
    \hat \sigma^2_{\omega_0} &= \sigma_{\omega_0}^2 + o_p(1)
\end{align}
The latter three statements follow from the standard assumptions required for the consistency and asymptotic normality of the GMM estimator $\hat \theta,$ and homoscedasticity of the error terms.
To derive the non-centrality parameter, it is also useful to note:
\begin{align}
\sqrt{n}\hat A_{\Delta z}\hat A_{zz}^{-1} & = \Gamma_n + o_p(1)\\
\sqrt{n}\hat A_{\Delta z}\hat A_{zz}^{-1} z & = \tilde\Delta_n + o_p(1)\\
\sqrt{n}\hat A_{\Delta z}\hat A_{zz}^{-1} \sqrt{n}\hat A_{z\Delta} &= \sqrt{n}\hat A_{\Delta z}\hat A_{zz}^{-1}\hat A_{zz}\hat A_{zz}^{-1} \sqrt{n}\hat A_{z\Delta}  \\&=E[\rho' A_{zz}^{-1} z_i z_i' A_{zz}^{-1} \rho] + o_p(1) \\&= E[\tilde\Delta_{ni}\tilde\Delta_{ni}'] + o_p(1)
\end{align}
These statements are either definitions, or follow from the assumptions above.

We assume in the proposition that the true parameter is $\theta_0$ and the null hypothesis for AR, EB and Cox is model $m$ such that $\theta_m\neq\theta_0$. We also define the constant:
\begin{align}
c = (\theta_0 - \theta_m)'E[\tilde\Delta_{ni}\tilde\Delta_{ni}'](\theta_0 - \theta_m).
\end{align}


\item[\textbf{(i) - EB}] For EB, notice that - since under our assumptions the variance of the estimator is 
\begin{align}
    \hat V_{\theta} = (\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1} \hat \sigma^2_{\omega_0}
\end{align}

the Wald test statistic for the null $\theta_0 = \theta_m$ can be written as :
\begin{align}
T^{EB,m} &= \frac{\zeta'\zeta}{\hat \sigma^2_{\omega_0}/ \sigma_{\omega_0}^2} \label{eq:TestStatEB_Pesaran}
\end{align}
where 
\begin{align}
    \zeta = \frac{(\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{1/2}}{\sigma_{\omega_0}}(\sqrt{n}(\hat\theta - \theta_m))
\end{align}
Notice moreover that
\begin{align*}
\hat\theta  &= (\Delta'P_z\Delta)^{-1}\Delta'P_zp \\
&= \theta_0 + (\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}\hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{n},
\end{align*}
so that 
\begin{align*}
    \zeta &= \frac{(\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{1/2}}{\sigma_{\omega_0}}(\sqrt{n}(\theta_0 - \theta_m)) + \frac{(\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1/2}}{\sigma_{\omega_0}} \hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{\sqrt{n}}\\
    &= \frac{(\sqrt{n}\hat A_{\Delta z} \hat A_{z z}^{-1}  \sqrt{n} \hat A_{z\Delta})^{1/2}}{\sigma_{\omega_0}}(\theta_0 - \theta_m) + \frac{(\sqrt{n}\hat A_{\Delta z} \hat A_{z z}^{-1} \sqrt{n}\hat A_{z\Delta})^{-1/2}}{\sigma_{\omega_0}} \sqrt{n}\hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{\sqrt{n}}
\end{align*}
from which it follows that, by applying the generalized Slutsky theorem and the facts stated above, that:

\begin{align*}
    \zeta \rightarrow_d N\bigg(\frac{(\rho' A_{z z}^{-1}  \rho)^{1/2}}{\sigma_{\omega_0}}(\theta_0 - \theta_m),1\bigg).
\end{align*}

Hence, using the definition of the EB test statistic in Equation (\ref{eq:TestStatEB_Pesaran}), we have the following convergence in distribution result:

\begin{align}
    T^{EB}\rightarrow_d\chi^2_{2}\bigg(\frac{c}{\sigma_{\omega_0}^2}\bigg),
\end{align}
since
\begin{align*}
    (\theta_0 - \theta_m)'\rho' A_{z z}^{-1}  \rho(\theta_0 - \theta_m) = c.   
\end{align*}

\item[\textbf{(ii) - AR}] For AR, we first consider the estimator $\hat\pi_m$
\begin{align*}
\hat\pi_m  &= (z'z)^{-1}z'(p - \Delta\theta_m)\\
&= \hat A_{zz}^{-1}\hat A_{z'\Delta}(\theta_0-\theta_m) + \hat A_{zz}^{-1}\frac{z'\omega_0}{n}, 
\end{align*}
and, under the assumption of homoskedasticity, $\hat V_{\pi_m}$, a consistent estimator of the asymptotic variance $V_{\pi_m}$,  is:
\begin{align}
V_{\pi_m} = \sigma^2_{\omega_{0}}A_{z z}^{-1} .  
\end{align}

So, we have
\begin{align}
\sqrt{n}\hat V_{\pi_m}^{-1/2} \hat\pi_m &=\bigg( \frac{\hat A_{zz}^{-1/2} \sqrt{n} \hat A_{z \Delta}'(\theta_0-\theta_m) +\hat A_{zz}^{-1/2} \frac{z'\omega_0}{\sqrt{n}}}{\hat\sigma_{\omega_0}}\bigg)\\
&\rightarrow_d \mathcal{N}\bigg( \frac{A_{zz}^{-1/2}\rho(\theta_0-\theta_m) }{\sigma_{\omega_0}},1\bigg),
\end{align}
and we can derive the asymptotic distribution of the AR test statistic:
\begin{align}
T^{AR,m} &\rightarrow_d \chi^2_{d_z}\bigg(\frac{(\theta_0-\theta_m)'\rho A_{zz}^{-1}\rho(\theta_0-\theta_m)}{\sigma^2_{\omega_{0}}}\bigg)\\
& =\chi^2_{d_z}\bigg(\frac{c}{\sigma^2_{\omega_{0}}}\bigg).
\end{align}


\item[\textbf{(iii) - RV}] First consider the object :
\begin{align*}
 Q_1 - Q_2&= g_1'Wg_1 - g_2'Wg_2\\
&=\frac{\omega^{I\prime} z}{n}(\frac{z'z}{n})^{-1}\frac{z'\omega^I}{n} - \frac{\omega^{II\prime} z}{n}(\frac{z'z}{n})^{-1}\frac{z'\omega^{II}}{n}\\
&= \frac{1}{n}(\Delta(\theta_0 - \theta_1)+ \omega_0)' P_z(\Delta(\theta_0 - \theta_1)+ \omega_0)- \frac{1}{n}(\Delta(\theta_0 -\theta_2)+ \omega_0)'  P_z(\Delta(\theta_0 - \theta_2)+ \omega_0)\\
&= -(\theta_1 - \theta_2)'\hat A_{z\Delta}'\hat A_{zz}^{-1}\hat A_{z\Delta}(\theta_1 - \theta_2)- 2(\theta_2 - \theta_1)'\hat A_{z\Delta}'\hat A_{zz}^{-1}\frac{z'\omega_0}{n}.
\end{align*}
Under the assumption of homoskedasticity, the estimator of the asymptotic variance of $\sqrt{n} (Q_1 - Q_2)$ is:
\begin{align}
    \hat\sigma_{RV}^2 = 4\hat\sigma_{\omega_0}^2(\theta_2 - \theta_1)'\hat A_{z \Delta}'\hat A_{zz}^{-1}\hat A_{z \Delta}(\theta_2 - \theta_1),
\end{align}
So that we can write:
\begin{align}
T^{RV} &= \sqrt{n}\frac{Q_1-Q_2}{\hat\sigma_{RV}}\\
&=-\frac{1}{2\hat\sigma_{\omega_0}}\bigg((\theta_2 - \theta_1)'\sqrt{n}\hat A_{z \Delta}'\hat A_{zz}^{-1}\sqrt{n}\hat A_{z \Delta}(\theta_2 - \theta_1)\bigg)^{1/2}\\
&\qquad  -\frac{1}{\hat\sigma_{\omega_0}}\bigg((\theta_2 - \theta_1)'\sqrt{n}\hat A_{z \Delta}'\hat A_{zz}^{-1}\sqrt{n}\hat A_{z \Delta}(\theta_2 - \theta_1)\bigg)^{-1/2}(\theta_2 - \theta_1)'\sqrt{n}\hat A_{z \Delta}'\hat A_{zz}^{-1}\frac{z'\omega_0}{\sqrt{n}}
\end{align}
For convergence in distribution, after applying the CLT, we have:
\begin{align}
T^{RV} &\rightarrow_d \mathcal{N}\bigg(\frac{\bigg((\theta_2 - \theta_1)'E[\tilde\Delta_{ni}\tilde\Delta_{ni}'](\theta_2 - \theta_1)\bigg)^{1/2}}{2\sigma_{\omega_0}},1\bigg)\\
&=\mathcal{N}\bigg(\frac{\bigg(E[(\tilde\Delta_{2ni}-\tilde\Delta_{1ni})^2]\bigg)^{1/2}}{2\sigma_{\omega_0}},1\bigg)\\
&=\mathcal{N}\bigg(\frac{\sqrt{c}}{2\sigma_{\omega_0}},1\bigg).
\end{align} 
Therefore
$$(T^{RV})^2\rightarrow_d \chi^2_{1}\bigg(\frac{c}{4\sigma^2_{\omega_0}} \bigg).$$


\item[\textbf{(iv) - Cox}] To derive the asymptotic distribution of the Cox test statistic, recall that $\theta_0 = \theta_{-m}$.  
Since the numerator of the test statistic is 
\begin{align*}
    \frac{\hat \sigma^{Cox,m}}{\sqrt{n}} T^{Cox,m} &=Q_{-m} - Q_m -(g_{-m} - g_m)'\hat A_{zz}^{-1}(g_{-m} - g_m),
\end{align*}
so that the first two terms equal the numerator of the RV test statistic. We conjecture (and verify at the end) that in this environment the asymptotic variance of the Cox test statistic is equal to the one of the RV test statistic, so that we can write
\begin{align*}
    T^{Cox,m} - T^{RV}=  - \frac{\sqrt{n}}{\hat \sigma^{RV}}(g_{-m} - g_m)'\hat A_{zz}^{-1}(g_{-m} - g_m),
\end{align*}
and for this term notice
\begin{align*}
- \frac{\sqrt{n}}{\hat \sigma^{RV}}(g_{-m} - g_m)'\hat A_{zz}^{-1}(g_{-m} - g_m)    &=-\frac{\sqrt{n}}{\hat \sigma^{RV}}(\theta_m - \theta_{-m})'\hat A_{z\Delta}' \hat A_{zz}^{-1} \hat A_{z\Delta}(\theta_m - \theta_{-m})\\
&= -\frac{1}{2 \hat \sigma_{\omega_0}}\bigg((\theta_m - \theta_{-m})'\sqrt{n}\hat A_{z\Delta}' \hat A_{zz}^{-1} \sqrt{n}\hat A_{z\Delta}(\theta_m - \theta_{-m})\bigg)^{1/2}\\
&\rightarrow_p -\frac{1}{2 \hat \sigma_{\omega_0}}\bigg((\theta_m - \theta_{-m})'E[\tilde\Delta_{ni}\tilde\Delta_{ni}'](\theta_m - \theta_{-m})\bigg)^{1/2}\\
&= -\frac{c^{1/2}}{2 \hat \sigma_{\omega_0}}
\end{align*}
So that, since this term converges in probability to a constant, the asymptotic variance for the Cox statistic that we conjecture is correct. In fact:
\begin{align}
    T^{Cox,m}\rightarrow_d N\bigg(\frac{c^{1/2}}{\hat \sigma_{\omega_0}},1\bigg)
\end{align}
\noindent Following the results above, we obtain 
\begin{align}
(T^{cox})^2 \rightarrow_d \chi^2_1\bigg(\frac{c}{\sigma^2_{\omega_0}}\bigg).
\end{align}

\end{proof}



==> Proofs/old/Pf_ConvergProb_NoMisspecification.tex <==
\begin{proof}
\noindent We start by proving the first part of the proposition in which we show that the modified test statistics converge in probability to constants that depend on $E[(\tilde\Delta_{0i}-\tilde\Delta_{mi})^2]$.
\begin{enumerate}
\item[\textbf{(i) - EB}] 
Consider the test statistic $T^{EB,m}$ under the assumptions of weight matrix $W=A_{zz}^{-1}$ and homoskedasticity. We first consider the object $\hat\theta$:
\begin{align*}
\hat\theta  &= \theta_0 + (\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}\hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{n}
\end{align*}
and
\begin{align}
\hat V_{\hat \theta}  &= \frac{\hat \sigma^2_{\omega_{0}}}{n}(\hat A_{\Delta z}  \hat A_{z z}^{-1}  \hat A_{z\Delta})^{-1}\\
&= \hat \sigma^2_{\omega_{0}}(\Delta' z (z' z)^{-1}  z'\Delta)^{-1}
\end{align}
so that:
\begin{align}
    T^{EB,m} =& (\theta_0 - \theta_m)'\hat V_{\hat \theta}^{-1} (\theta_0 - \theta_m) \\
    &+\frac{\frac{z'\omega_0}{\sqrt{n}} \hat A_{z z}^{-1}\hat A_{z \Delta }(\hat A_{\Delta z}  \hat A_{z z}^{-1}  \hat A_{z\Delta})^{-1}\hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{\sqrt{n}}} {\hat \sigma^2_{\omega_{0}}} \\
    &+2n\frac{(\theta_0 - \theta_m)'\hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{n}}{\hat\sigma^2_{\omega_{0}}}\\
= & \frac{(\tilde \Delta_0 - \tilde \Delta_m)'(\tilde \Delta_0 - \tilde \Delta_m)}{\hat \sigma^2_{\omega_0}} + \zeta_{EB}'\zeta_{EB} + \frac{2n}{\hat\sigma^2_{\omega_{0}}}\frac{(\tilde \Delta_0 - \tilde \Delta_m)'\omega_0}{n}
\end{align}

To derive the plim of the test statistic $T^{EB,m}$, we first consider the object $\hat\theta$:
\begin{align*}
\hat\theta  &= (\Delta'P_z\Delta)^{-1}\Delta'P_z(\Delta\theta_0 + \omega_0)\\
&= \theta_0 + (\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}\hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{n}\\
&\rightarrow_p \theta_0. 
\end{align*}

Now, from standard GMM theory the asymptotic variance of $\hat \theta$ under homoskedasticity of the error term is 
\begin{align}
V_{\theta}  &= \sigma^2_{\omega_{0}}(A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1} \\
    &= \sigma^2_{\omega_{0}}E[\tilde\Delta_{i}\tilde\Delta_{i}']^{-1}.
\end{align}

Since $\hat V_{\theta}$ is a consistent estimator of $V_{\theta}$ we have:
\begin{align}
\frac{T^{EB,m}}{n}&\rightarrow_p \frac{(\theta_0 - \theta_m)' E[\tilde\Delta_{i}\tilde\Delta_{i}'](\theta_0 - \theta_m)}{\sigma^2_{\omega_{0}}}\\
&= \frac{ E[(\tilde\Delta_{0i} - \tilde\Delta_{mi})^2]}{\sigma^2_{\omega_{0}}}
\end{align}



\item[\textbf{(ii) - AR}] 
To derive the plim of the test statistic $T^{AR,m}$, we first consider the object $\hat\pi_m$
\begin{align*}
\hat\pi_m  &= (z'z)^{-1}z'(\Delta\theta_0 + \omega_0 - \Delta\theta_m)\\
&= \hat A_{zz}^{-1}\hat A_{z'\Delta}(\theta_0-\theta_m) + \hat A_{zz}^{-1}\frac{z'\omega_0}{n} \\
&\rightarrow_p A_{zz}^{-1} A_{z'\Delta}(\theta_0-\theta_m) .
\end{align*}
Under the assumption of homoskedasticity, $V_{\pi_m}$  has the usual OLS form of:
\begin{align}
V_{\pi_m} &= \sigma^2_{\eta_{m}}A_{z z}^{-1}   
\end{align}
Since $\hat V_{\pi_m}$ is constructed to be a consistent estimator of $V_{\pi_m}$ we have
\begin{align}
\frac{T^{AR,m}}{n}&\rightarrow_p  (\theta_0-\theta_m)'  A_{\Delta'z}A_{zz}^{-1}V^{-1}_{\pi_m}A_{zz}^{-1} A_{z'\Delta}(\theta_0-\theta_m) \\
&=  \frac{(\theta_0-\theta_m)' \Gamma'E[z_iz_i']\Gamma(\theta_0-\theta_m) }{\sigma^2_{\eta_{m}}}\\
&=  \frac{E[(\tilde\Delta_{0i}-\tilde\Delta_{mi})^2] }{\sigma^2_{\eta_{m}}}.
\end{align}

\item[\textbf{(iii) - RV}] To derive the plim for $T^{RV}$, first consider the object $Q_1 - Q_2$:
\begin{align*}
Q_1 - Q_2 
&= g_1'Wg_1 - g_2'Wg_2\\
&= \frac{1}{n}(\Delta(\theta_0 - \theta_1)+ \omega_0)' P_z(\Delta(\theta_0 - \theta_1)+ \omega_0)- \frac{1}{n}(\Delta(\theta_0 -\theta_2)+ \omega_0)'  P_z(\Delta(\theta_0 - \theta_2)+ \omega_0)\\
& \rightarrow_p  E[(\tilde\Delta_{0i}-\tilde\Delta_{1i})^2]-E[(\tilde\Delta_{0i}-\tilde\Delta_{2i})^2]
\end{align*}
So that, assuming $\hat\sigma_{RV} \rightarrow_p \sigma_{RV}$, we have
\begin{align}
\frac{T^{RV}}{\sqrt{n}}&= \frac{Q_1 - Q_2}{\hat\sigma_{RV}} \\
&\rightarrow_p \frac{E[(\tilde\Delta_{0i}-\tilde\Delta_{1i})^2]-E[(\tilde\Delta_{0i}-\tilde\Delta_{2i})^2]}{\sigma_{RV}}
\end{align} 
which is consistent with Theorem 1 (ii) in \cite{rv02}.

\item[\textbf{(iv) - Cox}] For the Cox procedure, notice that the numerator of the test statistic is 
\begin{align*}
    Q_{-m} - Q_m -(g_{-m} - g_m)'A_{zz}^{-1}(g_{-m} - g_m), 
\end{align*}
for which we obtain
 \begin{align*}
&g_{-m}'A_{zz}^{-1}  g_{-m} -g_{m}'A_{zz}^{-1} g_m -(g_{-m} - g_m)'A_{zz}^{-1}(g_{-m} - g_m)\\
&\rightarrow_p (\theta_0 - \theta_{-m})'A_{z\Delta}'A_{zz}^{-1}A_{z\Delta}(\theta_0 - \theta_{-m}) - (\theta_0 - \theta_m)'A_{z\Delta}'A_{zz}^{-1}A_{z\Delta}(\theta_0 - \theta_m)\\
&\qquad-(\theta_m - \theta_{-m})'A_{z\Delta}'A_{zz}^{-1}A_{z\Delta}(\theta_m - \theta_{-m})\\
 &= E[(\tilde\Delta_{0i}-\tilde\Delta_{-mi})^2] -E[(\tilde\Delta_{0i}-\tilde\Delta_{mi})^2]  - E[(\tilde\Delta_{mi}-\tilde\Delta_{-mi})^2] \\
                          &= 2E[(\tilde\Delta_{0i}- \tilde\Delta_{mi})(\tilde\Delta_{-mi}-\tilde\Delta_{mi})]   
\end{align*}
So that, assuming $\hat\sigma_{Cox} \rightarrow_p \sigma_{Cox}$, we have
\begin{align}
\frac{T^{Cox,m}}{\sqrt{n}}&\rightarrow_p  \frac{ 2E[(\tilde\Delta_{0i}- \tilde\Delta_{mi})(\tilde\Delta_{-mi}-\tilde\Delta_{mi})] }{\sigma_{Cox}}.
\end{align} 

\end{enumerate}
To prove the second part of the proposition, that the tests are consistent, notice that for each test $y$, there exists an increasing function of n, $a_n$ such that
$\frac{T^{y,m}}{a_n} \rightarrow_p \zeta.$ The quantity $\zeta$ is positive and finite when $\theta_m\neq\theta_0$ and $E(\tilde\Delta_{0i}) \neq E(\tilde\Delta_{mi}).$ Hence, $T^{y,m}\rightarrow_p \infty,$ so that each test has power of one against fixed alternatives.
\end{proof}


==> Proofs/old/Pf_DemandSimSeq.tex <==
\begin{proof}
By definition of $\theta_m^{Dsim}$ and because $\theta^{Dseq}$ is the minimizer of $\mathcal{Q}^{dem}$, it must be that $\mathcal{Q}^{sim}_m(\theta_m^{Dsim}) < \mathcal{Q}^{sim}_m(\theta^{Dseq})$. In turn, this implies that $\mathcal{Q}_m(\theta_m^{Dsim}) < \mathcal{Q}_m(\theta^{Dseq})$ - if this inequality did not hold, we would need to have $\mathcal{Q}^{dem}(\theta^{Dseq})> \mathcal{Q}^{dem}(\theta^{Dsim})$. Since each objective function is assumed to have a unique minimizer, this last inequality is a contradiction. Moreover, in case 1. where cost shifters are correctly specified, we have  $\mathcal{Q}_{m}\left(\Delta(\theta^D)\right) = E[(\tilde \Delta^*_0 - \tilde \Delta_m(\theta^D))^2]$. Therefore, 
    \begin{align*}
        E[(\tilde \Delta^*_0 - \tilde \Delta_m(\theta_m^{Dsim}))^2] <         E[(\tilde \Delta^*_0 - \tilde \Delta_m(\theta^{Dseq}))^2].
    \end{align*}
In case 2. where cost shifters are misspecified, we have instead $\mathcal{Q}_{m}\left(\Delta(\theta^D)\right) = E[(\tilde \Delta^C_0 - \tilde \Delta_m(\theta^D))^2]$. Therefore, 
    \begin{align*}
        E[(\tilde \Delta^C_0 - \tilde \Delta_m(\theta_m^{Dsim}))^2] <         E[(\tilde \Delta^C_0 - \tilde \Delta_m(\theta^{Dseq}))^2].
    \end{align*}     
\end{proof}

==> Proofs/old/Pf_Fstats.tex <==
Specifically, we can compute F-statistics for two regressions (i) $2p-\Delta_1-\Delta_2$  on instruments and (ii) $\Delta_1-\Delta_2$ on instruments as follows, letting the residuals from these regressions be $\hat\zeta_1$ and $\hat\zeta_2$ respectively. 
\begin{align*}
    F_1 &= \frac{((z'z)^{-1}z'(2\Delta_0+2\omega_0-\Delta_1-\Delta_2))'z'z((z'z)^{-1}z'(z(2\Delta_0+2\omega_0-\Delta_1-\Delta_2))}{d_z\hat\sigma^2_{\zeta_1}},\\
&=    \frac{((z'z)^{-1}z'(z\frac{q_1+q_2}{\sqrt{n}}+\zeta_1))'z'z((z'z)^{-1}z'(z\frac{q_1+q_2}{\sqrt{n}}+\zeta_1))}{d_z\hat\sigma^2_{\zeta_1}},\\
&= \frac{ ( \hat A_{zz}^{1/2}(q_1+q_2)\hat A_{zz}^{-1/2}\frac{z'\zeta_1}{\sqrt{n}})'( \hat A_{zz}^{1/2}(q_1+q_2)+\hat A_{zz}^{-1/2}\frac{z'\zeta_1}{\sqrt{n}})}{d_z\hat\sigma^2_{\zeta_1}},\\
&= \frac{( \hat A_{zz}^{1/2}(q_1+q_2)+\hat A_{zz}^{-1/2}\frac{z'\zeta_1}{\sqrt{n}})'}{\sqrt{d_z}\hat\sigma_{\zeta_1}}\frac{( \hat A_{zz}^{1/2}(q_1+q_2)+\hat A_{zz}^{-1/2}\frac{z'\zeta_1}{\sqrt{n}})}{\sqrt{d_z}\hat\sigma_{\zeta_1}},\\
 d_z F_1&\rightarrow_d \chi^2_{d_z}(\pi_{01}'\pi_{01})
\end{align*}
where $\zeta_1=2\omega_0 + e_1 + e_2$ and $\sigma^2_{\zeta_1} = 4\sigma^2_{\omega_0} + \sigma^2_{e_1} + \sigma^2_{e_2} + 4\sigma_{\omega_0 e_1} + 4\sigma_{\omega_0 e_2} + 2\sigma_{e_1 e_2}=\Omega_{11}$.

Also, 
\begin{align*}
    F_2 &= \frac{(\hat\Gamma_1-\hat\Gamma_2)'z'z(\hat\Gamma_1-\hat\Gamma_2)}{d_z\hat\sigma^2_{\zeta_2}},\\
&=    \frac{((z'z)^{-1}z'(\Delta_1-\Delta_2))'z'z((z'z)^{-1}z'(\Delta_1-\Delta_2)}{d_z\hat\sigma^2_{\zeta_2}},\\
&=    \frac{((z'z)^{-1}z'(z\frac{q_1-q_2}{\sqrt{n}}+\zeta_2))'z'z((z'z)^{-1}z'(z\frac{q_1-q_2}{\sqrt{n}}+\zeta_2))}{d_z\hat\sigma^2_{\zeta_2}},\\
&= \frac{ ( \hat A_{zz}^{1/2}(q_1-q_2)+\hat A_{zz}^{-1/2}\frac{z'\zeta_2}{\sqrt{n}})'( \hat A_{zz}^{1/2}(q_1-q_2)+\hat A_{zz}^{-1/2}\frac{z'\zeta_2}{\sqrt{n}})}{d_z\hat\sigma^2_{\zeta_2}},\\
&= \frac{( \hat A_{zz}^{1/2}(q_1-q_2)+\hat A_{zz}^{-1/2}\frac{z'\zeta_2}{\sqrt{n}})'}{\sqrt{d_z}\hat\sigma_{\zeta_2}}\frac{( \hat A_{zz}^{1/2}(q_1-q_2)+\hat A_{zz}^{-1/2}\frac{z'\zeta_2}{\sqrt{n}})}{\sqrt{d_z}\hat\sigma_{\zeta_2}},\\
 d_z F_2&\rightarrow_d \chi^2_{d_z}(\pi_{02}'\pi_{02})
\end{align*}


==> Proofs/old/Pf_ManyInstr.tex <==


As a preliminary step, we define the first stage models as:
\begin{align*}
    \Delta &= z\Gamma + e\\
    \Delta^* &= z\Gamma^* + e^*.
\end{align*}
Further, we define $ \Sigma_{ee} = E[e_ie_i']$, $\Sigma_{ee^*} = E[e_ie^{*\prime}_i] $, and $\Sigma_{e\omega_0} = E[e_i\omega_{0i}']$.


\begin{proof}
We proceed in several steps:

\noindent \textbf{Step 1:} We first establish the following convergence in probability result:
\begin{align*}
    \hat A_{\Delta z}\hat A_{zz}^{-1}\hat A_{z\Delta} 
    %&= \frac{\Gamma'z'z\Gamma}{n} + \frac{\Gamma'z'e}{n} + \frac{e'z\Gamma}{n} + \frac{e'z(z'z)^{-1}z'e}{n}\\
    &\rightarrow_p H + \delta_z\Sigma_{ee}
\end{align*}
Note that, by plugging in the first stage equation for $\Delta$, we obtain:
\begin{align}
    \hat A_{\Delta z}\hat A_{zz}^{-1}\hat A_{z\Delta} 
    &= \underbrace{\frac{\Gamma'z'z\Gamma}{n}}_{I} + \underbrace{\frac{\Gamma'z'e}{n}}_{II} + \underbrace{\frac{e'z\Gamma}{n}}_{III} + \underbrace{\frac{e'z(z'z)^{-1}z'e}{n}}_{IV}
\end{align}
By Assumption \ref{as:manyinstr}, $I\rightarrow_p H$.  Now, consider $II$.  Following Hansen (2021, page 391), if we vectorize $II$, $Var(vec(II))\rightarrow_p 0$ which implies that $II \rightarrow_p0$.  By the same argument, $III\rightarrow_p 0$.  Finally, note that, by Equation 12.28 in Hansen 2021, for the $(j,k)^\text{th}$ element of IV, $E[IV_{jk} \mid z] \rightarrow_p \delta_{z} \Sigma_{ee}(j,k)$.  Further $Var[IV_{jk} \mid z] \rightarrow_p 0$.  Thus, by considering all elements and applying Markov's inequality,  in Equation 12.83, $IV\rightarrow_p \delta_z \Sigma$. \\ 

\noindent \textbf{Step 2:} We derive the plim of the RV numerator with a many instrument asymptotic:
\begin{align*}
Q_1 - Q_2 
&= (g_1-g_2)'W(g_1+g_2)\\
%&= \frac{1}{n}(\Delta(\theta_0 - \theta_1)+ \omega_0)' P_z(\Delta(\theta_0 - \theta_1)+ \omega_0)- \frac{1}{n}(\Delta(\theta_0 -\theta_2)+ \omega_0)'  P_z(\Delta(\theta_0 - \theta_2)+ \omega_0)\\
&= \frac{1}{n}\bigg(\theta_1-\theta_2\bigg)'\Delta'z(z'z)^{-1}z'\bigg(-2p + \Delta(\theta_1+\theta_2)\bigg)\\
    %&= \frac{1}{n}\bigg(\theta_1-\theta_2\bigg)'\Delta'z(z'z)^{-1}z'\Delta\bigg(\theta_1+\theta_2\bigg) -2 \frac{1}{n}\bigg(\theta_1-\theta_2\bigg)'\Delta'z(z'z)^{-1}z'p\\
   % &= \frac{1}{n}\bigg(\Delta_1-\Delta_2\bigg)'z(z'z)^{-1}z'\bigg(\Delta_1+\Delta_2\bigg) -2 \frac{1}{n}\bigg(\theta_1-\theta_2\bigg)'\Delta'z(z'z)^{-1}z'\Delta\hat\theta_{2SLS}\\
 %       &= \frac{1}{n}\bigg(\Gamma_1-\Gamma_2\bigg)(z'z)\bigg(\Gamma_1+\Gamma_2\bigg) -2 \frac{1}{n}\bigg(\theta_1-\theta_2\bigg)'\Gamma(z'z)\Gamma\hat\theta_{2SLS}\\
        &= \frac{1}{n}\bigg(\theta_1-\theta_2\bigg)'(\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})\bigg(\theta_1+\theta_2\bigg) -2 \frac{1}{n}\bigg(\theta_1-\theta_2\bigg)'(\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta}) \hat\theta_{2SLS}\\
        & \rightarrow_p  \bigg(\theta_1-\theta_2\bigg)(H+\delta_z \Sigma_{ee})\bigg(\theta_1+\theta_2\bigg) -2 \bigg(\theta_1-\theta_2\bigg)'(H+\delta_z \Sigma_{ee})\theta_{2SLS}, 
\end{align*}

\noindent Under the same many instrument asymptotics we derive $\theta_{2SLS}$, the plim of the 2SLS estimator:
\begin{align*}
\hat\theta_{2SLS}  &= (\Delta'P_z\Delta)^{-1}\Delta'P_zp\\
&=  (\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}\hat A_{\Delta z} \hat A_{z z}^{-1}\hat A_{z\Delta^*}\theta_0 +  (\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}\hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{n}\\
&=  \underbrace{(\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}}_{I}\underbrace{\hat A_{\Delta z} \hat A_{z z}^{-1}\hat A_{z\Delta^*}\theta_0}_{II} +  \underbrace{(\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}}_{I} \bigg(\underbrace{\frac{\Gamma'z'\omega_0}{n}}_{III} + \underbrace{\frac{e'z'(z'z)^{-1}z'\omega_0}{n}}_{IV}\bigg)
\end{align*}
By the results established in Step 1, $I\rightarrow_p H+\delta_z\Sigma_{ee}$.  By the same argument, $I\rightarrow_p H+\delta_z\Sigma_{ee^*}$.  Fianlly, we can show that $III\rightarrow_p \delta_z\Sigma_{e\omega_0}$.  Following the argument in Hansen (2021), $Var(vec(III))\rightarrow_p0$ so that $III\rightarrow_p 0$.  Finally, note that, by Equation 12.28 in Hansen 2021, for the $(j,k)^\text{th}$ element of IV, $E[IV_{jk} \mid z] \rightarrow_p \delta_{z} \Sigma_{e\omega_0}(j,k)$.  Further $Var[IV_{jk} \mid z] \rightarrow_p 0$.  Thus, by considering all elements and applying Markov's inequality,  in Equation 12.83, $IV\rightarrow_p \delta_z \Sigma_{e\omega_0}$.  Thus, $\theta_{2SLS}$ is given as
\begin{align*}
\theta_{2SLS} =  (H+\delta_z \Sigma_{ee})^{-1}(H^*+\delta_z \Sigma_{ee^*})\theta_0+(H+\delta_z \Sigma_{ee})^{-1}\delta_z \Sigma_{e \omega_0}
\end{align*}
So that:
\begin{align*}
    Q_1 - Q_2 %&\rightarrow_p \bigg(\theta_1-\theta_2\bigg)(H+\delta_z \Sigma_{ee})\bigg(\theta_1+\theta_2\bigg) -2 \bigg(\theta_1-\theta_2\bigg)'[(H^*+\delta_z \Sigma_{ee^*})\theta_0+\delta_z \Sigma_{e \omega_0}]\\
    &\rightarrow_p (\theta_1-\theta_2)\bigg(H(\theta_1+\theta_2)  -2 H^*\theta_0\bigg)  + \delta_z(\theta_1-\theta_2)'\bigg( \Sigma_{ee}(\theta_1+\theta_2)
    -2 \Sigma_{ee^*}\theta_0+ \Sigma_{e \omega_0}\bigg)
    %&= E[(\tilde\Delta_{1i}-\tilde\Delta^*_{0i})^2] - E[(\tilde\Delta_{2i}-\tilde\Delta^*_{0i})^2] + \delta_z\bigg( \sigma^2_{e_1}-\sigma^2_{e_2}
    %-2 \sigma_{e_0e^*_0}+2\sigma_{e_{-0}e^*_{0}}+ \sigma_{e_1 \omega_0}-\sigma_{e_2 \omega_0}\bigg)
\end{align*}

\noindent \textbf{Step 3:}  We show that when $\delta_z = 1$, $plim(Q_1-Q_2) = plim(Q^{RSS}_1-Q^{RSS}_2)$. Recall that, by Lemma \ref{lemma2}, $Q^{OLS}_1-Q^{OLS} = Q^{RSS}_1-Q^{RSS}$.  So, consider the numerator of the RSS statistic:
\begin{align*}
Q_1^{OLS} - Q_2^{OLS}
&= (g_1-g_2)'W(g_1+g_2)\\
%&= \frac{1}{n}(\omega_1'\Delta-\omega_2'\Delta)(\Delta'\Delta)^{-1}(\Delta'\omega_1+\Delta'\omega_2)\\
%&= ((p-\Delta_1)'-(p-\Delta_2)')\Delta(\Delta'\Delta)^{-1}\Delta'((p-\Delta_1)+(p-\Delta_2))\\
&= \frac{1}{n}(\Delta_2-\Delta_1)'\Delta(\Delta'\Delta)^{-1}\Delta'(2p-\Delta_1-\Delta_2)\\
%&= (\Delta_2-\Delta_1)'\Delta(\Delta'\Delta)^{-1}\Delta'(2\Delta^*_0-\Delta_1-\Delta_2) + (\Delta_2-\Delta_1)'\Delta(\Delta'\Delta)^{-1}\Delta'\omega_0 \\
&= \frac{1}{n}(\Delta_1-\Delta_2)'\Delta(\Delta'\Delta)^{-1}\Delta'(\Delta_1+\Delta_2) - 2\frac{1}{n}(\Delta_1-\Delta_2)'\Delta(\Delta'\Delta)^{-1}\Delta'p\\
%&= (\theta_1-\theta_2)'\Delta'\Delta(\Delta'\Delta)^{-1}\Delta'\Delta(\theta_1+\theta_2) - 2(\theta_1-\theta_2)'\Delta'\Delta\hat\theta_{OLS}\\
%&= (\theta_1-\theta_2)'\Delta'\Delta(\theta_1+\theta_2) - 2(\theta_1-\theta_2)'\Delta'\Delta\hat\theta_{OLS}\\
%&= \frac{1}{n}(\theta_1-\theta_2)'(z\Gamma+e)'(z\Gamma+e)(\theta_1+\theta_2) - 2\frac{1}{n}(\theta_1-\theta_2)'(z\Gamma+e)'(z\Gamma+e)\hat\theta_{OLS}\\
&= (\theta_1-\theta_2)'\bigg(\frac{\Gamma'z'z\Gamma}{n}+ \frac{\Gamma'z'e}{n} + \frac{e'z\Gamma}{n} + \frac{e'e}{n}\bigg) (\theta_1+\theta_2)  \\
&\qquad- 2(\theta_1-\theta_2)'\bigg(\frac{\Gamma'z'z\Gamma}{n}+ \frac{\Gamma'z'e}{n} + \frac{e'z\Gamma}{n} + \frac{e'e}{n}\bigg)\hat\theta_{OLS}\\
&\rightarrow_p (\theta_1-\theta_2)'(H + \Sigma_{ee}) (\theta_1+\theta_2)  
- 2(\theta_1-\theta_2)'(H + \Sigma_{ee})\theta_{OLS}
\end{align*}
It is easy to show that, when $\delta_z = 1$, $\theta_{2SLS} = \theta_{OLS}$.  Thus, when $\delta_z = 1$, $plim(Q_1-Q_2) = plim(Q^{OLS}_1-Q^{OLS}_2)$. We establish in Proposition \ref{prop:RSS} that $plim(Q^{OLS}_1-Q^{OLS}_2) = E[(\Delta_{1i}-\Delta_{OLSi})^2] - E[(\Delta_{2i}-\Delta_{OLSi})^2]$. \\

\noindent \textbf{Step 4:}  We show that $Q_1-Q_2$ can be expressed as a linear combination of numerators of the fixed instrument RV test statistic and the RSS test statistic.  Note that when $\delta_z = 0$, we are in a fixed instruments setup, so that the usual asymptotics obtains.  This means that, by Proposition \ref{prop:plims_TE2}: \begin{align}
    (\theta_1-\theta_2)\bigg(H(\theta_1+\theta_2)  -2 H^*\theta_0\bigg) =
E[(\tilde\Delta_{1i}-\tilde\Delta^*_{0i})^2] - E[(\tilde\Delta_{2i}-\tilde\Delta^*_{0i})^2] 
\end{align}
%and we can rewrite
%\begin{align*}
%    Q_1 - Q_2 &\rightarrow_p E[(\tilde\Delta_{1i}-\tilde\Delta^*_{0i})^2] - E[(\tilde\Delta_{2i}-\tilde\Delta^*_{0i})^2]  + \delta_z(\theta_1-\theta_2)'\bigg( \Sigma_{ee}(\theta_1+\theta_2)
 %   -2 \Sigma_{ee^*}\theta_0+ \Sigma_{e \omega_0}\bigg)
  %  \end{align*}

Therefore, by the results established in the previous steps,
% $$\delta_z(\theta_1-\theta_2)'\bigg( \Sigma_{ee}(\theta_1+\theta_2)
 %   -2 \Sigma_{ee^*}\theta_0+ \Sigma_{e \omega_0}\bigg) = E[(\Delta_{1i}-\Delta_{OLSi})^2] - E[(\Delta_{2i}-\Delta_{OLSi})^2]-E[(\tilde\Delta_{1i}-\tilde\Delta^*_{0i})^2] + E[(\tilde\Delta_{2i}-\tilde\Delta^*_{0i})^2]   $$
 %   so that
\begin{align*}
    Q_1-Q_2\rightarrow_p (1-\delta_z)\bigg(E[(\tilde\Delta_{1i}-\tilde\Delta^*_{0i})^2] - E[(\tilde\Delta_{2i}-\tilde\Delta^*_{0i})^2]\bigg) + \delta_z\bigg(E[(\Delta_{1i}-\Delta_{OLSi})^2] - E[(\Delta_{2i}-\Delta_{OLSi})^2]\bigg) 
\end{align*} 

\end{proof}


==> Proofs/old/Pf_RSS.tex <==
\subsection{The Problem with Testing without Instruments}\label{sec:RSS}

The RV test statistic depends on measures of fit formed with excluded instruments $z$.  However, implementations of the RV test based on residual sum of squares (RSS) have been popular in the applied IO literature.\footnote{For example, \cite{b87}, \cite{glv92}, \cite{bd10} and \cite{bdvk13} use RSS-based procedures to test hypotheses on conduct.}  These RSS-based tests are inconsistent.  To illustrate why, we briefly summarize how  one could implement an RSS based test.  First, one would impose model $m$ and rearrange the first order conditions of the firm as follows:
\begin{align}\label{OLSreg}
\mathbf{p} - \mathbf{\Delta}_m = \mathbf{w} \tau + \boldsymbol{\omega}_m.
\end{align}
Under the imposed model, $\mathbf{p} - \mathbf{\Delta}_m $ is observed and one can obtain an OLS residual $\hat{\boldsymbol{\omega}}_m$ from the regression (\ref{OLSreg}). Given that the OLS regression imposes that $\textbf{w}$ is orthogonal to $\boldsymbol \omega_m$, one can equivalently set $\hat{\boldsymbol{\omega}}_m = p - \Delta_m  = \hat{\omega}_m.$ One then constructs for model $m$ a measure of fit $Q_m^{RSS} = \frac{1}{n} \sum_i (\hat\omega_{mi})'(\hat\omega_{mi})$, and computes a test statistic as in  (\ref{RVt}):
\begin{align}
T^{RSS} = \frac{\sqrt{n}}{\hat  \sigma_{RSS}} (Q_1^{RSS} - Q_2^{RSS}), 
\end{align}
where $\hat  \sigma_{RSS}$ is a consistent estimator of the standard deviation of the difference in the RSS measures of fit. The formulation of the hypotheses is identical to what we have described for RV in Section \ref{sec:thetests}, except for the different measure of fit. 

Consider alternative moments
$g^{OLS}_m = \frac{\Delta'\hat\omega_m}{n}$,
which are the moments one would use to estimate Equation (\ref{eq:test}) by OLS. We define a measure of fit using these moments as $Q_m^{OLS} = g^{OLS\prime}_m(\frac{\Delta'\Delta}{n})^{-1} g^{OLS}_m$. Now we can prove the following lemma: 

\begin{lemma}\label{lemma2}

For any pair of models $m=1,2$,  
$T^{RSS} = \frac{\sqrt{n}}{\hat  \sigma_{RSS}} (Q_1^{OLS} - Q_2^{OLS}).$
\end{lemma}

\noindent The lemma establishes the equivalence between the RSS-based test and testing with OLS moments. As markups are endogenous,  tests based on $T^{RSS}$  have the wrong size and possibly no power against some fixed alternatives. Suppose that $\Delta_0=\Delta_1$ and consider testing two models:  the true model  and the OLS model with markups $\Delta^{OLS} = \Delta\theta^{OLS}$ where $\theta^{OLS}= E[\Delta_{i} \Delta_{i}']^{-1} E[\Delta_{i} p_i]$. As $Q_m^{OLS}$ is minimized at $\hat\theta^{OLS}$, $T^{RSS}$ asymptotically rejects for the wrong model. We formalize this in a proposition:\looseness=-1 
\begin{proposition}\label{prop:RSS} Assume that Assumptions \ref{as:momcond}, \ref{as:regcond} and \ref{as:homsked} are satisfied. Then:
\begin{align}
\frac{T^{RSS}}{\sqrt{n}} &\rightarrow_p  \frac{E[(\Delta^{OLS}_i -\Delta_{1i})^2 - (\Delta^{OLS}_i -\Delta_{2i})^2]	}{\sigma_{RSS}}
\end{align} 
\end{proposition}

When a researcher observes true markups, a valid way to perform model selection is to compare the implied markups for each model to the true markups.  This proposition shows that RSS-based tests asymptotically reject in favor of the model for which the implied markups are closer to the OLS markups. Thus, the RSS procedure implicitly uses the observed $\Delta^{OLS}$ in place of $\Delta_0$.  Since $\Delta$ is generally correlated with $\omega$, $\Delta^{OLS}$ may be very far from $\Delta_0$, making the RSS procedure inconsistent.\footnote{Our discussion thus far in this section is based on an RV-like test statistic because this has been used in the applied literature. In fact, other testing procedures (most notably, Cox and EB) could be performed using the moments $h$ based on OLS fit, thus incurring in the same problems.} An obvious solution is to test based on the moments formed with excluded instruments as in the procedures described in Section \ref{sec:thetests}. 




Useful objects for the proof: 
\begin{align*}
        \hat A_{\Delta \Delta} = \frac{\Delta'\Delta}{n}\\
        \hat A_{\Delta p} = \frac{\Delta'p}{n}
\end{align*}
and the facts:
\begin{align*}
    \hat A_{\Delta \Delta} &= A_{\Delta \Delta} + o_p(1)\\
    \hat A_{\Delta p} &= A_{\Delta p} + o_p(1).
\end{align*}
Notice moreover that:
\begin{align*}
    E[\hat\theta_{OLS}] = A_{\Delta \Delta}^{-1} A_{\Delta p} = \theta_{OLS} \neq \theta_0.
\end{align*}
where the inequality comes from our assumption on the endogeneity of the markup term. We first prove a useful lemma:

\begin{lemma}

Define the RSS measure of fit as 

\begin{align}
Q^{RSS}(\theta) = \frac{1}{n} \sum \hat \omega_{jt}(\theta)^2.
\end{align}
Also define a GMM measure of fit constructed with the OLS moments as 
\begin{align}\label{eq:QnOLS}
Q^{OLS}(\theta) = h(\theta)'W h(\theta)
\end{align}
 for
\begin{align}\label{eq:gn_OLS}
h(\theta) = \frac{1}{n} \Delta'\hat\omega(\theta),
\end{align}
and $W$ equals to $(\Delta'\Delta)^{-1}$.
Then, the two functions $Q^{RSS}(\theta)$ and $Q^{OLS}(\theta)$ are equal up to a constant, and have the same minimizers. It follows that:
\begin{align*}
T^{RSS} &= \sqrt{n} \frac{Q_1^{OLS} - Q_2^{OLS}}{\hat\sigma_{RSS}}    
\end{align*}

\end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma2}]

We can rewrite (\ref{eq:QnOLS}) in matrix notation as:
\begin{align}
n\cdot Q^{OLS}(\theta) &= \hat \omega(\theta)' \Delta (\Delta'\Delta)^{-1} \Delta'\hat \omega(\theta)\\
&= p'\Delta (\Delta'\Delta)^{-1} \Delta'p + (\theta'\Delta' \Delta \theta) - 2p'\Delta \theta \\
&= p'p-p'p+p'\Delta (\Delta'\Delta)^{-1} \Delta'p + (\theta'\Delta' \Delta \theta) - 2p'\Delta \theta \\
&= n\cdot Q^{RSS}(\theta) -(p'p-p'\Delta (\Delta'\Delta)^{-1} \Delta'p)\\
&= n\cdot Q^{RSS}(\theta) + c_n.
\end{align}
Since the functions $Q^{OLS}$ and $Q^{RSS}$ are equal up to the constant  $\frac{c_n}{n}$,  they also have the same minimizer $( \hat \theta_{OLS})$. Moreover, 
\begin{align}
   Q^{RSS}(\theta_1) - Q^{RSS}(\theta_2) &= Q_1^{RSS} - Q_2^{RSS}\\          
   &=Q_1^{OLS} - Q_2^{OLS}. 
\end{align}
\end{proof}

\begin{proof}[Proof of Proposition 3:]

By Lemma 1, the RSS test statistic is:
\begin{align}
T^{RSS} &= \sqrt{n} \frac{Q_1^{OLS} - Q_2^{OLS}}{\hat\sigma_{RSS}}
\end{align}
where $\hat\sigma^{RSS}_{I,II} \rightarrow_p \sqrt{\sigma^{2,RSS}_{I,II}}$ and $\sigma^{2 RSS}_{I,II}$ is the asymptotic variance of $\sqrt{n}(Q_1^{OLS} - Q_2^{OLS})$. To
derive the plim of the test statistic, first consider the object:
\begin{align*}
Q_1^{OLS} - Q_2^{OLS}
&= g_1'Wg_1 - ng_2'Wg_2\\
&= -(\theta_1-\theta_2)'\hat A_{\Delta\Delta}(\theta_1-\theta_2)-2(\theta_1-\theta_2)'\frac{\Delta'\omega_0}{n}\\
& \rightarrow_p  -(\theta_1-\theta_2)'A_{\Delta\Delta}(\theta_1-\theta_2) -2(\theta_1-\theta_2)'E[\Delta'\omega_0]\\
&= -E[(\Delta_{1i} -\Delta_{2i} )^2] - 2(\theta_1-\theta_2)' E[\Delta_i\Delta_i'](\theta_{OLS} -\theta_0)\\
&= -E[(\Delta_{1i} -\Delta_{2i} )^2] -  2E[(\Delta_{1i}-\Delta_{2i})'(\Delta_{OLS,i} -\Delta_{1i})]\\
&=E[(\Delta_{OLS,i} -\Delta_{1i}))^2 - (\Delta_{OLS,i} -\Delta_{2i}))^2],	
\end{align*}
so that we have
\begin{align}
\frac{T^{RSS}}{\sqrt{n}} &\rightarrow_p  \frac{E[(\Delta_{OLS,i} -\Delta_{1i}))^2 - (\Delta_{OLS,i} -\Delta_{2i}))^2]	}{\sigma^{RSS}_{I,II}}.
\end{align} 
\end{proof}

==> Proofs/old/Pf_RVDistribWeakInstr.tex <==
We start by recapping our setup of weak instruments for testing. Recall our model:
\begin{align*}
    p = \Delta_0 + \omega_0,
\end{align*}
and for model $m$ we define a modified first stage regression:
\begin{align*}
    \Delta_0 - \Delta_m = z(\Gamma^*_0 - \Gamma_m) + e_m.
\end{align*}
Then, we adopt a weak instrument asymptotics similar to \cite{ss97}: $(\hat\Gamma^{*}_0-\hat\Gamma_m) = \frac{q_m}{\sqrt{n}} + o_p(n^{-1/2})$ for a finite vector $q_m$. This is a special case of weak instruments for testing as defined in Proposition \ref{prop:degen}. Under this weak instruments for testing asymptotics, we have:
\begin{align}
\frac{z'\omega_0}{\sqrt{n}} &\rightarrow_d \xi_{\omega_0}\\
\frac{z'e_m}{\sqrt{n}} &\rightarrow_d \xi_{e_m}\\ 
%\frac{z'p}{\sqrt{n}}&=\frac{z'\Delta_0^* +z'e_0^* + z'\omega_0 }{\sqrt{n}}\\ &\rightarrow_d A_{zz}'c^*_0 + \xi_{e^*_0} + \xi_{\omega_0}\\
\frac{z'(\Delta_0 - \Delta_m)}{\sqrt{n}} &\rightarrow_d A_{zz}q_m + \xi_{e_m}\\
\frac{z'(p-\Delta_m)}{\sqrt{n}} &\rightarrow_d A_{zz}q_m + \xi_{e_m}+ \xi_{\omega_0}\\
\hat A_{zz}^{-1/2}\frac{z'(p-\Delta_m)}{\sqrt{n}} &\rightarrow_d A_{zz}^{1/2} q_m + A_{zz}^{-1/2}\bigg(\xi_{e_m}+ \xi_{\omega_0}\bigg)\\
&= D_m
%\Delta'z(z'z)^{-1}z'\Delta &\rightarrow_d ((A_{zz} C + \xi_e)' A^{-1}_{zz}(A_{zz} C + \xi_e))\\
%\hat\theta_{2SLS} &\rightarrow_d ((A_{zz} C + \xi_e)' A^{-1}_{zz}(A_{zz} C + \xi_e))^{-1}((A_{zz} C + \xi_e)' A^{-1}_{zz}(A_{zz} c^*_0 + \xi_{e^*_0}))\\
%&\qquad + ((A_{zz} C + \xi_e)' A^{-1}_{zz}(A_{zz} C + \xi_e))^{-1}((A_{zz} C + \xi_e)' A^{-1}_{zz}\xi_{\omega_0})
\end{align}
where, if we denote $\xi = (\xi_{\omega_0},\xi_{e_1},\xi_{e_2})$ and $u = (\omega_0, e_1, e_2)$ then $vec(\xi) \sim N(0,E[u_i u_i' \otimes z_i z_i'])$. We also define $$E[u_iu_i'] = \begin{bmatrix} \sigma^2_{\omega_0} & 
\sigma_{\omega_0e_1} &
\sigma_{\omega_0e_2} \\  
\sigma_{\omega_0e_1} &  
\sigma^2_{e_1} &
\sigma_{e_1e_2}\\
\sigma_{\omega_0e_2} & 
\sigma_{e_1e_2} &
\sigma^2_{e_2}
\end{bmatrix}.
$$

Thus, letting $D = (D_1,D_2)'$, the joint distribution of $D$ is given as $D \sim N( D_0 , V)$
where $D_0 = (A_{zz}^{1/2} q_1,A_{zz}^{1/2} q_2)'$ and $$V = \begin{bmatrix}
\sigma^2_{\omega_0} + \sigma^2_{e_1} + 2 \sigma_{\omega_0 e_1} &\sigma^2_{\omega_0} + \sigma_{\omega_0 e_1}+ \sigma_{\omega_0 e_2} + \sigma_{e_1 e_2} \\
\sigma^2_{\omega_0} + \sigma_{\omega_0 e_1}+ \sigma_{\omega_0 e_2} + \sigma_{e_1 e_2} & \sigma^2_{\omega_0} + \sigma^2_{e_2} + 2 \sigma_{\omega_0 e_2}
\end{bmatrix}\otimes I_{d_z}$$.

With the preliminaries defined, we now use them to derive the distribution of the RV test statistic under a weak instruments for testing asymptotic.  We first consider the numerator of $T^{RV}$.  First note the following:
\begin{align*}
   Q_1 - Q_2 
&= (g_1-g_2)'W(g_1+g_2)\\
&= \frac{1}{n}\bigg((p-\Delta_1)-(p-\Delta_2)\bigg)'z(z'z)^{-1}z'\bigg(p - \Delta_1 +(p-\Delta_2)\bigg)\\
&= \bigg(\frac{(p-\Delta_1)'z}{n}\hat A_{zz}^{-1/2}-\frac{(p-\Delta_2)'z}{n}\hat A_{zz}^{-1/2}\bigg)\bigg( \hat A_{zz}^{-1/2}\frac{z'(p - \Delta_1)}{n} + \hat A_{zz}^{-1/2}\frac{z'(p-\Delta_2)}{n}\bigg)
\end{align*}

so that:
\begin{align*}
     n(Q_1 - Q_2) & = \bigg(\frac{(p-\Delta_1)'z}{\sqrt{n}}\hat A_{zz}^{-1/2}-\frac{(p-\Delta_2)'z}{\sqrt{n}}\hat A_{zz}^{-1/2}\bigg)\bigg( \hat A_{zz}^{-1/2}\frac{z'(p - \Delta_1)}{\sqrt{n}} + \hat A_{zz}^{-1/2}\frac{z'(p-\Delta_2)}{\sqrt{n}}\bigg)\\ &\rightarrow_d  (D_1-D_2)'(D_1+D_2)
     %\bigg( A_{zz}c_2 + \xi_{e_2}- A_{zz}c_1 - \xi_{e_1}\bigg)'A_{zz}^{-1}\bigg(2A_{zz}c^*_0 + 2\xi_{e^*_0} + 2\xi_{\omega_0} - A_{zz}c_1 - \xi_{e_1}- A_{zz}c_2 - \xi_{e_2}\bigg)\\
     %&= \bigg( A_{zz}^{1/2}c_2 + A_{zz}^{-1/2}\xi_{e_2}- A_{zz}^{1/2}c_1 - A_{zz}^{-1/2}\xi_{e_1}\bigg)'\\
     %&\qquad \times \bigg(2A_{zz}^{1/2}c^*_0 + 2A_{zz}^{-1/2}\xi_{e^*_0} + 2A_{zz}^{-1/2}\xi_{\omega_0} - A_{zz}^{1/2}c_1 - A_{zz}^{-1/2}\xi_{e_1}- A_{zz}^{1/2}c_2 - A_{zz}^{-1/2}\xi_{e_2}\bigg)\\
     %&= \bigg( \iota_1 - \iota_2 + A_{zz}^{-1/2}\xi_{e_2} -A_{zz}^{-1/2}\xi_{e^*_0} - A_{zz}^{-1/2}\xi_{e_1}+A_{zz}^{-1/2}\xi_{e^*_0}
     %+A_{zz}^{-1/2}\xi_{\omega_0}-A_{zz}^{-1/2}\xi_{\omega_0}\bigg)'\\
     %&\qquad \times \bigg(\iota_1 + \iota_2 + 2A_{zz}^{-1/2}\xi_{e^*_0} + 2A_{zz}^{-1/2}\xi_{\omega_0} - A_{zz}^{-1/2}\xi_{e_1} - A_{zz}^{-1/2}\xi_{e_2}\bigg)\\
\end{align*}



Now we consider the denominator of the test statistic.  In particular, we define an estimator of the asymptotic variance, denoted $\hat \sigma^2_{RV}$, as:\footnote{See \cite{hp11} for the exact asymptotic variance of the RV test statistic without weak instruments.} 
\begin{align}
    \hat\sigma_{RV}^2 
&= 4g_1'\hat A_{zz}^{-1}\Sigma_1 \hat A_{zz}^{-1}g_1 +4g_2'\hat A_{zz}^{-1}\Sigma_2 \hat A_{zz}^{-1} g_2 - 8g_1'\hat A_{zz}^{-1}\Sigma_{1,2} \hat A_{zz}^{-1} g_2.
\end{align}
where
\begin{align}
&\Sigma_m = \frac{1}{n}\sum_{i=1}^n \bigg( z_i\hat \omega_{mi} \bigg) \bigg(z_i \hat\omega_{mi} \bigg)'\label{eq:Sigma_m}\\
%
&\Sigma_{1,2} = \frac{1}{n}\sum_{i=1}^n \bigg( z_i \hat \omega_{1i} \bigg) \bigg( z_i \hat \omega_{2i} \bigg) '
\end{align}

We first examine the convergence of $g_1$ and $g_2$:
\begin{align*}
    \sqrt{n} g_m &= \hat A_{zz}^{1/2} \hat A_{zz}^{-1/2}\frac{z'\Delta^*_0-z'\Delta_m + z'\omega_0}{\sqrt{n}}\\
    &\rightarrow_d A_{zz}^{1/2} \bigg(A_{zz}^{1/2}c^*_0 + A_{zz}^{-1/2}\xi_{e^*_0} + A_{zz}^{-1/2}\xi_{\omega_0} - A_{zz}^{1/2}c_m - A_{zz}^{-1/2}\xi_{e_m}\bigg)\\
        &= A_{zz}^{1/2} D_m
\end{align*}

Now, we examine the convergence of $\Sigma_m$.  In doing so, it is convenient to define $u_{mi} = \omega_{0i}+e_{mi}$:
\begin{align}
       \Sigma_m &= \frac{1}{n}\sum_{i=1}^n ( z_i \hat \omega_m) ( z_i \hat \omega_m)'\\
       %&=\frac{1}{n}\sum_{i=1}^n \bigg( z_i( p_i-\Delta_{mi}) \bigg) \bigg( z_i( p_i-\Delta_{mi}) \bigg)'\\
       &=\frac{1}{n}\sum_{i=1}^n \bigg( z_i( \Delta^*_{0i}+\omega_{0i}-\Delta_{mi}) \bigg) \bigg( z_i(\Delta^*_{0i}+\omega_{0i}-\Delta_{mi}) \bigg)'\\
       &=\frac{1}{n}\sum_{i=1}^n \bigg(  z_iz_{i}'\frac{q_m}{\sqrt{n}}+z_i(e_{mi}+\omega_{0i}) \bigg) \bigg( z_iz_{i}'\frac{q_m}{\sqrt{n}}+z_i(e_{mi}+\omega_{0i}) \bigg)'\\
     %&=\frac{1}{n}\sum_{i=1}^n \bigg(  z_iz_{i}'\frac{q_m}{\sqrt{n}}+z_iu_{mi} \bigg) \bigg( z_iz_{i}'\frac{q_m}{\sqrt{n}}+z_iu_{mi} \bigg)'\\
       &=\frac{1}{n}\sum_{i=1}^n  z_iz_{i}'\frac{q_m}{\sqrt{n}}\frac{q_m'}{\sqrt{n}}z_iz_{i}'+ \frac{1}{n}\sum_{i=1}^n  z_iz_{i}'\frac{q_m}{\sqrt{n}}'u_{mi}z_i'
 +\frac{1}{n}\sum_{i=1}^n z_iu_{mi}'\frac{q_m'}{\sqrt{n}}z_iz_{i}' +\frac{1}{n}\sum_{i=1}^n z_iu_{mi}'u_{mi} z_i'\\
 &\rightarrow_p (\sigma^2_{\omega_0} + \sigma^2_{e_m}  +2\sigma_{\omega_0e_m}) A_{zz}
\end{align}
By similar steps,  $\Sigma_{12}\rightarrow_p (\sigma^2_{\omega_0} + \sigma_{\omega_0e_1} +\sigma_{\omega_0e_2} + \sigma_{e_1e_2}) A_{zz}$.

Thus, the denominator of the RV test converges in distribution as follows:
\begin{align*}
    \hat\sigma^2&=4g_1'\hat A_{zz}^{-1}\Sigma_1 \hat A_{zz}^{-1}g_1 +4g_2'\hat A_{zz}^{-1}\Sigma_2 \hat A_{zz}^{-1} g_2 - 8g_1'\hat A_{zz}^{-1}\Sigma_{1,2} \hat A_{zz}^{-1} g_2\\
    &\rightarrow_d %4\sigma^2_{u_1}D_1'A_{zz}^{1/2} A_{zz}^{-1}A_{zz}A_{zz}^{-1}A_{zz}^{1/2} D_1 + 4\sigma^2_{u_2}D_2'A_{zz}^{1/2} A_{zz}^{-1}A_{zz}A_{zz}^{-1}A_{zz}^{1/2} D_2 - 8\sigma^2_{u_{12}}D_1'A_{zz}^{1/2} A_{zz}^{-1}A_{zz}A_{zz}^{-1}A_{zz}^{1/2} D_2\\
    4\sigma^2_{u_1}D_1'D_1 + 4\sigma^2_{u_2}D_2'D_2 - 8\sigma^2_{u_{12}}D_1'D_2\\
    &= 4 \bigg(D'\begin{bmatrix}I_{d_z} & 0 \\0 &-I_{d_z} \end{bmatrix}V\begin{bmatrix}I_{d_z} &0 \\0 &-I_{d_z} \end{bmatrix}D\bigg)
\end{align*}



Using the convergence results for the numerator and denominator, we can thus construct an asymptotic distribution for the test statistic $T^{RV}$. 
\begin{align}
    T^{RV} &\rightarrow_d\frac{D_1'D_1 - D_2'D_2}{2\sqrt{D'\begin{bmatrix}I_{d_z} & 0 \\0 &-I_{d_z} \end{bmatrix}V\begin{bmatrix}I_{d_z} &0 \\0 &-I_{d_z} \end{bmatrix}D}}
\end{align}
It is useful to consider an equivalent representation of the asymptotic distribution of $T^{RV}$. This representation is based on the rotation proposed in Magnolfi, Soelvsten, and Sullivan (2021). Consider $\pi = (\pi_1,\pi_2)' = (D_1+D_2,D_1-D_2)' = RD$ where $R = \begin{bmatrix} 1 & 1 \\ 1 & -1\end{bmatrix}$.  Thus, the distribution of $\pi$ is given as: $\pi \sim N(R D_0, \Omega)$ where $\Omega = R V R$.  Then we can write $T^{RV}$ as a function of $\pi$.

\begin{align}
    T^{RV} 
  &\rightarrow_d \frac{(D_1+D_2)'(D_1-D_2)}{2\sqrt{D'\begin{bmatrix}I_{d_z} & 0 \\0 &-I_{d_z} \end{bmatrix}V\begin{bmatrix}I_{d_z} &0 \\0 &-I_{d_z} \end{bmatrix}D}} \\ 
      %&= \frac{(D_1'+D_2)'(D_1-D_2)}{2\sqrt{D'\begin{bmatrix}I_{d_z} & I_{d_z}  \\I_{d_z}  &-I_{d_z} \end{bmatrix}\begin{bmatrix}0& I_{d_z}  \\I_{d_z}  &0 \end{bmatrix}\begin{bmatrix}.5I_{dz} &.5I_{dz} \\.5I_{dz} &-.5I_{dz} \end{bmatrix}V\begin{bmatrix}.5I_{dz} &.5I_{dz} \\.5I_{dz} &-.5I_{dz} \end{bmatrix}\begin{bmatrix}0& I_{d_z}  \\I_{d_z}  &0 \end{bmatrix}\begin{bmatrix}I_{d_z} & I_{d_z}  \\I_{d_z}  &-I_{d_z} \end{bmatrix}D}} \\ 
       &= \frac{(D_1+D_2)'(D_1-D_2)}{\sqrt{D'\begin{bmatrix}I_{d_z} & I_{d_z}  \\I_{d_z}  &-I_{d_z} \end{bmatrix}\begin{bmatrix}0& I_{d_z}  \\I_{d_z}  &0 \end{bmatrix}\begin{bmatrix}I_{dz} &I_{dz} \\I_{dz} &-I_{dz} \end{bmatrix}V\begin{bmatrix}I_{dz} &I_{dz} \\I_{dz} &-I_{dz} \end{bmatrix}\begin{bmatrix}0& I_{d_z}  \\I_{d_z}  &0 \end{bmatrix}\begin{bmatrix}I_{d_z} & I_{d_z}  \\I_{d_z}  &-I_{d_z} \end{bmatrix}D}} \\ 
       &= \frac{(D_1+D_2)'(D_1-D_2)}{\sqrt{D'R S_p R V R S_p R D}} \\ 
        &= \frac{\pi_1'\pi_2}{\sqrt{\pi' S_p\Omega S_p \pi}} 
\end{align}
where $S_p = \begin{bmatrix} 0 & I_{d_z} \\ I_{d_z} & 0 \end{bmatrix}$.

It is further useful to standardize $\pi$.  We partition $\Omega$ into four $d_z \times d_z$ block matrices.  Let $\pi^{std} = (\Omega_{11}^{-1/2} \pi_1,\Omega_{22}^{-1/2} \pi_2)\sim N(\pi_0^{std}, \Omega^{std}\otimes I_{d_z} )$, where $\pi^{std}_{01} =  \Omega_{11}^{-1/2} A^{1/2}_{zz} (q_1 + q_2) $ and $\pi^{std}_{02} =  \Omega_{22}^{-1/2} A^{1/2}_{zz} (q_1 - q_2)$ and  $\Omega^{std} = \begin{bmatrix} 1 & \rho \\ \rho & 1 \end{bmatrix}$, and  $\rho$ is the correlation between $\pi_1^{std}$ and $\pi_2^{std}$. Then we can write the asymptotic distribution of the RV test statistic as a function of $\pi^{std}$.

%\begin{align}
%    V^{std} &= \begin{bmatrix}1 & \rho\\ \rho & 1\end{bmatrix}\\
%    &= \begin{bmatrix}V_{11}^{-1/2} & 0 \\ 0 & V_{22}^{-1/2}\end{bmatrix} \begin{bmatrix}V_{11} & V_{12}\\ V_{12} & V_{22}\end{bmatrix} \begin{bmatrix}V_{11}^{-1/2} & 0 \\ 0 & V_{22}^{-1/2}\end{bmatrix}\\
%    &= S_VVS_V
%\end{align}
%so that 
%\begin{align}V &= \begin{bmatrix}V_{11}^{1/2} & 0 \\ 0 & V_{22}^{1/2}\end{bmatrix} \begin{bmatrix} 1& \rho \\ \rho & 1\end{bmatrix} \begin{bmatrix}V_{11}^{1/2} & 0 \\ 0 & V_{22}^{1/2}\end{bmatrix}\\
%&=S_V^{-1} V^{std} S_V^{-1}\end{align}

\begin{align}
     \frac{\pi_1'\pi_2}{\sqrt{\pi' S_p\Omega S_p \pi}} 
    &= \frac{\pi_1'\pi_2}{\sqrt{\pi' S_p\begin{bmatrix}\Omega_{11}^{1/2} I_{dz} & 0 \\ 0 & \Omega_{22}^{1/2} I_{dz}\end{bmatrix}\Omega^{std} \begin{bmatrix}\Omega_{11}^{1/2} I_{dz} & 0 \\ 0 & \Omega_{22}^{1/2} I_{dz}\end{bmatrix}S_p \pi}} \\
    %&= \frac{\pi_1'\pi_2}{\sqrt{\pi' S_p S^{-1}_\Omega\Omega^{std} S^{-1}_\Omega S_p \pi}} \\
    &= \frac{\pi_1'\pi_2}{\sqrt{\begin{bmatrix}\Omega_{11}^{1/2} \pi_2'  &  \Omega_{22}^{1/2} \pi_1'  \end{bmatrix}\Omega^{std} \begin{bmatrix}  \Omega_{11}^{1/2} \pi_2\\ \Omega_{22}^{1/2} \pi_1  \end{bmatrix}}} \\
        &=\frac{\Omega_{11}^{-1/2}\Omega_{22}^{-1/2}}{\Omega_{11}^{-1/2}\Omega_{22}^{-1/2}} \frac{\pi_1'\pi_2}{\sqrt{\begin{bmatrix}\Omega_{11}^{1/2} \pi_2'  &  \Omega_{22}^{1/2} \pi_1'  \end{bmatrix}\Omega^{std} \begin{bmatrix}  \Omega_{11}^{1/2} \pi_2\\ \Omega_{22}^{1/2} \pi_1  \end{bmatrix}}} \\
                %&=\frac{\pi_1^{std}'\pi_2^{std}}{\sqrt{\begin{bmatrix}\Omega_{22}^{-1/2} \pi_2'  &  \Omega_{11}^{-1/2} \pi_1'  \end{bmatrix}\Omega^{std} \begin{bmatrix}  \Omega_{22}^{-1/2} \pi_2\\ \Omega_{11}^{-1/2} \pi_1  \end{bmatrix}}} \\
                &=\frac{\pi_1^{std\prime}\pi_2^{std}}{\sqrt{\begin{bmatrix}\Omega_{11}^{-1/2} \pi_1 \\\Omega_{22}^{-1/2} \pi_2    \end{bmatrix}'S_p\Omega^{std} S_p\begin{bmatrix}  \Omega_{11}^{-1/2} \pi_1 \\\Omega_{22}^{-1/2} \pi_2 \end{bmatrix}}}\\          %&=\frac{\pi_1^{std}'\pi_2^{std}}{\sqrt{(S_\Omega\pi)'S_p\Omega^{std} S_\Omega\pi}}\\
     &=\frac{\pi_1^{std\prime}\pi_2^{std}}{\sqrt{\pi^{std\prime}S_p\Omega^{std} S_p\pi^{std}}}
\end{align}
Finally,
\begin{align}
    T^{RV} \rightarrow_d \frac{\pi_1^{std}'\pi_2^{std}}{\sqrt{\pi^{std}'S_p\Omega^{std} S_p\pi^{std}}}
\end{align}

%$V = \begin{bmatrix}
%\sigma^2_{\omega_0} + \sigma^2_{e_1} + 2 \sigma_{\omega_0 e_1} &\sigma^2_{\omega_0} + \sigma_{\omega_0 e_1}+ \sigma_{\omega_0 e_2} + \sigma_{e_1 e_2} \\
%\sigma^2_{\omega_0} + \sigma_{\omega_0 e_1}+ \sigma_{\omega_0 e_2} + \sigma_{e_1 e_2} & \sigma^2_{\omega_0} + \sigma^2_{e_2} + 2 \sigma_{\omega_0 e_2}
%\end{bmatrix}\otimes I_{d_z}$
%\begin{align}
%    \Omega &= RVR\\
 %   &= R \begin{bmatrix}
%\sigma^2_{\omega_0} + \sigma^2_{e_1} + 2 \sigma_{\omega_0 e_1} &\sigma^2_{\omega_0} + \sigma_{\omega_0 e_1}+ \sigma_{\omega_0 e_2} + \sigma_{e_1 e_2} \\
%\sigma^2_{\omega_0} + \sigma_{\omega_0 e_1}+ \sigma_{\omega_0 e_2} + \sigma_{e_1 e_2} & \sigma^2_{\omega_0} + \sigma^2_{e_2} + 2 \sigma_{\omega_0 e_2}
%\end{bmatrix}\otimes I_{d_z} R\\
%&=  \begin{bmatrix}
%2\sigma^2_{\omega_0} + \sigma^2_{e_1} + 3  \sigma_{\omega_0 e_1} + \sigma_{\omega_0 e_2} + \sigma_{e_1 e_2} &2\sigma^2_{\omega_0} + \sigma^2_{e_2} + \sigma_{\omega_0 e_1}+ 3\sigma_{\omega_0 e_2} + \sigma_{e_1 e_2} \\
%\sigma^2_{e_1}+ \sigma_{\omega_0 e_1}- \sigma_{\omega_0 e_2} - \sigma_{e_1 e_2} & -\sigma^2_{e_2} -  \sigma_{\omega_0 e_2} + \sigma_{\omega_0 e_1} + \sigma_{e_1e_2}
%\end{bmatrix}\otimes I_{d_z}R\\
%&=  \begin{bmatrix}
%4\sigma^2_{\omega_0} + \sigma^2_{e_1} + \sigma^2_{e_2} + 4  \sigma_{\omega_0 e_1} + 4 \sigma_{\omega_0 e_2} + 2\sigma_{e_1 e_2} &\sigma^2_{e_1} - \sigma^2_{e_2} + 2\sigma_{\omega_0 e_1}-2\sigma_{\omega_0 e_2}  \\
%\sigma^2_{e_1} - \sigma^2_{e_2} + 2\sigma_{\omega_0 e_1}-2\sigma_{\omega_0 e_2}& \sigma^2_{e_1} +  \sigma^2_{e_2} - 2 \sigma_{e_1e_2}
%\end{bmatrix}\otimes I_{d_z}
%\end{align}
Notice that the asymptotic distribution of the  RV test statistic depends on three paramaters, $\pi_{01}, \pi_{02}$, and $\rho$. The null space in this parameterization is characterized by $\pi_{01}'\pi_{02} = 0$.  In the null space, but far from the origin, instruments are relatively strong and the RV test statistic converges to a standard normal.  However, close to the origin, the RV test suffers from a size distortion due to degeneracy.   


==> Proofs/old/Pf_absfit.tex <==
\begin{proposition}\label{prop:absfit}
Suppose that the markups $\Delta$ are unobserved and that Assumptions \ref{as:momcond} and \ref{as:regcond}  are satisfied.  Then $\hat{\tilde{\Delta}}^{2SLS} \rightarrow_p \Delta^z_{0}$
\end{proposition}


\begin{proof}
From the proof of Proposition \ref{prop:plims_TE2}, part 1, we have established that the 2SLS estimator of $\theta$ converges in probability to the following:
\begin{align*}
    \hat\theta \rightarrow _p (A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1} A_{\Delta z}  A_{z z}^{-1}A_{z\Delta^*}\theta_0
\end{align*}
Thus, for each observation $i$, the predicted markups implied by the 2SLS estimate of $\theta$ asymptotically converge to:
\begin{align*}
\hat{\tilde{\Delta}}_{2SLS,i} &\rightarrow_p  \tilde\Delta(A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1} A_{\Delta z}  A_{z z}^{-1}A_{z\Delta^*}\theta_0\\
 %&=  zA_{zz}^{-1}A_{z\Delta}(A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1} A_{\Delta z}  A_{z z}^{-1}A_{z\Delta^*}\theta_0\\
 &=  zA_{zz}^{-1}A_{z\Delta}(A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1} A_{\Delta z}  A_{z z}^{-1}A_{z\Delta^*_0}\\
 &=  ztr(A_{zz}^{-1}A_{z\Delta}(A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1} A_{\Delta z}  A_{z z}^{-1}A_{z\Delta^*_0}\\
&=  ztr(A_{z\Delta}'A_{zz}^{-1}A_{\Delta z}'(A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1}A_{z\Delta^*_0}'A_{z z}^{-1\prime})\\
 &=  ztr( A_{z\Delta^*_0}'A_{z z}^{-1\prime})\\
&=  ztr( A_{z z}^{-1}A_{z\Delta^*_0})\\
&=  z A_{z z}^{-1}A_{z\Delta^*_0}\\
&=\tilde{\Delta}^*_{0i}
\end{align*}
\end{proof}



==> Submission/ECTA/Appendices/AltCost.tex <==
In this appendix we show that the results of the paper are preserved under a more flexible specification of marginal cost, including specifications where marginal cost depends on quantity sold. Let $\boldsymbol{q}_i$ denote quantity, and consider the separable expression in Equation (11) of \cite{bh14}:
\begin{align}
    \boldsymbol{c}_i = \bar c(\boldsymbol{q}_i,\textbf{w}_i) + \omega_i.
\end{align}
The specification of marginal cost that we adopt in the paper is a special case where $\bar c(\boldsymbol{q}_i,\textbf{w}_i) = \textbf{w}_i \tau$. We can define $\bar{\boldsymbol{\Delta}}_{mi} = \boldsymbol{\Delta}_{mi} + \bar c(\boldsymbol{q}_i,\textbf{w}_i)$: this term is pinned down by a model of conduct $m$, and a cost function $\bar c$. Assuming that $\bar c$ is fully specified by the researcher, we can test alternative pairs of models of conduct and cost functions with the methods described in the paper. In particular, that can be done by replacing ${{\Delta}}_{m}$ in the paper with $\bar{\boldsymbol{\Delta}}_{m}$. The set of instruments $\boldsymbol{z}$ must include $\textbf{w}$ in this case, but since $\bar c$ is fully specified, there is no additional requirement on instruments. 

Alternatively, the function $\bar c$ could be specified up to some cost parameters $\bar \tau$. These can be estimated under a model of conduct $m$ either as a preliminary step, or simultaneously with testing, analogous to demand estimation. In both cases, instruments are needed to estimate parameters $\bar \tau$, and thus must be sufficient to identify $\bar \tau$ under the true model of conduct. If a researcher pursues a sequential approach, the researcher can construct $\bar{\boldsymbol{\Delta}}_{mi} = \boldsymbol{\Delta}_{mi} + c(\boldsymbol{q}_i,\textbf{w}_i;\bar{\tau}_m)$ and perform testing after having estimated $\bar{\tau}_m$ under each model. Doing so requires adjusting the standard errors of the test statistic and the effective $F$-statistic $F_\rho$. 

This discussion makes it explicit that testing firm conduct also jointly tests models of marginal cost. In fact,  $\bar{\boldsymbol{\Delta}}_{m} $ generalizes the term $\Breve{\boldsymbol{\Delta}}_{m}$ defined in Section \ref{sec:globalmis}. In that section we show that cost misspecification can be incorporated in  $\Breve{\boldsymbol{\Delta}}_{m}$, and thus be understood as markup misspecification. Here, misspecification of $\bar c$ is manifested as misspecification of  $\bar{\boldsymbol{\Delta}}_{m} $. If one is flexible in specifying $\bar c$, misspecification of $\bar{\boldsymbol{\Delta}}_{m} $ largely concerns misspecification of ${\boldsymbol{\Delta}}_{m} $, and therefore conduct. Finally, this formulation shows that the methods described in the paper can be used to test models of cost, even when conduct is known.\looseness=-1




==> Submission/ECTA/Appendices/Robustness.tex <==

This appendix provides additional details and robustness exercises for our empirical application. We first discuss the candidate conduct models in more detail.

\noindent \textbf{Description of the Models of Conduct:} Following \cite{v07}, the markups in market $t$ for a model $m$ among those we consider can be written in the following form:
\[\boldsymbol{\Delta}_{mt}=\underbrace{-(\boldsymbol{\Omega}^r_{mt} \odot \boldsymbol{D}^r_t)^{-1} \boldsymbol{s}_t}_{\boldsymbol{\Delta}^\text{downstream}_{mt}}\underbrace{-(\boldsymbol{\Omega}^w_{mt} \odot \boldsymbol{D}^w_t )^{-1} \boldsymbol{s}_t}_{\boldsymbol{\Delta}^\text{upstream}_{mt}}\]
where $\boldsymbol{\Omega}^r_{mt}$ and $\boldsymbol{\Omega}^w_{mt}$ are ownership matrices, $\boldsymbol{D}^w_t$ is the jacobian of retail share $\boldsymbol{s}_t$ with respect to wholesale price, and $\boldsymbol{D}^r_t$ is the jacobian of retail share with respect to retail price. The markup $\boldsymbol{\Delta}_{mt}$ implied by each model is the sum of downstream markups $\boldsymbol{\Delta}^\text{downstream}_{mt}$ and upstream markups $\boldsymbol{\Delta}^\text{upstream}_{mt}$. We can derive each model by using different assumptions on the ownership matrices:
\begin{enumerate}
    \item \textit{Zero wholesale margin}: Set $\boldsymbol{\Omega}^w_{mt}$ to a matrix of zeros, set $\boldsymbol{\Omega}^r_{mt}$ to a matrix of ones.
    \item \textit{Zero retail margin}: Set $\boldsymbol{\Omega}^w_{mt}$ to a matrix of zeros, and set $\boldsymbol{\Omega}^r_{mt}$ to a matrix  with element $(i,j)$ that is equal to one if products $i$ and $j$ are produced by the same manufacturer, and to zero otherwise. 
    \item \textit{Linear pricing}: Set $\boldsymbol{\Omega}^r_{mt}$ to a matrix of ones, and set $\boldsymbol{\Omega}^w_{mt}$ to a matrix  with element $(i,j)$ that is equal to one if products $i$ and $j$ are produced by the same manufacturer, and to zero otherwise. 
    \item \textit{Hybrid model}: Set $\boldsymbol{\Omega}^r_{mt}$ to a matrix of ones, and set $\boldsymbol{\Omega}^w_{mt}$ to a matrix  with element $(i,j)$ that is equal to one if products $i$ and $j$ are produced by the same manufacturer and $i$ is not a private label, and to zero otherwise. 
    \item \textit{Wholesale Collusion}: Set $\boldsymbol{\Omega}^r_{mt}$ and $\boldsymbol{\Omega}^w_{mt}$ to matrices of ones. \looseness=-1
    
\end{enumerate}

\noindent \textbf{Distributions of Predicted Markups:} To build intuition on the mechanics of the RV test, we report in Figure \ref{fig:Pmkups_plot} the distributions of predicted markups for the three sets of instruments that we use in the main text. All distributions are 
\begin{figure}[H] 
\centering \caption{Distributions of Predicted Markups}
\label{fig:Pmkups_plot}
    \begin{subfigure}{.49\linewidth}
    \centering
    \includegraphics[scale=0.49]{Figures/AppendixPCM_BLPiv.png}
    \caption{BLP95 IVs}
    \end{subfigure}
    \begin{subfigure}{.49\linewidth}
    \includegraphics[scale=0.49]{Figures/AppendixPCM_GHiv.png}
    \caption{GH20 IVs}
    \end{subfigure}
    \begin{subfigure}{.49\linewidth}
    \includegraphics[scale=0.49]{Figures/AppendixPCM_Costiv.png}
    \caption{Rival Cost Shifters IVs}
    \end{subfigure}
    \caption*{\footnotesize{We report the distributions of $\Delta^z_{mi}$, the residualized predicted markups, for each model.}}
\vspace{-0.5cm}
\end{figure}     
\noindent centered at zero, since markups are residualized. The BLP95 instruments appear to generate meaningful differences in the distributions of predicted markups across models, thus making the test powerful. In contrast, the GH20 instruments generate distributions of predicted markups for the five models that are indistinguishable - the RV test has no power in this case. Finally, for the rival cost shifters instruments there is a clear distinction between the distribution of predicted markups for model 5 and all other distributions.  

While the figure helps interpretation, visual inspection of these distributions cannot substitute for formal RV testing, followed by the weak instruments diagnostic. In fact, interpreting the differences across distributions in terms of valid statistical statements requires the testing procedure we define.

\begin{comment}

\noindent \textbf{Alternative Demand Specifications:} Demand specification is an important input in the testing procedure, as it affects markups implied by different models. We report here test results for alternative demand specifications. We start with a basic logit model of demand, corresponding to the estimates reported in column 2 of Table \ref{Tab:demand}. Although this demand model is very restrictive, and quite far from the BLP model we use in our main specification, the testing results are mostly unaffected. 

We report in Table \ref{Tab:Dem_Rob} values of $F_\rho$ and MCS $p$-values for all pairs of models obtained by testing with logit demand. We use throughout BLP95 instruments for testing.



\begin{table}[htb]
\footnotesize
\caption{$F_\rho$ and MCS for Alternative Demand}
\label{Tab:Dem_Rob}
\centering
\begin{threeparttable}
\input{Tables/Dem_robustness}
\begin{tablenotes}[flushleft]
    \footnotesize
    \item[] This table reports $F_\rho$ and MCS $p$-values for different demand specifications. In each panel, we report $F_\rho$ for the pairwise combinations of the five candidate models, and the MCS $p$-values that correspond to each model. Test statistics are reported for pairs of models $i,j$, where model $i$ corresponds to the row and model $j$ corresponds to the column. Hence, a negative value of the test statistic suggests better fit of the row model. Critical values for $F_\rho$ are in Table \ref{tab:Tab_StockYogo_Combined_new} for $d_z=2$. MCS $p$-values below 0.05 indicate that a row model can be rejected.  Standard errors are adjusted to account for the two-step estimation error --- see Appendix \ref{sect:TwoStep} for details.\looseness=-1
\end{tablenotes}
\end{threeparttable}
\end{table}    
\end{comment}

    
\noindent \textbf{Alternative Sets of Instruments:} We perform RV testing using alternative sets of instruments. First, we combine the three sets of instruments that we use in the main text: BLP95, GH20 and rival cost shifters.\footnote{Results obtained using BLP95 and GH20 instruments together are similar.} We report in  Panel A of Table \ref{Tab:Instr_Rob} the effective $F$-statistics and MCS $p$-values for testing with these instruments. Combining the strong BLP95 instruments with the weak GH20 and rival cost shifters instruments lowers the effective $F$-statistics. In this case, while the instruments remain powerful and model 5 is firmly rejected, the MCS $p$-values for models 3 and 4 increase to 0.09 --- though still below the confidence level of 0.1 considered in \cite{hln11} and thus consistent with the RV test conducted with BLP95 instruments.

\begin{table}[htb]
\footnotesize
\caption{$F_\rho$ and MCS for Alternative Instruments}
\label{Tab:Instr_Rob}
\centering
\begin{threeparttable}
\input{Tables/Instr_robustness}
\begin{tablenotes}[flushleft]
    \footnotesize
    \item[]Each panel reports $F_\rho$ for the pair of models indicated by the row and column, and the MCS $p$-values for each row model. With MCS $p$-values below 0.05 a row model is rejected at a confidence level $\alpha=0.05$.  Values of $F_\rho$ and MCS standard errors account for two-step estimation error; see Appendix \ref{sect:TwoStep} for details.
\end{tablenotes}
\end{threeparttable}
\end{table}    

In  Panel B of Table \ref{Tab:Instr_Rob} we construct rival cost shifters instruments by taking the sum of squared differences between own and rival transportation cost. This different functional form also results in an instrument that is weak for size (at the $0.10$ target) and power (at the $0.50$ target), now for every combination of models. Testing based on this instrument is uninformative.

Panel C of Table \ref{Tab:Instr_Rob} helps to shed light on the source of power of the BLP95 instruments. In this panel we perform testing using as instruments only the number of other products produced by the firm, and the number of total products produced by rival firms. These instruments are powerful, and deliver identical results to the BLP95 instrument set. Hence, the number of products is a key dimension of variation in the data for testing conduct in this application. \looseness=-1 




==> Submission/ECTA/Appendices/TwoStep.tex <==

This appendix extends all our previously introduced statistics to take into account uncertainty stemming from preliminary demand estimation as well as dependence across observations. We suppose that $\Delta_m$ is a function of demand parameters $\theta^D$ that are estimated using a GMM estimator $\hat \theta^D$. We therefore let $W^D$ denote the GMM weight matrix and $h(\theta)=\frac{1}{n} \sum_{i=1}^n h_i(\theta)$ the GMM sample moment function used. Furthermore, we let $ H=\nabla_\theta h(\hat\theta^D)$ be the gradient of the sample moment function $ h$ and let $ G_m=-\frac{1}{n} \hat z' \nabla_{\theta} \hat \Delta_m(\hat\theta^D)$ be the gradient of $\hat g_m$. Both gradients are with respect to $\theta^D$.

\noindent\textbf{RV test:}
The RV statistic with a two-step adjustment replaces $\hat V_{\ell k}^\text{RV}$ in the definition of $\hat\sigma^2_\text{RV}$ with $\tilde V_{\ell k}^\text{RV} = \frac{1}{n} \sum_{i=1}^n \tilde \psi_{\ell i} \tilde \psi_{k i}'$. Here, the influence function $\tilde \psi_{mi}$ adjusts $\hat \psi_{mi}$ to account for preliminary demand estimation:
\begin{align}
      \tilde \psi_{mi} &= \hat \psi_{mi} - \hat W^{1/2} G_m \Phi \!\left(h_i(\hat\theta^D)- h(\hat\theta^D)\right)
\end{align}
where $\Phi=(H'W^DH)^{-1}H'W^D$. This is a standard adjustment for first-step estimation based on the asymptotic approximation $\hat \theta^D - \theta^D \approx -\Phi h(\theta^D).$

\noindent\textbf{AR test:}
Analogously to the above, the AR statistics with a two-step adjustment replaces $\hat V_{mm}^\text{AR}$ with $\tilde V_{mm}^\text{AR}$ where $\tilde V_{\ell k}^\text{AR} = \frac{1}{n} \sum_{i=1}^n \tilde \phi_{\ell i} \tilde \phi_{k i}'$. Here, the influence function $\tilde \phi_{mi}$ adjusts $\hat \phi_{mi} = \hat W \hat z_i(\hat p_i- \hat \Delta_{mi} - \hat z_i'\hat \pi_i)$ to account for preliminary demand estimation using the same approximation to $\hat \theta^D$ as above:
\begin{align}
      \tilde \phi_{mi} &= \hat \phi_{mi} - \hat W G_m \Phi_m \!\left(h_i(\hat\theta^D)- h(\hat\theta^D)\right).
\end{align}

% Analogous to the solution in \citeA{mw17}'s appendix D, a consistent estimator for the asymptotic variance of $\hat\pi_m$ that takes into account the uncertainty from the demand estimate $\hat\theta^D$ is:

% \[(G^{S\prime}_mWG^S_m)^{-1}G^{S\prime}_mW\Sigma_m WG^S_m(G^{S\prime}_mWG^S_m)^{-1}\]
% where $\hat g_m=n^{-1}z^{\prime}\hat\omega_m=n^{-1}z^{\prime}(p-\hat\Delta_m(\hat\theta^D)-z\hat\pi_m)$, $G^S_m=\nabla_\pi \hat g_m=n^{-1}z'z$ and:
% \[
% \Sigma_m = \sum_{i=1}^n \bigg(z^{\prime}_i\hat\omega_{m,i}-\hat g_m + \hat\Phi_m \left(z_i^{D\prime}\xi_i(\hat\theta^D)-\hat h(\hat\theta^D)\right) \bigg) \bigg( z^{\prime}_i\hat\omega_{m,i}-\hat g_m + \hat\Phi_m  \left(z_i^{D\prime}\xi_i(\hat\theta^D) -\hat h(\hat\theta^D)\right)\bigg)'
% \]
% where $\hat\Phi_m$ is defined as in the RV test case.

\noindent\textbf{$F$-statistic:}
The $F$-statistic with a two-step adjustment replaces $\hat \sigma_1^2$, $\hat \sigma_2^2$, and $\hat \sigma_{12}$ in the definition of $F_\rho$ and $\hat \rho^2$ with $\tilde \sigma_m^2 = d_z\inverse \text{trace}\big( \tilde V_{mm}^\text{AR} \hat W^{-1} \big)$ for $m\in\{1,2\}$ and $\tilde \sigma_{12} = d_z\inverse  \text{trace}\big(  \tilde V_{\ell k}^\text{AR}\hat W^{-1} )$. Here, $ \tilde V_{\ell k}^\text{AR}$ and $\tilde \phi_{mi}$ were introduced for the two-step correction of AR.

An extension of Proposition \ref{prop:wkinstrF} that accounts for two-step estimation can be established under homoskedasticity, i.e., when $\hat W^{-1/2} \tilde V_{\ell k}^\text{AR} \hat W^{-1/2}$ for $\ell,k \in \{1,2\}$ converge in probability to diagonal matrices. In the absence of homoskedasticity, $F_\rho$ is still informative about the strength of the instruments, but the exact thresholds for size control reported in Table \ref{tab:Tab_StockYogo_Combined_new} may only be approximations to the true thresholds.

%\noindent\textbf{EB test:}
%Analogous to the AR test correction, except that instead of $n^{-1}z^{\prime}(p-\hat\Delta_m(\hat\theta^D)-z\hat\pi_m)$ the supply side moment is now $z^{\prime}(p-\theta\hat\Delta(\hat\theta^D))$ and we take derivatives with respect to $\theta$ to compute $G_m$. This formulation is analogous to \citeA{mw17}, Appendix D.

%\noindent\textbf{Cox test:}
%The Cox statistic with a two-step adjustment replaces $ \hat V_{mm}^\text{AR} $ in the definition of $\hat\sigma^2_\text{Cox}$ with $\tilde V_{mm}^\text{AR}$. Here, $\tilde V_{mm}^\text{AR}$ was introduced for the two-step correction of AR.


\noindent\textbf{Dependence:}
Dependent data, e.g., cluster sampling, is easily accommodated by adjustments to $\hat V_{\ell k}^\text{RV}$ and $\hat V_{\ell k}^\text{AR}$. If we let $c_{ij}$ take the value one if observations $i$ and $j$ are deemed dependent and zero otherwise, then the variance estimators used in the paper can be replaced by 
\begin{align}
    \Breve V_{\ell k}^\text{RV} = \frac{1}{n} \sum_{i=1}^n\sum_{j=1}^n c_{ij} \hat\psi_{\ell i} \hat\psi_{k j}'
    \quad \text{and} \quad 
    \Breve V_{\ell k}^\text{AR} = \frac{1}{n} \sum_{i=1}^n\sum_{j=1}^n c_{ij} \hat\phi_{\ell i} \hat\phi_{k j}'.
\end{align}
Combinations of two-step estimation and dependence are also be handled by simply replacing $\hat \psi$ and $\hat \phi$ by $\tilde \psi$ and $\tilde \phi$ in the definitions of $\Breve V_{\ell k}^\text{RV}$ and $\Breve V_{\ell k}^\text{AR}$. Provided that suitable central limit theorem and laws of large numbers can be alluded to under the type of dependence considered, any claims on asymptotic validity under strong instruments made in the paper continue to hold. For clustered data, we refer to \citeA{ha19} for such results.

% Define $\hat g_{3} = \hat g_1-\hat g_2$ and $\hat Q_{3} = \hat g_{3}'\hat W\hat g_{3}$. Analogous to what we show for the RV test, we can show that a consistent estimator for the limiting variance of $\sqrt{n}(\hat Q_1-\hat Q_2-\hat Q_3)$ is:

% \[ \hat\sigma^2=4\hat g_1'\Sigma_1\hat g_1 + 4\hat g_2'\Sigma_2\hat  g_2 +4\hat g_{3}'\Sigma_{3}\hat g_{3}- 8\hat g_1'\Sigma_{1,2}\hat g_2 - 8\hat g_1'\Sigma_{1,3}  g_3 + 8g_2'\Sigma_{2,3}  g_3 \]
% where:
% \[
% \Sigma_{m,l} = \sum_{i=1}^n \bigg(z^{\prime}_i\omega_{m,i}-\hat g_m + \hat\Phi_m\left( z_i^{D\prime}\xi_i(\hat\theta^D)-\hat h(\hat\theta^D)\right) \bigg) \bigg( z^{\prime}_i\hat\omega_{l,i}-\hat g_l + \hat\Phi_l  \left(z_i^{D\prime}\xi_i(\hat\theta^D)-\hat h(\hat\theta^D)\right) \bigg)'\\
% \]
% and $\hat\Phi_m$ is defined as in the RV test case.



==> Submission/ECTA/Figures/ModelSel_slides.tex <==

\begin{tikzpicture}[scale = 0.85]
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=-1,xmax=5.5,ymin=-1.0,ymax=5.5,
  tick style={draw=none},
  xticklabels=\empty,
  yticklabels=\empty,
  xlabel={$E[(\Delta^z_0-\Delta^z_1)^2]$},
  ylabel={$E[(\Delta^z_0-\Delta^z_2)^2]$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.8,0.15)},anchor=north},
    y label style={at={(axis description cs:0.15,.75)},rotate=90,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  title={Model Selection},
  grid=major,
  grid style={thin,densely dotted,white!20}]

%45-deg lines
\addplot [domain=0:5.5,samples=2, color = black] {x} node[right]{};


%shading
\tikzstyle{rej1}=[draw=none,line width=10pt,preaction={clip, postaction={pattern=horizontal lines, pattern color=blue, opacity=0.3}}]
\tikzstyle{rej2}=[draw=none,line width=1pt,preaction={clip, postaction={pattern=vertical lines, pattern color=red, opacity=0.3}}]

\draw<3>[rej1] (100,300) -- (100,850) -- (650,850)   -- cycle;
\draw<3>[rej2] (300,100) -- (850,100) -- (850,650)   -- cycle;

\draw<4>[rej1] (100,150) -- (100,850) -- (800,850)   -- cycle;
\draw<4>[rej2] (150,100) -- (850,100) -- (850,800)   -- cycle;



\draw<3-4>[draw=black,line width=0.5pt,dashed]  (100,300) -- (700,900)  -- cycle;

\draw<3-4>[draw=black,line width=0.5pt,dashed]  (300,100) -- (900,700)  -- cycle;



\draw<4>[draw=black,line width=0.5pt,dashed]  (100,150) -- (700,750)  -- cycle;

\draw<4>[draw=black,line width=0.5pt,dashed]  (150,100) -- (750,700)  -- cycle;








%\node<1>[text width=5.9cm,rotate = 40,color = black,fill = none] at (600,620) {{${Q}_1 = {Q}_2$}};

\node<1->[text width=3.0cm,rotate = 0,color = black,fill = none] at (550,250) {{${Q}_1 > {Q}_2$}};

\node<1->[text width=5.9cm,rotate = 40,color = black,fill = none] at (500,540) {{$H_0^{RV}$: ${Q}_1 = {Q}_2$}};


\node<1-4>[text width=3.0cm,rotate = 0,color = black,fill = none] at (300,450) {{${Q}_1 < {Q}_2$}};

%\draw<2> [->] (100,450)--(190,310);
%\draw<2> [->] (100,450)--(500,310);


%\node<2>[text width=3.0cm,rotate = -55,color = black,fill = none] at (200,240) {{Low Bias}};

%\node<2>[text width=3.0cm,rotate = -15,color = black,fill = none] at (550,320) {{High Bias}};

\draw<4> [->] (150,350)--(225,275);
\draw<4> [->] (300,500)--(375,425);
\draw<4> [->] (450,650)--(525,575);

\draw<4> [->] (350,150)--(275,225);
\draw<4> [->] (500,300)--(425,375);
\draw<4> [->] (650,450)--(575,525);

%\draw<2->[black, fill=black] (200,300) circle (10) ;
\end{axis}

\end{tikzpicture}\hfill
\begin{tikzpicture}[scale = 0.85]
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=-1,xmax=5.5,ymin=-1.0,ymax=5.5,
  tick style={draw=none},
  xticklabels=\empty,
  yticklabels=\empty,
  xlabel={$E[(\Delta^z_0-\Delta^z_1)^2]$},
  ylabel={$E[(\Delta^z_0-\Delta^z_2)^2]$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.8,0.15)},anchor=north},
    y label style={at={(axis description cs:0.15,.75)},rotate=90,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  title={Model Assessment},
  grid=major,
  grid style={thin,densely dotted,white!20}]


%shading
\tikzstyle{rej1}=[draw=none,line width=10pt,preaction={clip, postaction={pattern=horizontal lines, pattern color=blue, opacity=0.3}}]
\tikzstyle{rej2}=[draw=none,line width=1pt,preaction={clip, postaction={pattern=vertical lines, pattern color=red, opacity=0.3}}]
\draw<3>[rej1] (250,200) -- (250,850) -- (100,850) -- (100,200)   -- cycle;
\draw<3>[rej2] (250,100) -- (250,200) -- (850,200) -- (850,100)   -- cycle;


\draw<4>[rej1] (150,150) -- (150,850) -- (100,850) -- (100,150)   -- cycle;
\draw<4>[rej2] (150,100) -- (150,150) -- (850,150) -- (850,100)   -- cycle;


\draw<4> [<-] (160,600)--(250,600);
\draw<4> [<-] (160,450)--(250,450);
\draw<4> [<-] (160,300)--(250,300);

\draw<4> [<-] (300,160)--(300,200);
\draw<4> [<-] (450,160)--(450,200);
\draw<4> [<-] (600,160)--(600,200);


\node<1->[text width=5.9cm,rotate = 90,color = black,fill = none] at (130,520) {{$H_{0,1}^{AR}$: ${Q}_1 = 0$}};
\node<1->[text width=5.9cm,rotate = 0,color = black,fill = none] at (520,130) {{$H_{0,2}^{AR}$: ${Q}_2 = 0$}};



\draw<3-4>[draw=black,line width=0.5pt,dashed]  (250,100) -- (250,700)  -- cycle;

\draw<3-4>[draw=black,line width=0.5pt,dashed]  (100,200) -- (700,200)  -- cycle;


\draw<4>[draw=black,line width=0.5pt,dashed]  (150,100) -- (150,700)  -- cycle;

\draw<4>[draw=black,line width=0.5pt,dashed]  (100,150) -- (700,150)  -- cycle;

%\draw<3->[black, fill=black] (200,300) circle (10) ;

\end{axis}

\end{tikzpicture}




==> Submission/ECTA/Figures/bresnahan.tex <==

\hspace{-1cm}\begin{tikzpicture}[scale=\tikzscale]
\begin{axis}[
            width=\textwidth,
            height=\axisdefaultheight,
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=0,xmax=6,ymin=0.0,ymax=10,
  xlabel={$q$},
  ylabel={$p$},
  xtick = none,
   ytick = {3.75,5.5,7.25},
        yticklabels = {$\tilde p_{2t}$,$p_t$,$\tilde p_{1t}$},
  %extra y ticks={9,10},
  %  extra y tick labels={$92\rightarrow$,$153.3\rightarrow$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.99,-0.02)},anchor=north},
    y label style={at={(axis description cs:-0.03,.92)},rotate=0,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  %title={Relationship Between Null and Degeneracy},
  grid=major,
  grid style={thin,densely dotted,white!20}]

%Demand
\addplot [domain=0:3.95,samples=2, color = blue!70!green,line width=1.2,opacity=0.4] {8.5-1.9*x} node[right]{};
\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (430,5) {{$D_t$ for $(z_t,\xi_t)$}};


%Omegas
\addplot [domain=0:4,samples=2, color = red!60!yellow] {2} node[right]{};
\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (480,19) {{$p_t-\Delta_{1t}$}};

\addplot [domain=0:4,samples=2, color = red!60!yellow] {5.5} node[right]{};
\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (480,55) {{$p_t-\Delta_{2t}$}};



%tilde p's
\addplot [domain=0:2.5,samples=2, color = black] {3.75} node[right]{};

\addplot [domain=0:2.5,samples=2, color = black] {7.25} node[right]{};

%Moments

\draw [decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
(245,55) -- (245,72.5) node [black,midway,xshift=2.35cm] {
$E[z_t(p_t-\Delta_{1t})]=0$};
\draw [decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
(245,37.5) -- (245,55) node [black,midway,xshift=3.75cm] {
$E[z_t(p_t-\Delta_{2t})]=E[z_t(\Delta_{1t}-\Delta_{2t})]$};

%Equilibria


\draw[black, fill=black] (65,72) ellipse (.1cm and .1cm);
\draw[black, fill=black] (160,55) ellipse (.1cm and .1cm);
\draw[black, fill=black] (250,38) ellipse (.1cm and .1cm);


\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (125,65) {{$\tilde{\mathcal{E}}_{1t}=(\cdot,\Delta_{1t})$}};
\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (220,48) {{${\mathcal{E}}_{t}$}};
\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (310,30) {{$\tilde{\mathcal{E}}_{2t}=(\cdot,\Delta_{2t})$}};







\end{axis}

\end{tikzpicture}


==> Submission/ECTA/Figures/noise.tex <==

\begin{tikzpicture}[scale = 1]
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=-1,xmax=5.5,ymin=-1.0,ymax=5.5,
  tick style={draw=none},
  xticklabels=\empty,
  yticklabels=\empty,
  xlabel={$E[(\Delta^z_0-\Delta^z_1)^2]$},
  ylabel={$E[(\Delta^z_0-\Delta^z_2)^2]$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.8,0.15)},anchor=north},
    y label style={at={(axis description cs:0.15,.75)},rotate=90,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  title={A. Model Selection - High Noise},
  grid=major,
  grid style={thin,densely dotted,white!20}]

%45-deg lines
\addplot [domain=0:5.5,samples=2, color = black] {x} node[right]{};


%shading
\tikzstyle{rej1}=[draw=none,line width=10pt,preaction={clip, postaction={pattern=horizontal lines, pattern color=blue, opacity=0.3}}]
\tikzstyle{rej2}=[draw=none,line width=1pt,preaction={clip, postaction={pattern=vertical lines, pattern color=red, opacity=0.3}}]

\draw[rej1] (100,300) -- (100,850) -- (650,850)   -- cycle;
\draw[rej2] (300,100) -- (850,100) -- (850,650)   -- cycle;




\draw[draw=black,line width=0.5pt,dashed]  (100,300) -- (700,900)  -- cycle;

\draw[draw=black,line width=0.5pt,dashed]  (300,100) -- (900,700)  -- cycle;







\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (550,180) {{${Q}_1 > {Q}_2$}};

\node[text width=5.9cm,rotate = 40,color = black,fill = none] at (500,540) {{$H^\text{RV}_0$: ${Q}_1 = {Q}_2$}};


\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (300,550) {{${Q}_1 < {Q}_2$}};



%\draw[black, fill=black] (200,350) circle (10) ;
%\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (350,380) {{$G$}};

\end{axis}

\end{tikzpicture}\hfill
\begin{tikzpicture}[scale = 1]
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=-1,xmax=5.5,ymin=-1.0,ymax=5.5,
  tick style={draw=none},
  xticklabels=\empty,
  yticklabels=\empty,
  xlabel={$E[(\Delta^z_0-\Delta^z_1)^2]$},
  ylabel={$E[(\Delta^z_0-\Delta^z_2)^2]$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.8,0.15)},anchor=north},
    y label style={at={(axis description cs:0.15,.75)},rotate=90,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  title={B. Model Assessment - High Noise},
  grid=major,
  grid style={thin,densely dotted,white!20}]


%shading
\tikzstyle{rej1}=[draw=none,line width=10pt,preaction={clip, postaction={pattern=horizontal lines, pattern color=blue, opacity=0.3}}]
\tikzstyle{rej2}=[draw=none,line width=1pt,preaction={clip, postaction={pattern=vertical lines, pattern color=red, opacity=0.3}}]
\draw[rej1] (250,200) -- (250,850) -- (100,850) -- (100,200)   -- cycle;
\draw[rej2] (250,100) -- (250,200) -- (850,200) -- (850,100)   -- cycle;





\node[text width=5.9cm,rotate = 90,color = black,fill = none] at (130,550) {{$H_{0,1}^\text{AR}$: ${Q}_1 = 0$}};
\node[text width=5.9cm,rotate = 0,color = black,fill = none] at (550,140) {{$H^\text{AR}_{0,2}$: ${Q}_2 = 0$}};



\draw[draw=black,line width=0.5pt,dashed]  (250,100) -- (250,700)  -- cycle;

\draw[draw=black,line width=0.5pt,dashed]  (100,200) -- (700,200)  -- cycle;

%\draw[black, fill=black] (200,350) circle (10) ;
%\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (350,380) {{$G$}};
\end{axis}

\end{tikzpicture}



\begin{tikzpicture}[scale = 1]
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=-1,xmax=5.5,ymin=-1.0,ymax=5.5,
  tick style={draw=none},
  xticklabels=\empty,
  yticklabels=\empty,
  xlabel={$E[(\Delta^z_0-\Delta^z_1)^2]$},
  ylabel={$E[(\Delta^z_0-\Delta^z_2)^2]$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.8,0.15)},anchor=north},
    y label style={at={(axis description cs:0.15,.75)},rotate=90,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  title={C. Model Selection - Low Noise},
  grid=major,
  grid style={thin,densely dotted,white!20}]

%45-deg lines
\addplot [domain=0:5.5,samples=2, color = black] {x} node[right]{};


%shading
\tikzstyle{rej1}=[draw=none,line width=10pt,preaction={clip, postaction={pattern=horizontal lines, pattern color=blue, opacity=0.3}}]
\tikzstyle{rej2}=[draw=none,line width=1pt,preaction={clip, postaction={pattern=vertical lines, pattern color=red, opacity=0.3}}]



\draw[rej1] (100,180) -- (100,870) -- (800,870)   -- cycle;
\draw[rej2] (180,100) -- (870,100) -- (870,800)   -- cycle;



%\draw[draw=black,line width=0.5pt,dashed]  (100,300) -- (700,900)  -- cycle;

%\draw[draw=black,line width=0.5pt,dashed]  (300,100) -- (900,700)  -- cycle;



\draw[draw=black,line width=0.5pt,dashed]  (100,180) -- (700,770)  -- cycle;

\draw[draw=black,line width=0.5pt,dashed]  (180,100) -- (770,700)  -- cycle;





\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (550,180) {{${Q}_1 > {Q}_2$}};

\node[text width=5.9cm,rotate = 40,color = black,fill = none] at (500,540) {{$H^\text{RV}_0$: ${Q}_1 = {Q}_2$}};


\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (300,550) {{${Q}_1 < {Q}_2$}};



%\draw [->] (150,350)--(225,275);
%\draw [->] (300,500)--(375,425);
%\draw [->] (450,650)--(525,575);

%\draw [->] (350,150)--(275,225);
%\draw [->] (500,300)--(425,375);
%\draw [->] (650,450)--(575,525);

%\draw[black, fill=black] (200,350) circle (10) ;
%\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (350,380) {{$G$}};
\end{axis}

\end{tikzpicture}\hfill\hfill
\begin{tikzpicture}[scale = 1]
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=-1,xmax=5.5,ymin=-1.0,ymax=5.5,
  tick style={draw=none},
  xticklabels=\empty,
  yticklabels=\empty,
  xlabel={$E[(\Delta^z_0-\Delta^z_1)^2]$},
  ylabel={$E[(\Delta^z_0-\Delta^z_2)^2]$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.8,0.15)},anchor=north},
    y label style={at={(axis description cs:0.15,.75)},rotate=90,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  title={D. Model Assessment - Low Noise},
  grid=major,
  grid style={thin,densely dotted,white!20}]


%shading
\tikzstyle{rej1}=[draw=none,line width=10pt,preaction={clip, postaction={pattern=horizontal lines, pattern color=blue, opacity=0.3}}]
\tikzstyle{rej2}=[draw=none,line width=1pt,preaction={clip, postaction={pattern=vertical lines, pattern color=red, opacity=0.3}}]
%\draw<3>[rej1] (250,200) -- (250,850) -- (100,850) -- (100,200)   -- cycle;
%\draw<3>[rej2] (250,100) -- (250,200) -- (850,200) -- (850,100)   -- cycle;


\draw[rej1] (165,165) -- (165,850) -- (100,850) -- (100,165)   -- cycle;
\draw[rej2] (165,100) -- (165,165) -- (850,165) -- (850,100)   -- cycle;


%\draw<4> [<-] (160,600)--(250,600);
%\draw<4> [<-] (160,450)--(250,450);
%\draw<4> [<-] (160,300)--(250,300);

%\draw<4> [<-] (300,160)--(300,200);
%\draw<4> [<-] (450,160)--(450,200);
%\draw<4> [<-] (600,160)--(600,200);


\node[text width=5.9cm,rotate = 90,color = black,fill = none] at (130,550) {{$H_{0,1}^\text{AR}$: ${Q}_1 = 0$}};
\node[text width=5.9cm,rotate = 0,color = black,fill = none] at (550,130) {{$H_{0,2}^\text{AR}$: ${Q}_2 = 0$}};



%\draw<3-4>[draw=black,line width=0.5pt,dashed]  (250,100) -- (250,700)  -- cycle;

%\draw<3-4>[draw=black,line width=0.5pt,dashed]  (100,200) -- (700,200)  -- cycle;


\draw[draw=black,line width=0.5pt,dashed]  (165,100) -- (165,700)  -- cycle;

\draw[draw=black,line width=0.5pt,dashed]  (100,165) -- (700,165)  -- cycle;

%\draw[black, fill=black] (200,350) circle (10) ;
%\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (350,380) {{$G$}};
\end{axis}

\end{tikzpicture}


==> Submission/ECTA/Figures/space_degeneracy.tex <==
\begin{tikzpicture}
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=-1,xmax=5.5,ymin=-1.0,ymax=5.5,
  tick style={draw=none},
  xticklabels=\empty,
  yticklabels=\empty,
  xlabel={$E[(\Delta^z_0-\Delta^z_1)^2]$},
  ylabel={$E[(\Delta^z_0-\Delta^z_2)^2]$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.8,0.15)},anchor=north},
    y label style={at={(axis description cs:0.15,.75)},rotate=90,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  %title={Relationship Between Null and Degeneracy},
  grid=major,
  grid style={thin,densely dotted,white!20}]

%45-deg lines
\addplot [domain=0:5.5,samples=2, color = black] {x} node[right]{};


%shading
\tikzstyle{rej1}=[draw=none,line width=10pt,preaction={clip, postaction={pattern=horizontal lines, pattern color=blue, opacity=0.2}}]
\tikzstyle{rej2}=[draw=none,line width=1pt,preaction={clip, postaction={pattern=vertical lines, pattern color=red, opacity=0.2}}]
%\draw[rej1] (100,100) -- (100,850) -- (850,850)   -- cycle;
%\draw[rej2] (100,100) -- (850,100) -- (850,850)   -- cycle;



%\node<5-6>[text width=1.0cm,rotate = 90,color = black,fill = none] at (70,50) {{$TE1$}};


\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (400,130) {{$\Gamma_2 = \Gamma_0$}};




\node[text width=5.9cm,rotate = 40,color = black,fill = none] at (410,370) {{ $\Gamma_1 = \Gamma_2$}};



\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (550,250) {{${Q}_1 > {Q}_2$}};

\node[text width=5.9cm,rotate = 40,color = black,fill = none] at (500,540) {{$H^\text{RV}_0$: ${Q}_1 = {Q}_2$}};


\node[text width=2.0cm,rotate = 0,color = black,fill = none] at (300,30) {{$\sigma^2_\text{RV} = 0$}};




\node[text width=3.0cm,rotate = 90,color = black,fill = none] at (125,350) {{$\Gamma_1 = \Gamma_0$}};

\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (300,450) {{${Q}_1 < {Q}_2$}};



\draw[-stealth,decorate,decoration={snake,amplitude=4pt,pre length=3pt,post length=4pt}] (100,100) -- ++(100,-70);
\draw[-stealth,decorate,decoration={snake,amplitude=4pt,pre length=3pt,post length=4pt}] (100,100) -- ++(100,-70);


%origin
\draw[red, fill=red] (100,100) circle (10) ;


\end{axis}

\end{tikzpicture}

==> Submission/ECTA/Proofs/Pf_ConvergProb_Misspecification.tex <==
\begin{proof}[Proof of Proposition \ref{prop:distrib_TE2}.]
For $(i)$, we use \eqref{eq:line2}, \eqref{eq:line5}, and the definition of the local alternative in \eqref{eq:local selection} to write
\begin{align}
\sqrt{n}\left( Q_1 -Q_2 \right) &= \sqrt{n}\left( (\Gamma_0-\Gamma_1) - (\Gamma_0-\Gamma_2) \right)\!' E[z_iz_i']\!\left( (\Gamma_0-\Gamma_1) + (\Gamma_0-\Gamma_2) \right)\! \\
&= q'E[z_iz_i']\!\left( (\Gamma_0-\Gamma_1) + (\Gamma_0-\Gamma_2) \right)\!.
\end{align}
%From Lemma 1 in \cite{rv02} or the proof of Proposition \ref{prop:degen}, we have that Assumption \ref{as:nodegen} implies that $\sqrt{n}\left( Q_1 -Q_2 \right)$ is bounded away from zero.
%From Proposition \ref{prop:degen} and its proof, we have that Assumption \ref{as:nodegen} and the local alternative in \eqref{eq:local selection} implies that $(\Gamma_0-\Gamma_1) + (\Gamma_0-\Gamma_2)$ is bounded away from zero. Furthermore, 
Assumption \ref{as:regcond}, part (iii), implies that $(\Gamma_0-\Gamma_1) + (\Gamma_0-\Gamma_2) $ is bounded. We therefore assume essentially without loss of generality that $\sqrt{n}\left( Q_1 -Q_2 \right)$ is a constant, say $c$.\footnote{This assumption is essentially without loss of generality since the boundedness of $(\Gamma_0-\Gamma_1) + (\Gamma_0-\Gamma_2)$, and therefore of $\sqrt{n}\left( Q_1 -Q_2 \right)$, allows us to otherwise argue along subsequences where $\sqrt{n}\left( Q_1 -Q_2 \right)$ converges to a constant.} From \eqref{eq:line1} and \eqref{eq:line5}, we can also write 
\begin{align}
    c &= \sqrt{n} \!\left( E\!\left[(\Delta_{0i}^{z}-\Delta_{1i}^z)^2\right] - E\!\left[(\Delta_{0i}^{z}-\Delta_{2i}^z)^2\right] \right) \\
    &= E\!\big[(\Delta_{0i}^{\text{RV},z}-\Delta_{1i}^{\text{RV},z})^2\big] - E\!\big[(\Delta_{0i}^{\text{RV},z}-\Delta_{2i}^{\text{RV},z})^2\big].
\end{align}

As in Remark \ref{rem:validity}, a first order Taylor expansion, Lemma \ref{lem:asymp norm}, parts $(i)$ and $(ii)$, together with consistency of $\hat \sigma^2_\text{RV}$ now leads to
\begin{align}
    T^\text{RV} = \frac{c}{\sigma_\text{RV}} + \frac{g_1'W^{1/2} \hat W^{1/2}\hat g_1 - g_2'W^{1/2} \hat W^{1/2}\hat g_2}{\sigma_\text{RV}} + o_p(1) \xrightarrow{d} N(c,1).
\end{align}

For $(ii)$, we first note that Assumption \ref{as:homsked} implies that
\begin{align}
    V^\text{AR}_{mm} = E[z_iz_i']\inverse E[e_{mi}^2 z_iz_i'] E[z_iz_i']\inverse = \sigma_m^2 E[z_iz_i'].
\end{align}
Thus we have from \eqref{eq:line2} and \eqref{eq:line5} that 
\begin{align}
    \sigma_m^2 n\pi_m'\big( V^\text{AR}_{mm}\big)\inverse\pi_m = n(\Gamma_0-\Gamma_m)'E[z_i z_i'](\Gamma_0-\Gamma_m) = q_m'E[z_i z_i']q_m
\end{align}
which in turn yields that $n\pi_m'\big( V^\text{AR}_{mm}\big)\inverse\pi_m = E\big[(\Delta^{\text{AR},z}_{0i}-\Delta^{\text{AR},z}_{mi}) ^2\big]/\sigma_m^2$ is a constant, say $c_m$. From Lemma \ref{lem:asymp norm}, parts $(iii)$ and $(iv)$, and continuous mapping we then have
\begin{align}
    T_m^\text{AR} &= n \hat \pi_m'\big( \hat V^\text{AR}_{mm}\big)\inverse \hat \pi_m = n \hat \pi_m'\big( V^\text{AR}_{mm}\big)\inverse \hat \pi_m + o_p(1) \xrightarrow{d} \chi^2_{d_z}(c_m). \qedhere
\end{align}
%
\begin{comment}
It is useful to note the following identities for each model $m$:
\begin{align}
\omega_m &= p-\Delta\theta_m\\
\omega_m &= \Delta^{*}\theta_0-\Delta\theta_m + \omega_0\\
\omega_m &= \Delta^{*}_0-\Delta_m + \omega_0.
\end{align}
Since in this environment true markups $\Delta^*$ differ from observed markups $\Delta$, we need the following definitions:
\begin{align}
A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta^*} &=  E[\tilde\Delta_{i} \tilde\Delta^{*\prime}_{i}], 
\end{align}
and
\begin{align}
    \lambda = E[\tilde\Delta_{i} \tilde\Delta_{i}']^{-1}E[\tilde\Delta_{i} \tilde\Delta^{*\prime}_{i}].
\end{align}

\begin{enumerate}
\item[\textbf{(i) - EB}] For EB, we first consider the object $\hat\theta$
\begin{align*}
\hat\theta  &= (\Delta'P_z\Delta)^{-1}\Delta'P_zp\\
&=  (\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}\hat A_{\Delta z} \hat A_{z z}^{-1}\hat A_{z\Delta^*}\theta_0+  (\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}\hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{n}\\
&\rightarrow_p (A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1} A_{\Delta z}  A_{z z}^{-1}A_{z\Delta^*}\theta_0+ (A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1} A_{\Delta z}  A_{z z}^{-1} E[z_i \omega_{0i}']\\
&=\lambda\theta_0
\end{align*}
So we have, approximating the asymptotic variance with the expression (\ref{eq:avarapprox})\footnote{Since the proposition concerns the plim of the test statistic, adopting this approximation does not alter the result.}:
\begin{align}
{n}(\hat\theta - \theta_m)'\hat V_{\theta}^{-1} (\hat\theta - \theta_m)
&\rightarrow_p \lim_{n\rightarrow\infty} {n}( (\lambda\theta_0- \theta_m)' V_{\theta}^{-1}( \lambda\theta_0- \theta_m))\\
&\approx \lim_{n\rightarrow\infty} {n}\frac{( \lambda\theta_0- \theta_m)'  E[\tilde\Delta_{i}\tilde\Delta_{i}']( \lambda\theta_0- \theta_m)}{\sigma^2_{\omega_0}}\\
&= \lim_{n\rightarrow\infty} {n}\frac{E[(\theta_0'\lambda\tilde\Delta_{i}-\tilde\Delta_{mi})^2]}{\sigma^2_{\omega_0}}\\
&=\lim_{n\rightarrow\infty} {n}\frac{ E\bigg[\bigg((\tilde{\tilde{\Delta}}^{*}_{0i}-\tilde\Delta_{0i})+(\tilde\Delta_{0i}-\tilde\Delta_{mi})\bigg)^2\bigg] }{\sigma^2_{\omega_{0}}}.
\end{align}
Note that, by Proposition \ref{prop:absfit}, $\tilde{\tilde{\Delta}}^*_{0i} = \tilde\Delta^*_{0i}$
\item[\textbf{(ii) - AR}] To derive the plim of the AR test statistic, we first consider the object $\hat\pi_m$
\begin{align*}
\hat\pi_m &= (z'z)^{-1}z'(\Delta^*\theta_0 + \omega_0 - \Delta\theta_m)\\
&= \hat A_{zz}^{-1}(\hat A_{z\Delta^*}\theta_0-\hat A_{z\Delta}\theta_m) + \hat A_{zz}^{-1}\frac{z'\omega_0}{n} \\
&\rightarrow_p A_{zz}^{-1} (A_{z\Delta^*}\theta_0-A_{z\Delta}\theta_m) + A_{zz}^{-1}E[z_i\omega_{0i}']\\
&=  \Gamma^*\theta_0-\Gamma\theta_m 
\end{align*}
So we have, under the approximation of the asymptotic variance given in (\ref{eq:avarapprox}):
\begin{align*}
T^{AR,m}&\rightarrow_p \lim_{n\rightarrow\infty} {n}(\Gamma^*\theta_0-\Gamma\theta_m)' V_{\pi_m}^{-1} (\Gamma^*\theta_0-\Gamma\theta_m)  \\
&\approx\lim_{n\rightarrow\infty} {n}\frac{(\Gamma^*\theta_0-\Gamma\theta_m)' A_{zz} (\Gamma^*\theta_0-\Gamma\theta_m)}{\sigma^2_{\omega_{0}}}  \\
&=\lim_{n\rightarrow\infty} {n}\frac{ E[(\tilde\Delta^*_{0i}-\tilde\Delta_{mi})^2] }{\sigma^2_{\omega_{0}}}  \\
&=\lim_{n\rightarrow\infty} {n}\frac{ E\bigg[\bigg((\tilde\Delta^*_{0i}-\tilde\Delta_{0i})+(\tilde\Delta_{0i}-\tilde\Delta_{mi})\bigg)^2\bigg] }{\sigma^2_{\omega_{0}}}  \\
\end{align*}

\item[\textbf{(iii) - RV}] To derive the plim of the RV test statistic we start from the object:

\begin{align*}
Q_1 - Q_2 
&= g_1'Wg_1 - g_2'Wg_2\\
&= \frac{1}{n}(\Delta^*\theta_0 - \Delta\theta_1+ \omega_0)' P_z(\Delta^*\theta_0 - \Delta\theta_1+ \omega_0)- \frac{1}{n}(\Delta^*\theta_0 - \Delta\theta_2+ \omega_0)'  P_z(\Delta^*\theta_0 - \Delta\theta_2+ \omega_0)\\
&= (\theta_0\hat A_{\Delta^*z} -\theta_1\hat A_{\Delta z})' \hat A_{zz}^{-1}(\hat A_{\Delta^*z}\theta_0 - \hat A_{\Delta z}\theta_1) - (\theta_0\hat A_{\Delta^*z} -\theta_2\hat A_{\Delta z})' \hat A_{zz}^{-1}(\hat A_{\Delta^*z}\theta_0 - \hat A_{\Delta z}\theta_2) \\
&\qquad+ 2(\theta_2-\theta_1)\hat A_{\Delta z} A_{zz}^{-1} \frac{\omega_0'z}{n}\\
& \rightarrow_p   (\theta_0 A_{\Delta^*z} -\theta_1 A_{\Delta z})'  A_{zz}^{-1}A_{zz}A_{zz}^{-1}( A_{\Delta^*z}\theta_0 - A_{\Delta z}\theta_1) \\
&\qquad- (\theta_0 A_{\Delta^*z} -\theta_2 A_{\Delta z})' A_{zz}^{-1}A_{zz}A_{zz}^{-1}( A_{\Delta^*z}\theta_0 -  A_{\Delta z}\theta_2)\\
& =  E[(\theta_0 \tilde\Delta^*_{i} -\theta_1 \tilde\Delta_i)^2] - E[(\theta_0 \tilde\Delta^*_{i} -\theta_2 \tilde\Delta_i)^2]
\end{align*}



\item[\textbf{(iv) - Cox}] For Cox, the numerator of the test statistic when using the formulation in Smith (1992) is:
 \begin{align*}
&  g_{-m}'A_{zz}^{-1}  g_{-m} - g_{m}'A_{zz}^{-1} g_m -(g_{-m} - g_m)'A_{zz}^{-1}(g_{-m} - g_m)\\
&= Q_{-m} - Q_m - (\theta_m'\hat A_{z\Delta*}' - \theta_{-m}'\hat A_{z\Delta}')\hat A_{z'z}^{-1}(\hat A_{z\Delta*}\theta_m - \hat A_{z\Delta}\theta_{-m}))\\
&\rightarrow_p  E[(\tilde\Delta^*_{0i}-\tilde\Delta_{-mi})^2] -E[(\tilde\Delta^*_{0i}-\tilde\Delta_{mi})^2]  - E[(\tilde\Delta^*_{mi}-\tilde\Delta_{-mi})^2] 
\end{align*}
So we have, under the approximation of the asymptotic variance given in (\ref{eq:avarapprox}):
\begin{align}
T^{cox,m}
&\rightarrow_p  2\lim_{n\rightarrow\infty} \sqrt{n}\frac{  E[(\tilde\Delta^*_{0i}-\tilde\Delta_{-mi})^2] -E[(\tilde\Delta^*_{0i}-\tilde\Delta_{mi})^2]  - E[(\tilde\Delta^*_{mi}-\tilde\Delta_{-mi})^2]  }{\sigma_{cox}} \\
&\approx 2\lim_{n\rightarrow\infty} \sqrt{n}\frac{  E[(\tilde\Delta^*_{0i}-\tilde\Delta_{-mi})^2] -E[(\tilde\Delta^*_{0i}-\tilde\Delta_{mi})^2]  - E[(\tilde\Delta^*_{mi}-\tilde\Delta_{-mi})^2]  }{2\sigma_{\omega_0} \sqrt{E[(\tilde\Delta_{1i}-\tilde\Delta_{2i})^2]}}.
\end{align} 
\end{enumerate}
\end{comment}
\end{proof}

==> Submission/ECTA/Proofs/Pf_Degeneracy.tex <==
\begin{proof}[Proof of Proposition \ref{prop:degen} and Corollary \ref{cor:degen}]

From \eqref{eq:line1} and \eqref{eq:line2}, we have equivalence between $E[(\Delta^z_{0i}-\Delta^z_{mi})^2] = 0$ and $\Gamma_0-\Gamma_m=0$. Furthermore, we recall that $\pi_m=\Gamma_0-\Gamma_m$. Thus, we only need to show that $\sigma^2_\text{RV}=0$ if and only if $\pi_m=0$ for all $m\in\{1,2\}$. Rewriting \eqref{eq:sig2rv} in matrix notation, we have
\begin{align}
    \sigma^2_\text{RV} = 4 
    \begin{pmatrix} W^{-1/2}\pi_1 \\ W^{-1/2}\pi_2 \end{pmatrix}'
    \begin{bmatrix}    V^\text{RV}_{11} & - V^\text{RV}_{12} \\ - V^\text{RV}_{12} & V^\text{RV}_{22}\end{bmatrix}
    \begin{pmatrix} W^{-1/2}\pi_1 \\ W^{-1/2}\pi_2 \end{pmatrix}.
\end{align}
Therefore, the claims to be proven follow from positive definiteness of the variance matrix $V^\text{RV} = E[(\psi_{1i}',\psi_{2i}')'(\psi_{1i}',\psi_{2i}')]$, which is the matrix with $V^\text{RV}_{11}$, $V^\text{RV}_{12}$, and $V^\text{RV}_{22}$ as its entries.

To show that $V^\text{RV}$ is positive definite, we take an arbitrary non-zero, non-random vector $v=(v_1',v_2')' \in \mathbb{R}^{2d_z}$. $V^\text{RV}$ is positive definite if $E(v_1'\psi_{1i}+v_2'\psi_{2i})^2 > 0$ for any such $v$. For certain implied non-random $u = (u_1',u_2')'$, $t=(t_1',t_2')'$ where $t$ is non-zero, we have $E(v_1'\psi_{1i}+v_2'\psi_{2i})^2 = E(u_1'z_i \cdot u_2'z_i + t_1'z_i \cdot e_{1i} + t_2'z_i \cdot e_{2i} )^2$. Because $\sigma_{12}^2 < \sigma_1^2\sigma_2^2$ (Assumption \ref{as:homsked}), we have that $E(t_1'z_i \cdot e_{1i} + t_2'z_i \cdot e_{2i} )^2 > 0$. Therefore, we can only have $E(v_1'\psi_{1i}+v_2'\psi_{2i})^2 = 0$ if $e_{1i}$ or $e_{2i}$ is a linear function of $z_i$ almost surely. However, because $E[z_ie_{mi}]=0$, such dependence is ruled out by $\sigma_m^2>0$ (Assumption \ref{as:homsked}).
%
%
%
%
% We begin by noting that Lemma 1 in \citeA{rv02} shows that $\sigma^2_{RV}=0$ if and only if $   \sqrt{n}(Q_1-Q_2)=o_p(1)$.
% Thus, for Proposition \ref{prop:weakinstr}, we need to show the equivalence
% $$\sqrt{n}(\hat Q_1-\hat Q_2) = o_p(1) \qquad \Leftrightarrow  \qquad E[(\Delta^z_{0i}-\Delta^z_{mi})^2] = 0 \qquad\text{for both $m=1,2$}$$
% From \eqref{eq:line1}, \eqref{eq:line4}, and the positive definiteness of $E[z_iz_i']$, $E[(\Delta^z_{0i}-\Delta^z{m_i})^2] = 0$ iff $g_m = 0$. By \eqref{eq:sig2rv}, if $g_1$ and $g_2$ = 0, then $\sigma^2_{RV} = 0$.  Furthermore, if $\sigma^2_{RV} = 0$ 
%
%
% Consider $Q_1-Q_2$:
% \begin{align*}
% Q_1-Q_2 &=
% %\frac{1}{n} \omega_1'z(z'z)^{-1}z'\omega_1  -  \frac{1}{n}\omega_2'z(z'z)^{-1}z'\omega_2 \\ &=
% \frac{1}{n} \bigg(\omega_1-\omega_2\bigg)'z(z'z)^{-1}z'\bigg(\omega_1+\omega_2\bigg) \\
% % &= \frac{1}{n}\bigg(p-\Delta_1-p+\Delta_2\bigg)'z(z'z)^{-1}z'\bigg(p-\Delta_1+p-\Delta_2\bigg) \\
%   &= \frac{1}{n}\bigg(p-\Delta_1-p+\Delta_2\bigg)'z(z'z)^{-1}z'\bigg(2p-\Delta_1-\Delta_2\bigg) \\
%   &= \frac{1}{n}\bigg(p-\Delta_1-p+\Delta_2\bigg)'z(z'z)^{-1}z'\bigg(2\Delta^*_0 +2\omega_0-\Delta_1-\Delta_2\bigg) \\
% %    &= \frac{1}{n}\bigg(\Delta_2-\Delta_1\bigg)'z(z'z)^{-1}z'\bigg(\Delta_1 +2\omega_0-\Delta_2\bigg) \\
%       &= \frac{1}{n}\bigg(\Delta_2-\Delta_1\bigg)'z(z'z)^{-1}z'\bigg(\Delta^*_0 - \Delta_1 + \Delta^*_0 -\Delta_2\bigg) +2\frac{1}{n}\bigg(\Delta_2-\Delta_1\bigg)'z(z'z)^{-1}z'\omega_0 \\
% %  &= \frac{1}{n}\bigg(\Delta_2-\Delta_1\bigg)'z(z'z)^{-1}z'z(z'z)^{-1}z'\bigg(\Delta_1-\Delta_2\bigg) +2\frac{1}{n}\bigg(\Delta_2-\Delta_1\bigg)'z(z'z)^{-1}z'\omega_0 \\
%   &= \frac{1}{n}\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'z'z\bigg(\hat\Gamma_0 - \hat\Gamma_1 + \hat\Gamma_0 -\hat\Gamma_2\bigg) +2\frac{1}{n}\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'z'\omega_0 
%   \end{align*}
% %  So we have:
% %  \begin{align*}
% %    \sqrt{n}(Q_1-Q_2) &= \frac{1}{\sqrt{n}}\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'z'z\bigg(\hat\Gamma_0 - \hat\Gamma_1 + \hat\Gamma_0 -\hat\Gamma_2\bigg) +2\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'\frac{z'\omega_0}{\sqrt{n}}
% %  \end{align*}
%
% %If $\hat \gamma = \hat \Gamma_1-\hat \Gamma_2 = o_p(1)$, $\hat \Gamma_0-\frac{\hat \Gamma_1 + \hat\Gamma_2}{2} = \frac{O_p(1)}{\sqrt{n}} =  o_p(1)$, and $\frac{z'\omega_0}{\sqrt{n}} = O_p(1)$, then we have:
% %  \begin{align*}
% %      \sqrt{n}(Q_1-Q_2) &=\sqrt{n}\bigg(\hat\Gamma_0 - \hat\Gamma_1 + \hat\Gamma_0 -\hat\Gamma_2\bigg)'\frac{z'z}{n}\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg) +2\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'\frac{z'\omega_0}{\sqrt{n}}
% %  \end{align*}
% %    \begin{align*}
%  %     \sqrt{n}(Q_1-Q_2) &=\underbrace{\sqrt{n}\bigg(\hat\Gamma_1 - \hat\Gamma_0 + \hat\Gamma_2 -\hat\Gamma_0\bigg)'}_{= O_p(1)}\underbrace{\frac{z'z}{n}}_{\rightarrow A_{zz}}\underbrace{\bigg(\hat\Gamma_1-\hat\Gamma_2\bigg)}_{=o_p(1)} +\underbrace{2\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'}_{=o_p(1)}\underbrace{\frac{z'\omega_0}{\sqrt{n}}}_{= O_p(1)}
%  % \end{align*}
%  % so that $ \sqrt{n}(Q_1-Q_2) = o_p(1)$ if and only if $\hat \gamma = o_p(1)$.
% 
%  For $m = 0,1,2$, given that $\hat\Gamma_m$ is a OLS regression coefficient and given the regularity conditions in Assumptions \ref{as:regcond}, $\hat\Gamma_m \rightarrow_p \Gamma_m$ so that $\hat\Gamma_m - \Gamma_m = o_p(1)$ and $\sqrt{n}(\hat\Gamma_m-\Gamma_m) = O_p(1)$.  Let $\hat\psi_m = (\hat\Gamma_m-\Gamma_m)$.
%       \begin{align*}
%       \sqrt{n}(Q_1-Q_2) &=\sqrt{n}\bigg(\hat\Gamma_1 - \hat\Gamma_0 + \hat\Gamma_2 -\hat\Gamma_0\bigg)'\frac{z'z}{n}\bigg(\hat\Gamma_1-\hat\Gamma_2\bigg) + 2\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'\frac{z'\omega_0}{\sqrt{n}}\\
%       &= \bigg(\sqrt{n}\bigg(\hat\psi_1-2\hat\psi_0 +  \hat\psi_2 \bigg) +\sqrt{n}(\Gamma_1 + \Gamma_2 - 2\Gamma_0)\bigg)'\frac{z'z}{n}\bigg(\hat\psi_1 -\hat\psi_2+\Gamma_1 - \Gamma_2\bigg)+\\&\qquad 2\bigg(\hat\psi_2-\hat\psi_1 +\Gamma_2-\Gamma_1\bigg)'\frac{z'\omega_0}{\sqrt{n}}
%   \end{align*}
%   Notice that, by Assumptions \ref{as:momcond} and \ref{as:regcond}, $\frac{z'\omega_0}{\sqrt{n}} = O_p(1)$ and $\frac{z'z}{n} = O_p(1)$.  Using the following facts\footnote{See page 12 of van der Vaart's \textit{Asymptotic Statistics}} $O_p(1)o_p(1) = o_p(1)$, $o_p(1) + o_p(1) = o_p(1)$, we can show that $\sqrt{n}(Q_1-Q_2) = o_p(1)$ if and only if the following two conditions hold: (i) $\Gamma_2 = \Gamma_1$ and (ii) $\Gamma_0 = \frac{\Gamma_1+\Gamma_2}{2}$.  To show the if part of the statement, if both (i) and (ii) hold, then:
%   \begin{align*}
%       \sqrt{n}(Q_1-Q_2) &=\bigg(\sqrt{n}\bigg(\hat\psi_1-2\hat\psi_0 +  \hat\psi_2 \bigg)\bigg)'\frac{z'z}{n}\bigg(\hat\psi_1 -\hat\psi_2\bigg)+ 2\bigg(\hat\psi_2-\hat\psi_1 \bigg)'\frac{z'\omega_0}{\sqrt{n}}\\
%       &= O_p(1)(O_p(1)o_p)) + o_p(1)O_p(1)\\
%       &= o_p(1) + o_p(1)\\
%       & = o_p(1)
%   \end{align*}
% Now to show the only if part of the statement, first suppose (i) holds but (ii) does not.  Then we have
%   \begin{align*}
%       \sqrt{n}(Q_1-Q_2) &=
%       \bigg(O_p(1) +\sqrt{n}(\Gamma_1 + \Gamma_2 - 2\Gamma_0)\bigg)'o_p(1)+ o_p(1) \\
%       &=
%       o_p(1) +\sqrt{n}(\Gamma_1 + \Gamma_2 - 2\Gamma_0)o_p(1)\\
%     &= o_p(1) + o_p(\sqrt{n}(\Gamma_1 + \Gamma_2 - 2\Gamma_0)\\
%     &\neq o_p(1)
%     \end{align*}
%   Now suppose (ii) holds but (i) does not. 
%   \begin{align*}
%       \sqrt{n}(Q_1-Q_2) &= O_p(1)(o_p(1) + \Gamma_1-\Gamma_2) + o_p + (\Gamma_1-\Gamma_2)O_p(1)\\
% &= o_p(1) + O_p(1)(\Gamma_1-\Gamma_2)\\
% &\neq o_p(1)
%       \end{align*}
%
% Thus, we have established $\sqrt{n}(Q_1-Q_2) = o_p(1)$ iff $\Gamma_1 = \Gamma_2$ and $\Gamma_0 = \frac{\Gamma_1 + \Gamma_2}{2}$.  Notice, that, if we combine conditions (i) and (ii), $\sqrt{n}(Q_1-Q_2) = o_p(1)$ iff $\Gamma_1 = \Gamma_2 = \Gamma_0$.  Thus, we can express this in terms of weak instruments.  Specifically,  $\sqrt{n}(Q_1-Q_2) = o_p(1)$ iff $\hat\Gamma_0 - \hat\Gamma_m = o_p(1)$ for $m = 1,2$.  We can also express degeneracy in terms of predicted markups.  $E[(\tilde\Delta^*_{0i}-\tilde\Delta_{mi})^2] = E[(\Gamma_0-\Gamma_m)z_iz_i'(\Gamma_0-\Gamma_m)] = (\Gamma_0-\Gamma_m)E[z_iz_i'](\Gamma_0-\Gamma_m)] = 0$  So under Assumption \ref{as:regcond}, $\sqrt{n}(Q_1-Q_2) = o_p(1)$ iff $E[(\tilde\Delta^*_{0i} - \tilde\Delta_{mi})^2] = 0$ for $m =1,2$.  We could also write $E[(\tilde\Delta_{0i}-\tilde\Delta_{mi}] = E[((\Gamma_0-\Gamma_m)z_i] = (\Gamma_0-\Gamma_m)E[z_i] $ but this is always 0 due to the orthogonalization
\end{proof}


==> Submission/ECTA/Proofs/Pf_Nulls.tex <==
\begin{proof}[Proof of Proposition \ref{prop:nulls}]
For $(i)$, we need to show the equivalence
\begin{align}\label{eq:equiv_prop1_ar}
\pi_m = 0 \qquad \Leftrightarrow \qquad   E[(\Delta^z_{0i}-\Delta^z_{mi})^2] = 0  
\end{align}
This equivalence is a consequence of \eqref{eq:line1}, \eqref{eq:line5}, and $E[z_i z_i']$ being positive definite.
For $(ii)$, we we need to show the equivalence
\begin{align}
    {Q}_1-{Q}_2 =0  \qquad \Leftrightarrow \qquad  E[(\Delta^z_{0i}-\Delta^z_{1i})^2]-E[(\Delta^z_{0i}-\Delta^z_{2i})^2]=0. 
\end{align}
This equivalence is a consequence of \eqref{eq:line1} and \eqref{eq:line5}.
%
\begin{comment}
\begin{align}\label{eq:equiv_prop1_ar}
\pi_m = 0 \qquad \Leftrightarrow \qquad   E[(\Delta^z_{0i}-\Delta^z_{mi})^2] = 0  
\end{align}
By definition of the OLS estimator, $\pi_m$ is:
\begin{align}
    \pi_m &= E[z_iz_i']^{-1}E[z_i(p_i-\Delta_{mi})] \\
        %&=E[z_iz_i']^{-1}E[z_i(\Delta_{0i}-\Delta_{mi})]\\
        &=(\Gamma_{0}-\Gamma_{m})
    \end{align}
where the second equality follows from Assumption \ref{as:momcond}, $E[z_i w_{0i}]=0$, and $\Delta_{0i} = p_i - \omega_{0i}$.  From the Proof of Lemma 1, it follows that $E[(\Delta^z_{0i}-\Delta^z_{mi})^2]=\pi_m'E[z_i'z_i]\pi_m$. 
The equivalence in \eqref{eq:equiv_prop1_ar} now follows from $E[z_i z_i']$ being positive definite.\\
For (ii), we can directly show the equivalence ${Q}_m = E[(\Delta^z_{0i}-\Delta^z_{mi})^2] $.
\begin{align*}
{Q}_m &= E[\omega_{mi}z_i]'E[z_i z_i']^{-1}E[\omega_{mi}z_i]\\
&=E[(\Delta_{0i}-\Delta_{mi})z_i]'E[z_i z_i']^{-1}E[(\Delta_{0i}-\Delta_{mi})z_i]\\
%&=E[(\Delta_{0i}-\Delta_{mi})z_i]'E[z_i z_i']^{-1}E[z_i z_i']E[z_i z_i']^{-1}E[(\Delta_{0i}-\Delta_{mi})z_i]\\
&=(\Gamma_0-\Gamma_m)'E[z_i z_i'](\Gamma_0-\Gamma_m)\\
&=E[(\Delta^z_{0i}-\Delta^z_{mi})^2]
\end{align*}     
where the second equality follows from  Assumption \ref{as:momcond}, $E[z_i w_{0i}]=0$, $\Delta_{mi} = p_i-\omega_{mi}$, and  $\Delta_{0i} = p_i - \omega_{0i}$. The last equality is proven in the Proof of Lemma 1.  Thus, ${Q}_1-{Q}_2 = E[(\Delta^z_{0i}-\Delta^z_{1i})^2]-E[(\Delta^z_{0i}-\Delta^z_{2i})^2] $
\end{comment}
%
\begin{comment}
\begin{enumerate}
    \item Note that for AR, the OLS estimator is given as:
    \begin{align}
    \pi_m &= E[z_iz_i']^{-1}E[z_i(p_i-\Delta_{mi})] \\
    &=E[z_iz_i']^{-1}E[z_i(\Delta_{0i}-\Delta_{mi})] + E[z_iz_i']^{-1}E[z_i\omega_{0i})]\\
        &=E[z_iz_i']^{-1}E[z_i(\Delta_{0i}-\Delta_{mi})]\\
        &=(\Gamma_{0i}-\Gamma_{mi})
    \end{align}
    We can rewrite the moment in Lemma \ref{lemma1} as:
    \begin{align}
        E[(\Delta^z_{0i}-\Delta^z_{mi})^2] &=E[(z_iE[z_iz_i']^{-1}E[z_i(\Delta_{0i}-\Delta_{mi})])^2]\\
        &=E[(z_i\pi_m)^2]\\
         &=E[z_i\pi_m \pi_m'z_i']\\
         &=E[\pi_m'z_i'z_i\pi_m ]\\
                  &=\pi_m'E[z_i'z_i]\pi_m 
    \end{align}
    Since $E[z_i'z_i]$ is positive definite, then it immediately follows from the definition of positive definite that $E[(\Delta^z_{0i}-\Delta^z_{mi})^2] = 0$ iff $\pi_m = 0$.
\item 
\begin{align*}
\mathcal{Q}_m &= E[\omega_{mi}z_i]'E[z_i z_i']^{-1}E[\omega_{mi}z_i]\\
&= E[(\Delta_{0i}-\Delta_{mi}+\omega_{0i})z_i]'E[z_i z_i']^{-1}E[(\Delta_{0i}-\Delta_{mi}+\omega_{0i})z_i]\\
&=E[(\Delta_{0i}-\Delta_{mi})z_i]'E[z_i z_i']^{-1}E[(\Delta_{0i}-\Delta_{mi})z_i]\\
&=E[(\Delta_{0i}-\Delta_{mi})z_i]'E[z_i z_i']^{-1}E[z_i z_i']E[z_i z_i']^{-1}E[(\Delta_{0i}-\Delta_{mi})z_i]\\
&=(\Gamma_0-\Gamma_m)'E[z_i z_i'](\Gamma_0-\Gamma_m)\\
&=E[(\Gamma_0-\Gamma_m)'z_i z_i'(\Gamma_0-\Gamma_m)]\\
&=E[(\Delta^z_{0i}-\Delta^z_{mi})'(\Delta^z_{0i}-\Delta^z_{mi})]\\
&=E[(\Delta^z_{0i}-\Delta^z_{mi})^2]
\end{align*}     
Since $\mathcal{Q}_m = E[(\Delta^z_{0i}-\Delta^z_{mi})^2] $, $\mathcal{Q}_1-\mathcal{Q}_2 = E[(\Delta^z_{0i}-\Delta^z_{1i})^2]-E[(\Delta^z_{0i}-\Delta^z_{2i})^2] $
\end{enumerate}
\end{comment}
\end{proof}

==> Submission/ECTA/Proofs/Pf_Plims.tex <==
\begin{proof}[Proof of Lemma \ref{cor:modelmisc}.] For $(i)$, suppose for concreteness that $E[(\Delta^z_{0i}-\Delta^z_{1i})^2]<E[(\Delta^z_{0i}-\Delta^z_{2i})^2]$. We need to show that $\Pr\big( T^\text{RV} < -q_{1-\alpha/2}(N) \big) \rightarrow 1$ where $q_{1-\alpha/2}(N)$ is the $(1-\alpha/2)$-th quantile of a standard normal distribution. From Proposition \ref{prop:nulls}, part $(ii)$, we have $Q_1 < Q_2$. Lemma \ref{lem:asymp norm}, parts $(i)$ and $(ii)$, together with Remark \ref{rem:validity} yields $T^\text{RV}/\sqrt{n} = \frac{ \hat Q_1-\hat Q_2}{\hat \sigma_\text{RV}} \xrightarrow{p}  \frac{Q_1-Q_2}{\sigma_\text{RV}} < 0$. Therefore, $\Pr\big( T^\text{RV}/\sqrt{n} < -q_{1-\alpha/2}(N_{0,1})/\sqrt{n} \big) \rightarrow 1$.

For $(ii)$, suppose that $E[(\Delta^z_{0i}-\Delta^z_{mi})^2]\neq 0$ for some $m \in \{1,2\}$.  We need to show that $\Pr\big( \text{reject } H^\text{AR}_{0,m} \big) \rightarrow 1$. From Proposition \ref{prop:nulls}, part $(i)$, it follows that $\pi_m \neq 0$ and since $V^\text{AR}_{mm}$ is positive definite we have $\pi_m'V^\text{AR}_{mm}\inverse \pi_m > 0$. Using Lemma \ref{lem:asymp norm}, parts $(iii)$ and $(iv)$, we have $(\hat \pi_m,\hat V^\text{AR}_{mm}) \xrightarrow{p} (\pi_m,V^\text{AR}_{mm})$ so that $T^\text{AR}_m/n = \hat\pi_m'\big(\hat V^\text{AR}_{mm}\big)\inverse \hat\pi_m \xrightarrow{p} \pi_m'\big( V^\text{AR}_{mm}\big)\inverse \pi_m > 0$. Therefore, $\Pr\big( \text{reject } H^\text{AR}_{0,m} \big) = \Pr\big( T^\text{AR}_m/n > q_{1-\alpha}(\chi^2_{d_z})/n \big) \rightarrow 1$ where $q_{1-\alpha}(\chi^2_{d_z})/n ) \rightarrow 1$ where $q_{d_z}(1-\alpha)$ denotes the $(1-\alpha)$-th quantile of a $\chi^2_{d_z}$ distribution.
\begin{comment}
\begin{itemize}

\item[(i)]  Consider anly model $m$ such that $E[(\Delta^z_{0i}-\Delta^z_{mi})^2]\neq 0$.  By \eqref{eq:line1}, \eqref{eq:line5} and the positive definiteness of $E[z_iz_i']$, $\pi_m\neq 0$, representing a fixed alternative of the AR test under $H^{AR}_{A,m}$.  From Lemma A.1 (iii) $\hat\pi_m\rightarrow\pi_m$, and from  (iv) $\hat V_m\rightarrow V_m$. Thus, $\hat\pi_m'\hat V_m\hat\pi_m\rightarrow_p \pi_m' V_m\pi_m >0$, where the inequality hold because  $V_m$ is positive definite. It immediately follows that $T^{AR} \rightarrow \infty$ and $\Pr(\text{reject } H^{AR}_{0,m}) \rightarrow 1$.  

    \item[(ii)]  By Lemma A.1 (i), $\hat Q_m \rightarrow_p Q_m$ for $m=1,2$ and  by (ii), $\hat\sigma^2_{RV} \rightarrow_p \sigma^2_{RV} \neq 0$ under Assumption \ref{as:nodegen}. Thus, $T^{RV} = \frac{\sqrt{n} (\hat Q_1-Q_2)}{\hat \sigma_{RV}} \rightarrow_p \lim_{n\rightarrow\infty }  \frac{\sqrt{n}(Q_1-Q_2)}{\sigma_{RV}}$. For any pair of models $1,2$ by which     $E[(\Delta^z_{0i}-\Delta^z_{1i})^2]<E[(\Delta^z_{0i}-\Delta^z_{2i})^2]$, $Q_1<Q_2$  from \eqref{eq:line1} and \eqref{eq:line5}.  Thus, the models represent a fixed alternative satisfying $H^{RV}_{1}$
 In this case  $T^{RV}\rightarrow_p -\infty$ so that $\Pr(\text{reject } H^{RV}_0 \text{ for } m=1) \rightarrow 1$ as $n\rightarrow\infty$. Likewise for fixed alternatives satisfying $H^{RV}_{2}$,  $Q_1>Q_2$ and, from \eqref{eq:line1} and \eqref{eq:line5}, $E[(\Delta^z_{0i}-\Delta^z_{1i})^2]>E[(\Delta^z_{0i}-\Delta^z_{1i})^2]$ .  In this case  $T^{RV}\rightarrow_p \infty$ so that $\Pr(\text{reject } H^{RV}_0 \text{ for } m=2) \rightarrow 1$ as $n\rightarrow\infty$.
\end{itemize}
\end{comment} 
\end{proof}

==> Submission/ECTA/Proofs/Pf_Testability.tex <==
\begin{proof}[Proof of Lemma \ref{lemma1}.]

% \noindent Let model 1 be the true model. We want to show that if and only if the condition     \begin{align}\label{eq:testability3}
%     E[(\tilde\Delta_{1i} - \tilde\Delta_{2i})^2] \neq 0
%     \end{align}
% a candidate model $m=2$ is falsified, in the sense of Definition 1:
% \begin{align}\label{eq:testability2}
% E[z_i(p_i-\Delta_{2i})]\neq0. 
% \end{align}
% As a useful preliminary, recall that the first stage is:
% \begin{align*}
% \Delta_i &= z_i\Gamma + \eta_i\\
%         &= \tilde \Delta_i + \eta_i,
% \end{align*}
% where $\eta$   is projection error orthogonal to $z$ by construction, so that $E[z_i\eta_i] = 0$.

% We first prove that (\ref{eq:testability3}) implies (\ref{eq:testability2}). Notice that a necessary and sufficient for (\ref{eq:testability3}) to be true is that there exists some nonzero measure subset $Z$ of the support of $z_i$ such that for $z_i\in Z$ we have $\tilde \Delta_{1i}\neq\tilde \Delta_{2i}.$ In turn, because of the definition of projection, it must be that for $z_i\in Z$ we have $z_i \Gamma_1 \neq z_i \Gamma_2.$ Then, we know that $\Gamma_1 \neq  \Gamma_2$ which in turn implies $E[z_i\Delta_{1i}] \neq E[z_i\Delta_{2i}]$ since $\Gamma = E[z_iz_i']^{-1}E[z_i\Delta_i] $. Condition (\ref{eq:testability2}) follows immediately from the fact that model $m=1$ is the true model.

% Now we prove that (\ref{eq:testability2}) implies (\ref{eq:testability3}). To do so, we proceed by contradiction: suppose that (\ref{eq:testability2}) holds, but $ E[(\tilde\Delta_{1i} - \tilde\Delta_{2i})^2]=0.$ Then, almost surely $\tilde \Delta_{1i}=\tilde \Delta_{2i}$. Hence we can write:
% \begin{align*}
%     E[z_i(p_i - \tilde \Delta_{1i})] = E[z_i(p_i - \tilde \Delta_{2i})],
% \end{align*}
% and since $E[z_i\eta_i] = 0$ we have:
% \begin{align*}
%     E[z_i(p_i - \tilde \Delta_{1i} - \eta_{1i})] = E[z_i(p_i - \tilde \Delta_{2i} - \eta_{2i})],
% \end{align*}
% which leads to a contradiction of (\ref{eq:testability2}). Hence, when (\ref{eq:testability2}) holds, (\ref{eq:testability3}) must hold as well.


We need to show the equivalence
\begin{align}\label{eq:equivalence}
    E[(\Delta_{0i}^{z}-\Delta_{mi}^z)^2] \neq 0 \quad  \Leftrightarrow \quad E[z_i(p_i-\Delta_{mi})] \neq 0.
\end{align}
This equivalence follows from \eqref{eq:line1}, \eqref{eq:line4}, and $E[z_i z_i']$ being positive definite.
%
% Part (ii) of Assumption \ref{as:regcond} implies that $E[z'z]$ and $E[z_i z_i']$ are positive definite so that $\Gamma_m = E[z'z]^{-1} E[z'\Delta_m] = E[z_iz_i']^{-1} E[z_i\Delta_{mi}]$ and $\Delta_{mi}^z = z_i'\Gamma_m$ are well-defined. We can then note that
% \begin{align}
%     E[(\Delta_{0i}^{z}-\Delta_{mi}^z)^2] &= E[(z_i'(\Gamma_0-\Gamma_m))^2] \\
%     &= (\Gamma_0-\Gamma_m)'E[z_i z_i'](\Gamma_0-\Gamma_m) \\
%     &= E[z_i(\Delta_{0i}-\Delta_{mi})]'E[z_i z_i']^{-1}E[z_i(\Delta_{0i}-\Delta_{mi})]\\
%     &= E[z_i(p_i-\Delta_{mi})]'E[z_i z_i']^{-1}E[z_i(p_i-\Delta_{mi})]
% \end{align}
% where the last equality follows from Assumption \ref{as:momcond}, $E[z_i w_{0i}]=0$, and $\Delta_{0i} = p_i - \omega_{0i}$. The equivalence in \eqref{eq:equivalence} now follows from $E[z_i z_i']$ being positive definite.
\end{proof}

==> Submission/ECTA/Proofs/Pf_WkInstrAsymptotic_Trv_F.tex <==
\begin{proof}[Proof of Proposition \ref{prop:wkinstrF}.]
The proof proceeds in three steps. Step (1) provides a function of the data $(\tilde \Psi_-',\tilde \Psi_+')'$ and two constants $\mu_-$, $\mu_+$ such that $(\tilde \Psi_-',\tilde \Psi_+')' \xrightarrow{d} (\Psi_-',  \Psi_+')'$. All of $(\tilde \Psi_-',\tilde \Psi_+')'$, $\mu_-$, and $\mu_+$ are also functions of the DGP. Step (2) establishes parts $(ii)$--$(iv)$. Step (3) shows that $\abs{T^\text{RV}} = \abs{\tilde \Psi_-'\tilde \Psi_+}/\big(\norm{\tilde \Psi_-}^2 + \norm{\tilde \Psi_+}^2 + 2 \rho \tilde \Psi_-'\tilde \Psi_+ + o_p(1) \big)^{1/2}$ and $F=\big( \norm{\tilde \Psi_-}^2 + \norm{\tilde \Psi_+}^2 - 2\rho \tilde \Psi_-'\tilde \Psi_+ \big)/\big(2d_z(1-\rho^2) \big) + o_p(1)$. Part $(i)$ follows from continuous mapping, step (1), and step (3).
	
	
\noindent \textbf{Step (1)} We first provide definitions of $\mu_-$ and $\mu_+$. Let $\tau_+ = 2(\sigma_1^2 + \sigma_2^2 + 2\sigma_{12})^{1/2}$ and $\tau_- = 2(\sigma_1^2 + \sigma_2^2 - 2\sigma_{12})^{1/2}$ and use these two positive constants to define% the vectors
\begin{align}
		\begin{pmatrix}
			 \mu_1 \\  \mu_2
		\end{pmatrix}  =
		\left(\frac{1}{{\tau_-}} + \frac{1}{{\tau_+}}\right)\! \begin{pmatrix} \sqrt{n} W^{1/2} g_1    \\	 	-\sqrt{n} W^{1/2}  g_2		\end{pmatrix}
		+
		\left(\frac{1}{{\tau_-}} - \frac{1}{{\tau_+}}\right)\!\begin{pmatrix}	-\sqrt{n} W^{1/2}  g_2  \\ 		\sqrt{n} W^{1/2}  g_1 		\end{pmatrix}\!.
\end{align}
Defining $\kappa = 1 + \mathbf{1}\{ \norm{\mu_1} \le \norm{\mu_2}  \}$, we then let $\mu_- = \norm{\mu_\kappa} - \norm{\mu_{3-\kappa}}$ and $\mu_+ = \norm{\mu_1} + \norm{\mu_2}$. Since the instruments are weak for testing, we have that $\sqrt{n} W^{1/2} g_m = E[z_i z_i']^{1/2} q_m$ so $\mu_-$ and $\mu_+$ do not depend on $n$. 
	
	
To introduce $\tilde \Psi_-$ and $\tilde \Psi_+$, we let ${\cal Q}_m \in \R^{d_z \times d_z}$ be a non-random orthogonal matrix $({\cal Q}_m{\cal Q}_m'={\cal Q}_m'{\cal Q}_m=I_{d_z})$ such that ${\cal Q}_m \mu_m = \norm{\mu_m} \boldsymbol e_1$. With these matrices in hand, we define $\tilde \Psi_- = \tilde \mu_\kappa - \tilde \mu_{3-\kappa}$ and $\tilde \Psi_+ = \tilde \mu_1 + \tilde \mu_2$ where
\begin{align}
		\begin{pmatrix}
			\tilde \mu_1 \\ \tilde \mu_2
		\end{pmatrix} = 
		\left(\frac{1}{{\tau_-}} + \frac{1}{{\tau_+}}\right)\! \begin{pmatrix} \sqrt{n} {\cal Q}_1\hat W^{1/2} \hat g_1    \\	 	-\sqrt{n} {\cal Q}_2\hat W^{1/2}  \hat g_2		\end{pmatrix}
		+
		\left(\frac{1}{{\tau_-}} - \frac{1}{{\tau_+}}\right)\!\begin{pmatrix}	-\sqrt{n} {\cal Q}_1\hat W^{1/2}  \hat g_2  \\ 		\sqrt{n} {\cal Q}_2\hat W^{1/2}  \hat g_1 		\end{pmatrix}\!.
\end{align}
	
	
The preceding definitions imply that $(\tilde \Psi_-',\tilde \Psi_+')' = \sqrt{n} A (\hat g_1'\hat W^{1/2},\hat g_2'\hat W^{1/2} )'$ for a particular non-random matrix $A \in \mathbb{R}^{2d_z \times 2d_z}$ with $\sqrt{n} A ( g_1' W^{1/2}, g_2' W^{1/2} )' = (\mu_-\boldsymbol e_1',\mu_+\boldsymbol e_1')'$. Since $\mu_-$ and $\mu_+$ do not depend on $n$, it therefore follows from Lemma \ref{lem:asymp norm}, part $(i)$, that $(\tilde \Psi_-',\tilde \Psi_+')' \xrightarrow{d} (\Psi_-',  \Psi_+')'$ provided that $AV^\text{RV}A' \rightarrow {\tiny \begin{bmatrix} 1 & \rho \\ \rho & 1 \end{bmatrix} }\otimes I_{d_z}$ where $\rho$ is the correlation between $e_{\kappa i}-e_{3-\kappa i}$ and $e_{1i}+e_{2i}$. To see why this convergence occurs, note first that weak instruments for testing (Assumption \ref{as:wkinstr}) implies that $g_m = O(n^{-1/2})$ for $m=1,2$, which in turn yields that the second part of $\psi_{mi}$ is $O_p(n^{-1/2})$. From Assumption \ref{as:homsked}, we then have
\begin{align}\label{eq:varconv}
		V^\text{RV}_{\ell k} = W^{1/2} E[ e_{\ell i} e_{k i} z_iz_i'] W^{1/2} + O(n^{-1/2}) = \sigma_{\ell k} I_{d_z} + O(n^{-1/2})
\end{align}
where we write $\sigma_{mm}$ for $\sigma_m^2$. Thus, we have that $V^\text{RV} \rightarrow {\tiny \begin{bmatrix} \sigma_1^2 & \sigma_{12} \\ \sigma_{12} & \sigma_{2}^2 \end{bmatrix} }\otimes I_{d_z} .$ Furthermore, we note that $A$ takes the form
\begin{align}
			A = 
			\begin{bmatrix}	(-1)^{3-\kappa}I & (-1)^\kappa I \\ I & I	\end{bmatrix}
			\begin{bmatrix}	{\cal Q}_1 & 0 \\ 0 & {\cal Q}_2	\end{bmatrix}
			\begin{bmatrix}	I & I \\ I & -I	\end{bmatrix}
			\begin{bmatrix}	I\tau_-^{-1} & 0 \\ 0 & I\tau_+^{-1}	\end{bmatrix}
			\begin{bmatrix}	I & -I \\ I & I	\end{bmatrix}
\end{align}
and leave the verification of $A\big( {\tiny \begin{bmatrix} \sigma_1^2 & \sigma_{12} \\ \sigma_{12} & \sigma_{2}^2 \end{bmatrix} }\otimes I_{d_z} \big)A' = {\tiny \begin{bmatrix} 1 & \rho \\ \rho & 1 \end{bmatrix} }\otimes I_{d_z}$ to the reader.
	
	
\noindent \textbf{Step (2)} Part $(iv)$ is an immediate implication of the triangle inequality and the definitions $\mu_- = \norm{\mu_\kappa} - \norm{\mu_{3-\kappa}}$ and $\mu_+ = \norm{\mu_1} + \norm{\mu_2}$. For part $(ii)$, we have that $\mu_-=0$ if and only if $\norm{\mu_1}^2 - \norm{\mu_2}^2 =0$. In turn, we have that
\begin{align}
		\norm{\mu_1}^2 - \norm{\mu_2}^2 &= n\!\left( \!\left(\tau_-^{-1} + \tau_+^{-1} \right)^2  - \!\left(\tau_-^{-1} - \tau_+^{-1} \right)^2 \right)\! \left( Q_1 - Q_2\right) \\
		&=4n (\tau_+ \tau_-)^{-1} \left( Q_1 - Q_2\right),
\end{align}
from which part $(ii)$ is immediate. For part $(iii)$, we have that $\mu_+=0$ if and only if $\norm{\mu_1}^2 + \norm{\mu_2}^2 =0$. We now have,
\begin{align}
			\norm{\mu_1}^2 \!+\! \norm{\mu_2}^2
			&\!=\! n\!\begin{pmatrix} W^{1/2}g_1  \\ W^{1/2}g_2	\end{pmatrix}'\!
			A'A 
			\!\begin{pmatrix} W^{1/2}g_1  \\ W^{1/2}g_2	\end{pmatrix} \!
			=\! n\!\begin{pmatrix} W^{-1/2}\pi_1  \\ W^{-1/2}\pi_2	\end{pmatrix}'\!
			A'A 
			\!\begin{pmatrix} W^{-1/2}\pi_1  \\ W^{-1/2}\pi_2	\end{pmatrix} \!
\end{align}
so part $(iii)$ follows from the positive definiteness of both $W$ and the matrix $A'A = 4 \!{\tiny \begin{bmatrix} \tau_+^{-2} + \tau_-^{-2} & \tau_+^{-2} - \tau_-^{-2} \\ \tau_+^{-2} - \tau_-^{-2} & \tau_+^{-2} + \tau_-^{-2} \end{bmatrix} }\!\otimes I_{d_z}$.

		
\noindent \textbf{Step (3)} For $T^\text{RV}$ we first consider the numerator. Here, we observe that
\begin{align}
		\tilde \Psi_-' \tilde\Psi_+ = \tilde \mu_\kappa'\tilde \mu_\kappa - \tilde \mu_{3-\kappa}'\tilde \mu_{3-\kappa} = 4n (\tau_+ \tau_-)^{-1} \!\left( \hat Q_\kappa - \hat Q_{3-\kappa}\right)
\end{align}
so that $\sqrt{n}\abs{\hat Q_1-\hat Q_2} = (\tau_+\tau_-/4)\abs{\tilde\Psi_-' \tilde\Psi_+}/\sqrt{n}$. For the denominator, we initially note that Lemma \ref{lem:asymp norm}, part $(ii)$, and \eqref{eq:varconv} yields that
\begin{align}
		(\tau_+ \tau_-/4)^{-2} n \hat \sigma^2_\text{RV} = \tfrac{4^3n}{\tau_+^2\tau_-^2}\!\left[ \sigma_1^2 \hat Q_1 + \sigma_2^2 \hat Q_2 - 2\sigma_{12} \hat g_1' \hat W \hat g_2  \right] + o_p(1).
\end{align}	
Similarly, we can calculate that
\begin{align}
		\norm{\tilde \Psi_-}^2  &+ \norm{\tilde \Psi_+}^2  + 2\rho \tilde \Psi_-'\tilde \Psi_+ 
		= n \begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix}
		'A' \bigg( {\tiny \begin{bmatrix} 1 & \rho \\ \rho & 1 \end{bmatrix} }\otimes  I_{d_z}  \bigg)A
		\begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix}\\
		&= {4^2n}{} \begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix}'
		\bigg( \! \tfrac{4}{\tau_+^2\tau_-^2}{\tiny \begin{bmatrix} \sigma_1^2 \! & \! -\sigma_{12} \\ -\sigma_{12} \! & \! \sigma_2^2 \end{bmatrix}} \!\otimes I_{d_z}  \bigg)
		\begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix} \\
		&= \tfrac{4^3n}{\tau_+^2\tau_-^2}\!\left[ \sigma_1^2 \hat Q_1 + \sigma_2^2 \hat Q_2 - 2\sigma_{12} \hat g_1' \hat W \hat g_2  \right]
\end{align}
where the second equality follows from the last sentences of steps (1) and (2) together with
\begin{align}
		{\tiny \begin{bmatrix} \tau_+^{-2} + \tau_-^{-2} & \tau_+^{-2} - \tau_-^{-2} \\ \tau_+^{-2} - \tau_-^{-2} & \tau_+^{-2} + \tau_-^{-2} \end{bmatrix} \begin{bmatrix} \sigma_1^2 & \sigma_{12} \\ \sigma_{12} & \sigma_{2}^2 \end{bmatrix}  \begin{bmatrix} \tau_+^{-2} + \tau_-^{-2} & \tau_+^{-2} - \tau_-^{-2} \\ \tau_+^{-2} - \tau_-^{-2} & \tau_+^{-2} + \tau_-^{-2} \end{bmatrix} = \begin{bmatrix} \sigma_1^2 & -\sigma_{12} \\ -\sigma_{12} & \sigma_2^2 \end{bmatrix} } \tfrac{4}{\tau_+^2\tau_-^2}.
\end{align}
Thus we have the desired conclusion
		\begin{align}
		\abs{T^\text{RV}} &= \sqrt{n}\frac{\abs{\hat Q_1 - \hat Q_2}}{\hat \sigma_\text{RV}} = \frac{4n (\tau_+ \tau_-)^{-1/2} \!\abs{ \hat Q_1 - \hat Q_2}}{\left( (\tau_+ \tau_-/4^2)\inverse n \hat \sigma^2_\text{RV}  \right)^{1/2}} \\
		&=
		 \abs{\tilde \Psi_-'\tilde \Psi_+}/\big(\norm{\tilde \Psi_-}^2 + \norm{\tilde \Psi_+}^2 + 2\kappa \tilde \Psi_-'\tilde \Psi_+  + o_p(1) \big)^{1/2}
\end{align}
	
	
For $F_\rho$, we first note that standard arguments lead to
\begin{align}
		2d_zF_\rho &=n(1-\hat \rho^2)\frac{\hat \sigma_2^2 \hat g_1' \hat W \hat g_1 + \hat \sigma_1^2 \hat g_2' \hat W \hat g_2 - 2\hat \sigma_{12} \hat g_1' \hat W \hat g_2}{\hat \sigma_1^2 \hat \sigma_2^2 - \hat \sigma_{12}^2 } \\
		&=n(1-\rho^2)\frac{\sigma_2^2 \hat Q_1 +  \sigma_1^2 \hat Q_2 - 2 \sigma_{12} \hat g_1' \hat W \hat g_2}{ \sigma_1^2  \sigma_2^2 -  \sigma_{12}^2 } + o_p(1).
\end{align}
Similarly, we can calculate that
\begin{align}
		\norm{\tilde \Psi_-}^2  &+ \norm{\tilde \Psi_+}^2  - 2\rho \tilde \Psi_-'\tilde \Psi_+ 
		= n \begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix}'
		A' \bigg( {\tiny \begin{bmatrix} 1 & -\rho \\ -\rho & 1 \end{bmatrix} }\otimes  I_{d_z}   \bigg)A
		\begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix} \\
		&= {n}{} \begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix}'
		\bigg(  {\tiny \begin{bmatrix} \sigma_1^2  &  \sigma_{12} \\ \sigma_{12}  &  \sigma_2^2 \end{bmatrix}}\inverse \otimes I_{d_z}  \bigg)
		\begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix} \\
		&= n\frac{\sigma_2^2 \hat Q_1 +  \sigma_1^2 \hat Q_2 - 2 \sigma_{12} \hat g_1' \hat W \hat g_2}{ \sigma_1^2  \sigma_2^2 -  \sigma_{12}^2 }
\end{align}
which follows from inverting the equality in the last sentence of step (1).
\end{proof}

==> Submission/ECTA/Proofs/Pf_plims_cost.tex <==
\begin{proof}[Proof of Lemma \ref{cor:cost_misc}.] 
Since $\textbf{w}_\textbf{a}$ is a subset of $\textbf{w}$, the proof follows immediately by replacing any variable $y$ residualized with respect to $\textbf{w}$ in the Proof of Lemma \ref{cor:modelmisc}, with $y^\textbf{a}$ which has been residualized with respect to $\textbf{w}_\textbf{a}$.
%
\begin{comment}
For $\textbf{w}_\textbf{a}\neq \textbf{w}$, by Equation \eqref{eq:cost_mispec2}, $p_i =  \Delta^\textbf{a}_{0i} + \omega_{0i}$, where $p_i = \boldsymbol{p}_m-\textbf{w}_{\textbf{a}}E[\textbf{w}_{\textbf{a}}'\textbf{w}_{\textbf{a}}]^{-1}E[\textbf{w}_{\textbf{a}}'\boldsymbol{p}_m]$ and $\Delta^a_m = \boldsymbol{\Delta}^{\textbf{a}}_m-\textbf{w}_{\textbf{a}}E[\textbf{w}_{\textbf{a}}'\textbf{w}_{\textbf{a}}]^{-1}E[\textbf{w}_{\textbf{a}}'\boldsymbol{\Delta}^{\textbf{a}}_m]$.  Define $\Delta^{\textbf{a}z}_{0i} = z_iE[z_iz_i']E[z_i\Delta^{\textbf{a}z}_{0i}]$.  Further, define $\Delta_m = \boldsymbol{\Delta}_m-\textbf{w}_{\textbf{a}}E[\textbf{w}_{\textbf{a}}'\textbf{w}_{\textbf{a}}]^{-1}E[\textbf{w}_{\textbf{a}}'\boldsymbol{\Delta}_m]$ and $\Delta^{z}_{mi} = z_iE[z_iz_i']E[z_i\Delta^{z}_{mi}]$.  Let $z = \boldsymbol{z}-\textbf{w}_{\textbf{a}}E[\textbf{w}_{\textbf{a}}'\textbf{w}_{\textbf{a}}]^{-1}E[\textbf{w}_{\textbf{a}}'\boldsymbol{z}]$. By Equation \eqref{eq:omega_costmisc} and under Assumption \ref{as:misspmc}, the right hand side of \eqref{eq:line4} can be rewritten as
$$E[z_i(\Delta^\textbf{a}_{0i}-\Delta_{mi})]'E[z_iz_i']^{-1}E[z_i(\Delta^\textbf{a}_{0i}-\Delta_{mi})].$$  Thus, replacing $\Delta^z_{0i}$ with $\Delta^{\textbf{a}z}_{0i}$ the equality between \eqref{eq:line1} and \eqref{eq:line4} holds as does the equality between \eqref{eq:line4} and \eqref{eq:line5}. 

\begin{itemize}
\item[(i)]  Under Assumption \ref{as:misspmc} and by the equality of \eqref{eq:line1}, \eqref{eq:line5}, and the positive definiteness of $E[z_iz_i']$, $\pi_m = 0$ iff $E[(\Delta^{\textbf{a}z}_{0i}-\Delta^{\textbf{a}z}_{mi})^2]=0$.  The proof then follows from the Proof of Lemma 2 (i). 
    \item[(ii)]  Under Assumption \ref{as:misspmc} and by the equality of \eqref{eq:line1}, \eqref{eq:line5}, and the positive definiteness of $E[z_iz_i']$, $Q_1=Q_2$ iff $E[(\Delta^{\textbf{a}z}_{0i}-\Delta^{z}_{1i})^2]=E[(\Delta^{\textbf{a}z}_{0i}-\Delta^{z}_{2i})^2]$ The proof then follows from the Proof of Lemma 2 (ii). 
\end{itemize}
\end{comment}
\end{proof}

==> Submission/ECTA/SubmissionInfo.tex <==
Title: Testing Firm Conduct
Keywords: testing, non-nested, weak instruments, firm conduct
Abstract: We study inference on firm conduct without data on markups.  Berry and Haile (2014) provide a testability condition requiring instruments.  Implementing a test using this condition involves choosing both hypotheses and instruments, which affect inference. While the IO literature has adopted model selection and model assessment approaches to formulating hypotheses, we present the advantages of the Rivers and Vuong (2002) (RV) model selection test under misspecification. However, the RV test may suffer from degeneracy, whereby inference is invalid. We characterize degeneracy as a weak instruments problem via a novel definition of weak instruments for testing. This characterization enables us to provide a diagnostic for reliable inference. We illustrate our results in the setting of Villas-Boas (2007). We test conduct with three standard sets of instruments, one strong and two weak. Weak instruments cause the RV test to have no power. With strong instruments, models of double marginalization are rejected.


==> Submission/ECTA/Tables/AR_results.tex <==
%\renewcommand{\arraystretch}{1.2}
\begin{widetable}{.98\columnwidth}{lcccc}
\toprule
\textbf{BLP95 IVs} & 2 & 3 & 4 & 5 \\
\cmidrule(lr){2-5}
1. Zero wholesale margin&262.2$\,$,$\,$673.7&262.2$\,$,$\,$216.8&262.2$\,$,$\,$220.4&262.2$\,$,$\,$221\\
2. Zero retail margin &&673.7$\,$,$\,$216.8 & 673.7$\,$,$\,$220.4&673.7$\,$,$\,$221\\
3. Linear pricing&&&216.8$\,$,$\,$220.4&216.8$\,$,$\,$221\\
4. Hybrid model&&&&220.4$\,$,$\,$221\\
5. Wholesale collusion&&&&\\
\bottomrule
\end{widetable}




==> Submission/ECTA/Tables/FStats_supply_all.tex <==
%\renewcommand{\arraystretch}{1.2}
\begin{widetable}{.98\columnwidth}{lrrrr}
\toprule
\textbf{Panel A: BLP95 IVs} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5} \\
\cmidrule(lr){2-5}
1. Zero wholesale margin&66.3&26.3&26.2&90.7\\
2. Zero retail margin&&36.4&36.6&79.0\\
3. Simple linear pricing&&&50.8&27.2\\
4. Hybrid model&&&&26.9\\
5. Wholesale collusion&&&&\\
\midrule
\textbf{Panel B: GH20 IVs} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5} \\
\cmidrule(lr){2-5}
1. Zero wholesale margin&5.7&2.5&2.5&3.7\\
2. Zero retail margin&&2.2&2.2&4.3\\
3. Simple linear pricing&&&1.0&2.5\\
4. Hybrid model&&&&2.5\\
5. Wholesale collusion&&&&\\
\midrule
\textbf{Panel C: Rival Cost Shifters IVs} &\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5} \\
\cmidrule(lr){2-5}
1. Zero wholesale margin&68.6&1.1&1.3&131.6\\
2. Zero retail margin&&44.8&47.0&112.9\\
3. Linear pricing&&&5.2&33.7\\
4. Hybrid model&&&&34.6\\
5. Wholesale collusion&&&&\\
\bottomrule
\end{widetable}


==> Submission/ECTA/Tables/F_critical_values.tex <==

%\newcolumntype{d}[1]{D{.}{.}{#1}}
%\renewcommand{\arraystretch}{1.05}
\begin{widetable}{.98\columnwidth}{r*{3}{>{\raggedleft\arraybackslash}p{4em}}c*{3}{>{\raggedleft\arraybackslash}p{4em}}}
\toprule
&  \multicolumn{3}{c}{\textbf{Panel A:} Maximal Size ${cv^s},\,\, r^s = $} &&  \multicolumn{3}{c}{\textbf{Panel B:} Maximal Power ${cv^p},\,\, r^p = $}\\ 
\cmidrule(lr){2-4}\cmidrule(lr){6-8} 
$d_z$  & 0.075 & 0.10 & 0.125 & & 0.95 & 0.75 & 0.50\\
\midrule
1&31.4&14.5&8.4&&31.1&22.6&18.0\\
2&0&0&0&&18.9&13.2&10.4\\
3&0&0&0&&14.6&10.2&8.0\\
4&0&0&0&&12.3&8.8&6.9\\
5&0&0&0&&10.8&7.8&6.2\\
6&0&0&0&&9.8&7.2&5.8\\
7&0&0&0&&9.0&6.7&5.4\\
8&0&0&0&&8.4&6.4&5.2\\
9&0.3&0&0&&8.0&6.1&5.0\\
10&1.7&0.4&0&&7.6&5.8&4.8\\
11&3.3&1.3&0.5&&7.2&5.6&4.6\\
12&5.0&2.1&1.1&&7.0&5.4&4.5\\
13&6.9&3.1&1.8&&6.7&5.3&4.4\\
14&8.8&4.0&2.4&&6.5&5.1&4.3\\
15&10.8&5.0&3.1&&6.3&5.0&4.2\\
20&21.1&10.2&6.6&&5.6&4.6&3.9\\
25&31.8&15.7&10.3&&5.1&4.2&3.7\\
30&42.8&21.2&14.1&&4.8&4.0&3.5\\
\bottomrule
\end{widetable}

==> Submission/ECTA/Tables/Instr_robustness.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{widetable}{.98\columnwidth}{lrrrrc}
\toprule
\textbf{Panel A: BLP95 + GH20 + Rival Cost} & \multicolumn{4}{c}{$F_\rho$}& MCS $p$-values\\
\multicolumn{1}{l}{($d_z=8$)}&\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&65.7&21.5&21.5&91.7&0.71 \\
2. Zero retail margin&&30.1&30.2&80.1&1.00 \\
3. Linear pricing&&&36.3&33.1&0.09 \\
4. Hybrid model&&&&33.0&0.09 \\
5. Wholesale collusion&&&&&0.00 \\
\midrule
\textbf{Panel B: Difference in Cost Shifters IVs} & \multicolumn{4}{c}{$F_\rho$}& MCS $p$-values\\
\multicolumn{1}{l}{($d_z=1$)}&\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&12.1&3.8&3.8&4.8&0.72\\
2. Zero retail margin&&7.1&7.0&8.1&0.19\\
3. Linear pricing&&&1.8&2.8&0.72\\
4. Hybrid model&&&&2.8&0.70\\
5. Wholesale collusion&&&&&1.00\\
\midrule
\textbf{Panel C: BLP Constant IVs} & \multicolumn{4}{c}{$F_\rho$}& MCS $p$-values\\
\multicolumn{1}{l}{($d_z=2$)}&\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&63.6&28.0&28.0&91.3&0.61\\
2. Zero retail margin&&37.8&37.9&78.5&1.00\\
3. Linear pricing&&&50.1&29.3&0.02\\
4. Hybrid model&&&&29.1&0.02\\
5. Wholesale collusion&&&&&0.00\\
\bottomrule
\end{widetable}


==> Submission/ECTA/Tables/RV_application_full.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{widetable}{.98\columnwidth}{lrrrrc}
\toprule
\textbf{Panel A: BLP95 IVs} & \multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& MCS $p$-values \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&0.65&$-$3.45&$-$3.45&$-$5.37&0.52\\
2. Zero retail margin&&$-$3.18&$-$3.17&$-$4.25&1.00\\
3. Linear pricing&&&0.17&$-$4.47&0.04\\
4. Hybrid model&&&&$-$4.48&0.04\\
5. Wholesale collusion&&&&&0.00\\
\midrule
\textbf{Panel B: GH20 IVs} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& MCS $p$-values \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&0.77&0.40&0.39&$-$1.05&0.74 \\
2. Zero retail margin&&0.29&0.28&$-$1.02&0.78 \\
3. Linear pricing&&&$-$1.18&$-$0.81&1.00 \\
4. Hybrid model&&&&$-$0.80&0.78 \\
5. Wholesale collusion&&&&&0.55 \\
\midrule
\textbf{Panel C: Rival Cost Shifters IVs} & \multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}&MCS $p$-values \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&-0.76&-0.33&-0.46&-4.06&1.00\\
2. Zero retail margin&&0.82&0.80&-3.01&0.45\\
3. Linear pricing&&&-1.33&-3.94&0.75\\
4. Hybrid model&&&&-3.95&0.67\\
5. Wholesale collusion&&&&&0.00\\
\bottomrule
\end{widetable}


==> Submission/ECTA/Tables/demand_models.tex <==
\begin{widetable}{.98\columnwidth}{lrrrrrr}
\toprule
& \multicolumn{2}{c}{(1) Logit-OLS}  & \multicolumn{2}{c}{(2) Logit-2SLS}  & \multicolumn{2}{c}{(3) BLP}   \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
& coef. & \multicolumn{1}{c}{s.e.}
& coef. & \multicolumn{1}{c}{s.e.}
& coef. & \multicolumn{1}{c}{s.e.}    \\
\midrule
 Prices         &    $-1.750$ &   (0.019)    &    $-6.519$  &   (0.209)    &  $-12.001$  & (0.777)\\
 Size           &    0.037 &    (0.001)   &    0.018 &   (0.001)    &  $-0.060$  & (0.013) \\
 Light          &    0.259  &   (0.010)  &    0.413 &   (0.014)    &  $-0.270$  & (0.144) \\
 Plain   &    0.508 &   (0.007)   &    0.423  &   (0.009)   &  0.439 & (0.012) \\
 log(\#Flavors)   &    1.127  &   (0.004)  &    1.106 &   (0.005)    &  1.135    & (0.007) \\
 Income $\times$ price &      &       &        &      &  4.333   & (0.378)\\
 Income $\times$ light &     &        &        &      &  0.215  & (0.069)\\
Age $\times$ light    &      &       &      &        & $-0.565$  & (0.113)  \\
 Age $\times$ size     &    &         &   &           & $-0.067$& (0.008)  \\
\midrule 
Own elasticity-mean     &    \multicolumn{2}{c}{$-1.320$}    &    \multicolumn{2}{c}{$-4.917$}    & \multicolumn{2}{c}{$-6.306$}  \\
Own elasticity-median   &   \multicolumn{2}{c}{$-1.177$}    &    \multicolumn{2}{c}{$-4.384$ }   & \multicolumn{2}{c}{$-6.187$}  \\
 $J$-statistic         &   \multicolumn{2}{c}{2.0e-23}  &    \multicolumn{2}{c}{1.9e-21}    & \multicolumn{2}{c}{2.5e-01} \\
\bottomrule
\end{widetable}


==> Submission/ECTA/Tables/summary_stat.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Mar 12, 2021 - 03:58:35 PM
%\renewcommand{\arraystretch}{1.05}
\begin{widetable}{.98\columnwidth}{lrrrrr} 
\toprule
Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Median}  & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Pctl(75)} \\ 
\midrule
Price (\$) & 0.76 & 0.30 & 0.68 &  0.55 & 0.91 \\ 
Sales (6 oz. units) & 1,461 & 3,199 & 503  & 213 & 1,301 \\ 
Shares & 0.007 & 0.012 & 0.003 & 0.001 & 0.007 \\ 
Outside Share & 0.710 & 0.111 & 0.708 & 0.631 & 0.788 \\ 
Size (oz.) & 17.82 & 10.57 & 16  & 6 & 32 \\ 
Frac. Light & 0.93 & 0.26 & 1 &  1 & 1 \\ 
Number Flavors & 5.39 & 5.81 & 3  & 1 & 8 \\ 
Frac. Private Label & 0.09 & 0.28 & 0  & 0 & 0 \\ 
Distance to Plant (mi.) & 493 & 477 & 392  & 199 & 546 \\ 
Freight Cost (\$) & 212 & 242 & 164  & 52 & 271 \\ 
\bottomrule
\end{widetable} 


==> Submission/QE/Appendices/AltCost.tex <==
In this appendix we discuss how the results of the paper are preserved in a more general setting where marginal cost depends on quantity sold. While in the paper, we derive results assuming constant marginal cost, this is an important extension. It is well known going back to \citeA{b82} and \citeA{l82} that the requirements for testing conduct are greater when marginal cost is non-constant.  Thus, the reader may wonder if the results of our paper would be qualitatively different in a more general setting.


Let $\boldsymbol{q}_i$ denote quantity, and consider a separable cost function:
\begin{align}
    \boldsymbol{c}_i = \bar{\boldsymbol{c}}(\boldsymbol{q}_i,\textbf{w}_i;\tau) + \omega_i,
\end{align}
where $\bar c$ is specified up to some cost parameters $\tau$.  The specification of marginal cost that we adopt in the paper is a special case where $\bar{\boldsymbol{c}}(\boldsymbol{q}_i,\textbf{w}_i;\tau) = \textbf{w}_i \tau$.


There are two additional cases to consider. The first concerns the researcher knowing the true value of $\tau$. We can define $\bar{\boldsymbol{\Delta}}_{mi} = \boldsymbol{\Delta}_{mi} + \bar{\boldsymbol{c}}(\boldsymbol{q}_i,\textbf{w}_i;\tau)$: this term is pinned down by a model of conduct $m$, and a cost function $\bar{\boldsymbol{c}}$. In this case, we can test alternative pairs of models of conduct and cost functions with the methods described in the paper. In particular, that can be done by replacing ${{\Delta}}_{m}$ in the paper with $\bar{\boldsymbol{\Delta}}_{m}$. The set of instruments $\boldsymbol{z}$ must include $\textbf{w}$ in this case, but since $\bar{\boldsymbol{c}}$ is fully specified, there is no additional requirement on instruments. 

Alternatively, when $\tau$ is unknown to the researcher, she can estimate it under a model of conduct $m$ either as a preliminary step, or simultaneously with testing, as she would in the case of constant marginal cost. However, excluded instruments that rotate residual marginal revenue are now needed to estimate $\tau$, and thus must be sufficient to identify $\tau$ under the true model of conduct. If a researcher pursues a sequential approach, the researcher can construct $\bar{\boldsymbol{\Delta}}_{mi} = \boldsymbol{\Delta}_{mi} + \bar{\boldsymbol{c}}(\boldsymbol{q}_i,\textbf{w}_i;{\tau}_m)$ and perform testing after having estimated ${\tau}_m$ under each model. 

The results in the paper are still applicable as long as the researcher adjusts the standard errors of the RV test statistic and the effective $F$-statistic. As there may exist models, falsified by a set of instruments under constant marginal cost, which are not falsified by those same instruments with a more flexible marginal cost specification, degeneracy is more likely to occur when cost is non-constant. This is akin to the classic example of demand shifters in \cite{b82}. More specifically, as shown in \cite{mqsw22}, the researcher needs to use instruments corresponding to economically different sources of exogenous variation in order to pin down cost parameters and perform the test. As this setup places additional requirements on the instruments, evaluating the quality of the inference on conduct using our diagnostic is even more necessary in this setting. However, beyond the extra burden, the testing problem is fundamentally unchanged, therefore the results in this paper apply.   

This discussion makes it explicit that testing firm conduct also jointly tests models of marginal cost. In fact,  $\bar{\boldsymbol{\Delta}}_{m} $ generalizes the term $\Breve{\boldsymbol{\Delta}}_{m}$ defined in Section \ref{sec:globalmis}. In that section we show that cost misspecification can be incorporated in  $\Breve{\boldsymbol{\Delta}}_{m}$, and thus be understood as markup misspecification. Here, misspecification of $\bar c$ is manifested as misspecification of  $\bar{\boldsymbol{\Delta}}_{m} $. If one is flexible in specifying $\bar c$, misspecification of $\bar{\boldsymbol{\Delta}}_{m} $ largely concerns misspecification of ${\boldsymbol{\Delta}}_{m} $, and therefore conduct. Finally, this formulation shows that the methods described in the paper can be used to test models of cost, even when conduct is known.\looseness=-1




==> Submission/QE/Appendices/MCS.tex <==
%This Appendix details our construction of the model confidence set (MCS) $M^*$ for a given set of instruments. Suppose the set of models is $M=\{1,\dots,M_0\}$. Let $K = {M_0 \choose 2}$ denote the total number of unique pairwise model comparisons and let $T^\text{RV}(T^\text{RV}_1,\dots,T_K^\text{RV})$

In this appendix, we provide further details on the construction of the model confidence set.  The construction is iterative where in each step a $p$-value for a model of worst fit is computed.  For a set of instruments $z_\ell$, the MCS $M^*_\ell$ is the collection of models with a $p$-value above the significance level.

For a researcher testing a set of candidate models $M$, we now describe the construction of the MCS $p$-values at each step of the algorithm.  
At iteration $k$, there are $M_k\subset M$ models under current consideration.  Denoting $\abs{M_k}$ as the cardinality of $M_k$, this results in $K = \binom{\abs{M_k}}{2}$ distinct pairs of models and therefore RV test statistics. To make notation compact, we define $\Pi$ as a one-to-one mapping from unique model pairs to $\{1,\hdots,K\}$, and let $T^\text{RV}_{\Pi(m_1,m_2)}=  {\sqrt{n}(\hat{Q}_{m_1}-\hat{Q}_{m_2})}/{\hat\sigma_{\text{RV},\Pi(m_1,m_2)}}$.  In this iteration, we find the pair of models $(m_1,m_2)$ associated with the largest test statistic in magnitude, denoted $\bar{T}^\text{RV}$.  If $\bar{T}^\text{RV}$ is positive (negative), then $m_1$ ($m_2$) is the model of worst fit for which we compute the MCS $p$-value.  This model will be dropped from $M_{k+1}$ in the next iteration.

For computation of the MCS $p$-values, we utilize that $    \big(T^\text{RV}_1,\hdots,T^\text{RV}_K \big)'$ is asymptotically normal with zero mean and a variance $\Sigma$ under no degeneracy and a null of equal fit.  This observation follows by extending Lemma \ref{lem:asymp norm} to $\abs{M_k}$ models and alluding to a first order Taylor approximation as in Remark \ref{rem:validity}.  We estimate $\Sigma$ using $\hat\Sigma$.  The diagonal entries of $\hat\Sigma$ are all one.  For any off-diagonal element $\hat\Sigma_{ij}$ with $(i,j) = (\Pi(m_1,m_2),\Pi(m_3,m_4)) $ we have:\looseness=-1
\begin{align}
    \hat\Sigma_{ij} = 4\hat\sigma^{-1}_{\text{RV},i}\hat\sigma^{-1}_{\text{RV},j}&\bigg(\hat g_{m_1}'\hat W^{1/2}\hat V^{\text{RV}}_{m_1m_3}\hat W^{1/2}\hat g_{m_3} -\hat g_{m_2}'\hat W^{1/2}\hat V^{\text{RV}}_{m_2m_3}\hat W^{1/2}\hat g_{m_3} \\&\qquad- \hat g_{m_1}'\hat W^{1/2}\hat V^{\text{RV}}_{m_1m_4}\hat W^{1/2}\hat g_{m_4} +  \hat g_{m_2}'\hat W^{1/2}\hat V^{\text{RV}}_{m_2m_4}\hat W^{1/2}\hat g_{m_4}\bigg).
\end{align}



%\cite{hln11} define a version of the MCS procedure where you obtain $p$- values for model under consideration and then, for a level $\alpha$, the MCS is obtained as the set of models with a $p$-value above $\alpha$. We implement this iterative procedure as the do.  As we are able to derive the asymptotic distribution of the test statistics above, 
We take 99,999 draws from this distribution and for each draw compute the max of the absolute value of the $K$ simulated test statistics denoted $\bar{T}^{\text{RV},sim}$.  The $p$-value is then computed as the fraction of draws for which  $\bar{T}^{\text{RV},sim} > \abs{\bar T^\text{RV}}$.

This procedure is computationally expedient.  In particular, one does not need to bootstrap both demand estimation and the testing procedure, which can be prohibitively costly.  Instead, using the adjustments derived in Appendix \ref{sect:TwoStep}, $\hat\Sigma$ can incorporate adjustments for demand estimation and clustering. 


==> Submission/QE/Appendices/Robustness.tex <==

This appendix provides additional details for our empirical application. 

\noindent \textbf{Code Details:} Below is the definition of the demand estimation problem in \texttt{PyBLP} and the testing problem in \texttt{pyRVtest}.
\begin{figure}[ht]
    \centering
    \caption{Code for Demand Estimation and Testing}
    %\hspace{-1cm}
    \begin{subfigure}[t]{0.47\textwidth}
        \centering
        \caption*{Panel A. Demand Estimation Code}
        \includegraphics[scale=0.24]{Submission/QE/Figures/demand_code.png}
    \end{subfigure}
    %\hspace{-.5cm}
    \begin{subfigure}[t]{0.52\textwidth}
        \centering
        \caption*{Panel B. Testing Code}
        \includegraphics[scale=0.24]{Figures/code_test.png}
    \end{subfigure}
    \caption*{\footnotesize{Panels A and B report the definitions of the demand estimation problem in \texttt{PyBLP} and the testing problem in \texttt{pyRVtest}, respectively.}}
\end{figure}

\vspace{-0.8cm}

\noindent \textbf{Description of the Models of Conduct:} Following \cite{v07}, the markups in market $t$ for a model $m$ among those we consider can be written in the following form:
\[\boldsymbol{\Delta}_{mt}=\underbrace{-(\boldsymbol{\Omega}^r_{mt} \odot \boldsymbol{D}^r_t)^{-1} \boldsymbol{s}_t}_{=\boldsymbol{\Delta}^\text{downstream}_{mt}}\underbrace{-(\boldsymbol{\Omega}^w_{mt} \odot \boldsymbol{D}^w_t )^{-1} \boldsymbol{s}_t}_{=\boldsymbol{\Delta}^\text{upstream}_{mt}}\]
where $\boldsymbol{\Omega}^r_{mt}$ and $\boldsymbol{\Omega}^w_{mt}$ are ownership matrices, $\boldsymbol{D}^w_t$ is the jacobian of retail share $\boldsymbol{s}_t$ with respect to wholesale price, and $\boldsymbol{D}^r_t$ is the jacobian of retail share with respect to retail price. The markup $\boldsymbol{\Delta}_{mt}$ implied by each model is the sum of downstream markups $\boldsymbol{\Delta}^\text{downstream}_{mt}$ and upstream markups $\boldsymbol{\Delta}^\text{upstream}_{mt}$. We can derive each model by using different assumptions on the ownership matrices:
\begin{enumerate}
    \item \textit{Zero wholesale margin}: Set $\boldsymbol{\Omega}^w_{mt}$ to a matrix of zeros, set $\boldsymbol{\Omega}^r_{mt}$ to a matrix of ones.
    \item \textit{Zero retail margin}: Set $\boldsymbol{\Omega}^w_{mt}$ to a matrix of zeros, and set $\boldsymbol{\Omega}^r_{mt}$ to a matrix  with element $(i,j)$ that is equal to one if products $i$ and $j$ are produced by the same manufacturer, and to zero otherwise. 
    \item \textit{Linear pricing}: Set $\boldsymbol{\Omega}^r_{mt}$ to a matrix of ones, and set $\boldsymbol{\Omega}^w_{mt}$ to a matrix  with element $(i,j)$ that is equal to one if products $i$ and $j$ are produced by the same manufacturer, and to zero otherwise. 
    \item \textit{Hybrid model}: Set $\boldsymbol{\Omega}^r_{mt}$ to a matrix of ones, and set $\boldsymbol{\Omega}^w_{mt}$ to a matrix  with element $(i,j)$ that is equal to one if products $i$ and $j$ are produced by the same manufacturer and $i$ is not a private label, and to zero otherwise. 
    \item \textit{Wholesale Collusion}: Set $\boldsymbol{\Omega}^r_{mt}$ and $\boldsymbol{\Omega}^w_{mt}$ to matrices of ones. \looseness=-1
    
\end{enumerate}

\noindent \textbf{Assessment Tests Results:}
We present in Table \ref{Tab:Cox_EB} the test results from the two other model assessment procedures defined in Appendix \ref{sect:EBCox}. With NoProd instruments, the EB and Cox tests reject all models. Similar to the AR results in Table \ref{Tab:Model_assessment_all}, the Cox and EB results illustrate the pitfalls of using model assessment tests for conduct, formally discussed in Section \ref{sec:globalmis}.

\begin{table}[ht]
\footnotesize
\caption{Cox and EB Test Results}
\label{Tab:Cox_EB}
\centering
\begin{threeparttable}
\input{Submission/QE/Tables/CoxEB.tex}
\begin{tablenotes}[flushleft]
    \setlength\labelsep{0pt}
    \footnotesize
    \item Each cell reports the respective pair of test statistics $T_i,T_j$ for row model $i$ and column model $j$, with NoProd instruments. For 95\% confidence, the critical value for Cox is $\pm1.95$, and EB is $5.98$. Standard errors account for two-step estimation error and clustering at the market level; see Appendix \ref{sect:TwoStep}.\looseness=-1
\end{tablenotes}
\end{threeparttable}
\end{table}    


\noindent \textbf{Pooling all Instrument Sets:}  We present in Table \ref{Tab:Instr_Rob} the test results obtained by pooling all instrument sets used in Section \ref{sec:empiricaleg}.  Two observations emerge from the table. First, the $F$-statistics with the pooled instruments, although above the corresponding critical values for 95\% best-case power, are below those for the NoProd instrument set. This confirms our observation that pooling instruments may result in lower $F$-statistics, and potentially weak instruments. Second, the MCS for both sets of pooled instruments now includes not only model 2, but also model 1 at a confidence level $\alpha = 0.05$. Hence, pooled instrument sets lead to less sharp conclusions in this example.

\begin{table}[ht]
\footnotesize
\caption{RV Test Results with Alternative Instruments}
\label{Tab:Instr_Rob}
\centering
\begin{threeparttable}
\input{Submission/QE/Tables/CombinedInstr}
\begin{tablenotes}[flushleft]
    \setlength\labelsep{0pt}
    \footnotesize
    \item Table reports the RV test statistics $T^\text{RV}$ and the effective $F$-statistic for all pairs of models, and the MCS $p$-values (details on their computation are in Appendix F). A negative RV test statistic suggests better fit of the row model. With MCS $p$-values below 0.05 a row model is rejected from the model confidence set. All $F$-statistics exceed the appropriate critical values for a worst-case size of  0.075 and best-case power of 0.95. Both $T^\text{RV}$ and the $F$-statistics account for two-step estimation error and clustering at the market level; see Appendix \ref{sect:TwoStep} for details.  \looseness=-1
\end{tablenotes}
\end{threeparttable}
\end{table}    


    


==> Submission/QE/Appendices/TwoStep.tex <==

This appendix extends all our previously introduced statistics to take into account uncertainty stemming from preliminary demand estimation as well as dependence across observations. We suppose that $\Delta_m$ is a function of demand parameters $\theta^D_0$ that are estimated using a GMM estimator $\hat \theta^D$. We therefore let $W^D$ denote the GMM weight matrix and $h(\theta^D)=\frac{1}{n} \sum_{i=1}^n h_i(\theta^D)$ the GMM sample moment function used. Furthermore, we let $ H=\nabla_\theta h(\hat\theta^D)$ be the gradient of the sample moment function $ h$ and let $ G_m=-\frac{1}{n} \hat z' \nabla_{\theta} \hat \Delta_m(\hat\theta^D)$ be the gradient of $\hat g_m$. Both gradients are with respect to $\theta^D$.

\noindent\textbf{RV test:}
The RV statistic with a two-step adjustment replaces $\hat V_{\ell k}^\text{RV}$ in the definition of $\hat\sigma^2_\text{RV}$ with $\tilde V_{\ell k}^\text{RV} = \frac{1}{n} \sum_{i=1}^n \tilde \psi_{\ell i} \tilde \psi_{k i}'$. Here, the influence function $\tilde \psi_{mi}$ adjusts $\hat \psi_{mi}$ to account for preliminary demand estimation:
\begin{align}
      \tilde \psi_{mi} &= \hat \psi_{mi} - \hat W^{1/2} G_m \Phi \!\left(h_i(\hat\theta^D)- h(\hat\theta^D)\right)
\end{align}
where $\Phi=(H'W^DH)^{-1}H'W^D$. This is a standard adjustment for first-step estimation based on the asymptotic approximation $\hat \theta^D - \theta^D_0 = -\Phi h(\theta^D_0) + o_p\big(n^{-1/2}\big).$

\noindent\textbf{AR test:}
Analogously to the above, the AR statistics with a two-step adjustment replaces $\hat V_{mm}^\text{AR}$ with $\tilde V_{mm}^\text{AR}$ where $\tilde V_{\ell k}^\text{AR} = \frac{1}{n} \sum_{i=1}^n \tilde \phi_{\ell i} \tilde \phi_{k i}'$. Here, the influence function $\tilde \phi_{mi}$ adjusts $\hat \phi_{mi} = \hat W \hat z_i(\hat p_i- \hat \Delta_{mi} - \hat z_i'\hat \pi_i)$ to account for preliminary demand estimation using the same approximation to $\hat \theta^D$ as above:
\begin{align}
      \tilde \phi_{mi} &= \hat \phi_{mi} - \hat W G_m \Phi_m \!\left(h_i(\hat\theta^D)- h(\hat\theta^D)\right).
\end{align}

% Analogous to the solution in \citeA{mw17}'s appendix D, a consistent estimator for the asymptotic variance of $\hat\pi_m$ that takes into account the uncertainty from the demand estimate $\hat\theta^D$ is:

% \[(G^{S\prime}_mWG^S_m)^{-1}G^{S\prime}_mW\Sigma_m WG^S_m(G^{S\prime}_mWG^S_m)^{-1}\]
% where $\hat g_m=n^{-1}z^{\prime}\hat\omega_m=n^{-1}z^{\prime}(p-\hat\Delta_m(\hat\theta^D)-z\hat\pi_m)$, $G^S_m=\nabla_\pi \hat g_m=n^{-1}z'z$ and:
% \[
% \Sigma_m = \sum_{i=1}^n \bigg(z^{\prime}_i\hat\omega_{m,i}-\hat g_m + \hat\Phi_m \left(z_i^{D\prime}\xi_i(\hat\theta^D)-\hat h(\hat\theta^D)\right) \bigg) \bigg( z^{\prime}_i\hat\omega_{m,i}-\hat g_m + \hat\Phi_m  \left(z_i^{D\prime}\xi_i(\hat\theta^D) -\hat h(\hat\theta^D)\right)\bigg)'
% \]
% where $\hat\Phi_m$ is defined as in the RV test case.

\noindent\textbf{$F$-statistic:}
The $F$-statistic with a two-step adjustment replaces $\hat \sigma_1^2$, $\hat \sigma_2^2$, and $\hat \sigma_{12}$ in the definition of $F$ and $\hat \rho^2$ with $\tilde \sigma_m^2 = d_z\inverse \text{trace}\big( \tilde V_{mm}^\text{AR} \hat W^{-1} \big)$ for $m\in\{1,2\}$ and $\tilde \sigma_{12} = d_z\inverse  \text{trace}\big(  \tilde V_{\ell k}^\text{AR}\hat W^{-1} )$. Here, $ \tilde V_{\ell k}^\text{AR}$ and $\tilde \phi_{mi}$ were introduced in the preceding paragraph.

An extension of Proposition \ref{prop:wkinstrF} that accounts for two-step estimation can be established under homoskedasticity, i.e., when $\hat W^{-1/2} \tilde V_{\ell k}^\text{AR} \hat W^{-1/2}$ for $\ell,k \in \{1,2\}$ converge in probability to diagonal matrices. In the absence of homoskedasticity, $F$ is still informative about the strength of the instruments, but the exact thresholds for size control reported in Table \ref{tab:Tab_StockYogo_Combined_new} may only be approximations to the true thresholds.

%\noindent\textbf{EB test:}
%Analogous to the AR test correction, except that instead of $n^{-1}z^{\prime}(p-\hat\Delta_m(\hat\theta^D)-z\hat\pi_m)$ the supply side moment is now $z^{\prime}(p-\theta\hat\Delta(\hat\theta^D))$ and we take derivatives with respect to $\theta$ to compute $G_m$. This formulation is analogous to \citeA{mw17}, Appendix D.

%\noindent\textbf{Cox test:}
%The Cox statistic with a two-step adjustment replaces $ \hat V_{mm}^\text{AR} $ in the definition of $\hat\sigma^2_\text{Cox}$ with $\tilde V_{mm}^\text{AR}$. Here, $\tilde V_{mm}^\text{AR}$ was introduced for the two-step correction of AR.


\noindent\textbf{Dependence:}
Dependent data, e.g., cluster sampling, is easily accommodated by adjustments to $\hat V_{\ell k}^\text{RV}$ and $\hat V_{\ell k}^\text{AR}$. If we let $c_{ij}$ take the value one if observations $i$ and $j$ are deemed dependent and zero otherwise, then the variance estimators used in the paper can be replaced by 
\begin{align}
    \Breve V_{\ell k}^\text{RV} = \frac{1}{n} \sum_{i=1}^n\sum_{j=1}^n c_{ij} \hat\psi_{\ell i} \hat\psi_{k j}'
    \quad \text{and} \quad 
    \Breve V_{\ell k}^\text{AR} = \frac{1}{n} \sum_{i=1}^n\sum_{j=1}^n c_{ij} \hat\phi_{\ell i} \hat\phi_{k j}'.
\end{align}
Combinations of two-step estimation and dependence are also handled by simply replacing $\hat \psi$ and $\hat \phi$ by $\tilde \psi$ and $\tilde \phi$ in the definitions of $\Breve V_{\ell k}^\text{RV}$ and $\Breve V_{\ell k}^\text{AR}$. Provided that suitable central limit theorem and laws of large numbers can be alluded to under the type of dependence considered, any claims on asymptotic validity under strong instruments made in the paper continue to hold. For clustered data, we refer to \citeA{ha19} for such results.

% Define $\hat g_{3} = \hat g_1-\hat g_2$ and $\hat Q_{3} = \hat g_{3}'\hat W\hat g_{3}$. Analogous to what we show for the RV test, we can show that a consistent estimator for the limiting variance of $\sqrt{n}(\hat Q_1-\hat Q_2-\hat Q_3)$ is:

% \[ \hat\sigma^2=4\hat g_1'\Sigma_1\hat g_1 + 4\hat g_2'\Sigma_2\hat  g_2 +4\hat g_{3}'\Sigma_{3}\hat g_{3}- 8\hat g_1'\Sigma_{1,2}\hat g_2 - 8\hat g_1'\Sigma_{1,3}  g_3 + 8g_2'\Sigma_{2,3}  g_3 \]
% where:
% \[
% \Sigma_{m,l} = \sum_{i=1}^n \bigg(z^{\prime}_i\omega_{m,i}-\hat g_m + \hat\Phi_m\left( z_i^{D\prime}\xi_i(\hat\theta^D)-\hat h(\hat\theta^D)\right) \bigg) \bigg( z^{\prime}_i\hat\omega_{l,i}-\hat g_l + \hat\Phi_l  \left(z_i^{D\prime}\xi_i(\hat\theta^D)-\hat h(\hat\theta^D)\right) \bigg)'\\
% \]
% and $\hat\Phi_m$ is defined as in the RV test case.



==> Submission/QE/Figures/flowchart.tex <==
\begin{tikzpicture}[node distance=2cm]



\node (start) [flowbox] {Step 0: Get MCS $M^*_\ell$  for each\\ instrument set $z_\ell$};
\node (in1) [flowbox, right of=start, xshift = 2cm] {Step 1: Check for conflicting evidence.\\ No conflict: $\forall \ell,\ell'$, $M^*_\ell\subseteq M^*_{\ell'} \,\, \text{or}$ \\$M^*_{\ell'}\subseteq M^*_{\ell}$ };
\node (pro1) [flowbox, right of=in1, yshift = 1.5cm, xshift = 6cm] {Step 2: $M^* = M$};
\node (pro2) [flowbox, right of=in1, yshift = -1.5cm, xshift = 6cm] {Step 2: Set $M^*$ as smallest MCS.\\ Then $\forall$ $\ell$ add $M^*_\ell$ to $M^*$ if $z_\ell$ strong for all model pairs};
%\node (pro3) [flowbox, below  of=pro2, yshift=0.2cm] {$\forall$ $l$ add $M^*_\ell$ to $M^*$ if $z_\ell$ strong for all pairs of models};

\draw [arrow] (start) -- (in1);
\draw [arrow] (in1) -- node[anchor=east,rotate=10,xshift=2cm,yshift = 0.25cm] {conflicting evidence} (pro1);
\draw [arrow] (in1) -- node[anchor=south, rotate=-10.5] {no conflicting evidence} (pro2);
%\draw [arrow] (pro2) -- (pro3);
%\draw [arrow] (pro2b) |- (pro1);
%\draw [arrow] (pro2a) -- (out1);
%\draw [arrow] (out1) -- (stop);


\end{tikzpicture}

==> Submission/QE/Figures/noise.tex <==

\begin{tikzpicture}[scale = 0.9]
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=-1,xmax=5.5,ymin=-1.0,ymax=5.5,
  tick style={draw=none},
  xticklabels=\empty,
  yticklabels=\empty,
  xlabel={$E[(\Delta^z_0-\Delta^z_1)^2]$},
  ylabel={$E[(\Delta^z_0-\Delta^z_2)^2]$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.8,0.15)},anchor=north},
    y label style={at={(axis description cs:0.15,.75)},rotate=90,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  title={A. Model Selection - High Noise},
  grid=major,
  grid style={thin,densely dotted,white!20}]

%45-deg lines
\addplot [domain=0:5.5,samples=2, color = black] {x} node[right]{};


%shading
\tikzstyle{rej1}=[draw=none,line width=10pt,preaction={clip, postaction={pattern=horizontal lines, pattern color=blue, opacity=0.3}}]
\tikzstyle{rej2}=[draw=none,line width=1pt,preaction={clip, postaction={pattern=vertical lines, pattern color=red, opacity=0.3}}]

\draw[rej1] (100,300) -- (100,850) -- (650,850)   -- cycle;
\draw[rej2] (300,100) -- (850,100) -- (850,650)   -- cycle;




\draw[draw=black,line width=0.5pt]  (100,300) -- (700,900)  -- cycle;

\draw[draw=black,line width=0.5pt]  (300,100) -- (900,700)  -- cycle;







\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (550,180) {{${Q}_1 > {Q}_2$}};

\node[text width=5.9cm,rotate = 40,color = black,fill = none] at (500,540) {{$H^\text{RV}_0$: ${Q}_1 = {Q}_2$}};


\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (300,550) {{${Q}_1 < {Q}_2$}};



%\draw[black, fill=black] (200,350) circle (10) ;
%\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (350,380) {{$G$}};

\end{axis}

\end{tikzpicture}\hfill
\begin{tikzpicture}[scale = 0.9]
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=-1,xmax=5.5,ymin=-1.0,ymax=5.5,
  tick style={draw=none},
  xticklabels=\empty,
  yticklabels=\empty,
  xlabel={$E[(\Delta^z_0-\Delta^z_1)^2]$},
  ylabel={$E[(\Delta^z_0-\Delta^z_2)^2]$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.8,0.15)},anchor=north},
    y label style={at={(axis description cs:0.15,.75)},rotate=90,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  title={B. Model Assessment - High Noise},
  grid=major,
  grid style={thin,densely dotted,white!20}]


%shading
\tikzstyle{rej1}=[draw=none,line width=10pt,preaction={clip, postaction={pattern=horizontal lines, pattern color=blue, opacity=0.3}}]
\tikzstyle{rej2}=[draw=none,line width=1pt,preaction={clip, postaction={pattern=vertical lines, pattern color=red, opacity=0.3}}]
\draw[rej1] (250,200) -- (250,850) -- (100,850) -- (100,200)   -- cycle;
\draw[rej2] (250,100) -- (250,200) -- (850,200) -- (850,100)   -- cycle;





\node[text width=5.9cm,rotate = 90,color = black,fill = none] at (130,550) {{$H_{0,1}^\text{AR}$: ${Q}_1 = 0$}};
\node[text width=5.9cm,rotate = 0,color = black,fill = none] at (550,140) {{$H^\text{AR}_{0,2}$: ${Q}_2 = 0$}};



\draw[draw=black,line width=0.5pt]  (250,100) -- (250,700)  -- cycle;

\draw[draw=black,line width=0.5pt]  (100,200) -- (700,200)  -- cycle;

%\draw[black, fill=black] (200,350) circle (10) ;
%\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (350,380) {{$G$}};
\end{axis}

\end{tikzpicture}



\begin{tikzpicture}[scale = 0.9]
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=-1,xmax=5.5,ymin=-1.0,ymax=5.5,
  tick style={draw=none},
  xticklabels=\empty,
  yticklabels=\empty,
  xlabel={$E[(\Delta^z_0-\Delta^z_1)^2]$},
  ylabel={$E[(\Delta^z_0-\Delta^z_2)^2]$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.8,0.15)},anchor=north},
    y label style={at={(axis description cs:0.15,.75)},rotate=90,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  title={C. Model Selection - Low Noise},
  grid=major,
  grid style={thin,densely dotted,white!20}]

%45-deg lines
\addplot [domain=0:5.5,samples=2, color = black] {x} node[right]{};


%shading
\tikzstyle{rej1}=[draw=none,line width=10pt,preaction={clip, postaction={pattern=horizontal lines, pattern color=blue, opacity=0.3}}]
\tikzstyle{rej2}=[draw=none,line width=1pt,preaction={clip, postaction={pattern=vertical lines, pattern color=red, opacity=0.3}}]



\draw[rej1] (100,180) -- (100,870) -- (800,870)   -- cycle;
\draw[rej2] (180,100) -- (870,100) -- (870,800)   -- cycle;



%\draw[draw=black,line width=0.5pt,dashed]  (100,300) -- (700,900)  -- cycle;

%\draw[draw=black,line width=0.5pt,dashed]  (300,100) -- (900,700)  -- cycle;



\draw[draw=black,line width=0.5pt]  (100,180) -- (700,770)  -- cycle;

\draw[draw=black,line width=0.5pt]  (180,100) -- (770,700)  -- cycle;





\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (550,180) {{${Q}_1 > {Q}_2$}};

\node[text width=5.9cm,rotate = 40,color = black,fill = none] at (500,540) {{$H^\text{RV}_0$: ${Q}_1 = {Q}_2$}};


\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (300,550) {{${Q}_1 < {Q}_2$}};



%\draw [->] (150,350)--(225,275);
%\draw [->] (300,500)--(375,425);
%\draw [->] (450,650)--(525,575);

%\draw [->] (350,150)--(275,225);
%\draw [->] (500,300)--(425,375);
%\draw [->] (650,450)--(575,525);

%\draw[black, fill=black] (200,350) circle (10) ;
%\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (350,380) {{$G$}};
\end{axis}

\end{tikzpicture}\hfill\hfill
\begin{tikzpicture}[scale = 0.9]
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=-1,xmax=5.5,ymin=-1.0,ymax=5.5,
  tick style={draw=none},
  xticklabels=\empty,
  yticklabels=\empty,
  xlabel={$E[(\Delta^z_0-\Delta^z_1)^2]$},
  ylabel={$E[(\Delta^z_0-\Delta^z_2)^2]$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.8,0.15)},anchor=north},
    y label style={at={(axis description cs:0.15,.75)},rotate=90,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  title={D. Model Assessment - Low Noise},
  grid=major,
  grid style={thin,densely dotted,white!20}]


%shading
\tikzstyle{rej1}=[draw=none,line width=10pt,preaction={clip, postaction={pattern=horizontal lines, pattern color=blue, opacity=0.3}}]
\tikzstyle{rej2}=[draw=none,line width=1pt,preaction={clip, postaction={pattern=vertical lines, pattern color=red, opacity=0.3}}]
%\draw<3>[rej1] (250,200) -- (250,850) -- (100,850) -- (100,200)   -- cycle;
%\draw<3>[rej2] (250,100) -- (250,200) -- (850,200) -- (850,100)   -- cycle;


\draw[rej1] (165,165) -- (165,850) -- (100,850) -- (100,165)   -- cycle;
\draw[rej2] (165,100) -- (165,165) -- (850,165) -- (850,100)   -- cycle;


%\draw<4> [<-] (160,600)--(250,600);
%\draw<4> [<-] (160,450)--(250,450);
%\draw<4> [<-] (160,300)--(250,300);

%\draw<4> [<-] (300,160)--(300,200);
%\draw<4> [<-] (450,160)--(450,200);
%\draw<4> [<-] (600,160)--(600,200);


\node[text width=5.9cm,rotate = 90,color = black,fill = none] at (130,550) {{$H_{0,1}^\text{AR}$: ${Q}_1 = 0$}};
\node[text width=5.9cm,rotate = 0,color = black,fill = none] at (550,130) {{$H_{0,2}^\text{AR}$: ${Q}_2 = 0$}};



%\draw<3-4>[draw=black,line width=0.5pt,dashed]  (250,100) -- (250,700)  -- cycle;

%\draw<3-4>[draw=black,line width=0.5pt,dashed]  (100,200) -- (700,200)  -- cycle;


\draw[draw=black,line width=0.5pt]  (165,100) -- (165,700)  -- cycle;

\draw[draw=black,line width=0.5pt]  (100,165) -- (700,165)  -- cycle;

%\draw[black, fill=black] (200,350) circle (10) ;
%\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (350,380) {{$G$}};
\end{axis}

\end{tikzpicture}


==> Submission/QE/Figures/space_degeneracy.tex <==
\begin{tikzpicture}[scale = 0.75]
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=-1,xmax=5.5,ymin=-1.0,ymax=5.5,
  tick style={draw=none},
  xticklabels=\empty,
  yticklabels=\empty,
  xlabel={$E[(\Delta^z_0-\Delta^z_1)^2]$},
  ylabel={$E[(\Delta^z_0-\Delta^z_2)^2]$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.8,0.15)},anchor=north},
    y label style={at={(axis description cs:0.15,.75)},rotate=90,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  %title={Relationship Between Null and Degeneracy},
  grid=major,
  grid style={thin,densely dotted,white!20}]

%45-deg lines
\addplot [domain=0:5.5,samples=2, color = black] {x} node[right]{};


%shading
\tikzstyle{rej1}=[draw=none,line width=10pt,preaction={clip, postaction={pattern=horizontal lines, pattern color=blue, opacity=0.2}}]
\tikzstyle{rej2}=[draw=none,line width=1pt,preaction={clip, postaction={pattern=vertical lines, pattern color=red, opacity=0.2}}]
%\draw[rej1] (100,100) -- (100,850) -- (850,850)   -- cycle;
%\draw[rej2] (100,100) -- (850,100) -- (850,850)   -- cycle;



%\node<5-6>[text width=1.0cm,rotate = 90,color = black,fill = none] at (70,50) {{$TE1$}};


\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (400,130) {{$\Gamma_2 = \Gamma_0$}};




\node[text width=5.9cm,rotate = 40,color = black,fill = none] at (410,370) {{ $\Gamma_1 = \Gamma_2$}};



\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (550,250) {{${Q}_1 > {Q}_2$}};

\node[text width=5.9cm,rotate = 40,color = black,fill = none] at (500,540) {{$H^\text{RV}_0$: ${Q}_1 = {Q}_2$}};


\node[text width=2.0cm,rotate = 0,color = black,fill = none] at (300,30) {{$\sigma^2_\text{RV} = 0$}};




\node[text width=3.0cm,rotate = 90,color = black,fill = none] at (125,350) {{$\Gamma_1 = \Gamma_0$}};

\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (300,450) {{${Q}_1 < {Q}_2$}};



\draw[-stealth,decorate,decoration={snake,amplitude=4pt,pre length=3pt,post length=4pt}] (100,100) -- ++(100,-70);
\draw[-stealth,decorate,decoration={snake,amplitude=4pt,pre length=3pt,post length=4pt}] (100,100) -- ++(100,-70);


%origin
\draw[red, fill=red] (100,100) circle (10) ;


\end{axis}

\end{tikzpicture}

==> Submission/QE/Proofs/Pf_ConvergProb_Misspecification.tex <==
\begin{proof}[Proof of Proposition \ref{prop:distrib_TE2}.]
For $(i)$, we use Equations \eqref{eq:line2} and \eqref{eq:line5} in addition to the definition of the local alternative in Equation \eqref{eq:local selection} to write
\begin{align}
\sqrt{n}\left( Q_1 -Q_2 \right) &= \sqrt{n}\left( (\Gamma_0-\Gamma_1) - (\Gamma_0-\Gamma_2) \right)\!' E[z_iz_i']\!\left( (\Gamma_0-\Gamma_1) + (\Gamma_0-\Gamma_2) \right)\! \\
&= q'E[z_iz_i']\!\left( (\Gamma_0-\Gamma_1) + (\Gamma_0-\Gamma_2) \right)\!.
\end{align}
%From Lemma 1 in \cite{rv02} or the proof of Proposition \ref{prop:degen}, we have that Assumption \ref{as:nodegen} implies that $\sqrt{n}\left( Q_1 -Q_2 \right)$ is bounded away from zero.
%From Proposition \ref{prop:degen} and its proof, we have that Assumption \ref{as:nodegen} and the local alternative in \eqref{eq:local selection} implies that $(\Gamma_0-\Gamma_1) + (\Gamma_0-\Gamma_2)$ is bounded away from zero. Furthermore, 
Assumption \ref{as:regcond}, part (iii), implies that $(\Gamma_0-\Gamma_1) + (\Gamma_0-\Gamma_2) $ is bounded. We therefore assume essentially without loss of generality that $\sqrt{n}\left( Q_1 -Q_2 \right)$ is a constant, say $c$.\footnote{This assumption is essentially without loss of generality since the boundedness of $(\Gamma_0-\Gamma_1) + (\Gamma_0-\Gamma_2)$, and therefore of $\sqrt{n}\left( Q_1 -Q_2 \right)$, allows us to otherwise argue along subsequences where $\sqrt{n}\left( Q_1 -Q_2 \right)$ converges to a constant.} From Equations \eqref{eq:line1} and \eqref{eq:line5}, we can also write 
\begin{align}
    c &= \sqrt{n} \!\left( E\!\left[(\Delta_{0i}^{z}-\Delta_{1i}^z)^2\right] - E\!\left[(\Delta_{0i}^{z}-\Delta_{2i}^z)^2\right] \right) \\
    &= E\!\big[(\Delta_{0i}^{\text{RV},z}-\Delta_{1i}^{\text{RV},z})^2\big] - E\!\big[(\Delta_{0i}^{\text{RV},z}-\Delta_{2i}^{\text{RV},z})^2\big].
\end{align}

As in Remark \ref{rem:validity}, a first order Taylor expansion, Lemma \ref{lem:asymp norm}, parts $(i)$ and $(ii)$, together with consistency of $\hat \sigma^2_\text{RV}$ now leads to
\begin{align}
    T^\text{RV} = \frac{c}{\sigma_\text{RV}} + \frac{g_1'W^{1/2} \hat W^{1/2}\hat g_1 - g_2'W^{1/2} \hat W^{1/2}\hat g_2}{\sigma_\text{RV}} + o_p(1) \xrightarrow{d} N(c,1).
\end{align}

For $(ii)$, we first note that Assumption \ref{as:homsked} implies that
\begin{align}
    V^\text{AR}_{mm} = E[z_iz_i']\inverse E[e_{mi}^2 z_iz_i'] E[z_iz_i']\inverse = \sigma_m^2 E[z_iz_i'].
\end{align}
Thus we have from Equations \eqref{eq:line2} and \eqref{eq:line5} that 
\begin{align}
    \sigma_m^2 n\pi_m'\big( V^\text{AR}_{mm}\big)\inverse\pi_m = n(\Gamma_0-\Gamma_m)'E[z_i z_i'](\Gamma_0-\Gamma_m) = q_m'E[z_i z_i']q_m
\end{align}
which in turn yields that $n\pi_m'\big( V^\text{AR}_{mm}\big)\inverse\pi_m = E\big[(\Delta^{\text{AR},z}_{0i}-\Delta^{\text{AR},z}_{mi}) ^2\big]/\sigma_m^2$ is a constant, say $c_m$. From Lemma \ref{lem:asymp norm}, parts $(iii)$ and $(iv)$, and continuous mapping we then have
\begin{align}
    T_m^\text{AR} &= n \hat \pi_m'\big( \hat V^\text{AR}_{mm}\big)\inverse \hat \pi_m = n \hat \pi_m'\big( V^\text{AR}_{mm}\big)\inverse \hat \pi_m + o_p(1) \xrightarrow{d} \chi^2_{d_z}(c_m). \qedhere
\end{align}
%
\begin{comment}
It is useful to note the following identities for each model $m$:
\begin{align}
\omega_m &= p-\Delta\theta_m\\
\omega_m &= \Delta^{*}\theta_0-\Delta\theta_m + \omega_0\\
\omega_m &= \Delta^{*}_0-\Delta_m + \omega_0.
\end{align}
Since in this environment true markups $\Delta^*$ differ from observed markups $\Delta$, we need the following definitions:
\begin{align}
A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta^*} &=  E[\tilde\Delta_{i} \tilde\Delta^{*\prime}_{i}], 
\end{align}
and
\begin{align}
    \lambda = E[\tilde\Delta_{i} \tilde\Delta_{i}']^{-1}E[\tilde\Delta_{i} \tilde\Delta^{*\prime}_{i}].
\end{align}

\begin{enumerate}
\item[\textbf{(i) - EB}] For EB, we first consider the object $\hat\theta$
\begin{align*}
\hat\theta  &= (\Delta'P_z\Delta)^{-1}\Delta'P_zp\\
&=  (\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}\hat A_{\Delta z} \hat A_{z z}^{-1}\hat A_{z\Delta^*}\theta_0+  (\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}\hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{n}\\
&\rightarrow_p (A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1} A_{\Delta z}  A_{z z}^{-1}A_{z\Delta^*}\theta_0+ (A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1} A_{\Delta z}  A_{z z}^{-1} E[z_i \omega_{0i}']\\
&=\lambda\theta_0
\end{align*}
So we have, approximating the asymptotic variance with the expression (\ref{eq:avarapprox})\footnote{Since the proposition concerns the plim of the test statistic, adopting this approximation does not alter the result.}:
\begin{align}
{n}(\hat\theta - \theta_m)'\hat V_{\theta}^{-1} (\hat\theta - \theta_m)
&\rightarrow_p \lim_{n\rightarrow\infty} {n}( (\lambda\theta_0- \theta_m)' V_{\theta}^{-1}( \lambda\theta_0- \theta_m))\\
&\approx \lim_{n\rightarrow\infty} {n}\frac{( \lambda\theta_0- \theta_m)'  E[\tilde\Delta_{i}\tilde\Delta_{i}']( \lambda\theta_0- \theta_m)}{\sigma^2_{\omega_0}}\\
&= \lim_{n\rightarrow\infty} {n}\frac{E[(\theta_0'\lambda\tilde\Delta_{i}-\tilde\Delta_{mi})^2]}{\sigma^2_{\omega_0}}\\
&=\lim_{n\rightarrow\infty} {n}\frac{ E\bigg[\bigg((\tilde{\tilde{\Delta}}^{*}_{0i}-\tilde\Delta_{0i})+(\tilde\Delta_{0i}-\tilde\Delta_{mi})\bigg)^2\bigg] }{\sigma^2_{\omega_{0}}}.
\end{align}
Note that, by Proposition \ref{prop:absfit}, $\tilde{\tilde{\Delta}}^*_{0i} = \tilde\Delta^*_{0i}$
\item[\textbf{(ii) - AR}] To derive the plim of the AR test statistic, we first consider the object $\hat\pi_m$
\begin{align*}
\hat\pi_m &= (z'z)^{-1}z'(\Delta^*\theta_0 + \omega_0 - \Delta\theta_m)\\
&= \hat A_{zz}^{-1}(\hat A_{z\Delta^*}\theta_0-\hat A_{z\Delta}\theta_m) + \hat A_{zz}^{-1}\frac{z'\omega_0}{n} \\
&\rightarrow_p A_{zz}^{-1} (A_{z\Delta^*}\theta_0-A_{z\Delta}\theta_m) + A_{zz}^{-1}E[z_i\omega_{0i}']\\
&=  \Gamma^*\theta_0-\Gamma\theta_m 
\end{align*}
So we have, under the approximation of the asymptotic variance given in (\ref{eq:avarapprox}):
\begin{align*}
T^{AR,m}&\rightarrow_p \lim_{n\rightarrow\infty} {n}(\Gamma^*\theta_0-\Gamma\theta_m)' V_{\pi_m}^{-1} (\Gamma^*\theta_0-\Gamma\theta_m)  \\
&\approx\lim_{n\rightarrow\infty} {n}\frac{(\Gamma^*\theta_0-\Gamma\theta_m)' A_{zz} (\Gamma^*\theta_0-\Gamma\theta_m)}{\sigma^2_{\omega_{0}}}  \\
&=\lim_{n\rightarrow\infty} {n}\frac{ E[(\tilde\Delta^*_{0i}-\tilde\Delta_{mi})^2] }{\sigma^2_{\omega_{0}}}  \\
&=\lim_{n\rightarrow\infty} {n}\frac{ E\bigg[\bigg((\tilde\Delta^*_{0i}-\tilde\Delta_{0i})+(\tilde\Delta_{0i}-\tilde\Delta_{mi})\bigg)^2\bigg] }{\sigma^2_{\omega_{0}}}  \\
\end{align*}

\item[\textbf{(iii) - RV}] To derive the plim of the RV test statistic we start from the object:

\begin{align*}
Q_1 - Q_2 
&= g_1'Wg_1 - g_2'Wg_2\\
&= \frac{1}{n}(\Delta^*\theta_0 - \Delta\theta_1+ \omega_0)' P_z(\Delta^*\theta_0 - \Delta\theta_1+ \omega_0)- \frac{1}{n}(\Delta^*\theta_0 - \Delta\theta_2+ \omega_0)'  P_z(\Delta^*\theta_0 - \Delta\theta_2+ \omega_0)\\
&= (\theta_0\hat A_{\Delta^*z} -\theta_1\hat A_{\Delta z})' \hat A_{zz}^{-1}(\hat A_{\Delta^*z}\theta_0 - \hat A_{\Delta z}\theta_1) - (\theta_0\hat A_{\Delta^*z} -\theta_2\hat A_{\Delta z})' \hat A_{zz}^{-1}(\hat A_{\Delta^*z}\theta_0 - \hat A_{\Delta z}\theta_2) \\
&\qquad+ 2(\theta_2-\theta_1)\hat A_{\Delta z} A_{zz}^{-1} \frac{\omega_0'z}{n}\\
& \rightarrow_p   (\theta_0 A_{\Delta^*z} -\theta_1 A_{\Delta z})'  A_{zz}^{-1}A_{zz}A_{zz}^{-1}( A_{\Delta^*z}\theta_0 - A_{\Delta z}\theta_1) \\
&\qquad- (\theta_0 A_{\Delta^*z} -\theta_2 A_{\Delta z})' A_{zz}^{-1}A_{zz}A_{zz}^{-1}( A_{\Delta^*z}\theta_0 -  A_{\Delta z}\theta_2)\\
& =  E[(\theta_0 \tilde\Delta^*_{i} -\theta_1 \tilde\Delta_i)^2] - E[(\theta_0 \tilde\Delta^*_{i} -\theta_2 \tilde\Delta_i)^2]
\end{align*}



\item[\textbf{(iv) - Cox}] For Cox, the numerator of the test statistic when using the formulation in Smith (1992) is:
 \begin{align*}
&  g_{-m}'A_{zz}^{-1}  g_{-m} - g_{m}'A_{zz}^{-1} g_m -(g_{-m} - g_m)'A_{zz}^{-1}(g_{-m} - g_m)\\
&= Q_{-m} - Q_m - (\theta_m'\hat A_{z\Delta*}' - \theta_{-m}'\hat A_{z\Delta}')\hat A_{z'z}^{-1}(\hat A_{z\Delta*}\theta_m - \hat A_{z\Delta}\theta_{-m}))\\
&\rightarrow_p  E[(\tilde\Delta^*_{0i}-\tilde\Delta_{-mi})^2] -E[(\tilde\Delta^*_{0i}-\tilde\Delta_{mi})^2]  - E[(\tilde\Delta^*_{mi}-\tilde\Delta_{-mi})^2] 
\end{align*}
So we have, under the approximation of the asymptotic variance given in (\ref{eq:avarapprox}):
\begin{align}
T^{cox,m}
&\rightarrow_p  2\lim_{n\rightarrow\infty} \sqrt{n}\frac{  E[(\tilde\Delta^*_{0i}-\tilde\Delta_{-mi})^2] -E[(\tilde\Delta^*_{0i}-\tilde\Delta_{mi})^2]  - E[(\tilde\Delta^*_{mi}-\tilde\Delta_{-mi})^2]  }{\sigma_{cox}} \\
&\approx 2\lim_{n\rightarrow\infty} \sqrt{n}\frac{  E[(\tilde\Delta^*_{0i}-\tilde\Delta_{-mi})^2] -E[(\tilde\Delta^*_{0i}-\tilde\Delta_{mi})^2]  - E[(\tilde\Delta^*_{mi}-\tilde\Delta_{-mi})^2]  }{2\sigma_{\omega_0} \sqrt{E[(\tilde\Delta_{1i}-\tilde\Delta_{2i})^2]}}.
\end{align} 
\end{enumerate}
\end{comment}
\end{proof}

==> Submission/QE/Proofs/Pf_Degeneracy.tex <==
\begin{proof}[Proof of Proposition \ref{prop:degen} and Corollary \ref{cor:degen}]

From Equations \eqref{eq:line1} and \eqref{eq:line2}, we have equivalence between $E[(\Delta^z_{0i}-\Delta^z_{mi})^2] = 0$ and $\Gamma_0-\Gamma_m=0$. Furthermore, we recall that $\pi_m=\Gamma_0-\Gamma_m$. Thus, we only need to show that $\sigma^2_\text{RV}=0$ if and only if $\pi_m=0$ for all $m\in\{1,2\}$. Rewriting Equation \eqref{eq:sig2rv} in matrix notation, we have
\begin{align}
    \sigma^2_\text{RV} = 4 
    \begin{pmatrix} W^{-1/2}\pi_1 \\ W^{-1/2}\pi_2 \end{pmatrix}'
    \begin{bmatrix}    V^\text{RV}_{11} & - V^\text{RV}_{12} \\ - V^\text{RV}_{12} & V^\text{RV}_{22}\end{bmatrix}
    \begin{pmatrix} W^{-1/2}\pi_1 \\ W^{-1/2}\pi_2 \end{pmatrix}.
\end{align}
Therefore, the claims to be proven follow from positive definiteness of the variance matrix $V^\text{RV} = E[(\psi_{1i}',\psi_{2i}')'(\psi_{1i}',\psi_{2i}')]$, which is the matrix with $V^\text{RV}_{11}$, $V^\text{RV}_{12}$, and $V^\text{RV}_{22}$ as its entries.

To show that $V^\text{RV}$ is positive definite, we take an arbitrary non-zero, non-random vector $v=(v_1',v_2')' \in \mathbb{R}^{2d_z}$. $V^\text{RV}$ is positive definite if $E(v_1'\psi_{1i}+v_2'\psi_{2i})^2 > 0$ for any such $v$. For certain implied non-random $u = (u_1',u_2')'$ and $t=(t_1',t_2')'$ where $t$ is non-zero, we have $E(v_1'\psi_{1i}+v_2'\psi_{2i})^2 = E(u_1'z_i \cdot u_2'z_i + t_1'z_i \cdot e_{1i} + t_2'z_i \cdot e_{2i} )^2$. Because $\sigma_{12}^2 < \sigma_1^2\sigma_2^2$ (Assumption \ref{as:homsked}), we have that $E(t_1'z_i \cdot e_{1i} + t_2'z_i \cdot e_{2i} )^2 > 0$. Therefore, we can only have $E(v_1'\psi_{1i}+v_2'\psi_{2i})^2 = 0$ if $e_{1i}$ or $e_{2i}$ is a linear function of $z_i$ almost surely. However, because $E[z_ie_{mi}]=0$, such dependence is ruled out by $\sigma_m^2>0$ (Assumption \ref{as:homsked}).
%
%
%
%
% We begin by noting that Lemma 1 in \citeA{rv02} shows that $\sigma^2_{RV}=0$ if and only if $   \sqrt{n}(Q_1-Q_2)=o_p(1)$.
% Thus, for Proposition \ref{prop:weakinstr}, we need to show the equivalence
% $$\sqrt{n}(\hat Q_1-\hat Q_2) = o_p(1) \qquad \Leftrightarrow  \qquad E[(\Delta^z_{0i}-\Delta^z_{mi})^2] = 0 \qquad\text{for both $m=1,2$}$$
% From \eqref{eq:line1}, \eqref{eq:line4}, and the positive definiteness of $E[z_iz_i']$, $E[(\Delta^z_{0i}-\Delta^z{m_i})^2] = 0$ iff $g_m = 0$. By \eqref{eq:sig2rv}, if $g_1$ and $g_2$ = 0, then $\sigma^2_{RV} = 0$.  Furthermore, if $\sigma^2_{RV} = 0$ 
%
%
% Consider $Q_1-Q_2$:
% \begin{align*}
% Q_1-Q_2 &=
% %\frac{1}{n} \omega_1'z(z'z)^{-1}z'\omega_1  -  \frac{1}{n}\omega_2'z(z'z)^{-1}z'\omega_2 \\ &=
% \frac{1}{n} \bigg(\omega_1-\omega_2\bigg)'z(z'z)^{-1}z'\bigg(\omega_1+\omega_2\bigg) \\
% % &= \frac{1}{n}\bigg(p-\Delta_1-p+\Delta_2\bigg)'z(z'z)^{-1}z'\bigg(p-\Delta_1+p-\Delta_2\bigg) \\
%   &= \frac{1}{n}\bigg(p-\Delta_1-p+\Delta_2\bigg)'z(z'z)^{-1}z'\bigg(2p-\Delta_1-\Delta_2\bigg) \\
%   &= \frac{1}{n}\bigg(p-\Delta_1-p+\Delta_2\bigg)'z(z'z)^{-1}z'\bigg(2\Delta^*_0 +2\omega_0-\Delta_1-\Delta_2\bigg) \\
% %    &= \frac{1}{n}\bigg(\Delta_2-\Delta_1\bigg)'z(z'z)^{-1}z'\bigg(\Delta_1 +2\omega_0-\Delta_2\bigg) \\
%       &= \frac{1}{n}\bigg(\Delta_2-\Delta_1\bigg)'z(z'z)^{-1}z'\bigg(\Delta^*_0 - \Delta_1 + \Delta^*_0 -\Delta_2\bigg) +2\frac{1}{n}\bigg(\Delta_2-\Delta_1\bigg)'z(z'z)^{-1}z'\omega_0 \\
% %  &= \frac{1}{n}\bigg(\Delta_2-\Delta_1\bigg)'z(z'z)^{-1}z'z(z'z)^{-1}z'\bigg(\Delta_1-\Delta_2\bigg) +2\frac{1}{n}\bigg(\Delta_2-\Delta_1\bigg)'z(z'z)^{-1}z'\omega_0 \\
%   &= \frac{1}{n}\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'z'z\bigg(\hat\Gamma_0 - \hat\Gamma_1 + \hat\Gamma_0 -\hat\Gamma_2\bigg) +2\frac{1}{n}\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'z'\omega_0 
%   \end{align*}
% %  So we have:
% %  \begin{align*}
% %    \sqrt{n}(Q_1-Q_2) &= \frac{1}{\sqrt{n}}\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'z'z\bigg(\hat\Gamma_0 - \hat\Gamma_1 + \hat\Gamma_0 -\hat\Gamma_2\bigg) +2\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'\frac{z'\omega_0}{\sqrt{n}}
% %  \end{align*}
%
% %If $\hat \gamma = \hat \Gamma_1-\hat \Gamma_2 = o_p(1)$, $\hat \Gamma_0-\frac{\hat \Gamma_1 + \hat\Gamma_2}{2} = \frac{O_p(1)}{\sqrt{n}} =  o_p(1)$, and $\frac{z'\omega_0}{\sqrt{n}} = O_p(1)$, then we have:
% %  \begin{align*}
% %      \sqrt{n}(Q_1-Q_2) &=\sqrt{n}\bigg(\hat\Gamma_0 - \hat\Gamma_1 + \hat\Gamma_0 -\hat\Gamma_2\bigg)'\frac{z'z}{n}\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg) +2\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'\frac{z'\omega_0}{\sqrt{n}}
% %  \end{align*}
% %    \begin{align*}
%  %     \sqrt{n}(Q_1-Q_2) &=\underbrace{\sqrt{n}\bigg(\hat\Gamma_1 - \hat\Gamma_0 + \hat\Gamma_2 -\hat\Gamma_0\bigg)'}_{= O_p(1)}\underbrace{\frac{z'z}{n}}_{\rightarrow A_{zz}}\underbrace{\bigg(\hat\Gamma_1-\hat\Gamma_2\bigg)}_{=o_p(1)} +\underbrace{2\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'}_{=o_p(1)}\underbrace{\frac{z'\omega_0}{\sqrt{n}}}_{= O_p(1)}
%  % \end{align*}
%  % so that $ \sqrt{n}(Q_1-Q_2) = o_p(1)$ if and only if $\hat \gamma = o_p(1)$.
% 
%  For $m = 0,1,2$, given that $\hat\Gamma_m$ is a OLS regression coefficient and given the regularity conditions in Assumptions \ref{as:regcond}, $\hat\Gamma_m \rightarrow_p \Gamma_m$ so that $\hat\Gamma_m - \Gamma_m = o_p(1)$ and $\sqrt{n}(\hat\Gamma_m-\Gamma_m) = O_p(1)$.  Let $\hat\psi_m = (\hat\Gamma_m-\Gamma_m)$.
%       \begin{align*}
%       \sqrt{n}(Q_1-Q_2) &=\sqrt{n}\bigg(\hat\Gamma_1 - \hat\Gamma_0 + \hat\Gamma_2 -\hat\Gamma_0\bigg)'\frac{z'z}{n}\bigg(\hat\Gamma_1-\hat\Gamma_2\bigg) + 2\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'\frac{z'\omega_0}{\sqrt{n}}\\
%       &= \bigg(\sqrt{n}\bigg(\hat\psi_1-2\hat\psi_0 +  \hat\psi_2 \bigg) +\sqrt{n}(\Gamma_1 + \Gamma_2 - 2\Gamma_0)\bigg)'\frac{z'z}{n}\bigg(\hat\psi_1 -\hat\psi_2+\Gamma_1 - \Gamma_2\bigg)+\\&\qquad 2\bigg(\hat\psi_2-\hat\psi_1 +\Gamma_2-\Gamma_1\bigg)'\frac{z'\omega_0}{\sqrt{n}}
%   \end{align*}
%   Notice that, by Assumptions \ref{as:momcond} and \ref{as:regcond}, $\frac{z'\omega_0}{\sqrt{n}} = O_p(1)$ and $\frac{z'z}{n} = O_p(1)$.  Using the following facts\footnote{See page 12 of van der Vaart's \textit{Asymptotic Statistics}} $O_p(1)o_p(1) = o_p(1)$, $o_p(1) + o_p(1) = o_p(1)$, we can show that $\sqrt{n}(Q_1-Q_2) = o_p(1)$ if and only if the following two conditions hold: (i) $\Gamma_2 = \Gamma_1$ and (ii) $\Gamma_0 = \frac{\Gamma_1+\Gamma_2}{2}$.  To show the if part of the statement, if both (i) and (ii) hold, then:
%   \begin{align*}
%       \sqrt{n}(Q_1-Q_2) &=\bigg(\sqrt{n}\bigg(\hat\psi_1-2\hat\psi_0 +  \hat\psi_2 \bigg)\bigg)'\frac{z'z}{n}\bigg(\hat\psi_1 -\hat\psi_2\bigg)+ 2\bigg(\hat\psi_2-\hat\psi_1 \bigg)'\frac{z'\omega_0}{\sqrt{n}}\\
%       &= O_p(1)(O_p(1)o_p)) + o_p(1)O_p(1)\\
%       &= o_p(1) + o_p(1)\\
%       & = o_p(1)
%   \end{align*}
% Now to show the only if part of the statement, first suppose (i) holds but (ii) does not.  Then we have
%   \begin{align*}
%       \sqrt{n}(Q_1-Q_2) &=
%       \bigg(O_p(1) +\sqrt{n}(\Gamma_1 + \Gamma_2 - 2\Gamma_0)\bigg)'o_p(1)+ o_p(1) \\
%       &=
%       o_p(1) +\sqrt{n}(\Gamma_1 + \Gamma_2 - 2\Gamma_0)o_p(1)\\
%     &= o_p(1) + o_p(\sqrt{n}(\Gamma_1 + \Gamma_2 - 2\Gamma_0)\\
%     &\neq o_p(1)
%     \end{align*}
%   Now suppose (ii) holds but (i) does not. 
%   \begin{align*}
%       \sqrt{n}(Q_1-Q_2) &= O_p(1)(o_p(1) + \Gamma_1-\Gamma_2) + o_p + (\Gamma_1-\Gamma_2)O_p(1)\\
% &= o_p(1) + O_p(1)(\Gamma_1-\Gamma_2)\\
% &\neq o_p(1)
%       \end{align*}
%
% Thus, we have established $\sqrt{n}(Q_1-Q_2) = o_p(1)$ iff $\Gamma_1 = \Gamma_2$ and $\Gamma_0 = \frac{\Gamma_1 + \Gamma_2}{2}$.  Notice, that, if we combine conditions (i) and (ii), $\sqrt{n}(Q_1-Q_2) = o_p(1)$ iff $\Gamma_1 = \Gamma_2 = \Gamma_0$.  Thus, we can express this in terms of weak instruments.  Specifically,  $\sqrt{n}(Q_1-Q_2) = o_p(1)$ iff $\hat\Gamma_0 - \hat\Gamma_m = o_p(1)$ for $m = 1,2$.  We can also express degeneracy in terms of predicted markups.  $E[(\tilde\Delta^*_{0i}-\tilde\Delta_{mi})^2] = E[(\Gamma_0-\Gamma_m)z_iz_i'(\Gamma_0-\Gamma_m)] = (\Gamma_0-\Gamma_m)E[z_iz_i'](\Gamma_0-\Gamma_m)] = 0$  So under Assumption \ref{as:regcond}, $\sqrt{n}(Q_1-Q_2) = o_p(1)$ iff $E[(\tilde\Delta^*_{0i} - \tilde\Delta_{mi})^2] = 0$ for $m =1,2$.  We could also write $E[(\tilde\Delta_{0i}-\tilde\Delta_{mi}] = E[((\Gamma_0-\Gamma_m)z_i] = (\Gamma_0-\Gamma_m)E[z_i] $ but this is always 0 due to the orthogonalization
\end{proof}


==> Submission/QE/Proofs/Pf_Nulls.tex <==
\begin{proof}[Proof of Proposition \ref{prop:nulls}]
For $(i)$, we need to show the equivalence
\begin{align}\label{eq:equiv_prop1_ar}
\pi_m = 0 \qquad \Leftrightarrow \qquad   E[(\Delta^z_{0i}-\Delta^z_{mi})^2] = 0  
\end{align}
This equivalence is a consequence of Equations \eqref{eq:line1} and \eqref{eq:line5} in addition to $E[z_i z_i']$ being positive definite.
For $(ii)$, we we need to show the equivalence
\begin{align}
    {Q}_1-{Q}_2 =0  \qquad \Leftrightarrow \qquad  E[(\Delta^z_{0i}-\Delta^z_{1i})^2]-E[(\Delta^z_{0i}-\Delta^z_{2i})^2]=0. 
\end{align}
This equivalence is a consequence of Equations \eqref{eq:line1} and \eqref{eq:line5}.
%
\begin{comment}
\begin{align}\label{eq:equiv_prop1_ar}
\pi_m = 0 \qquad \Leftrightarrow \qquad   E[(\Delta^z_{0i}-\Delta^z_{mi})^2] = 0  
\end{align}
By definition of the OLS estimator, $\pi_m$ is:
\begin{align}
    \pi_m &= E[z_iz_i']^{-1}E[z_i(p_i-\Delta_{mi})] \\
        %&=E[z_iz_i']^{-1}E[z_i(\Delta_{0i}-\Delta_{mi})]\\
        &=(\Gamma_{0}-\Gamma_{m})
    \end{align}
where the second equality follows from Assumption \ref{as:momcond}, $E[z_i w_{0i}]=0$, and $\Delta_{0i} = p_i - \omega_{0i}$.  From the Proof of Lemma 1, it follows that $E[(\Delta^z_{0i}-\Delta^z_{mi})^2]=\pi_m'E[z_i'z_i]\pi_m$. 
The equivalence in \eqref{eq:equiv_prop1_ar} now follows from $E[z_i z_i']$ being positive definite.\\
For (ii), we can directly show the equivalence ${Q}_m = E[(\Delta^z_{0i}-\Delta^z_{mi})^2] $.
\begin{align*}
{Q}_m &= E[\omega_{mi}z_i]'E[z_i z_i']^{-1}E[\omega_{mi}z_i]\\
&=E[(\Delta_{0i}-\Delta_{mi})z_i]'E[z_i z_i']^{-1}E[(\Delta_{0i}-\Delta_{mi})z_i]\\
%&=E[(\Delta_{0i}-\Delta_{mi})z_i]'E[z_i z_i']^{-1}E[z_i z_i']E[z_i z_i']^{-1}E[(\Delta_{0i}-\Delta_{mi})z_i]\\
&=(\Gamma_0-\Gamma_m)'E[z_i z_i'](\Gamma_0-\Gamma_m)\\
&=E[(\Delta^z_{0i}-\Delta^z_{mi})^2]
\end{align*}     
where the second equality follows from  Assumption \ref{as:momcond}, $E[z_i w_{0i}]=0$, $\Delta_{mi} = p_i-\omega_{mi}$, and  $\Delta_{0i} = p_i - \omega_{0i}$. The last equality is proven in the Proof of Lemma 1.  Thus, ${Q}_1-{Q}_2 = E[(\Delta^z_{0i}-\Delta^z_{1i})^2]-E[(\Delta^z_{0i}-\Delta^z_{2i})^2] $
\end{comment}
%
\begin{comment}
\begin{enumerate}
    \item Note that for AR, the OLS estimator is given as:
    \begin{align}
    \pi_m &= E[z_iz_i']^{-1}E[z_i(p_i-\Delta_{mi})] \\
    &=E[z_iz_i']^{-1}E[z_i(\Delta_{0i}-\Delta_{mi})] + E[z_iz_i']^{-1}E[z_i\omega_{0i})]\\
        &=E[z_iz_i']^{-1}E[z_i(\Delta_{0i}-\Delta_{mi})]\\
        &=(\Gamma_{0i}-\Gamma_{mi})
    \end{align}
    We can rewrite the moment in Lemma \ref{lemma1} as:
    \begin{align}
        E[(\Delta^z_{0i}-\Delta^z_{mi})^2] &=E[(z_iE[z_iz_i']^{-1}E[z_i(\Delta_{0i}-\Delta_{mi})])^2]\\
        &=E[(z_i\pi_m)^2]\\
         &=E[z_i\pi_m \pi_m'z_i']\\
         &=E[\pi_m'z_i'z_i\pi_m ]\\
                  &=\pi_m'E[z_i'z_i]\pi_m 
    \end{align}
    Since $E[z_i'z_i]$ is positive definite, then it immediately follows from the definition of positive definite that $E[(\Delta^z_{0i}-\Delta^z_{mi})^2] = 0$ iff $\pi_m = 0$.
\item 
\begin{align*}
\mathcal{Q}_m &= E[\omega_{mi}z_i]'E[z_i z_i']^{-1}E[\omega_{mi}z_i]\\
&= E[(\Delta_{0i}-\Delta_{mi}+\omega_{0i})z_i]'E[z_i z_i']^{-1}E[(\Delta_{0i}-\Delta_{mi}+\omega_{0i})z_i]\\
&=E[(\Delta_{0i}-\Delta_{mi})z_i]'E[z_i z_i']^{-1}E[(\Delta_{0i}-\Delta_{mi})z_i]\\
&=E[(\Delta_{0i}-\Delta_{mi})z_i]'E[z_i z_i']^{-1}E[z_i z_i']E[z_i z_i']^{-1}E[(\Delta_{0i}-\Delta_{mi})z_i]\\
&=(\Gamma_0-\Gamma_m)'E[z_i z_i'](\Gamma_0-\Gamma_m)\\
&=E[(\Gamma_0-\Gamma_m)'z_i z_i'(\Gamma_0-\Gamma_m)]\\
&=E[(\Delta^z_{0i}-\Delta^z_{mi})'(\Delta^z_{0i}-\Delta^z_{mi})]\\
&=E[(\Delta^z_{0i}-\Delta^z_{mi})^2]
\end{align*}     
Since $\mathcal{Q}_m = E[(\Delta^z_{0i}-\Delta^z_{mi})^2] $, $\mathcal{Q}_1-\mathcal{Q}_2 = E[(\Delta^z_{0i}-\Delta^z_{1i})^2]-E[(\Delta^z_{0i}-\Delta^z_{2i})^2] $
\end{enumerate}
\end{comment}
\end{proof}

==> Submission/QE/Proofs/Pf_Plims.tex <==
\begin{proof}[Proof of Lemma \ref{cor:modelmisc}.] For $(i)$, suppose for concreteness that $E[(\Delta^z_{0i}-\Delta^z_{1i})^2]<E[(\Delta^z_{0i}-\Delta^z_{2i})^2]$. We need to show that $\Pr\big( T^\text{RV} < -q_{1-\alpha/2}(N) \big) \rightarrow 1$ where $q_{1-\alpha/2}(N)$ is the $(1-\alpha/2)$-th quantile of a standard normal distribution. From Proposition \ref{prop:nulls}, part $(ii)$, we have $Q_1 < Q_2$. Lemma \ref{lem:asymp norm}, parts $(i)$ and $(ii)$, together with Remark \ref{rem:validity} yields $T^\text{RV}/\sqrt{n} = \frac{ \hat Q_1-\hat Q_2}{\hat \sigma_\text{RV}} \xrightarrow{p}  \frac{Q_1-Q_2}{\sigma_\text{RV}} < 0$. Therefore, $\Pr\big( T^\text{RV}/\sqrt{n} < -q_{1-\alpha/2}(N_{0,1})/\sqrt{n} \big) \rightarrow 1$.

For $(ii)$, suppose that $E[(\Delta^z_{0i}-\Delta^z_{mi})^2]\neq 0$ for some $m \in \{1,2\}$.  We need to show that $\Pr\big( \text{reject } H^\text{AR}_{0,m} \big) \rightarrow 1$. From Proposition \ref{prop:nulls}, part $(i)$, it follows that $\pi_m \neq 0$ and since $V^\text{AR}_{mm}$ is positive definite we have $\pi_m'(V^\text{AR}_{mm})\inverse \pi_m > 0$. Using Lemma \ref{lem:asymp norm}, parts $(iii)$ and $(iv)$, we have $(\hat \pi_m,\hat V^\text{AR}_{mm}) \xrightarrow{p} (\pi_m,V^\text{AR}_{mm})$ so that $T^\text{AR}_m/n = \hat\pi_m'\big(\hat V^\text{AR}_{mm}\big)\inverse \hat\pi_m \xrightarrow{p} \pi_m'\big( V^\text{AR}_{mm}\big)\inverse \pi_m > 0$. Therefore, $\Pr\big( \text{reject } H^\text{AR}_{0,m} \big) = \Pr\big( T^\text{AR}_m/n > q_{1-\alpha}(\chi^2_{d_z})/n \big) \rightarrow 1$ where $q_{1-\alpha}(\chi^2_{d_z})/n ) \rightarrow 1$ where $q_{d_z}(1-\alpha)$ denotes the $(1-\alpha)$-th quantile of a $\chi^2_{d_z}$ distribution.
\begin{comment}
\begin{itemize}

\item[(i)]  Consider anly model $m$ such that $E[(\Delta^z_{0i}-\Delta^z_{mi})^2]\neq 0$.  By \eqref{eq:line1}, \eqref{eq:line5} and the positive definiteness of $E[z_iz_i']$, $\pi_m\neq 0$, representing a fixed alternative of the AR test under $H^{AR}_{A,m}$.  From Lemma A.1 (iii) $\hat\pi_m\rightarrow\pi_m$, and from  (iv) $\hat V_m\rightarrow V_m$. Thus, $\hat\pi_m'\hat V_m\hat\pi_m\rightarrow_p \pi_m' V_m\pi_m >0$, where the inequality hold because  $V_m$ is positive definite. It immediately follows that $T^{AR} \rightarrow \infty$ and $\Pr(\text{reject } H^{AR}_{0,m}) \rightarrow 1$.  

    \item[(ii)]  By Lemma A.1 (i), $\hat Q_m \rightarrow_p Q_m$ for $m=1,2$ and  by (ii), $\hat\sigma^2_{RV} \rightarrow_p \sigma^2_{RV} \neq 0$ under Assumption \ref{as:nodegen}. Thus, $T^{RV} = \frac{\sqrt{n} (\hat Q_1-Q_2)}{\hat \sigma_{RV}} \rightarrow_p \lim_{n\rightarrow\infty }  \frac{\sqrt{n}(Q_1-Q_2)}{\sigma_{RV}}$. For any pair of models $1,2$ by which     $E[(\Delta^z_{0i}-\Delta^z_{1i})^2]<E[(\Delta^z_{0i}-\Delta^z_{2i})^2]$, $Q_1<Q_2$  from \eqref{eq:line1} and \eqref{eq:line5}.  Thus, the models represent a fixed alternative satisfying $H^{RV}_{1}$
 In this case  $T^{RV}\rightarrow_p -\infty$ so that $\Pr(\text{reject } H^{RV}_0 \text{ for } m=1) \rightarrow 1$ as $n\rightarrow\infty$. Likewise for fixed alternatives satisfying $H^{RV}_{2}$,  $Q_1>Q_2$ and, from \eqref{eq:line1} and \eqref{eq:line5}, $E[(\Delta^z_{0i}-\Delta^z_{1i})^2]>E[(\Delta^z_{0i}-\Delta^z_{1i})^2]$ .  In this case  $T^{RV}\rightarrow_p \infty$ so that $\Pr(\text{reject } H^{RV}_0 \text{ for } m=2) \rightarrow 1$ as $n\rightarrow\infty$.
\end{itemize}
\end{comment} 
\end{proof}

==> Submission/QE/Proofs/Pf_Testability.tex <==
\begin{proof}[Proof of Lemma \ref{as:falsify}.]

% \noindent Let model 1 be the true model. We want to show that if and only if the condition     \begin{align}\label{eq:testability3}
%     E[(\tilde\Delta_{1i} - \tilde\Delta_{2i})^2] \neq 0
%     \end{align}
% a candidate model $m=2$ is falsified, in the sense of Definition 1:
% \begin{align}\label{eq:testability2}
% E[z_i(p_i-\Delta_{2i})]\neq0. 
% \end{align}
% As a useful preliminary, recall that the first stage is:
% \begin{align*}
% \Delta_i &= z_i\Gamma + \eta_i\\
%         &= \tilde \Delta_i + \eta_i,
% \end{align*}
% where $\eta$   is projection error orthogonal to $z$ by construction, so that $E[z_i\eta_i] = 0$.

% We first prove that (\ref{eq:testability3}) implies (\ref{eq:testability2}). Notice that a necessary and sufficient for (\ref{eq:testability3}) to be true is that there exists some nonzero measure subset $Z$ of the support of $z_i$ such that for $z_i\in Z$ we have $\tilde \Delta_{1i}\neq\tilde \Delta_{2i}.$ In turn, because of the definition of projection, it must be that for $z_i\in Z$ we have $z_i \Gamma_1 \neq z_i \Gamma_2.$ Then, we know that $\Gamma_1 \neq  \Gamma_2$ which in turn implies $E[z_i\Delta_{1i}] \neq E[z_i\Delta_{2i}]$ since $\Gamma = E[z_iz_i']^{-1}E[z_i\Delta_i] $. Condition (\ref{eq:testability2}) follows immediately from the fact that model $m=1$ is the true model.

% Now we prove that (\ref{eq:testability2}) implies (\ref{eq:testability3}). To do so, we proceed by contradiction: suppose that (\ref{eq:testability2}) holds, but $ E[(\tilde\Delta_{1i} - \tilde\Delta_{2i})^2]=0.$ Then, almost surely $\tilde \Delta_{1i}=\tilde \Delta_{2i}$. Hence we can write:
% \begin{align*}
%     E[z_i(p_i - \tilde \Delta_{1i})] = E[z_i(p_i - \tilde \Delta_{2i})],
% \end{align*}
% and since $E[z_i\eta_i] = 0$ we have:
% \begin{align*}
%     E[z_i(p_i - \tilde \Delta_{1i} - \eta_{1i})] = E[z_i(p_i - \tilde \Delta_{2i} - \eta_{2i})],
% \end{align*}
% which leads to a contradiction of (\ref{eq:testability2}). Hence, when (\ref{eq:testability2}) holds, (\ref{eq:testability3}) must hold as well.

%This is now the proof that our definition corresponds to that in BH14 under parametric restrictions.\\

In our parametric framework, the falsifiable condition in Equation (28) of \cite{bh14} is\footnote{See Section 6, Case 2 in \cite{bh14} for a discussion of their non-parametric environment.}
\begin{align}\label{eq:BH14}
    E[ \boldsymbol{p}_i-\boldsymbol{\Delta}_{mi} \mid z_i,\textbf{w}_i ] = \textbf{w}_i \tau + E[ \omega_{0i} \mid z_i,\textbf{w}_i ] \quad \text{a.s.}
\end{align}
This equation, together with residualization against $\textbf{w}_i$ and integration over the distribution of  $\textbf{w}_i$, then implies that
\begin{align}\label{eq:BH14}
    E[ {p}_i-{\Delta}_{mi} \mid z_i ] = E[ \omega_{0i} \mid z_i] \quad \text{a.s.}
\end{align}
Integrating the above against $z_i$, using the assumption $E[z_i\omega_{0i} ]=0$, and relying on the law of iterated expectations, then yields
\begin{align}
    E[z_i(p_i-\Delta_{mi})] = 0
\end{align}
Finally, we note the equivalence
\begin{align}\label{eq:equivalence}
    E[(\Delta_{0i}^{z}-\Delta_{mi}^z)^2] = 0 \quad  &\Leftrightarrow \quad E[z_i(p_i-\Delta_{mi})] = 0 
\end{align}
which follows from \eqref{eq:line1}, \eqref{eq:line4}, and $E[z_i z_i']$ being positive definite. Thus we have shown that Equation (28) of \cite{bh14} implies \eqref{eq:testability}.
%
%
%{The falsifiable condition in Equation (28) of \cite{bh14} is the right most expression in \eqref{eq:equivalence}, as our environment is nested in their nonparametric testing setup. See Section 6, Case 2 in \cite{bh14} for a discussion of their environment.  After conditioning on $\textbf{w}$, the marginal revenue function for model $m$ is $p_i - \Delta_{mi}$.  So, under constant marginal costs, condition (28) in \cite{bh14} for a model to be testable becomes the one above:$ E[p_i - \Delta_{mi} \!\mid\! z_i,\textbf{w}_i]=0$ with probability one.}
%
% Part (ii) of Assumption \ref{as:regcond} implies that $E[z'z]$ and $E[z_i z_i']$ are positive definite so that $\Gamma_m = E[z'z]^{-1} E[z'\Delta_m] = E[z_iz_i']^{-1} E[z_i\Delta_{mi}]$ and $\Delta_{mi}^z = z_i'\Gamma_m$ are well-defined. We can then note that
% \begin{align}
%     E[(\Delta_{0i}^{z}-\Delta_{mi}^z)^2] &= E[(z_i'(\Gamma_0-\Gamma_m))^2] \\
%     &= (\Gamma_0-\Gamma_m)'E[z_i z_i'](\Gamma_0-\Gamma_m) \\
%     &= E[z_i(\Delta_{0i}-\Delta_{mi})]'E[z_i z_i']^{-1}E[z_i(\Delta_{0i}-\Delta_{mi})]\\
%     &= E[z_i(p_i-\Delta_{mi})]'E[z_i z_i']^{-1}E[z_i(p_i-\Delta_{mi})]
% \end{align}
% where the last equality follows from Assumption \ref{as:momcond}, $E[z_i w_{0i}]=0$, and $\Delta_{0i} = p_i - \omega_{0i}$. The equivalence in \eqref{eq:equivalence} now follows from $E[z_i z_i']$ being positive definite.
\end{proof}

==> Submission/QE/Proofs/Pf_WkInstrAsymptotic_Trv_F.tex <==
\begin{proof}[Proof of Proposition \ref{prop:wkinstrF}.]
The proof proceeds in three steps. Step (1) provides a function of the data $(\tilde \Psi_-',\tilde \Psi_+')'$ and two constants $\mu_-$, $\mu_+$ such that $(\tilde \Psi_-',\tilde \Psi_+')' \xrightarrow{d} (\Psi_-',  \Psi_+')'$. All of $(\tilde \Psi_-',\tilde \Psi_+')'$, $\mu_-$, and $\mu_+$ are also functions of the DGP. Step (2) establishes parts $(ii)$--$(iv)$. Step (3) shows that $\abs{T^\text{RV}} = \abs{\tilde \Psi_-'\tilde \Psi_+}/\big(\norm{\tilde \Psi_-}^2 + \norm{\tilde \Psi_+}^2 + 2 \rho \tilde \Psi_-'\tilde \Psi_+ + o_p(1) \big)^{1/2}$ and $F=\big( \norm{\tilde \Psi_-}^2 + \norm{\tilde \Psi_+}^2 - 2\rho \tilde \Psi_-'\tilde \Psi_+ \big)/\big(2d_z \big) + o_p(1)$. Part $(i)$ follows from continuous mapping, step (1), and step (3).
	
	
\noindent \textbf{Step (1)} We first provide definitions of $\mu_-$ and $\mu_+$. Let $\tau_+ = 2(\sigma_1^2 + \sigma_2^2 + 2\sigma_{12})^{1/2}$ and $\tau_- = 2(\sigma_1^2 + \sigma_2^2 - 2\sigma_{12})^{1/2}$ and use these two positive constants to define% the vectors
\begin{align}
		\begin{pmatrix}
			 \mu_1 \\  \mu_2
		\end{pmatrix}  =
		\left(\frac{1}{{\tau_-}} + \frac{1}{{\tau_+}}\right)\! \begin{pmatrix} \sqrt{n} W^{1/2} g_1    \\	 	-\sqrt{n} W^{1/2}  g_2		\end{pmatrix}
		+
		\left(\frac{1}{{\tau_-}} - \frac{1}{{\tau_+}}\right)\!\begin{pmatrix}	-\sqrt{n} W^{1/2}  g_2  \\ 		\sqrt{n} W^{1/2}  g_1 		\end{pmatrix}\!.
\end{align}
Defining $\kappa = 1 + \mathbf{1}\{ \norm{\mu_1} \le \norm{\mu_2}  \}$, we then let $\mu_- = \norm{\mu_\kappa} - \norm{\mu_{3-\kappa}}$ and $\mu_+ = \norm{\mu_1} + \norm{\mu_2}$. Since the instruments are weak for testing, we have that $\sqrt{n} W^{1/2} g_m = E[z_i z_i']^{1/2} q_m$ so $\mu_-$ and $\mu_+$ do not depend on $n$. 
	
	
To introduce $\tilde \Psi_-$ and $\tilde \Psi_+$, we let ${\cal Q}_m \in \mathbb{R}^{d_z \times d_z}$ be a non-random orthogonal matrix $({\cal Q}_m{\cal Q}_m'={\cal Q}_m'{\cal Q}_m=I_{d_z})$ such that ${\cal Q}_m \mu_m = \norm{\mu_m} \boldsymbol e_1$. With these matrices in hand, we define $\tilde \Psi_- = \tilde \mu_\kappa - \tilde \mu_{3-\kappa}$ and $\tilde \Psi_+ = \tilde \mu_1 + \tilde \mu_2$ where
\begin{align}
		\begin{pmatrix}
			\tilde \mu_1 \\ \tilde \mu_2
		\end{pmatrix} = 
		\left(\frac{1}{{\tau_-}} + \frac{1}{{\tau_+}}\right)\! \begin{pmatrix} \sqrt{n} {\cal Q}_1\hat W^{1/2} \hat g_1    \\	 	-\sqrt{n} {\cal Q}_2\hat W^{1/2}  \hat g_2		\end{pmatrix}
		+
		\left(\frac{1}{{\tau_-}} - \frac{1}{{\tau_+}}\right)\!\begin{pmatrix}	-\sqrt{n} {\cal Q}_1\hat W^{1/2}  \hat g_2  \\ 		\sqrt{n} {\cal Q}_2\hat W^{1/2}  \hat g_1 		\end{pmatrix}\!.
\end{align}
	
	
The preceding definitions imply that $(\tilde \Psi_-',\tilde \Psi_+')' = \sqrt{n} A (\hat g_1'\hat W^{1/2},\hat g_2'\hat W^{1/2} )'$ for a particular non-random matrix $A \in \mathbb{R}^{2d_z \times 2d_z}$ with $\sqrt{n} A ( g_1' W^{1/2}, g_2' W^{1/2} )' = (\mu_-\boldsymbol e_1',\mu_+\boldsymbol e_1')'$. Since $\mu_-$ and $\mu_+$ do not depend on $n$, it therefore follows from Lemma \ref{lem:asymp norm}, part $(i)$, that $(\tilde \Psi_-',\tilde \Psi_+')' \xrightarrow{d} (\Psi_-',  \Psi_+')'$ provided that $AV^\text{RV}A' = {\tiny \begin{bmatrix} 1 & \rho \\ \rho & 1 \end{bmatrix} }\otimes I_{d_z}$ where $\rho$ is the correlation between $e_{\kappa i}-e_{3-\kappa, i}$ and $e_{1i}+e_{2i}$. To see why this convergence occurs, note first that weak instruments for testing (Assumption \ref{as:wkinstr}) implies that $g_m = O(n^{-1/2})$ for $m=1,2$, which in turn yields that the second part of $\psi_{mi}$ is $O_p(n^{-1/2})$. From Assumption \ref{as:homsked}, we then have
\begin{align}\label{eq:varconv}
		V^\text{RV}_{\ell k} = W^{1/2} E[ e_{\ell i} e_{k i} z_iz_i'] W^{1/2} + O(n^{-1/2}) = \sigma_{\ell k} I_{d_z} + O(n^{-1/2})
\end{align}
where we write $\sigma_{mm}$ for $\sigma_m^2$. Thus, we have that $V^\text{RV} = {\tiny \begin{bmatrix} \sigma_1^2 & \sigma_{12} \\ \sigma_{12} & \sigma_{2}^2 \end{bmatrix} }\otimes I_{d_z} .$ Furthermore, we note that $A$ takes the form
\begin{align}
			A = 
			\begin{bmatrix}	(-1)^{3-\kappa}I & (-1)^\kappa I \\ I & I	\end{bmatrix}
			\begin{bmatrix}	{\cal Q}_1 & 0 \\ 0 & {\cal Q}_2	\end{bmatrix}
			\begin{bmatrix}	I & I \\ I & -I	\end{bmatrix}
			\begin{bmatrix}	I\tau_-^{-1} & 0 \\ 0 & I\tau_+^{-1}	\end{bmatrix}
			\begin{bmatrix}	I & -I \\ I & I	\end{bmatrix}
\end{align}
and leave the verification of $A\big( {\tiny \begin{bmatrix} \sigma_1^2 & \sigma_{12} \\ \sigma_{12} & \sigma_{2}^2 \end{bmatrix} }\otimes I_{d_z} \big)A' = {\tiny \begin{bmatrix} 1 & \rho \\ \rho & 1 \end{bmatrix} }\otimes I_{d_z}$ to the reader.
	
	
\noindent \textbf{Step (2)} Part $(iv)$ is an immediate implication of the triangle inequality and the definitions $\mu_- = \norm{\mu_\kappa} - \norm{\mu_{3-\kappa}}$ and $\mu_+ = \norm{\mu_1} + \norm{\mu_2}$. For part $(ii)$, we have that $\mu_-=0$ if and only if $\norm{\mu_1}^2 - \norm{\mu_2}^2 =0$. In turn, we have that
\begin{align}
		\norm{\mu_1}^2 - \norm{\mu_2}^2 &= n\!\left( \!\left(\tau_-^{-1} + \tau_+^{-1} \right)^2  - \!\left(\tau_-^{-1} - \tau_+^{-1} \right)^2 \right)\! \left( Q_1 - Q_2\right) \\
		&=4n (\tau_+ \tau_-)^{-1} \left( Q_1 - Q_2\right),
\end{align}
from which part $(ii)$ is immediate. For part $(iii)$, we have that $\mu_+=0$ if and only if $\norm{\mu_1}^2 + \norm{\mu_2}^2 =0$. We now have,
\begin{align}
			\norm{\mu_1}^2 \!+\! \norm{\mu_2}^2
			&\!=\! n\!\begin{pmatrix} W^{1/2}g_1  \\ W^{1/2}g_2	\end{pmatrix}'\!
			A'A 
			\!\begin{pmatrix} W^{1/2}g_1  \\ W^{1/2}g_2	\end{pmatrix} \!
			=\! n\!\begin{pmatrix} W^{-1/2}\pi_1  \\ W^{-1/2}\pi_2	\end{pmatrix}'\!
			A'A 
			\!\begin{pmatrix} W^{-1/2}\pi_1  \\ W^{-1/2}\pi_2	\end{pmatrix} \!
\end{align}
so part $(iii)$ follows from the positive definiteness of both $W$ and the matrix $A'A = 4 \!{\tiny \begin{bmatrix} \tau_+^{-2} + \tau_-^{-2} & \tau_+^{-2} - \tau_-^{-2} \\ \tau_+^{-2} - \tau_-^{-2} & \tau_+^{-2} + \tau_-^{-2} \end{bmatrix} }\!\otimes I_{d_z}$.

		
\noindent \textbf{Step (3)} For $T^\text{RV}$ we first consider the numerator. Here, we observe that
\begin{align}
		\tilde \Psi_-' \tilde\Psi_+ = \tilde \mu_\kappa'\tilde \mu_\kappa - \tilde \mu_{3-\kappa}'\tilde \mu_{3-\kappa} = 4n (\tau_+ \tau_-)^{-1} \!\left( \hat Q_\kappa - \hat Q_{3-\kappa}\right)
\end{align}
so that $\sqrt{n}\abs{\hat Q_1-\hat Q_2} = (\tau_+\tau_-/4)\abs{\tilde\Psi_-' \tilde\Psi_+}/\sqrt{n}$. For the denominator, we initially note that Lemma \ref{lem:asymp norm}, part $(ii)$, and Equation \eqref{eq:varconv} yields that
\begin{align}
		(\tau_+ \tau_-/4)^{-2} n \hat \sigma^2_\text{RV} = \tfrac{4^3n}{\tau_+^2\tau_-^2}\!\left[ \sigma_1^2 \hat Q_1 + \sigma_2^2 \hat Q_2 - 2\sigma_{12} \hat g_1' \hat W \hat g_2  \right] + o_p(1).
\end{align}	
Similarly, we can calculate that
\begin{align}
		\norm{\tilde \Psi_-}^2  &+ \norm{\tilde \Psi_+}^2  + 2\rho \tilde \Psi_-'\tilde \Psi_+ 
		= n \begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix}
		'A' \bigg( {\tiny \begin{bmatrix} 1 & \rho \\ \rho & 1 \end{bmatrix} }\otimes  I_{d_z}  \bigg)A
		\begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix}\\
		&= {4^2n}{} \begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix}'
		\bigg( \! \tfrac{4}{\tau_+^2\tau_-^2}{\tiny \begin{bmatrix} \sigma_1^2 \! & \! -\sigma_{12} \\ -\sigma_{12} \! & \! \sigma_2^2 \end{bmatrix}} \!\otimes I_{d_z}  \bigg)
		\begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix} \\
		&= \tfrac{4^3n}{\tau_+^2\tau_-^2}\!\left[ \sigma_1^2 \hat Q_1 + \sigma_2^2 \hat Q_2 - 2\sigma_{12} \hat g_1' \hat W \hat g_2  \right]
\end{align}
where the second equality follows from the last sentences of steps (1) and (2) together with
\begin{align}
		{\tiny \begin{bmatrix} \tau_+^{-2} + \tau_-^{-2} & \tau_+^{-2} - \tau_-^{-2} \\ \tau_+^{-2} - \tau_-^{-2} & \tau_+^{-2} + \tau_-^{-2} \end{bmatrix} \begin{bmatrix} \sigma_1^2 & \sigma_{12} \\ \sigma_{12} & \sigma_{2}^2 \end{bmatrix}  \begin{bmatrix} \tau_+^{-2} + \tau_-^{-2} & \tau_+^{-2} - \tau_-^{-2} \\ \tau_+^{-2} - \tau_-^{-2} & \tau_+^{-2} + \tau_-^{-2} \end{bmatrix} = \begin{bmatrix} \sigma_1^2 & -\sigma_{12} \\ -\sigma_{12} & \sigma_2^2 \end{bmatrix} } \tfrac{4}{\tau_+^2\tau_-^2}.
\end{align}
Thus we have the desired conclusion
		\begin{align}
		\abs{T^\text{RV}} &= \sqrt{n}\frac{\abs{\hat Q_1 - \hat Q_2}}{\hat \sigma_\text{RV}} = \frac{4n (\tau_+ \tau_-)^{-1/2} \!\abs{ \hat Q_1 - \hat Q_2}}{\left( (\tau_+ \tau_-/4^2)\inverse n \hat \sigma^2_\text{RV}  \right)^{1/2}} \\
		&=
		 \abs{\tilde \Psi_-'\tilde \Psi_+}/\big(\norm{\tilde \Psi_-}^2 + \norm{\tilde \Psi_+}^2 + 2\kappa \tilde \Psi_-'\tilde \Psi_+  + o_p(1) \big)^{1/2}
\end{align}
	
	
For $F$, we first note that standard arguments lead to
\begin{align}
		2d_zF &=n(1-\hat \rho^2)\frac{\hat \sigma_2^2 \hat g_1' \hat W \hat g_1 + \hat \sigma_1^2 \hat g_2' \hat W \hat g_2 - 2\hat \sigma_{12} \hat g_1' \hat W \hat g_2}{\hat \sigma_1^2 \hat \sigma_2^2 - \hat \sigma_{12}^2 } \\
		&=n(1-\rho^2)\frac{\sigma_2^2 \hat Q_1 +  \sigma_1^2 \hat Q_2 - 2 \sigma_{12} \hat g_1' \hat W \hat g_2}{ \sigma_1^2  \sigma_2^2 -  \sigma_{12}^2 } + o_p(1).
\end{align}
Similarly, we can calculate that
\begin{align}
		\norm{\tilde \Psi_-}^2  &+ \norm{\tilde \Psi_+}^2  - 2\rho \tilde \Psi_-'\tilde \Psi_+ 
		= n \begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix}'
		A' \bigg( {\tiny \begin{bmatrix} 1 & -\rho \\ -\rho & 1 \end{bmatrix} }\otimes  I_{d_z}   \bigg)A
		\begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix} \\
		&= n(1-\rho^2) \begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix}'
		\bigg(  {\tiny \begin{bmatrix} \sigma_1^2  &  \sigma_{12} \\ \sigma_{12}  &  \sigma_2^2 \end{bmatrix}}\inverse \otimes I_{d_z}  \bigg)
		\begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix} \\
		&= n(1-\rho^2)\frac{\sigma_2^2 \hat Q_1 +  \sigma_1^2 \hat Q_2 - 2 \sigma_{12} \hat g_1' \hat W \hat g_2}{ \sigma_1^2  \sigma_2^2 -  \sigma_{12}^2 }
\end{align}
which follows from inverting the equality in the last sentence of step (1).
\end{proof}

==> Submission/QE/Proofs/Pf_plims_cost.tex <==
\begin{proof}[Proof of Lemma \ref{cor:cost_misc}.] 
Since $\textbf{w}_\textbf{a}$ is a subset of $\textbf{w}$, the proof follows immediately by replacing any variable $y$ residualized with respect to $\textbf{w}$ in the Proof of Lemma \ref{cor:modelmisc}, with $y^\textbf{a}$ which has been residualized with respect to $\textbf{w}_\textbf{a}$.
%
\begin{comment}
For $\textbf{w}_\textbf{a}\neq \textbf{w}$, by Equation \eqref{eq:cost_mispec2}, $p_i =  \Delta^\textbf{a}_{0i} + \omega_{0i}$, where $p_i = \boldsymbol{p}_m-\textbf{w}_{\textbf{a}}E[\textbf{w}_{\textbf{a}}'\textbf{w}_{\textbf{a}}]^{-1}E[\textbf{w}_{\textbf{a}}'\boldsymbol{p}_m]$ and $\Delta^a_m = \boldsymbol{\Delta}^{\textbf{a}}_m-\textbf{w}_{\textbf{a}}E[\textbf{w}_{\textbf{a}}'\textbf{w}_{\textbf{a}}]^{-1}E[\textbf{w}_{\textbf{a}}'\boldsymbol{\Delta}^{\textbf{a}}_m]$.  Define $\Delta^{\textbf{a}z}_{0i} = z_iE[z_iz_i']E[z_i\Delta^{\textbf{a}z}_{0i}]$.  Further, define $\Delta_m = \boldsymbol{\Delta}_m-\textbf{w}_{\textbf{a}}E[\textbf{w}_{\textbf{a}}'\textbf{w}_{\textbf{a}}]^{-1}E[\textbf{w}_{\textbf{a}}'\boldsymbol{\Delta}_m]$ and $\Delta^{z}_{mi} = z_iE[z_iz_i']E[z_i\Delta^{z}_{mi}]$.  Let $z = \boldsymbol{z}-\textbf{w}_{\textbf{a}}E[\textbf{w}_{\textbf{a}}'\textbf{w}_{\textbf{a}}]^{-1}E[\textbf{w}_{\textbf{a}}'\boldsymbol{z}]$. By Equation \eqref{eq:omega_costmisc} and under Assumption \ref{as:misspmc}, the right hand side of \eqref{eq:line4} can be rewritten as
$$E[z_i(\Delta^\textbf{a}_{0i}-\Delta_{mi})]'E[z_iz_i']^{-1}E[z_i(\Delta^\textbf{a}_{0i}-\Delta_{mi})].$$  Thus, replacing $\Delta^z_{0i}$ with $\Delta^{\textbf{a}z}_{0i}$ the equality between \eqref{eq:line1} and \eqref{eq:line4} holds as does the equality between \eqref{eq:line4} and \eqref{eq:line5}. 

\begin{itemize}
\item[(i)]  Under Assumption \ref{as:misspmc} and by the equality of \eqref{eq:line1}, \eqref{eq:line5}, and the positive definiteness of $E[z_iz_i']$, $\pi_m = 0$ iff $E[(\Delta^{\textbf{a}z}_{0i}-\Delta^{\textbf{a}z}_{mi})^2]=0$.  The proof then follows from the Proof of Lemma 2 (i). 
    \item[(ii)]  Under Assumption \ref{as:misspmc} and by the equality of \eqref{eq:line1}, \eqref{eq:line5}, and the positive definiteness of $E[z_iz_i']$, $Q_1=Q_2$ iff $E[(\Delta^{\textbf{a}z}_{0i}-\Delta^{z}_{1i})^2]=E[(\Delta^{\textbf{a}z}_{0i}-\Delta^{z}_{2i})^2]$ The proof then follows from the Proof of Lemma 2 (ii). 
\end{itemize}
\end{comment}
\end{proof}

==> Submission/QE/Tables/AR_results.tex <==
%\renewcommand{\arraystretch}{1.2}
\begin{widetable}{.98\columnwidth}{lccc}
\toprule
\textbf{NoProd IVs} & 2 & 3 & 4  \\
\cmidrule(lr){2-4}
1. Zero wholesale margin&315.34, 575.29&315.34, 398.27&315.34, 396.08\\
2. Zero retail margin &&575.29, 398.27&575.29, 396.08\\
3. Linear pricing&&&398.27, 396.08\\
4. Hybrid model&&&\\
\bottomrule
\end{widetable}




==> Submission/QE/Tables/CombinedInstr.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{comment}
\begin{widetable}{.98\columnwidth}{lrrrc}
\toprule
\multicolumn{1}{l}{\textbf{Panel A: BLP95 + Diff + Cost + Demo} ($d_z=8$) } \\
& \multicolumn{3}{c}{$F_\rho$}& MCS $p$-values\\
\multicolumn{1}{l}{Models}&\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}&\\
\cmidrule(lr){2-5}
1. Zero wholesale margin&106.7&50.0&49.7&0.17 \\
2. Zero retail margin&&61.4&61.3&1.00 \\
3. Linear pricing&&&60.0&0.00 \\
4. Hybrid model&&&&0.00 \\
\midrule
\multicolumn{5}{l}{\textbf{Panel B: No PCA BLP95 + No PCA Diff + Cost + Demo } ($d_z=22$) }\\
& \multicolumn{3}{c}{$F_\rho$}& MCS $p$-values\\
\multicolumn{1}{l}{Models}&\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}&\\
\cmidrule(lr){2-5}
1. Zero wholesale margin&77.6&28.3&28.3&1.00 \\
2. Zero retail margin&&37.2&37.3&0.57 \\
3. Linear pricing&&&31.7&0.00 \\
4. Hybrid model&&&&0.00 \\
\bottomrule
\end{widetable}


\begin{widetable}{.98\columnwidth}{lrrrc}
\toprule
& \multicolumn{3}{c}{$F$-statistics} & MCS $p$-values \\
\cmidrule(lr){2-4}  \cmidrule(lr){5-5}
\multicolumn{1}{l}{Models} & 2 & 3 & 4 & \\
\midrule
\multicolumn{1}{l}{\textbf{Panel A: BLP95 + Demo + Cost + Diff} ($d_z=11$) } \\
1. Zero wholesale margin&106.7&50.0&49.7&0.17 \\
2. Zero retail margin&&61.4&61.3&1.00 \\
3. Linear pricing&&&60.0&0.00 \\
4. Hybrid model&&&&0.00 \\
\cmidrule(lr){1-5}
\multicolumn{5}{l}{\textbf{Panel B: No PCA BLP95 + Demo + Cost + No PCA Diff } ($d_z=22$) }\\
1. Zero wholesale margin&77.6&28.3&28.3&1.00 \\
2. Zero retail margin&&37.2&37.3&0.57 \\
3. Linear pricing&&&31.7&0.00 \\
4. Hybrid model&&&&0.00 \\
\bottomrule
\end{widetable}
\end{comment}

\begin{widetable}{.98\columnwidth}{lrrrrrrc}
\toprule
& \multicolumn{3}{c}{$T^\text{RV}$}& \multicolumn{3}{c}{$F$-statistics}&  MCS $p$-values\\
\cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-8}  
Models & 2 & 3 &  4 & 2 & 3 & 4 & \\ 
\midrule
\multicolumn{8}{l}{\textbf{IVs: No. Products + Demo + Cost + Diff} ($d_z=11$)}  \\ 
1. Zero wholesale margin&1.664&  -8.827&  -8.838&105.3 &   {70.7}   &  {70.8}&0.096 \\
2. Zero retail margin&&-5.655 & -5.653&&{85.6}  &   {86.2} &1.0      \\
3. Linear pricing&&&-1.781&&&{101.1}&0.00 \\
4. Hybrid model&&&&&&&0.00 \\
%\cmidrule(lr){1-8}
%\multicolumn{8}{l}{\textbf{Panel B: No. Products + Demo + Cost + Diff} (no PCA, $d_z=14$)}  \\ 
%\multicolumn{8}{c}{\textbf{Panel B: No PCA BLP95 + Demo + Cost + No PCA Diff } ($d_z=22$)}\\
%1. Zero wholesale margin&1.662 & -8.858 & -8.869&$\underset{***\wedge\wedge\wedge}{100.2}$  &  $\underset{***\wedge\wedge\wedge}{63.0}$ &    $\underset{***\wedge\wedge\wedge}{63.1}$&0.097 \\
%2. Zero retail margin&&-5.659 & -5.657&&$\underset{***\wedge\wedge\wedge}{76.8}$   &  $\underset{***\wedge\wedge\wedge}{77.3}$&1.0 \\
%3. Linear pricing&&&-1.795&&&$\underset{***\wedge\wedge\wedge}{89.2}$&0.00 \\
%4. Hybrid model&&&&&&&0.00 \\
\bottomrule
\end{widetable}


==> Submission/QE/Tables/CoxEB.tex <==
\begin{widetable}{.98\columnwidth}{lccc}
\toprule
\textbf{Cox Test} & 2 & 3 & 4  \\
\cmidrule(lr){2-4}
1. Zero wholesale margin&-4.72, 3.99&4.34, -6.53&4.35, -6.55\\
2. Zero retail margin &&9.47, -12.42&9.47, -12.46\\
3. Linear pricing&&&0.01, -0.01\\
4. Hybrid model&&&\\
\midrule
\textbf{EB Test} & 2 & 3 & 4  \\
\cmidrule(lr){2-4}
1. Zero wholesale margin&253.16, 319.1&253.16, 338.14&253.16, 337.97\\
2. Zero retail margin &&319.1, 338.14&319.1, 337.97\\
3. Linear pricing&&&338.14, 337.97\\
4. Hybrid model&&&\\
\bottomrule
\end{widetable}

==> Submission/QE/Tables/F_critical_values.tex <==

%\newcolumntype{d}[1]{D{.}{.}{#1}}
%\renewcommand{\arraystretch}{1.05}
\begin{widetable}{.98\columnwidth}{lS r *{3}{S} r *{3}{S}}
\toprule
&&& \multicolumn{3}{c}{\textbf{Panel A:} Critical Values, ${cv^s}$} &&  \multicolumn{3}{c}{\textbf{Panel B:} Critical Values, ${cv^p}$}\\ 
\cmidrule(lr){4-10}
&&& \multicolumn{3}{c}{Worst-Case Size, $r^s$} &&  \multicolumn{3}{c}{Best-Case Power, $r^p$}\\ 
\cmidrule(lr){4-6} \cmidrule(lr){8-10} 
$\rho^2$ & \mc{$d_z$} && \mc{0.075} & \mc{0.10} &  \mc{0.125} & & \mc{0.95} & \mc{0.75} & \mc{0.50} \\
\midrule
%\multicolumn{9}{c}{$\rho^2 = 0.25$}\\
%\cmidrule(lr){1-9}
\multirow{8}{*}{$0.25$} 
& 1 && 0 & 0 & 0 && 20.5 & 15.5 & 12.4 \\
&2&&0&0&0&&10.7&8.1&6.6\\
&3&&0&0&0&&7.4&5.7&4.6\\
&4&&0&0&0&&5.7&4.4&3.7\\
&5&&0&0&0&&4.8&3.7&3.1\\
%6&0&0&0&&4.1&3.2&2.7\\
%7&0&0&0&&3.6&2.8&2.4\\
%8&0&0&0&&3.3&2.6&2.2\\
%9&0&0&0&&3&2.4&2\\
&10&&0&0&0&&2.8&2.2&1.9\\
%11&0&0&0&&2.6&2.1&1.8\\
%12&0&0&0&&2.4&2&1.7\\
%13&0&0&0&&2.3&1.9&1.6\\
%14&0&0&0&&2.2&1.8&1.5\\
%15&0&0&0&&2.1&1.7&1.5\\
&20&&4.3&2.0&1.1&&1.7&1.4&1.3\\
%25&7.3&3.7&2.4&&1.5&1.3&1.1\\
&30&&10.3&5.2&3.5&&1.4&1.2&1.1\\
\midrule
%\multicolumn{9}{c}{$\rho^2 = 0.75$}\\
%\cmidrule(lr){1-9}
\multirow{8}{*}{$0.75$} 
&1&&26.7&12.6&0&&6.5&4.9&3.9\\
&2&&0&0&0&&3.3&2.5&2.0\\
&3&&0&0&0&&2.2&1.7&1.4\\
&4&&0&0&0&&1.7&1.3&1.1\\
&5&&0&0&0&&1.4&1.1&0.9\\
&10&&0.8&0&0&&0.8&0.6&0.5\\
&20&&17.1&8.3&5.4&&0.4&0.4&0\\
&30&&34.4&17.0&11.3&&0.3&0&0\\
\bottomrule
\end{widetable}

==> Submission/QE/Tables/RV_accumul1.tex <==
\begin{widetable}{.98\columnwidth}{lrrrrrrc}
\toprule
& \multicolumn{3}{c}{$T^\text{RV}$}& \multicolumn{3}{c}{$F$-statistics}&  MCS $p$-values\\
\cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-8}  
Models & 2 & 3 &  4 & 2 & 3 & 4 & \\ 
\midrule
\textbf{Panel A: NoProd IVs} $(d_z = 2)$ \\ 
1. Zero wholesale margin& 4.33&$-$8.54& $-$8.56&143.9&126.2&126.8&0.00\\
2. Zero retail margin&&$-$7.35&$-$7.36&&100.2&100.8&{1.00}\\
3. Linear pricing&&&$-$3.10&&&204.9&0.00\\
4. Hybrid model&&&&&&&0.00\\
\cmidrule(lr){1-8}
\textbf{Panel B: Demo IVs} $(d_z = 3)$ \\
1. Zero wholesale margin& 2.42&$-$6.38& $-$6.41&30.7&52.4&53.1&0.02\\
2. Zero retail margin&&$-$5.36&$-$5.41&&37.8&38.1&{1.00}\\
3. Linear pricing&&&0.38&&&47.5&0.00\\
4. Hybrid model&&&&&&&0.00\\
\cmidrule(lr){1-8}
\textbf{Panel C: Cost IVs} $(d_z = 1)$\\
1. Zero wholesale margin& $-$1.99&$-$1.51& $-$1.80&106.8&6.0$^\dagger$&7.1$^\dagger$&{1.00}\\
2. Zero retail margin&&1.83&1.77&&86.7&87.7&{0.10}\\
3. Linear pricing&&&$-$2.97&&&91.7&{0.13}\\
4. Hybrid model&&&&&&&0.01\\
\cmidrule(lr){1-8}
\textbf{Panel D: Diff IVs} $(d_z = 5)$ \\
1. Zero wholesale margin& 0.81&0.52&0.51&6.2$^\dagger$&3.3$^\dagger$&3.3$^\dagger$&{0.67}\\
2. Zero retail margin&&0.37&0.36&&2.9$^\dagger$&2.9$^\dagger$&{0.71}\\
3. Linear pricing&&&$-$1.18&&&1.8$^\dagger$&{1.00}\\
4. Hybrid model&&&&&&&{0.56}\\
\midrule
\midrule
\textbf{Aggregating Evidence:} &\multicolumn{7}{c}{ $\boldsymbol{M^* = \{2\}}$}\\
\multicolumn{8}{c}{Step 0: $M^*_A = \{2\}$,  $M^*_B = \{2\}$, $M^*_C = \{1,2,3\}$, $ M^*_D = \{1,2,3,4\}$ \hfill Step 1: No conflicting evidence}\\
\multicolumn{8}{l}{Step 2:  Smallest MCS is $M^*_A= \{2\}$, no additional models supported by strong instruments}\\
%&\multicolumn{7}{c}{No Conflicting Evidence$\qquad$ $M^* = \{2\}$}\\
%Conflicting Evidence: \multicolumn{7}{c}{No}\\
%$M^*$: \multicolumn{7}{c}{$\{2\}$}\\
\bottomrule
\end{widetable}


==> Submission/QE/Tables/demand_models.tex <==
\begin{widetable}{.98\columnwidth}{lrrrrrr}
\toprule
& \multicolumn{2}{c}{(1) Logit-OLS}  & \multicolumn{2}{c}{(2) Logit-2SLS}  & \multicolumn{2}{c}{(3) BLP}   \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
& coef. & \multicolumn{1}{c}{s.e.}
& coef. & \multicolumn{1}{c}{s.e.}
& coef. & \multicolumn{1}{c}{s.e.}    \\
\midrule
 Prices         &    $-1.750$ &   (0.019)    &    $-6.519$  &   (0.209)    &  $-12.001$  & (0.777)\\
 Size           &    0.037 &    (0.001)   &    0.018 &   (0.001)    &  $-0.060$  & (0.013) \\
 Light          &    0.259  &   (0.010)  &    0.413 &   (0.014)    &  $-0.270$  & (0.144) \\
 Plain   &    0.508 &   (0.007)   &    0.423  &   (0.009)   &  0.439 & (0.012) \\
 log(\#Flavors)   &    1.127  &   (0.004)  &    1.106 &   (0.005)    &  1.135    & (0.007) \\
 Income $\times$ price &      &       &        &      &  4.333   & (0.378)\\
 Income $\times$ light &     &        &        &      &  0.215  & (0.069)\\
Age $\times$ light    &      &       &      &        & $-0.565$  & (0.113)  \\
 Age $\times$ size     &    &         &   &           & $-0.067$& (0.008)  \\
\midrule 
 Own price elasticity-mean       & \multicolumn{2}{c}{-1.32}  & \multicolumn{2}{c}{-4.917} & \multicolumn{2}{c}{-6.306} \\
 Own price elasticity-median     & \multicolumn{2}{c}{-1.177} & \multicolumn{2}{c}{-4.384} & \multicolumn{2}{c}{-6.187} \\
 Diversion outside option-mean   &  \multicolumn{2}{c}{0.72}  &  \multicolumn{2}{c}{0.72}  &  \multicolumn{2}{c}{0.39}  \\
 Diversion outside option-median &  \multicolumn{2}{c}{0.71}  &  \multicolumn{2}{c}{0.71}  &  \multicolumn{2}{c}{0.38}  \\
\bottomrule
\end{widetable}


==> Submission/QE/Tables/summary_stat.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Mar 12, 2021 - 03:58:35 PM
%\renewcommand{\arraystretch}{1.05}
\begin{widetable}{.98\columnwidth}{lrrrrr} 
\toprule
Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Median}  & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Pctl(75)} \\ 
\midrule
Price (\$) & 0.76 & 0.30 & 0.68 &  0.55 & 0.91 \\ 
Sales (6 oz. units) & 1,461 & 3,199 & 503  & 213 & 1,301 \\ 
Shares & 0.007 & 0.012 & 0.003 & 0.001 & 0.007 \\ 
Outside Share & 0.710 & 0.111 & 0.708 & 0.631 & 0.788 \\ 
Size (oz.) & 17.82 & 10.57 & 16  & 6 & 32 \\ 
Frac. Light & 0.93 & 0.26 & 1 &  1 & 1 \\ 
Number Flavors & 5.39 & 5.81 & 3  & 1 & 8 \\ 
Frac. Private Label & 0.09 & 0.28 & 0  & 0 & 0 \\ 
Distance to Plant (mi.) & 493 & 477 & 392  & 199 & 546 \\ 
Freight Cost (\$) & 212 & 242 & 164  & 52 & 271 \\ 
\bottomrule
\end{widetable} 


==> Submission/ReStud/Appendices/AltCost.tex <==
In this appendix we discuss how the results of the paper are preserved in a more general setting where marginal cost depends on quantity sold. While in the paper, we derive results assuming constant marginal cost, this is an important extension. It is well known going back to \citeA{b82} and \citeA{l82} that the requirements for testing conduct are greater when marginal cost is non-constant.  Thus, the reader may wonder if the results of our paper would be qualitatively different in a more general setting.


Let $\boldsymbol{q}_i$ denote quantity, and consider a separable cost function:
\begin{align}
    \boldsymbol{c}_i = \bar{\boldsymbol{c}}(\boldsymbol{q}_i,\textbf{w}_i;\tau) + \omega_i,
\end{align}
where $\bar c$ is specified up to some cost parameters $\tau$.  The specification of marginal cost that we adopt in the paper is a special case where $\bar{\boldsymbol{c}}(\boldsymbol{q}_i,\textbf{w}_i;\tau) = \textbf{w}_i \tau$.


There are two additional cases to consider. The first concerns the researcher knowing the true value of $\tau$. We can define $\bar{\boldsymbol{\Delta}}_{mi} = \boldsymbol{\Delta}_{mi} + \bar{\boldsymbol{c}}(\boldsymbol{q}_i,\textbf{w}_i;\tau)$: this term is pinned down by a model of conduct $m$, and a cost function $\bar{\boldsymbol{c}}$. In this case, we can test alternative pairs of models of conduct and cost functions with the methods described in the paper. In particular, that can be done by replacing ${{\Delta}}_{m}$ in the paper with $\bar{\boldsymbol{\Delta}}_{m}$. The set of instruments $\boldsymbol{z}$ must include $\textbf{w}$ in this case, but since $\bar{\boldsymbol{c}}$ is fully specified, there is no additional requirement on instruments. 

Alternatively, when $\tau$ is unknown to the researcher, she can estimate it under a model of conduct $m$ either as a preliminary step, or simultaneously with testing, as she would in the case of constant marginal cost. However, excluded instruments that rotate residual marginal revenue are now needed to estimate $\tau$, and thus must be sufficient to identify $\tau$ under the true model of conduct. If a researcher pursues a sequential approach, the researcher can construct $\bar{\boldsymbol{\Delta}}_{mi} = \boldsymbol{\Delta}_{mi} + \bar{\boldsymbol{c}}(\boldsymbol{q}_i,\textbf{w}_i;{\tau}_m)$ and perform testing after having estimated ${\tau}_m$ under each model. 

The results in the paper are still applicable as long as the researcher adjusts the standard errors of the RV test statistic and the effective $F$-statistic. As there may exist models, falsified by a set of instruments under constant marginal cost which are not falsified by those same instruments with a more flexible marginal cost specification, degeneracy is more likely to occur when cost is non-constant. This is akin to the classic example of demand shifters in \cite{b82}.  Thus, evaluating the quality of the inference on conduct using our diagnostic is even more necessary in this setting.    

This discussion makes it explicit that testing firm conduct also jointly tests models of marginal cost. In fact,  $\bar{\boldsymbol{\Delta}}_{m} $ generalizes the term $\Breve{\boldsymbol{\Delta}}_{m}$ defined in Section \ref{sec:globalmis}. In that section we show that cost misspecification can be incorporated in  $\Breve{\boldsymbol{\Delta}}_{m}$, and thus be understood as markup misspecification. Here, misspecification of $\bar c$ is manifested as misspecification of  $\bar{\boldsymbol{\Delta}}_{m} $. If one is flexible in specifying $\bar c$, misspecification of $\bar{\boldsymbol{\Delta}}_{m} $ largely concerns misspecification of ${\boldsymbol{\Delta}}_{m} $, and therefore conduct. Finally, this formulation shows that the methods described in the paper can be used to test models of cost, even when conduct is known.\looseness=-1




==> Submission/ReStud/Appendices/Emipirical.tex <==
\subsection{Data}\label{sec:data}

Our main source of data is the IRI Academic Dataset (see \cite{bkm08} for a description).  This dataset contains weekly price and quantity data for upcs sold in a sample of stores in the United States.  While this is the same data source as in \cite{v07}, it is not the same dataset as it covers a later time period and significantly more geographic markets.  Thus, our aim is not to replicate her findings; instead we seek to use this important empirical setting to illustrate our approach to testing. In cleaning the data, we try to mimic her choices as closely as possible.

Our data is for the year of 2010.\footnote{We choose to use only one year because the IRI dataset does not provide cross-reference for supermarket chains' identity across years and for computational reasons.} We define a market as a retail store-quarter.  We drop data coming from two geographic markets (``EAU CLAIRE'' and ``PITTSFIELD'') for which IRI does not provide geographical location information. We approximate the market size with a measure of the traffic in each store,  derived from the store-level revenue information from IRI. For approximately 5\% of stores, this approximation is poor resulting in an outside share below 50\%.  We drop these from our sample.  

In defining a product, we restrict attention to upcs labelled as ``yogurt'' in the IRI data and focus on the most commonly purchased sizes: 6, 16, 24 and 32oz.\footnote{For example, we drop products labelled ``soy yogurt'' and ``goat yogurt''}  Similar to \cite{v07}, we define a product as a brand-fat content-flavor-size, where flavor takes the value ``Plain'' or ``Other'' and fat content is either light (less than 4.5\% fat content) or whole.\footnote{Given that we lack detailed information for private label products,  we do not add other nutritional information.}  We further standardize package sizes to 6oz serving sizes.

Based on market shares, we exclude niche firms and products from the analysis. In particular, any firm which have less than a 5\% inside share  in all markets is dropped. We also drop products from a market which have an inside share lower than 0.1\% in that market and for which their cumulative inside share is not bigger than 1\%. After cleaning, our dataset has  205,123 observations for 5,034 markets corresponding to  1,309 stores.

We supplement our main dataset with county level demographics obtained from the Census Bureau's PUMS database which we match to the DMAs in the IRI data.  In particular, we draw 1000 households and record household income and age of the head of the household. We exclude households with income lower than \$12k or bigger than \$1 million. The demographic variables are adjusted to reflect their deviation from the mean.

We also measure transportation costs from manufacturer to retailer using average fuel cost times distance.  To do so, we use data on average regional on-highway diesel prices in dollars per gallon by quarter from the US Energy Information Administration.\footnote{https://www.eia.gov/dnav/pet/pet\_pri\_gnd\_dcus\_nus\_w.htm} Manufacturer plant locations were collected by hand.\footnote{We thank Xinrong Zhu for generously sharing this data with us.}
 
 Table \ref{Tab:summarystats} contains summary statistics for the main variables of interest in the paper.  
\begin{table}[!h]\footnotesize\caption{Summary Statistics}\label{Tab:summarystats}\centering
\input{Empirical/Tables/summary_stat}
%\input{Tables/summary_stat_count}
\end{table}    

\subsection{Demand Model, Identification, and Estimation}

\noindent \textbf{Demand Model:}
We begin by describing our model of demand which follows a standard framework from  \cite{blp95}, as in \cite{v07}.  Each consumer $i$ receives utility from purchasing product $j$ in market $t$ according to the following utility index:
\begin{align}\label{eq:utility}
    u_{ijt} = \beta_i x_j + \alpha_i p_{jt} + \xi_{t} + \xi_{s} + \xi_{b(j)} + \xi_{jt} + \epsilon_{ijt} 
\end{align}
where $x_j$ includes a set of product characteristics: package size and dummy variables for whether the yogurt is low fat and for whether it is plain flavored. We also include the log of the number of flavors offered in the market, following \cite{ar05}. $p_{jt}$ represents the price charged for product $j$ in market $t$.   
All specifications have fixed effects for quarter, store and brand producing product $j$, denoted $\xi_{t}$, $\xi_{s}$, and $\xi_{b(j)}$ respectively.  $\xi_{jt}$ and $\epsilon_{ijt}$ denotes unobservable shocks at the product-market and the individual product market level, respectively.  Finally, we allow consumer preferences for characteristics $\beta_i$ and price $\alpha_i$ to vary across individuals. As in \cite{v07}, we do so by interacting their mean with individual level demographics for income and age of the head of household so that
\begin{align}
    \alpha_i &= \bar\alpha + \tilde\alpha\times D_i\\
    \beta_i &= \bar\beta + \tilde\beta\times D_i
\end{align}    
where $\bar\alpha$ and $\bar\beta$ represent the mean taste across consumers and $D_i$ denotes demographics.


To close the model of demand, we make additional assumptions which are standard in the literature.  In particular, we normalize the utility consumer $i$ receives from consuming the outside option as $u_{i0t} = \epsilon_{i0t}$.  The idiosyncratic errors $\epsilon_{jt}$ and $\epsilon_{i0t}$ are assumed to be distributed i.i.d. Type I extreme value. Under the assumption that each consumer purchases one unit of the good that gives her the highest utility, including the outside good, the market share of product $j$ in market $t$ takes the following form:      
\begin{equation}\label{eq:shares}
s_{jt} = \int \frac{\exp({\beta_{i}x_{j}  + \alpha_i p_{jt} +\xi_{t} + \xi_{s} + \xi_{b(j)}  + \xi_{jt}})}{1 +\sum_{l\in{\mathcal{J}_{t}}} \exp({\beta_{i}x_{l}  + \alpha_i p_{lt} +\xi_{t} + \xi_{s} + \xi_{b(l)}  + \xi_{lt}})}f(\alpha_i,\beta_i) \text{d}\alpha_i\text{d}\beta_i
\end{equation}

\noindent \textbf{Identification and Estimation:}   Demand estimation and testing can either be performed \textit{sequentially}, in which demand estimation is a preliminary step, or \textit{simultaneously} by stacking the demand and supply moments.  Following \cite{v07}, we adopt a sequential approach.  For the purposes of illustrating the empirical relevance of the findings in Sections 4 and 5, the computationally simpler simultaneous approach is sufficient.  We estimate demand following the approach developed in \cite{blp95}.  Including brand, store, and quarter fixed effects in (\ref{eq:utility}) controls for all unobservables that are constant either within a brand, a store, or a quarter. Thus, the source of endogeneity which threatens identification is limited to the set of unobservables that vary across these dimensions, denoted as $\xi_{jt}$.  
As prices and shares may be correlated with  $\xi_{jt}$, instruments are then required to identify the coefficient on price $\alpha_i$ and parameters for the individual specific components of utility, $\tilde\alpha$ and $\tilde\beta$, as these latter parameters enter the model non-linearly.    

We use a standard set of instruments.  For each brand in each market, we interact the average highway fuel cost for the region of the country where that market is located with the distance from the store to the brand's nearest manufacturing plant.  As we lack information on plant location for some products, including private labels, we interact the unobserved vector of fuel costs for all observations with a dummy indicating that plant location is observed.  This cost shifter provides exogenous variation to identify the coefficient on price, $\alpha$. 

The non-linear parameters are identified using instrumental variables proposed in \cite{gh19}.  For the nonlinear price parameters on demographics $\tilde\alpha$, we interact the fuel cost instrument with the mean of the demographics for the DMA in which the market is located. For $\tilde\beta$, we interact the observed characteristics with the mean of the demographics for the DMA in which the market is located.  Under the timing assumptions of the model, \cite{gh19} demonstrate that this interaction provides exogenous cross-sectional variation to identify the parameters of interest.  

Estimation proceeds via GMM.     For each guess of the non-linear parameters, we employ the contraction presented in \cite{blp95} to recover the mean utility of each product in each market.  We then regress the mean utilities on price and a set of dummy variables for the fixed effects via two-stage least squares and recover the unobserved product market unobservables as residuals.  We then interact these residuals with the instruments to form the sample moments which enter the GMM objective function. The GMM procedure recovers estimates of the nonlinear parameters, $\tilde\alpha$ and $\tilde\beta$, as well as the price coefficient, $\alpha$, and the fixed effects.  We compute demand estimates using the PyBLP package developed in \cite{cg19}.\footnote{We refer to PyBLP documentation website https://pyblp.readthedocs.io/en/stable/index.html# for detailed information of the methods used.}.


\noindent \textbf{Results:} Results for demand estimation are reported in Table \ref{Tab:demand}.  As a reference, we report estimates of a standard logit model of demand in Columns 1 and 2.  In Column 1, the logit model is estimated via OLS while in Column 2, we use fuel cost as an instrument for price and estimate the model via 2SLS.  We see a large reduction in the price coefficient, indicative of endogenity not controlled for by the fixed effects.  Columns 3 and 4 report estimates of the full demand model.  Our full demand model generates reasonable elasticities which are comparable to those obtained in \cite{v07} who finds a mean own price elasticity of -5.64.      

\begin{table}[H]\footnotesize
\caption{Demand Estimates}\centering
    \input{Tables/demand_models}\label{Tab:demand}
\end{table}
 \begin{tablenotes}
 \item[] \footnotesize{In the table, we report demand estimates for a logit model of demand obtained from OLS estimation in column 1 and 2SLS  estimation in column 2. Column 3 corresponds to the full BLP model. All specifications have fixed effects for quarter, store and brand and are estimated with 205,123 observations.} 
\end{tablenotes}


%\begin{table}[!h]\footnotesize
%    \centering\caption{Markups Summary Stat}
%    \input{MarkupDescTable}
%\end{table}

%\begin{figure}[!h]
%    \centering\caption{Markups Distribution}
%    \subfloat[IV1]{\includegraphics[scale=0.5]{MarkupFig1.png}}
%    \subfloat[Mixed 2]{\includegraphics[scale=0.5]{MarkupFig2.png}}
    
%    \label{fig:my_label}
%\end{figure}

==> Submission/ReStud/Appendices/MCS.tex <==
%This Appendix details our construction of the model confidence set (MCS) $M^*$ for a given set of instruments. Suppose the set of models is $M=\{1,\dots,M_0\}$. Let $K = {M_0 \choose 2}$ denote the total number of unique pairwise model comparisons and let $T^\text{RV}(T^\text{RV}_1,\dots,T_K^\text{RV})$

In this appendix, we provide further details on the construction of the model confidence set.  The construction is iterative where in each step a $p$-value for a model of worst fit is computed.  For a set of instruments $z_\ell$, the MCS $M^*_\ell$ is the collection of models with a $p$-value above the significance level.

For a researcher testing a set of candidate models $M$, we now describe the construction of the MCS $p$-values at each step of the algorithm.  
At iteration $k$, there are $M_k\subset M$ models under current consideration.  Denoting $\abs{M_k}$ as the cardinality of $M_k$, this results in $K = {\abs{M_k}\choose 2}$ distinct pairs of models and therefore RV test statistics. To make notation compact, we define $\Pi$ as a one-to-one mapping from unique model pairs to $\{1,\hdots,K\}$, and let $T^\text{RV}_{\Pi(m_1,m_2)}=  {\sqrt{n}(\hat{Q}_{m_1}-\hat{Q}_{m_2})}/{\hat\sigma_{\text{RV},\Pi(m_1,m_2)}}$.  In this iteration, we find the pair of models $(m_1,m_2)$ associated with the largest test statistic in magnitude, denoted $\bar{T}^\text{RV}$.  If $\bar{T}^\text{RV}$ is positive (negative), then $m_1$ ($m_2$) is the model of worst fit for which we compute the MCS $p$-value.  This model will be dropped from $M_{k+1}$ in the next iteration.

For computation of the MCS $p$-values, we utilize that $    \big(T^\text{RV}_1,\hdots,T^\text{RV}_K \big)'$ is asymptotically normal with zero mean and a variance $\Sigma$ under no degeneracy and a null of equal fit.  This observation follows by extending Lemma \ref{lem:asymp norm} to $\abs{M_k}$ models and alluding to a first order Taylor approximation as in Remark \ref{rem:validity}.  We estimate $\Sigma$ using $\hat\Sigma$.  The diagonal entries of $\hat\Sigma$ are all one.  For any off-diagonal element $\hat\Sigma_{ij}$ with $(i,j) = (\Pi(m_1,m_2),\Pi(m_3,m_4)) $ we have:\looseness=-1
\begin{align}
    \hat\Sigma_{ij} = 4\hat\sigma^{-1}_{\text{RV},i}\hat\sigma^{-1}_{\text{RV},j}&\bigg(\hat g_{m_1}'\hat W^{1/2}\hat V^{\text{RV}}_{m_1m_3}\hat W^{1/2}\hat g_{m_3} -\hat g_{m_2}'\hat W^{1/2}\hat V^{\text{RV}}_{m_2m_3}\hat W^{1/2}\hat g_{m_3} \\&\qquad- \hat g_{m_1}'\hat W^{1/2}\hat V^{\text{RV}}_{m_1m_4}\hat W^{1/2}\hat g_{m_4} +  \hat g_{m_2}'\hat W^{1/2}\hat V^{\text{RV}}_{m_2m_4}\hat W^{1/2}\hat g_{m_4}\bigg).
\end{align}



%\cite{hln11} define a version of the MCS procedure where you obtain $p$- values for model under consideration and then, for a level $\alpha$, the MCS is obtained as the set of models with a $p$-value above $\alpha$. We implement this iterative procedure as the do.  As we are able to derive the asymptotic distribution of the test statistics above, 
We take 99,999 draws from this distribution and for each draw compute the max of the absolute value of the $K$ simulated test statistics denoted $\bar{T}^{\text{RV},sim}$.  The $p$-value is then computed as the fraction of draws for which  $\bar{T}^{\text{RV},sim} > \abs{\bar T^\text{RV}}$.

This procedure is computationally expedient.  In particular, one does not need to bootstrap both demand estimation and the testing procedure, which can be prohibitively costly.  Instead, using the adjustments derived in Appendix \ref{sect:TwoStep}, $\hat\Sigma$ can incorporate adjustments for demand estimation and clustering. 


==> Submission/ReStud/Appendices/ManyInstruments.tex <==
\subsection{Many Instruments for Testing: Bias of RV}\label{sec:manyinstr} 

The RV test fundamentally depends on predicting markups from the instruments.  When the first stage is viewed in this light, one may consider adding a large number of instruments in order to improve the predictions.  In light of Proposition \ref{prop:degen}, there may be benefits to doing so in the context of RV.  However, this comes at a cost.  The econometrics literature has discussed the problem of many instruments in an estimation context.  Specifically  \cite{b94} and \cite{cs05} show that the 2SLS estimator is inconsistent under a many instruments asymptotic.  More troubling, this asymptotic has been found to approximate well the finite sample distribution of the estimator, thus revealing substantial bias towards the OLS estimator.  The intuition, discussed in \cite{ad09} is that increasing the number of instruments overfits the endogenous variable.  In the extreme, one predicts the endogenous variable perfectly and thus reverts to OLS in the second stage.  

We show that the use of many instruments has a similar impact on the RV test that it does in 2SLS.  We first establish the analogue of OLS in testing.  Consider alternative moments
$g^{OLS}_m = \frac{\Delta'\hat\omega_m}{n}$,
which are the moments one would use to estimate Equation (\ref{eq:test}) by OLS. We define a measure of fit using these moments as $Q_m^{OLS} = g^{OLS\prime}_m(\frac{\Delta'\Delta}{n})^{-1} g^{OLS}_m$. Now we can define a version of the RV test statistic with the OLS moments: $T^{OLS} = \frac{\sqrt{n}}{\hat  \sigma_{RSS}} (Q_1^{OLS} - Q_2^{OLS}).$
As shown in Appendix XX, this test is inconsistent and has a plim given by:
$$\frac{T^{OLS}}{\sqrt{n}} &\rightarrow_p  \frac{E[(\Delta^{OLS}_i -\Delta_{1i})^2 - (\Delta^{OLS}_i -\Delta_{2i})^2]	}{\sigma_{OLS}}$$
This shows that OLS-based tests asymptotically reject in favor of the model for which the implied markups are closer to the OLS markups. Since $\Delta$ is generally correlated with $\omega$, $\Delta^{OLS}$ may be very far from $\Delta_0$.  While $T^{OLS}$ may seem artificial, we show in Appendix XX that it is equivalent to an implementation of the RV test based on residual sum of squares (RSS) which has been popular in the applied IO literature.\footnote{For example, \cite{b87}, \cite{glv92}, \cite{bd10} and \cite{bdvk13} use RSS-based procedures to test hypotheses on conduct.} 



Now, to formalize the bias of many instruments, 
we consider a many instrument asymptotic, following \cite{b94} and \cite{cs05}.   Specifically, letting $\Gamma = [\Gamma_1, \Gamma_2]$, we assume the following:

\begin{assumption}\label{as:manyinstr} Let the number of instruments grow at rate $n$ so that $\frac{d_z}{n} \rightarrow_p \delta_z > 0$.  Moreover, suppose:
(i) $\frac{\hat\Gamma'z'z\hat\Gamma}{n}\rightarrow H_1 + o_p(1)$ and (ii) $\frac{\hat\Gamma'z'z\hat\Gamma_0}{n}\rightarrow H_2 + o_p(1)$ for some matrices $H_1,H_2>0$.
\end{assumption}
The above assumption maintains that  the concentration parameters $\frac{\Gamma'z'z\Gamma}{n}$ and $\frac{\Gamma'z'z\Gamma_0}{n}$ are non-diverging as the number of instruments grows.  Thus, the variance of the predicted markups remains finite. One way to interpret this assumption is that additional instruments are eventually uninformative in predicting markups. Regardless of the interpretation, the econometrics literature has found that the asymptotic distribution obtained with this assumption is a good approximation of the finite sample performance even if $d_z$ is small (see \cite{b94} and \cite{ak95}).\looseness=-1


Under Assumption \ref{as:manyinstr}, we can characterize the behavior of the RV test statistic in a many instrument setting.  Specifically, we derive the following result:
\begin{proposition}\label{prop:biasmany} Suppose that Assumptions \ref{as:momcond}, \ref{as:regcond}, and \ref{as:manyinstr} are satisfied. Then:
\begin{align*}
    \frac{T^{RV}}{\sqrt{n}} \rightarrow_p 
    & \frac{1-\delta_z}{\sigma_{RV}}
    \bigg(E[(\Delta^z_{1i}-\Delta^z_{0i})^2] - E[(\Delta^z_{2i}-\Delta^z_{0i})^2]\bigg)
    \\&\qquad +\frac{\delta_z}{\sigma_{RV}}\bigg(E[(\Delta_{1i}-\Delta^{OLS}_i)^2] - E[(\Delta_{2i}-\Delta^{OLS}_i)^2]\bigg)
\end{align*}

\end{proposition}

Proposition \ref{prop:biasmany} sheds light on important aspects of testing with many instruments. In estimation, the presence of many instruments biases 2SLS estimates to their OLS counterpart.  Likewise, we see that the RV test is biased towards the RSS test discussed in Section \ref{sec:RSS}, which forms the moments with the endogenous markups.  The extent of the bias depends on the magnitude of $\delta_z$.  \cite{h20} states that although there is no set rule of thumb, many instruments are a serious concern whenever the number of instruments exceeds 5\% of the sample size. However, many instruments can still create significant bias below that threshold.  In fact, \cite{ak95} find severe bias in a setting where  $\frac{d_z}{n}$ is as small as 0.005.  


Thus, a researcher should be concerned when using many instruments \textit{even if they are valid}.  While valid instruments implement the condition in Lemma 1, there is no guarantee that using them to form the RV test will allow one to  achieving correct inference either in finite sample or asymptotically.  We return to the problem of many instruments in Section \ref{sec:sieveIJIVE} and propose a modification of the RV test statistic which removes the finite sample bias that they cause.

==> Submission/ReStud/Appendices/Robustness.tex <==

This appendix provides additional details for our empirical application. 

\noindent \textbf{Code Details:} Below is the definition of the demand estimation problem in \texttt{PyBLP} and the testing problem in \texttt{pyRVtest}.
\begin{figure}[H]
    \centering
    \caption{Code for Demand Estimation and Testing}
    \hspace{-2.5cm}
    \begin{subfigure}[t]{0.5\textwidth}
        \caption*{\hspace{-1.5cm}Panel A. Demand Estimation Code}
        \includegraphics[scale=0.32, trim={.1cm 0 0 0}, clip]{Figures/pyBLP_problem1.png} \\
        \includegraphics[scale=0.3, trim={.1cm 0 0 0}, clip]{Figures/pyBLP_problem2.png}\\
        \vspace{1.75cm}
    \end{subfigure}
    \hspace{-1cm}
    \begin{subfigure}[t]{0.4\textwidth}
        \caption*{\hspace{1.5cm}Panel B. Testing Code}
        \includegraphics[scale=0.32]{Figures/pyRVtest_problem.png}
    \end{subfigure}
    
    \caption*{\footnotesize{Panels A and B report the definitions of the demand estimation problem in \texttt{PyBLP} and the testing problem in \texttt{pyRVtest}, respectively.}}
\end{figure}

\vspace{-0.8cm}

\noindent \textbf{Description of the Models of Conduct:} Following \cite{v07}, the markups in market $t$ for a model $m$ among those we consider can be written in the following form:
\[\boldsymbol{\Delta}_{mt}=\underbrace{-(\boldsymbol{\Omega}^r_{mt} \odot \boldsymbol{D}^r_t)^{-1} \boldsymbol{s}_t}_{=\boldsymbol{\Delta}^\text{downstream}_{mt}}\underbrace{-(\boldsymbol{\Omega}^w_{mt} \odot \boldsymbol{D}^w_t )^{-1} \boldsymbol{s}_t}_{=\boldsymbol{\Delta}^\text{upstream}_{mt}}\]
where $\boldsymbol{\Omega}^r_{mt}$ and $\boldsymbol{\Omega}^w_{mt}$ are ownership matrices, $\boldsymbol{D}^w_t$ is the jacobian of retail share $\boldsymbol{s}_t$ with respect to wholesale price, and $\boldsymbol{D}^r_t$ is the jacobian of retail share with respect to retail price. The markup $\boldsymbol{\Delta}_{mt}$ implied by each model is the sum of downstream markups $\boldsymbol{\Delta}^\text{downstream}_{mt}$ and upstream markups $\boldsymbol{\Delta}^\text{upstream}_{mt}$. We can derive each model by using different assumptions on the ownership matrices:
\begin{enumerate}
    \item \textit{Zero wholesale margin}: Set $\boldsymbol{\Omega}^w_{mt}$ to a matrix of zeros, set $\boldsymbol{\Omega}^r_{mt}$ to a matrix of ones.
    \item \textit{Zero retail margin}: Set $\boldsymbol{\Omega}^w_{mt}$ to a matrix of zeros, and set $\boldsymbol{\Omega}^r_{mt}$ to a matrix  with element $(i,j)$ that is equal to one if products $i$ and $j$ are produced by the same manufacturer, and to zero otherwise. 
    \item \textit{Linear pricing}: Set $\boldsymbol{\Omega}^r_{mt}$ to a matrix of ones, and set $\boldsymbol{\Omega}^w_{mt}$ to a matrix  with element $(i,j)$ that is equal to one if products $i$ and $j$ are produced by the same manufacturer, and to zero otherwise. 
    \item \textit{Hybrid model}: Set $\boldsymbol{\Omega}^r_{mt}$ to a matrix of ones, and set $\boldsymbol{\Omega}^w_{mt}$ to a matrix  with element $(i,j)$ that is equal to one if products $i$ and $j$ are produced by the same manufacturer and $i$ is not a private label, and to zero otherwise. 
    \item \textit{Wholesale Collusion}: Set $\boldsymbol{\Omega}^r_{mt}$ and $\boldsymbol{\Omega}^w_{mt}$ to matrices of ones. \looseness=-1
    
\end{enumerate}



\noindent \textbf{Pooling all Instrument Sets:}  We present in Table \ref{Tab:Instr_Rob} the test results obtained by pooling all instrument sets used in Section \ref{sec:empiricaleg}. We do so first using the PCA BLP95 and Diff instruments (Panel A), and then using non PCA versions of these instruments (Panel B). Two observations emerge from the table. First, the $F$-statistics with the pooled instruments, although above the corresponding critical values for 95\% maximal power, are below those for the BLP95 instrument set. This confirms our observation that pooling instruments may result in lower $F$-statistics, and potentially weak instruments. Second, the MCS for both sets of pooled instruments now includes not only model 2, but also model 1 at a confidence level $\alpha = 0.05$. Hence, pooled instrument sets lead to less sharp conclusions in this example.

\begin{table}[H]
\footnotesize
\caption{RV Test Results with Alternative Instruments}
\label{Tab:Instr_Rob}
\centering
\begin{threeparttable}
\input{Tables/CombinedInstr}
\begin{tablenotes}[flushleft]
    \footnotesize
    Panels A and B report the RV test statistics $T^\text{RV}$ and the effective $F$-statistic for all pairs of models, and the MCS $p$-values (details on their computation are in Appendix F). A negative RV test statistic suggests better fit of the row model. With MCS $p$-values below 0.05 a row model is rejected from the model confidence set.    Both $T^\text{RV}$ and the $F$-statistics account for two-step estimation error and clustering at the market level; see Appendix \ref{sect:TwoStep} for details.  \looseness=-1
\end{tablenotes}
\end{threeparttable}
\end{table}    



==> Submission/ReStud/Appendices/SimSeqDemand.tex <==

Consider a setting where testing is performed in a GMM environment and the supply moments for a model of conduct $m$ are $g_m\left(\theta^{D}\right) = \frac{1}{n}z'(p-\Delta_m(\theta^{D}))$.  The supply moments depend on demand parameters $\theta^D$ through markups $\Delta_m=\Delta_m(\theta^D)$. Demand moments are $
 h\left(\theta^{D}\right) = \frac{1}{n}\textbf{z}^{D\prime}\boldsymbol{\xi}(\theta^{D})$,
where $\boldsymbol{\xi}(\theta^{D})$ is the value of the demand unobservable implied by $\theta^D$, and $\textbf{z}^{D}$ is a vector of demand instruments.\footnote{Demand moments could include micro-moments; our discussion in this section would still apply.} We assume that the dimension of $\textbf{z}^D$ is sufficient to identify $\theta^{D}$ from demand moments alone. \looseness=-1  

We define plim of the demand parameters obtained from sequential estimation as:
\begin{align*}
    \theta^{Dseq} = \arg\min_{\theta^D} \mathcal{Q}^D(\theta^D),
\end{align*}
where $\mathcal{Q}^D=plim(h(\theta^{D})'W^{D}h(\theta^{D}))$ and $W^{D} = (\frac{\textbf{z}^{D\prime}\textbf{z}^D}{n})^{-1}$. We construct the RV test statistic  in a second step  from a measure of fit based on supply moments.   The asymptotic value of the measure of fit for each model $m$ is:
\[
\mathcal{Q}_{m}(\theta^{Dseq})=\mathcal{g}_m(\theta^{Dseq})'W\mathcal{g}_m(\theta^{Dseq}).
\]



Alternatively, we could use the supply moments to estimate demand. Stacking the demand and supply moments, the simultaneous GMM objective function is:
\begin{align*}
Q_m^{sim}(\theta^D) = (g_m(\theta^D)',h(\theta^D)')W^{sim}(g_m(\theta^D)',h(\theta^D)')'
\end{align*}
%\begin{align*}
%Q_m^{sim}(\theta^D) & =\left[\begin{array}{c}
%g_m(\theta^D)\\
%h(\theta^D)
%\end{array}\right]^{\prime}W^{sim}\left[\begin{array}{c}
%g_m(\theta^D)\\
%h(\theta^D)
%\end{array}\right].
%\end{align*}
We maintain the following assumption on $W^{sim}$ for tractability:
\begin{assumption}\label{as:blockdiag}
    $W^{sim}$ is block diagonal, so that $W^{sim}=diag(W, W^D)$.  
\end{assumption}
\noindent The plim of the demand parameters obtained from simultaneous estimation are: $$\theta_m^{Dsim} = \arg\min_{\theta^{D}} \mathcal{Q}_m(\Delta(\theta^{D})) + \mathcal{Q}^{D}(\theta^{D}).$$ 
\noindent While the value of $\theta_m^{Dsim}$ is model specific, $\theta^{Dseq}$ is not. We now establish the following:
\begin{proposition}\label{prop:demand}
Let Assumption \ref{as:blockdiag} hold, $\textbf{w}$ be correctly specified, $\theta_m^{Dsim}$ be unique, and $\theta^{Dseq}\neq\theta_m^{Dsim}$ for model $m$. Then, $E[(\tilde \Delta_0 - \tilde \Delta_m(\theta_m^{Dsim}))^2] <         E[(\tilde \Delta_0 - \tilde \Delta_m(\theta^{Dseq}))^2]$.\footnote{ If cost shifters $\textbf{w}_a$ are not correctly specified but  Assumption \ref{as:misspmc} holds, then 
        $E[(\tilde \Delta^\textbf{a}_0 - \tilde \Delta_m(\theta_m^{Dsim}))^2] <         E[(\tilde \Delta^\textbf{a}_0 - \tilde \Delta_m(\theta^{Dseq}))^2]
    $
    where $\Delta^\textbf{a}_0=M_{\textbf{w}_a}(\boldsymbol{\Delta}_0+\textbf{w}\tau-\textbf{w}_a\tau_a)$.}
\end{proposition}    
    

The consequences of the proposition  depend on the model of conduct $m$ and the testing environment. Suppose $m=1$ is the true model and there is no misspecification.  Then $\theta^{Dseq}=\theta_1^{Dsim}$, and $ E[(\tilde \Delta_0 - \tilde \Delta_1(\theta_1^{Dsim}))^2] =         E[(\tilde \Delta_0 - \tilde \Delta_1(\theta^{Dseq}))^2] = 0.$   It follows that  $\mathcal{Q}_1 - \mathcal{Q}_2$ is smaller in magnitude under simultaneous estimation.  Instead, when demand is misspecified, the proposition implies that $B$ is smaller with a simultaneous approach. However, predicted markups for $m=2$ also get closer to the true ones.
Thus, a simultaneous approach provides a (weakly) better fit for both models. If the researcher assumes that the testing environment has low misspecification  and has a large dataset, a simultaneous approach may change the sign for the RV statistic and cause the researcher to conclude for a wrong model. However, if misspecification is severe or if the dataset is small, a simultaneous approach may offer advantages by improving the fit of a true model. We summarize these findings as follows:
\begin{corollary}\label{cor:demand}
Let Assumption \ref{as:blockdiag} hold, $\theta_m^{Dsim}$ be unique, and $\theta^{Dseq}\neq\theta_m^{Dsim}$ for model $m$. 
\begin{itemize}
    \item[(i)] Without misspecification, the plim of the RV numerator is smaller in magnitude under simultaneous estimation, but has the same sign as under sequential estimation.
    \item[(ii)]  With misspecification, the sign and magnitude of plim of the RV numerator could differ under simultaneous and sequential estimation.
\end{itemize}
\end{corollary}

\noindent While we focus on the numerator, the mode of demand estimation will also effect the denominator of $T^{RV}$. This effect on the power of RV is ambiguous even under our simplifying assumptions and we leave it to future research.
 

The demand estimation literature (see \cite{cg19}) has discussed how simultaneous and sequential estimation affect estimates and standard errors for the demand parameters. Our results show that simultaneous estimation does not guarantee demand parameter estimates closer to the true demand parameters. Instead, the supply moments pull the demand parameters towards values which improve the fit of the predicted markups under the assumed conduct model. Moreover, efficiency considerations that apply to estimation do not immediately apply to our setup as one of the models we consider is not correctly specified. \looseness=-1   


==> Submission/ReStud/Appendices/TwoStep.tex <==

This appendix extends all our previously introduced statistics to take into account uncertainty stemming from preliminary demand estimation as well as dependence across observations. We suppose that $\Delta_m$ is a function of demand parameters $\theta^D_0$ that are estimated using a GMM estimator $\hat \theta^D$. We therefore let $W^D$ denote the GMM weight matrix and $h(\theta^D)=\frac{1}{n} \sum_{i=1}^n h_i(\theta^D)$ the GMM sample moment function used. Furthermore, we let $ H=\nabla_\theta h(\hat\theta^D)$ be the gradient of the sample moment function $ h$ and let $ G_m=-\frac{1}{n} \hat z' \nabla_{\theta} \hat \Delta_m(\hat\theta^D)$ be the gradient of $\hat g_m$. Both gradients are with respect to $\theta^D$.

\noindent\textbf{RV test:}
The RV statistic with a two-step adjustment replaces $\hat V_{\ell k}^\text{RV}$ in the definition of $\hat\sigma^2_\text{RV}$ with $\tilde V_{\ell k}^\text{RV} = \frac{1}{n} \sum_{i=1}^n \tilde \psi_{\ell i} \tilde \psi_{k i}'$. Here, the influence function $\tilde \psi_{mi}$ adjusts $\hat \psi_{mi}$ to account for preliminary demand estimation:
\begin{align}
      \tilde \psi_{mi} &= \hat \psi_{mi} - \hat W^{1/2} G_m \Phi \!\left(h_i(\hat\theta^D)- h(\hat\theta^D)\right)
\end{align}
where $\Phi=(H'W^DH)^{-1}H'W^D$. This is a standard adjustment for first-step estimation based on the asymptotic approximation $\hat \theta^D - \theta^D_0 = -\Phi h(\theta^D_0) + o_p\big(n^{-1/2}\big).$

\noindent\textbf{AR test:}
Analogously to the above, the AR statistics with a two-step adjustment replaces $\hat V_{mm}^\text{AR}$ with $\tilde V_{mm}^\text{AR}$ where $\tilde V_{\ell k}^\text{AR} = \frac{1}{n} \sum_{i=1}^n \tilde \phi_{\ell i} \tilde \phi_{k i}'$. Here, the influence function $\tilde \phi_{mi}$ adjusts $\hat \phi_{mi} = \hat W \hat z_i(\hat p_i- \hat \Delta_{mi} - \hat z_i'\hat \pi_i)$ to account for preliminary demand estimation using the same approximation to $\hat \theta^D$ as above:
\begin{align}
      \tilde \phi_{mi} &= \hat \phi_{mi} - \hat W G_m \Phi_m \!\left(h_i(\hat\theta^D)- h(\hat\theta^D)\right).
\end{align}

% Analogous to the solution in \citeA{mw17}'s appendix D, a consistent estimator for the asymptotic variance of $\hat\pi_m$ that takes into account the uncertainty from the demand estimate $\hat\theta^D$ is:

% \[(G^{S\prime}_mWG^S_m)^{-1}G^{S\prime}_mW\Sigma_m WG^S_m(G^{S\prime}_mWG^S_m)^{-1}\]
% where $\hat g_m=n^{-1}z^{\prime}\hat\omega_m=n^{-1}z^{\prime}(p-\hat\Delta_m(\hat\theta^D)-z\hat\pi_m)$, $G^S_m=\nabla_\pi \hat g_m=n^{-1}z'z$ and:
% \[
% \Sigma_m = \sum_{i=1}^n \bigg(z^{\prime}_i\hat\omega_{m,i}-\hat g_m + \hat\Phi_m \left(z_i^{D\prime}\xi_i(\hat\theta^D)-\hat h(\hat\theta^D)\right) \bigg) \bigg( z^{\prime}_i\hat\omega_{m,i}-\hat g_m + \hat\Phi_m  \left(z_i^{D\prime}\xi_i(\hat\theta^D) -\hat h(\hat\theta^D)\right)\bigg)'
% \]
% where $\hat\Phi_m$ is defined as in the RV test case.

\noindent\textbf{$F$-statistic:}
The $F$-statistic with a two-step adjustment replaces $\hat \sigma_1^2$, $\hat \sigma_2^2$, and $\hat \sigma_{12}$ in the definition of $F$ and $\hat \rho^2$ with $\tilde \sigma_m^2 = d_z\inverse \text{trace}\big( \tilde V_{mm}^\text{AR} \hat W^{-1} \big)$ for $m\in\{1,2\}$ and $\tilde \sigma_{12} = d_z\inverse  \text{trace}\big(  \tilde V_{\ell k}^\text{AR}\hat W^{-1} )$. Here, $ \tilde V_{\ell k}^\text{AR}$ and $\tilde \phi_{mi}$ were introduced in the preceding paragraph.

An extension of Proposition \ref{prop:wkinstrF} that accounts for two-step estimation can be established under homoskedasticity, i.e., when $\hat W^{-1/2} \tilde V_{\ell k}^\text{AR} \hat W^{-1/2}$ for $\ell,k \in \{1,2\}$ converge in probability to diagonal matrices. In the absence of homoskedasticity, $F$ is still informative about the strength of the instruments, but the exact thresholds for size control reported in Table \ref{tab:Tab_StockYogo_Combined_new} may only be approximations to the true thresholds.

%\noindent\textbf{EB test:}
%Analogous to the AR test correction, except that instead of $n^{-1}z^{\prime}(p-\hat\Delta_m(\hat\theta^D)-z\hat\pi_m)$ the supply side moment is now $z^{\prime}(p-\theta\hat\Delta(\hat\theta^D))$ and we take derivatives with respect to $\theta$ to compute $G_m$. This formulation is analogous to \citeA{mw17}, Appendix D.

%\noindent\textbf{Cox test:}
%The Cox statistic with a two-step adjustment replaces $ \hat V_{mm}^\text{AR} $ in the definition of $\hat\sigma^2_\text{Cox}$ with $\tilde V_{mm}^\text{AR}$. Here, $\tilde V_{mm}^\text{AR}$ was introduced for the two-step correction of AR.


\noindent\textbf{Dependence:}
Dependent data, e.g., cluster sampling, is easily accommodated by adjustments to $\hat V_{\ell k}^\text{RV}$ and $\hat V_{\ell k}^\text{AR}$. If we let $c_{ij}$ take the value one if observations $i$ and $j$ are deemed dependent and zero otherwise, then the variance estimators used in the paper can be replaced by 
\begin{align}
    \Breve V_{\ell k}^\text{RV} = \frac{1}{n} \sum_{i=1}^n\sum_{j=1}^n c_{ij} \hat\psi_{\ell i} \hat\psi_{k j}'
    \quad \text{and} \quad 
    \Breve V_{\ell k}^\text{AR} = \frac{1}{n} \sum_{i=1}^n\sum_{j=1}^n c_{ij} \hat\phi_{\ell i} \hat\phi_{k j}'.
\end{align}
Combinations of two-step estimation and dependence are also handled by simply replacing $\hat \psi$ and $\hat \phi$ by $\tilde \psi$ and $\tilde \phi$ in the definitions of $\Breve V_{\ell k}^\text{RV}$ and $\Breve V_{\ell k}^\text{AR}$. Provided that suitable central limit theorem and laws of large numbers can be alluded to under the type of dependence considered, any claims on asymptotic validity under strong instruments made in the paper continue to hold. For clustered data, we refer to \citeA{ha19} for such results.

% Define $\hat g_{3} = \hat g_1-\hat g_2$ and $\hat Q_{3} = \hat g_{3}'\hat W\hat g_{3}$. Analogous to what we show for the RV test, we can show that a consistent estimator for the limiting variance of $\sqrt{n}(\hat Q_1-\hat Q_2-\hat Q_3)$ is:

% \[ \hat\sigma^2=4\hat g_1'\Sigma_1\hat g_1 + 4\hat g_2'\Sigma_2\hat  g_2 +4\hat g_{3}'\Sigma_{3}\hat g_{3}- 8\hat g_1'\Sigma_{1,2}\hat g_2 - 8\hat g_1'\Sigma_{1,3}  g_3 + 8g_2'\Sigma_{2,3}  g_3 \]
% where:
% \[
% \Sigma_{m,l} = \sum_{i=1}^n \bigg(z^{\prime}_i\omega_{m,i}-\hat g_m + \hat\Phi_m\left( z_i^{D\prime}\xi_i(\hat\theta^D)-\hat h(\hat\theta^D)\right) \bigg) \bigg( z^{\prime}_i\hat\omega_{l,i}-\hat g_l + \hat\Phi_l  \left(z_i^{D\prime}\xi_i(\hat\theta^D)-\hat h(\hat\theta^D)\right) \bigg)'\\
% \]
% and $\hat\Phi_m$ is defined as in the RV test case.



==> Submission/ReStud/Appendices/pyRV.tex <==
\begin{figure}[H]
    \centering
    \caption{Code for Demand Estimation and Testing}
    \hspace{-2.5cm}\begin{subfigure}[b]{0.5\textwidth}
          \caption*{\hspace{-1.5cm}Panel A. Demand Estimation Code}
         \includegraphics[scale=0.3, trim={.1cm 0 0 0}, clip]{Figures/pyBLP_problem1.png}\\
\includegraphics[scale=0.3, trim={.1cm 0 0 0}, clip]{Figures/pyBLP_problem2.png}\\
\vspace{1.75cm}
     \end{subfigure}
     \hspace{-1cm}\begin{subfigure}[b]{0.4\textwidth}
        
         \caption*{\hspace{1.5cm}Panel B. Testing Code}
         \includegraphics[scale=0.3]{Figures/pyRV_problem.png}
     \end{subfigure}
    
\subcaption*{Panel A and B respectively report the definition of the demand estimation problem in \texttt{PyBLP} and the testing problem in \texttt{pyRV}. }
\end{figure}

==> Submission/ReStud/Figures/ModelSel_slides.tex <==

\begin{tikzpicture}[scale = 0.85]
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=-1,xmax=5.5,ymin=-1.0,ymax=5.5,
  tick style={draw=none},
  xticklabels=\empty,
  yticklabels=\empty,
  xlabel={$E[(\Delta^z_0-\Delta^z_1)^2]$},
  ylabel={$E[(\Delta^z_0-\Delta^z_2)^2]$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.8,0.15)},anchor=north},
    y label style={at={(axis description cs:0.15,.75)},rotate=90,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  title={Model Selection},
  grid=major,
  grid style={thin,densely dotted,white!20}]

%45-deg lines
\addplot [domain=0:5.5,samples=2, color = black] {x} node[right]{};


%shading
\tikzstyle{rej1}=[draw=none,line width=10pt,preaction={clip, postaction={pattern=horizontal lines, pattern color=blue, opacity=0.3}}]
\tikzstyle{rej2}=[draw=none,line width=1pt,preaction={clip, postaction={pattern=vertical lines, pattern color=red, opacity=0.3}}]

\draw<3>[rej1] (100,300) -- (100,850) -- (650,850)   -- cycle;
\draw<3>[rej2] (300,100) -- (850,100) -- (850,650)   -- cycle;

\draw<4>[rej1] (100,150) -- (100,850) -- (800,850)   -- cycle;
\draw<4>[rej2] (150,100) -- (850,100) -- (850,800)   -- cycle;



\draw<3-4>[draw=black,line width=0.5pt,dashed]  (100,300) -- (700,900)  -- cycle;

\draw<3-4>[draw=black,line width=0.5pt,dashed]  (300,100) -- (900,700)  -- cycle;



\draw<4>[draw=black,line width=0.5pt,dashed]  (100,150) -- (700,750)  -- cycle;

\draw<4>[draw=black,line width=0.5pt,dashed]  (150,100) -- (750,700)  -- cycle;








%\node<1>[text width=5.9cm,rotate = 40,color = black,fill = none] at (600,620) {{${Q}_1 = {Q}_2$}};

\node<1->[text width=3.0cm,rotate = 0,color = black,fill = none] at (550,250) {{${Q}_1 > {Q}_2$}};

\node<1->[text width=5.9cm,rotate = 40,color = black,fill = none] at (500,540) {{$H_0^{RV}$: ${Q}_1 = {Q}_2$}};


\node<1-4>[text width=3.0cm,rotate = 0,color = black,fill = none] at (300,450) {{${Q}_1 < {Q}_2$}};

%\draw<2> [->] (100,450)--(190,310);
%\draw<2> [->] (100,450)--(500,310);


%\node<2>[text width=3.0cm,rotate = -55,color = black,fill = none] at (200,240) {{Low Bias}};

%\node<2>[text width=3.0cm,rotate = -15,color = black,fill = none] at (550,320) {{High Bias}};

\draw<4> [->] (150,350)--(225,275);
\draw<4> [->] (300,500)--(375,425);
\draw<4> [->] (450,650)--(525,575);

\draw<4> [->] (350,150)--(275,225);
\draw<4> [->] (500,300)--(425,375);
\draw<4> [->] (650,450)--(575,525);

%\draw<2->[black, fill=black] (200,300) circle (10) ;
\end{axis}

\end{tikzpicture}\hfill
\begin{tikzpicture}[scale = 0.85]
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=-1,xmax=5.5,ymin=-1.0,ymax=5.5,
  tick style={draw=none},
  xticklabels=\empty,
  yticklabels=\empty,
  xlabel={$E[(\Delta^z_0-\Delta^z_1)^2]$},
  ylabel={$E[(\Delta^z_0-\Delta^z_2)^2]$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.8,0.15)},anchor=north},
    y label style={at={(axis description cs:0.15,.75)},rotate=90,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  title={Model Assessment},
  grid=major,
  grid style={thin,densely dotted,white!20}]


%shading
\tikzstyle{rej1}=[draw=none,line width=10pt,preaction={clip, postaction={pattern=horizontal lines, pattern color=blue, opacity=0.3}}]
\tikzstyle{rej2}=[draw=none,line width=1pt,preaction={clip, postaction={pattern=vertical lines, pattern color=red, opacity=0.3}}]
\draw<3>[rej1] (250,200) -- (250,850) -- (100,850) -- (100,200)   -- cycle;
\draw<3>[rej2] (250,100) -- (250,200) -- (850,200) -- (850,100)   -- cycle;


\draw<4>[rej1] (150,150) -- (150,850) -- (100,850) -- (100,150)   -- cycle;
\draw<4>[rej2] (150,100) -- (150,150) -- (850,150) -- (850,100)   -- cycle;


\draw<4> [<-] (160,600)--(250,600);
\draw<4> [<-] (160,450)--(250,450);
\draw<4> [<-] (160,300)--(250,300);

\draw<4> [<-] (300,160)--(300,200);
\draw<4> [<-] (450,160)--(450,200);
\draw<4> [<-] (600,160)--(600,200);


\node<1->[text width=5.9cm,rotate = 90,color = black,fill = none] at (130,520) {{$H_{0,1}^{AR}$: ${Q}_1 = 0$}};
\node<1->[text width=5.9cm,rotate = 0,color = black,fill = none] at (520,130) {{$H_{0,2}^{AR}$: ${Q}_2 = 0$}};



\draw<3-4>[draw=black,line width=0.5pt,dashed]  (250,100) -- (250,700)  -- cycle;

\draw<3-4>[draw=black,line width=0.5pt,dashed]  (100,200) -- (700,200)  -- cycle;


\draw<4>[draw=black,line width=0.5pt,dashed]  (150,100) -- (150,700)  -- cycle;

\draw<4>[draw=black,line width=0.5pt,dashed]  (100,150) -- (700,150)  -- cycle;

%\draw<3->[black, fill=black] (200,300) circle (10) ;

\end{axis}

\end{tikzpicture}




==> Submission/ReStud/Figures/bresnahan.tex <==

\hspace{-1cm}\begin{tikzpicture}[scale=\tikzscale]
\begin{axis}[
            width=\textwidth,
            height=\axisdefaultheight,
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=0,xmax=6,ymin=0.0,ymax=10,
  xlabel={$q$},
  ylabel={$p$},
  xtick = none,
   ytick = {3.75,5.5,7.25},
        yticklabels = {$\tilde p_{2t}$,$p_t$,$\tilde p_{1t}$},
  %extra y ticks={9,10},
  %  extra y tick labels={$92\rightarrow$,$153.3\rightarrow$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.99,-0.02)},anchor=north},
    y label style={at={(axis description cs:-0.03,.92)},rotate=0,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  %title={Relationship Between Null and Degeneracy},
  grid=major,
  grid style={thin,densely dotted,white!20}]

%Demand
\addplot [domain=0:3.95,samples=2, color = blue!70!green,line width=1.2,opacity=0.4] {8.5-1.9*x} node[right]{};
\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (430,5) {{$D_t$ for $(z_t,\xi_t)$}};


%Omegas
\addplot [domain=0:4,samples=2, color = red!60!yellow] {2} node[right]{};
\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (480,19) {{$p_t-\Delta_{1t}$}};

\addplot [domain=0:4,samples=2, color = red!60!yellow] {5.5} node[right]{};
\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (480,55) {{$p_t-\Delta_{2t}$}};



%tilde p's
\addplot [domain=0:2.5,samples=2, color = black] {3.75} node[right]{};

\addplot [domain=0:2.5,samples=2, color = black] {7.25} node[right]{};

%Moments

\draw [decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
(245,55) -- (245,72.5) node [black,midway,xshift=2.35cm] {
$E[(\Delta^z_{0t}-\Delta^z_{1t})^2]=0$};
\draw [decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
(245,37.5) -- (245,55) node [black,midway,xshift=3.75cm] {
$E[(\Delta^z_{0t}-\Delta^z_{2t})^2]\neq 0$};

%Equilibria


\draw[black, fill=black] (65,72) ellipse (.1cm and .1cm);
\draw[black, fill=black] (160,55) ellipse (.1cm and .1cm);
\draw[black, fill=black] (250,38) ellipse (.1cm and .1cm);


\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (125,65) {{$\tilde{\mathcal{E}}_{1t}=(\cdot,\Delta_{1t})$}};
\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (220,48) {{${\mathcal{E}}_{t}$}};
\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (310,30) {{$\tilde{\mathcal{E}}_{2t}=(\cdot,\Delta_{2t})$}};







\end{axis}

\end{tikzpicture}


==> Submission/ReStud/Figures/flowchart.tex <==
\begin{tikzpicture}[node distance=2cm]

\node (start) [flowbox] {Step 0: Get MCS $M^*_\ell$  for each\\ instrument set $z_\ell$};
\node (in1) [flowbox, right of=start, xshift = 2cm] {Step 1: Check for conflicting evidence.\\ No conflict: $\forall \ell,\ell'$, $M^*_\ell\subseteq M^*_{\ell'} \,\, \text{or}$ \\$M^*_{\ell'}\subseteq M^*_{\ell}$ };
\node (pro1) [flowbox, right of=in1, yshift = 1.5cm, xshift = 6cm] {Step 2: $M^* = M$};
\node (pro2) [flowbox, right of=in1, yshift = -1.5cm, xshift = 6cm] {Step 2: Set $M^*$ as smallest MCS.\\ Then $\forall$ $\ell$ add $M^*_\ell$ to $M^*$ if $z_\ell$ strong for all model pairs};
%\node (pro3) [flowbox, below  of=pro2, yshift=0.2cm] {$\forall$ $l$ add $M^*_\ell$ to $M^*$ if $z_\ell$ strong for all pairs of models};

\draw [arrow] (start) -- (in1);
\draw [arrow] (in1) -- node[anchor=east,rotate=10,xshift=2cm,yshift = 0.25cm] {conflicting evidence} (pro1);
\draw [arrow] (in1) -- node[anchor=south, rotate=-10.5] {no conflicting evidence} (pro2);
%\draw [arrow] (pro2) -- (pro3);
%\draw [arrow] (pro2b) |- (pro1);
%\draw [arrow] (pro2a) -- (out1);
%\draw [arrow] (out1) -- (stop);


\end{tikzpicture}

==> Submission/ReStud/Figures/noise.tex <==

\begin{tikzpicture}[scale = 1]
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=-1,xmax=5.5,ymin=-1.0,ymax=5.5,
  tick style={draw=none},
  xticklabels=\empty,
  yticklabels=\empty,
  xlabel={$E[(\Delta^z_0-\Delta^z_1)^2]$},
  ylabel={$E[(\Delta^z_0-\Delta^z_2)^2]$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.8,0.15)},anchor=north},
    y label style={at={(axis description cs:0.15,.75)},rotate=90,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  title={A. Model Selection - High Noise},
  grid=major,
  grid style={thin,densely dotted,white!20}]

%45-deg lines
\addplot [domain=0:5.5,samples=2, color = black] {x} node[right]{};


%shading
\tikzstyle{rej1}=[draw=none,line width=10pt,preaction={clip, postaction={pattern=horizontal lines, pattern color=blue, opacity=0.3}}]
\tikzstyle{rej2}=[draw=none,line width=1pt,preaction={clip, postaction={pattern=vertical lines, pattern color=red, opacity=0.3}}]

\draw[rej1] (100,300) -- (100,850) -- (650,850)   -- cycle;
\draw[rej2] (300,100) -- (850,100) -- (850,650)   -- cycle;




\draw[draw=black,line width=0.5pt]  (100,300) -- (700,900)  -- cycle;

\draw[draw=black,line width=0.5pt]  (300,100) -- (900,700)  -- cycle;







\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (550,180) {{${Q}_1 > {Q}_2$}};

\node[text width=5.9cm,rotate = 40,color = black,fill = none] at (500,540) {{$H^\text{RV}_0$: ${Q}_1 = {Q}_2$}};


\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (300,550) {{${Q}_1 < {Q}_2$}};



%\draw[black, fill=black] (200,350) circle (10) ;
%\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (350,380) {{$G$}};

\end{axis}

\end{tikzpicture}\hfill
\begin{tikzpicture}[scale = 1]
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=-1,xmax=5.5,ymin=-1.0,ymax=5.5,
  tick style={draw=none},
  xticklabels=\empty,
  yticklabels=\empty,
  xlabel={$E[(\Delta^z_0-\Delta^z_1)^2]$},
  ylabel={$E[(\Delta^z_0-\Delta^z_2)^2]$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.8,0.15)},anchor=north},
    y label style={at={(axis description cs:0.15,.75)},rotate=90,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  title={B. Model Assessment - High Noise},
  grid=major,
  grid style={thin,densely dotted,white!20}]


%shading
\tikzstyle{rej1}=[draw=none,line width=10pt,preaction={clip, postaction={pattern=horizontal lines, pattern color=blue, opacity=0.3}}]
\tikzstyle{rej2}=[draw=none,line width=1pt,preaction={clip, postaction={pattern=vertical lines, pattern color=red, opacity=0.3}}]
\draw[rej1] (250,200) -- (250,850) -- (100,850) -- (100,200)   -- cycle;
\draw[rej2] (250,100) -- (250,200) -- (850,200) -- (850,100)   -- cycle;





\node[text width=5.9cm,rotate = 90,color = black,fill = none] at (130,550) {{$H_{0,1}^\text{AR}$: ${Q}_1 = 0$}};
\node[text width=5.9cm,rotate = 0,color = black,fill = none] at (550,140) {{$H^\text{AR}_{0,2}$: ${Q}_2 = 0$}};



\draw[draw=black,line width=0.5pt]  (250,100) -- (250,700)  -- cycle;

\draw[draw=black,line width=0.5pt]  (100,200) -- (700,200)  -- cycle;

%\draw[black, fill=black] (200,350) circle (10) ;
%\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (350,380) {{$G$}};
\end{axis}

\end{tikzpicture}



\begin{tikzpicture}[scale = 1]
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=-1,xmax=5.5,ymin=-1.0,ymax=5.5,
  tick style={draw=none},
  xticklabels=\empty,
  yticklabels=\empty,
  xlabel={$E[(\Delta^z_0-\Delta^z_1)^2]$},
  ylabel={$E[(\Delta^z_0-\Delta^z_2)^2]$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.8,0.15)},anchor=north},
    y label style={at={(axis description cs:0.15,.75)},rotate=90,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  title={C. Model Selection - Low Noise},
  grid=major,
  grid style={thin,densely dotted,white!20}]

%45-deg lines
\addplot [domain=0:5.5,samples=2, color = black] {x} node[right]{};


%shading
\tikzstyle{rej1}=[draw=none,line width=10pt,preaction={clip, postaction={pattern=horizontal lines, pattern color=blue, opacity=0.3}}]
\tikzstyle{rej2}=[draw=none,line width=1pt,preaction={clip, postaction={pattern=vertical lines, pattern color=red, opacity=0.3}}]



\draw[rej1] (100,180) -- (100,870) -- (800,870)   -- cycle;
\draw[rej2] (180,100) -- (870,100) -- (870,800)   -- cycle;



%\draw[draw=black,line width=0.5pt,dashed]  (100,300) -- (700,900)  -- cycle;

%\draw[draw=black,line width=0.5pt,dashed]  (300,100) -- (900,700)  -- cycle;



\draw[draw=black,line width=0.5pt]  (100,180) -- (700,770)  -- cycle;

\draw[draw=black,line width=0.5pt]  (180,100) -- (770,700)  -- cycle;





\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (550,180) {{${Q}_1 > {Q}_2$}};

\node[text width=5.9cm,rotate = 40,color = black,fill = none] at (500,540) {{$H^\text{RV}_0$: ${Q}_1 = {Q}_2$}};


\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (300,550) {{${Q}_1 < {Q}_2$}};



%\draw [->] (150,350)--(225,275);
%\draw [->] (300,500)--(375,425);
%\draw [->] (450,650)--(525,575);

%\draw [->] (350,150)--(275,225);
%\draw [->] (500,300)--(425,375);
%\draw [->] (650,450)--(575,525);

%\draw[black, fill=black] (200,350) circle (10) ;
%\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (350,380) {{$G$}};
\end{axis}

\end{tikzpicture}\hfill\hfill
\begin{tikzpicture}[scale = 1]
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,very thick,black},
  xmin=-1,xmax=5.5,ymin=-1.0,ymax=5.5,
  tick style={draw=none},
  xticklabels=\empty,
  yticklabels=\empty,
  xlabel={$E[(\Delta^z_0-\Delta^z_1)^2]$},
  ylabel={$E[(\Delta^z_0-\Delta^z_2)^2]$},
  axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.8,0.15)},anchor=north},
    y label style={at={(axis description cs:0.15,.75)},rotate=90,anchor=south},
  xlabel style = {black},
  ylabel style = {black},
  title={D. Model Assessment - Low Noise},
  grid=major,
  grid style={thin,densely dotted,white!20}]


%shading
\tikzstyle{rej1}=[draw=none,line width=10pt,preaction={clip, postaction={pattern=horizontal lines, pattern color=blue, opacity=0.3}}]
\tikzstyle{rej2}=[draw=none,line width=1pt,preaction={clip, postaction={pattern=vertical lines, pattern color=red, opacity=0.3}}]
%\draw<3>[rej1] (250,200) -- (250,850) -- (100,850) -- (100,200)   -- cycle;
%\draw<3>[rej2] (250,100) -- (250,200) -- (850,200) -- (850,100)   -- cycle;


\draw[rej1] (165,165) -- (165,850) -- (100,850) -- (100,165)   -- cycle;
\draw[rej2] (165,100) -- (165,165) -- (850,165) -- (850,100)   -- cycle;


%\draw<4> [<-] (160,600)--(250,600);
%\draw<4> [<-] (160,450)--(250,450);
%\draw<4> [<-] (160,300)--(250,300);

%\draw<4> [<-] (300,160)--(300,200);
%\draw<4> [<-] (450,160)--(450,200);
%\draw<4> [<-] (600,160)--(600,200);


\node[text width=5.9cm,rotate = 90,color = black,fill = none] at (130,550) {{$H_{0,1}^\text{AR}$: ${Q}_1 = 0$}};
\node[text width=5.9cm,rotate = 0,color = black,fill = none] at (550,130) {{$H_{0,2}^\text{AR}$: ${Q}_2 = 0$}};



%\draw<3-4>[draw=black,line width=0.5pt,dashed]  (250,100) -- (250,700)  -- cycle;

%\draw<3-4>[draw=black,line width=0.5pt,dashed]  (100,200) -- (700,200)  -- cycle;


\draw[draw=black,line width=0.5pt]  (165,100) -- (165,700)  -- cycle;

\draw[draw=black,line width=0.5pt]  (100,165) -- (700,165)  -- cycle;

%\draw[black, fill=black] (200,350) circle (10) ;
%\node[text width=3.0cm,rotate = 0,color = black,fill = none] at (350,380) {{$G$}};
\end{axis}

\end{tikzpicture}


==> Submission/ReStud/Proofs/Pf_ConvergDistrib_Misspecification.tex <==
\begin{proof}
%On top of the assumption of Proposition 2 that $\sqrt{n}\hat A_{z\Delta }= \rho + o_p(1),$ we also need a further assumption to define local alternatives, this time involving the true markups $\Delta^*$:
%\begin{align}
%    \sqrt{n}(\hat A_{z\Delta^* } - \hat A_{z\Delta })&= %\rho^* + o_p(1),
%\end{align}
%so that:
%\begin{align}
%\sqrt{n}(\hat A_{ z\Delta^* }\theta_0 -\hat A_{z\Delta}\theta_m)&= A_{zz}^{-1} \rho^*\theta_0 + A_{zz}^{-1}\rho(\theta_0-\theta_m) + o_p(1).
%\end{align}

%We formally state the assumption as:
%\begin{assumption}
%    We assume that the models we consider satisfy the %following local alternatives property:
%    \begin{align}
%    \sqrt{n}(\hat A_{z\Delta^* } - \hat A_{z\Delta })&= \rho^* + o_p(1),
%\end{align}    
%where $\rho^*$ is a finite matrix.
%\end{assumption}

It is useful to note the following:
\begin{align}
\sqrt{n}(\hat A_{ z\Delta^* }\theta_0 -\hat A_{z\Delta}\theta_m)\hat A_{zz}^{-1} \sqrt{n}(\hat A_{ z\Delta^* }\theta_0 -\hat A_{z\Delta}\theta_m)& = E\bigg[\bigg(\theta_0\tilde\Delta^*_{ni} - \theta_m\tilde\Delta_{ni}\bigg)\bigg(\tilde\Delta^*_{ni}\theta_0 - \tilde\Delta_{ni}\theta_m\bigg)\bigg]+ o_p(1)\\
&=E\bigg[\bigg(\tilde\Delta^*_{n,0i} - \tilde\Delta_{n,mi}\bigg)^2\bigg]+ o_p(1)
\end{align}


\begin{itemize}
\item[\textbf{(i) - EB }] To derive the distribution of the test statistic, we first consider:
\begin{align*}
\sqrt{n}(\Delta'P_z\Delta)^{1/2}(\hat\theta - \theta_0)  &= \sqrt{n}(\Delta'P_z\Delta)^{-1/2}\Delta'P_zp - \sqrt{n}(\Delta'P_z\Delta)^{1/2}\theta_0\\
&= \sqrt{n}(\Delta'P_z\Delta)^{-1/2}\Delta'P_z(\Delta^*\theta_0 + \omega_0)- \sqrt{n}(\Delta'P_z\Delta)^{1/2}\theta_0\\
&= \sqrt{n}(\Delta'P_z\Delta)^{-1/2}\Delta'P_z(\Delta^*-\Delta)\theta_0 + \sqrt{n}(\Delta'P_z\Delta)^{-1/2}\Delta'P_z \omega_0\\
&= (\sqrt{n}\hat A_{\Delta z} \hat A_{z z}^{-1} \sqrt{n}\hat A_{z\Delta})^{-1/2}\sqrt{n}\hat A_{\Delta z} \hat A_{z z}^{-1}\sqrt{n}(\hat A_{z\Delta^*}-\hat A_{z\Delta})\theta_0 \\
&\qquad+(\sqrt{n}\hat A_{\Delta z} \hat A_{z z}^{-1} \sqrt{n}\hat A_{z\Delta})^{-1/2}\sqrt{n}\hat A_{\Delta z} \hat A_{z z}^{-1}\frac{z'\omega_0}{\sqrt{n}}\\
&\rightarrow_d{N}\biggl((\rho A_{zz}^{-1}\rho)^{-1/2}\rho A_{zz}^{-1}\rho^*\theta_0,\sigma^2_{\omega_0}\biggr)
\end{align*}
so that 
\begin{align*}
\sqrt{n}\frac{(\Delta'P_z\Delta)^{1/2}}{\hat\sigma_{\omega_0}}(\hat\theta - \theta_m)  &= \sqrt{n}\frac{(\Delta'P_z\Delta)^{1/2}}{\hat\sigma_{\omega_0}}(\hat\theta- \theta_0)  + \sqrt{n}\frac{(\Delta'P_z\Delta)^{1/2}}{\hat\sigma_{\omega_0}}(\theta_0- \theta_m)\\
&= \sqrt{n}\frac{(\sqrt{n}\hat A_{\Delta z} \hat A_{zz}^{-1} \sqrt{n}\hat A_{z\Delta})^{1/2}}{\hat\sigma_{\omega_0}}(\hat\theta- \theta_0)  +\frac{(\sqrt{n}\hat A_{\Delta z} \hat A_{zz}^{-1} \sqrt{n}\hat A_{z\Delta})^{1/2}}{\hat\sigma_{\omega_0}} (\theta_0- \theta_m)\\
&\rightarrow_d{N}\biggl( \frac{(\rho A_{zz}^{-1}\rho)^{-1/2}\rho A_{zz}^{-1}\rho^*\theta_0+(\rho A_{zz}^{-1}\rho)^{1/2}(\theta_0 - \theta_m)}{\hat\sigma_{\omega_0}},1\biggr)\\
&\rightarrow_d{N}\biggl( \frac{(\rho A_{zz}^{-1}\rho)^{1/2}((1+\lambda)\theta_0 - \theta_m)}{\hat\sigma_{\omega_0}},1\biggr)\\
\end{align*}
where $\lambda =(\rho A_{zz}^{-1}\rho)^{-1}\rho A_{zz}^{-1}\rho^*$.  Thus,
\begin{align}
    T^{EB}&\rightarrow_d\chi^2_{2}\bigg(\frac{((1+\lambda)\theta_0 - \theta_m)'(\rho A_{zz}^{-1}\rho)((1+\lambda)\theta_0 - \theta_m)}{\sigma_{\omega_0}^2}\bigg)\\
    &= \chi^2_{2}\bigg(\frac{((1+\lambda)\theta_0 - \theta_m)' E[\tilde\Delta_{ni}\tilde\Delta_{ni}'] ((1+\lambda)\theta_0 - \theta_m)}{\sigma_{\omega_0}^2}\bigg)
\end{align}

\item[\textbf{(ii) - AR }] To derive the distribution of the test statistic, we first consider:
\begin{align*}
\sqrt{n}\hat\pi_m  &= \sqrt{n}(z'z)^{-1}z'(p - \Delta\theta_m)\\
&= \sqrt{n}(z'z)^{-1}z'(\Delta^*\theta_0 + \omega_0 - \Delta\theta_m)\\
&= \hat A_{zz}^{-1}\sqrt{n}(\hat A_{z'\Delta^*}\theta_0-\hat A_{z'\Delta}\theta_m) + \hat A_{zz}^{-1}\frac{z'\omega_0}{\sqrt{n}} \\
&\rightarrow_d \mathcal{N}\biggl(A_{zz}^{-1} \rho^*\theta_0 + A_{zz}^{-1}\rho(\theta_0-\theta_m) ,A_{zz}^{-1}\sigma^2_{\omega_0}\biggr) 
\end{align*}
Thus,
\begin{align}
    T^{AR}&\rightarrow_d\chi^2_{d_z}\bigg(\frac{( \rho^*\theta_0 +\rho(\theta_0-\theta_m))' A_{zz}^{-1}( \rho^*\theta_0 +\rho(\theta_0-\theta_m)) }{\sigma_{\omega_0}^2}\bigg)\\
  &=\chi^2_{d_z}\bigg(\frac{E[(\tilde\Delta^*_{n,0i} - \tilde\Delta_{n,mi})^2]}{\sigma_{\omega_0}^2}\bigg)  
\end{align}

\item[\textbf{(iii) - RV }]
\begin{align*}
\sqrt{n}(Q_1 - Q_2) &= \bigg(\sqrt{n}\bigg(\hat\psi_1-2\hat\psi_0 +  \hat\psi_2 \bigg) +\sqrt{n}(\Gamma_1 + \Gamma_2 - 2\Gamma_0)\bigg)'\frac{z'z}{n}\bigg(\hat\psi_1 -\hat\psi_2+\Gamma_1 - \Gamma_2\bigg)+\\&\qquad 2\bigg(\hat\psi_2-\hat\psi_1 +\Gamma_2-\Gamma_1\bigg)'\frac{z'\omega_0}{\sqrt{n}}
  \end{align*}
Suppose $\hat\Gamma_1 + \hat\Gamma_2 - 2\hat\Gamma_0 = \frac{c}{\sqrt{n}}$. Further suppose that $\hat\Gamma_1-\hat\Gamma_2 =d\neq 0$.  Then we have
\begin{align*}
\sqrt{n}(Q_1 - Q_2) &= \bigg( c\bigg)'\frac{z'z}{n}\bigg(d\bigg)+ 2\bigg(d\bigg)'\frac{z'\omega_0}{\sqrt{n}}\\
&\rightarrow_d \mathcal{N}(c'A_{zz}d,4dA_{zz}d\sigma^2_{\omega_0})\\
&\rightarrow_d \mathcal{N}(\Gamma_0-\Gamma_1+\Gamma_0-\Gamma_2)'E[z_iz_i'](\Gamma_0-\Gamma_1-(\Gamma_0-\Gamma_2)),4dA_{zz}d\sigma^2_{\omega_0})\\
&\rightarrow_d \mathcal{N}E[(\tilde\Delta_{0i}-\tilde\Delta_{1i}+\tilde\Delta_{0i}-\tilde\Delta_{2i})'(\tilde\Delta_{0i}-\tilde\Delta_{1i}-(\tilde\Delta_{0i}-\tilde\Delta_{2i})]),4dA_{zz}d\sigma^2_{\omega_0})\\
&= \mathcal{N}E[(\tilde\Delta_{0i}-\tilde\Delta_{1i})^2+(\tilde\Delta_{0i}-\tilde\Delta_{2i})^2],4E[((\tilde\Delta_{0i}-\tilde\Delta_{1i}- (\tilde\Delta_{0i}-\tilde\Delta_{2i}))^2](\sigma^2_{\omega_0})\\
  \end{align*}
  So we have, under the approximation of the asymptotic variance given in (\ref{eq:avarapprox}):
\begin{align}
 T^{RV} 
&\rightarrow_p \lim_{n\rightarrow\infty} \sqrt{n}\frac{E[(\theta_0 \tilde\Delta^*_{i} -\theta_1 \tilde\Delta_i)^2] - E[(\theta_0 \tilde\Delta^*_{i} -\theta_2 \tilde\Delta_i)^2]}{\sigma_{RV}}\\
&\approx\lim_{n\rightarrow\infty} \sqrt{n}\frac{ E[(\theta_0 \tilde\Delta^*_{i} -\theta_1 \tilde\Delta_i)^2] - E[(\theta_0 \tilde\Delta^*_{i} -\theta_2 \tilde\Delta_i)^2]}{2\sigma_{\omega_0}\sqrt{E[(\tilde\Delta_{1i}-\tilde\Delta_{2i})^2]]}}\\
&=\lim_{n\rightarrow\infty}\sqrt{n} \frac{E\bigg[\bigg((\tilde\Delta^*_{0i}-\tilde\Delta^*_{1i}) +(\tilde\Delta^*_{1i}-\tilde\Delta_{1i}) \bigg)^2-\bigg((\tilde\Delta^*_{0i}-\tilde\Delta^*_{2i}) +(\tilde\Delta^*_{2i}-\tilde\Delta_{2i}) \bigg)^2\bigg]}{2\sigma_{\omega_0} \sqrt{E[(\tilde\Delta_{1i}-\tilde\Delta_{2i})^2]}}.
\end{align} 



Define
$$\hat B = \bigg((\theta_2-\theta_1)'\hat A_{\Delta z} \hat A_{zz}^{-1} \hat A_{z\Delta} (\theta_2-\theta_1)\bigg)^{-1/2}$$
To derive the distribution of the test statistic, we first consider:
\begin{align*}
\sqrt{n}\hat B(Q_1 - Q_2) 
&= \sqrt{n}\hat B\frac{1}{n}(\Delta^*\theta_0 - \Delta\theta_1+ \omega_0)' P_z(\Delta^*\theta_0- \Delta\theta_1+ \sqrt{n}\hat B\omega_0) \\
&\qquad - \sqrt{n}\hat B\frac{1}{n}(\Delta^*\theta_0 - \sqrt{n}\hat B\Delta\theta_2+ \omega_0)'  P_z(\Delta^*\theta_0 - \Delta\theta_2+ \omega_0)\\
&= \bigg((\theta_2-\theta_1)'\sqrt{n}\hat A_{\Delta z} \hat A_{zz}^{-1} \sqrt{n}\hat A_{z\Delta} (\theta_2-\theta_1)\bigg)^{-1/2}\times\\
&\qquad\qquad\sqrt{n}(\theta_0\hat A_{\Delta^*z} -\theta_1\hat A_{\Delta z})' \hat A_{zz}^{-1}\sqrt{n}(\hat A_{\Delta^*z}\theta_0 - \hat A_{\Delta z}\theta_1) \\
&\,\,- \bigg((\theta_2-\theta_1)'\sqrt{n}\hat A_{\Delta z} \hat A_{zz}^{-1} \sqrt{n}\hat A_{z\Delta} (\theta_2-\theta_1)\bigg)^{-1/2}\times \\
&\qquad\qquad\sqrt{n}(\theta_0\hat A_{\Delta^*z} -\theta_2\hat A_{\Delta z})' \hat A_{zz}^{-1}\sqrt{n}(\hat A_{\Delta^*z}\theta_0 - \hat A_{\Delta z}\theta_2) \\
&\,\,+ 2\bigg((\theta_2-\theta_1)'\sqrt{n}\hat A_{\Delta z} \hat A_{zz}^{-1} \sqrt{n}\hat A_{z\Delta} (\theta_2-\theta_1)\bigg)^{-1/2}\times \\
&\qquad\qquad(\theta_2-\theta_1)\sqrt{n}\hat A_{\Delta z} \hat A_{zz}^{-1} \frac{\omega_0'z}{\sqrt{n}}\\
&\rightarrow_d\mathcal{N}\biggl( \bigg((\theta_2-\theta_1)'\rho A_{zz}^{-1} \rho (\theta_2-\theta_1)\bigg)^{-1/2} \mu^{I,II},4\sigma^2_{\omega_0}\biggr)
\end{align*}
where
$$\mu^{I,II}= \bigg(\rho^*\theta_0 + \rho(\theta_0-\theta_1)\bigg)'A_{zz}^{-1}\bigg(\rho^*\theta_0 + \rho(\theta_0-\theta_1)\bigg)-\bigg(\rho^*\theta_0 + \rho(\theta_0-\theta_2)\bigg)'A_{zz}^{-1}\bigg(\rho^*\theta_0 + \rho(\theta_0-\theta_2)\bigg)$$
So that, if we square the RV test statistic, we obtain:
 \begin{align}
 (T^{RV})^2 &\rightarrow_d\chi^2_{1}\bigg(\frac{1}{4\sigma_{\omega_0}^2}\bigg(\frac{E[(\tilde\Delta^*_{n,0i} - \tilde\Delta_{n,1i})^2]}{E[(\tilde\Delta_{n,1i} - \tilde\Delta_{n,2i})^2]^{1/2}}-\frac{E[(\tilde\Delta^*_{n,0i} - \tilde\Delta_{n,2i})^2]}{E[(\tilde\Delta_{n,1i} - \tilde\Delta_{n,2i})^2]^{1/2}}\bigg)^2\bigg).
% &= \chi^2_{1}\bigg(\frac{{c^*_{1}^2}/{c_{1,2}}-{c^*_{2}^2}/{c_{1,2}}}{4\sigma_{\omega_0}^2}\bigg) 
\end{align}

\item[\textbf{(iv) - Cox }] To derive the distribution of the test statistic consider:
\begin{align*}
\sqrt{n}\hat B T^{Cox,m}&= \sqrt{n}\hat B \bigg( Q_{-m}-Q_m -\frac{1}{n}(g_m - g_{-m} )'W(g_m - g_{-m} )\bigg)\\
&=\sqrt{n} \hat B ( Q_{-m}-Q_m)-\sqrt{n} \hat B (\theta_m - \theta_{-m})'\hat A_{\Delta z}\hat A_{zz}^{-1}\hat A_{z\Delta}(\theta_m - \theta_{-m})\\
&=\sqrt{n} \hat B ( Q_{-m}-Q_m) -  \bigg((\theta_2-\theta_1)'\sqrt{n}\hat A_{\Delta z} A_{zz}^{-1}\sqrt{n} \hat A_{z\Delta} (\theta_2-\theta_1)\bigg)^{-1/2}\times \\
&\qquad(\theta_m - \theta_{-m})'\sqrt{n}\hat A_{\Delta z}\hat A_{zz}^{-1}\sqrt{n}\hat A_{z\Delta}(\theta_m - \theta_{-m})\\
&\rightarrow_d\mathcal{N}( \bigg((\theta_m-\theta_{-m})'\rho A_{zz}^{-1} \rho (\theta_m-\theta_{-m})\bigg)^{-1/2} \mu^{cox,m},4\sigma^2_{\omega_0})
\end{align*}
where
\begin{align*}
\mu^{cox,m}&= \bigg(\rho^*\theta_0 + \rho(\theta_0-\theta_{-m})\bigg)'A_{zz}^{-1}\bigg(\rho^*\theta_0 + \rho(\theta_0-\theta_{-m})\bigg)\\
&\qquad-\bigg(\rho^*\theta_0 + \rho(\theta_0-\theta_m)\bigg)'A_{zz}^{-1}\bigg(\rho^*\theta_0 + \rho(\theta_0-\theta_m)\bigg)\\
&\qquad -(\theta_{-m}-\theta_{m})'\rho'A_{zz}^{-1}\rho(\theta_{-m}-\theta_{m})
\end{align*}
%\footnote{If $\theta_{-m} = \theta_0$ and $\Delta^* = \Delta$, then $\rho^* = 0$ and $\mu^{cox,m} = 2\mu^{I,II}$.  Meanwhile if $\theta_m = \theta_0$, $\mu^{cox,m} = 2\mu^{I,II} = 0$}
So that, if we square the Cox test statistic, we obtain:
 \begin{align}
 (T^{cox})^2 &\rightarrow_d\chi^2_{1}\bigg(
 \bigg(\frac{E[(\tilde\Delta^*_{n,0i} - \tilde\Delta_{n,1i})^2] - E[(\tilde\Delta^*_{n,0i} - \tilde\Delta_{n,2i})^2] - E[(\tilde\Delta_{n,1i} - \tilde\Delta_{n,2i})^2]}{2\sigma_{\omega_0}E[(\tilde\Delta_{n,1i} - \tilde\Delta_{n,2i})^2]^{1/2}}\bigg)^2\bigg)\\
 &= \chi^2_{1}\bigg(\frac{{c^{*2}_{1}}/{c_{1,2}}-{c^{*2}_{2}}/{c_{1,2}}-{c_{1,2}}}{4\sigma_{\omega_0}^2}\bigg) 
  \end{align}
  
\end{itemize}
\end{proof}

==> Submission/ReStud/Proofs/Pf_ConvergDistrib_NoMisspecification.tex <==
\textbf{Remarks on Local Alternatives} - We start with some preliminary discussion of our definition of local alternatives.
We assume in Proposition 2 that: 
\begin{align}
    \hat A_{z\Delta} = \frac{z'\Delta}{n} = \frac{\rho}{\sqrt{n}} + o_p(n^{-1/2}), \label{eq:localAltI}
\end{align}    
where $\rho$ is a finite matrix, which intuitively means that the covariation between instruments and markups implied by the two models vanishes as the sample size increases. In the spirit of local power analysis, this is not a restriction to take literally, but rather to use as a tool to approximate the finite sample power of the tests we consider in a challenging environment where the two models are hard to tell apart. 

Most standard local power analysis is done by imposing that the parameters that characterize the alternative hypothesis get closer to the truth at a certain rate. In the spirit of the literature on non-nested hypothesis testing and model testing (e.g. Pesaran, 1982; Smith, 1992), we adopt instead a restriction on the joint distribution of the data $(z,\Delta),$ imposing that a certain moment vanishes at a rate that allows to control the asymptotic distribution of the test statistics under the alternative hypothesis. 

It is worth noticing some of the implications of our assumption (\ref{eq:localAltI}). First, notice that our definition of local alternatives implies that:
\begin{align}
g_m=\frac{z'\omega_m}{n} = \frac{g}{\sqrt{n}} + o_p(n^{-1/2}). \label{eq:localAltII}
\end{align}
where $g$ is a finite $d_z-$vector.
In fact consider:
\begin{align}
    g_m &=\frac{z'(\omega_0 + \Delta(\theta_0 - \theta_m))}{n}\\
        &= \frac{z'\Delta}{n} (\theta_0 - \theta_m) + o_p(1)  \label{eq:localAltIII}
\end{align}
Then, if (\ref{eq:localAltI}) holds, it follows immediately that $g_m=\frac{\rho}{\sqrt{n}} (\theta_0 - \theta_m) + o_p(n^{-1/2})$, which implies that (\ref{eq:localAltII}) holds for $g=\rho (\theta_0 - \theta_m)$. The condition (\ref{eq:localAltII}) is similar to the definition of local alternatives adopted in Marmer and Otsu (2012).

Notice moreover that we can write the estimator of the first stage parameter $\hat \Gamma$ as:
\begin{align*}
    \hat \Gamma = (\frac{z'z}{n})^{-1}\frac{z'\Delta}{n},
\end{align*}
so that its population equivalent is 
\begin{align*}
    \Gamma = \Gamma_n = A_{zz}^{-1}\frac{g}{\sqrt{n}},
\end{align*}
where the last equality follows from assumption (\ref{eq:localAltI}). Hence, our assumption, though stronger, implies the condition on $\Gamma$ routinely used to analyze asymptotics with weak instruments (Stock and Staiger, 1997). 

\begin{proof}[Proof of Proposition 2]
We will use in what follows the following facts, which are a consequence of the assumptions of the proposition:
\begin{align}
    \sqrt{n}\hat A_{\Delta z} &= \rho + o_p(1)\\
    \hat A_{z z} &= A_{z z} + o_p(1)\\
    \frac{z'\omega_0}{\sqrt{n}} &\rightarrow_d N(0,A_{z z}\sigma_{\omega_0}^2)\\
    \hat \sigma^2_{\omega_0} &= \sigma_{\omega_0}^2 + o_p(1)
\end{align}
The latter three statements follow from the standard assumptions required for the consistency and asymptotic normality of the GMM estimator $\hat \theta,$ and homoscedasticity of the error terms.
To derive the non-centrality parameter, it is also useful to note:
\begin{align}
\sqrt{n}\hat A_{\Delta z}\hat A_{zz}^{-1} & = \Gamma_n + o_p(1)\\
\sqrt{n}\hat A_{\Delta z}\hat A_{zz}^{-1} z & = \tilde\Delta_n + o_p(1)\\
\sqrt{n}\hat A_{\Delta z}\hat A_{zz}^{-1} \sqrt{n}\hat A_{z\Delta} &= \sqrt{n}\hat A_{\Delta z}\hat A_{zz}^{-1}\hat A_{zz}\hat A_{zz}^{-1} \sqrt{n}\hat A_{z\Delta}  \\&=E[\rho' A_{zz}^{-1} z_i z_i' A_{zz}^{-1} \rho] + o_p(1) \\&= E[\tilde\Delta_{ni}\tilde\Delta_{ni}'] + o_p(1)
\end{align}
These statements are either definitions, or follow from the assumptions above.

We assume in the proposition that the true parameter is $\theta_0$ and the null hypothesis for AR, EB and Cox is model $m$ such that $\theta_m\neq\theta_0$. We also define the constant:
\begin{align}
c = (\theta_0 - \theta_m)'E[\tilde\Delta_{ni}\tilde\Delta_{ni}'](\theta_0 - \theta_m).
\end{align}


\item[\textbf{(i) - EB}] For EB, notice that - since under our assumptions the variance of the estimator is 
\begin{align}
    \hat V_{\theta} = (\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1} \hat \sigma^2_{\omega_0}
\end{align}

the Wald test statistic for the null $\theta_0 = \theta_m$ can be written as :
\begin{align}
T^{EB,m} &= \frac{\zeta'\zeta}{\hat \sigma^2_{\omega_0}/ \sigma_{\omega_0}^2} \label{eq:TestStatEB_Pesaran}
\end{align}
where 
\begin{align}
    \zeta = \frac{(\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{1/2}}{\sigma_{\omega_0}}(\sqrt{n}(\hat\theta - \theta_m))
\end{align}
Notice moreover that
\begin{align*}
\hat\theta  &= (\Delta'P_z\Delta)^{-1}\Delta'P_zp \\
&= \theta_0 + (\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}\hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{n},
\end{align*}
so that 
\begin{align*}
    \zeta &= \frac{(\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{1/2}}{\sigma_{\omega_0}}(\sqrt{n}(\theta_0 - \theta_m)) + \frac{(\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1/2}}{\sigma_{\omega_0}} \hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{\sqrt{n}}\\
    &= \frac{(\sqrt{n}\hat A_{\Delta z} \hat A_{z z}^{-1}  \sqrt{n} \hat A_{z\Delta})^{1/2}}{\sigma_{\omega_0}}(\theta_0 - \theta_m) + \frac{(\sqrt{n}\hat A_{\Delta z} \hat A_{z z}^{-1} \sqrt{n}\hat A_{z\Delta})^{-1/2}}{\sigma_{\omega_0}} \sqrt{n}\hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{\sqrt{n}}
\end{align*}
from which it follows that, by applying the generalized Slutsky theorem and the facts stated above, that:

\begin{align*}
    \zeta \rightarrow_d N\bigg(\frac{(\rho' A_{z z}^{-1}  \rho)^{1/2}}{\sigma_{\omega_0}}(\theta_0 - \theta_m),1\bigg).
\end{align*}

Hence, using the definition of the EB test statistic in Equation (\ref{eq:TestStatEB_Pesaran}), we have the following convergence in distribution result:

\begin{align}
    T^{EB}\rightarrow_d\chi^2_{2}\bigg(\frac{c}{\sigma_{\omega_0}^2}\bigg),
\end{align}
since
\begin{align*}
    (\theta_0 - \theta_m)'\rho' A_{z z}^{-1}  \rho(\theta_0 - \theta_m) = c.   
\end{align*}

\item[\textbf{(ii) - AR}] For AR, we first consider the estimator $\hat\pi_m$
\begin{align*}
\hat\pi_m  &= (z'z)^{-1}z'(p - \Delta\theta_m)\\
&= \hat A_{zz}^{-1}\hat A_{z'\Delta}(\theta_0-\theta_m) + \hat A_{zz}^{-1}\frac{z'\omega_0}{n}, 
\end{align*}
and, under the assumption of homoskedasticity, $\hat V_{\pi_m}$, a consistent estimator of the asymptotic variance $V_{\pi_m}$,  is:
\begin{align}
V_{\pi_m} = \sigma^2_{\omega_{0}}A_{z z}^{-1} .  
\end{align}

So, we have
\begin{align}
\sqrt{n}\hat V_{\pi_m}^{-1/2} \hat\pi_m &=\bigg( \frac{\hat A_{zz}^{-1/2} \sqrt{n} \hat A_{z \Delta}'(\theta_0-\theta_m) +\hat A_{zz}^{-1/2} \frac{z'\omega_0}{\sqrt{n}}}{\hat\sigma_{\omega_0}}\bigg)\\
&\rightarrow_d \mathcal{N}\bigg( \frac{A_{zz}^{-1/2}\rho(\theta_0-\theta_m) }{\sigma_{\omega_0}},1\bigg),
\end{align}
and we can derive the asymptotic distribution of the AR test statistic:
\begin{align}
T^{AR,m} &\rightarrow_d \chi^2_{d_z}\bigg(\frac{(\theta_0-\theta_m)'\rho A_{zz}^{-1}\rho(\theta_0-\theta_m)}{\sigma^2_{\omega_{0}}}\bigg)\\
& =\chi^2_{d_z}\bigg(\frac{c}{\sigma^2_{\omega_{0}}}\bigg).
\end{align}


\item[\textbf{(iii) - RV}] First consider the object :
\begin{align*}
 Q_1 - Q_2&= g_1'Wg_1 - g_2'Wg_2\\
&=\frac{\omega^{I\prime} z}{n}(\frac{z'z}{n})^{-1}\frac{z'\omega^I}{n} - \frac{\omega^{II\prime} z}{n}(\frac{z'z}{n})^{-1}\frac{z'\omega^{II}}{n}\\
&= \frac{1}{n}(\Delta(\theta_0 - \theta_1)+ \omega_0)' P_z(\Delta(\theta_0 - \theta_1)+ \omega_0)- \frac{1}{n}(\Delta(\theta_0 -\theta_2)+ \omega_0)'  P_z(\Delta(\theta_0 - \theta_2)+ \omega_0)\\
&= -(\theta_1 - \theta_2)'\hat A_{z\Delta}'\hat A_{zz}^{-1}\hat A_{z\Delta}(\theta_1 - \theta_2)- 2(\theta_2 - \theta_1)'\hat A_{z\Delta}'\hat A_{zz}^{-1}\frac{z'\omega_0}{n}.
\end{align*}
Under the assumption of homoskedasticity, the estimator of the asymptotic variance of $\sqrt{n} (Q_1 - Q_2)$ is:
\begin{align}
    \hat\sigma_{RV}^2 = 4\hat\sigma_{\omega_0}^2(\theta_2 - \theta_1)'\hat A_{z \Delta}'\hat A_{zz}^{-1}\hat A_{z \Delta}(\theta_2 - \theta_1),
\end{align}
So that we can write:
\begin{align}
T^{RV} &= \sqrt{n}\frac{Q_1-Q_2}{\hat\sigma_{RV}}\\
&=-\frac{1}{2\hat\sigma_{\omega_0}}\bigg((\theta_2 - \theta_1)'\sqrt{n}\hat A_{z \Delta}'\hat A_{zz}^{-1}\sqrt{n}\hat A_{z \Delta}(\theta_2 - \theta_1)\bigg)^{1/2}\\
&\qquad  -\frac{1}{\hat\sigma_{\omega_0}}\bigg((\theta_2 - \theta_1)'\sqrt{n}\hat A_{z \Delta}'\hat A_{zz}^{-1}\sqrt{n}\hat A_{z \Delta}(\theta_2 - \theta_1)\bigg)^{-1/2}(\theta_2 - \theta_1)'\sqrt{n}\hat A_{z \Delta}'\hat A_{zz}^{-1}\frac{z'\omega_0}{\sqrt{n}}
\end{align}
For convergence in distribution, after applying the CLT, we have:
\begin{align}
T^{RV} &\rightarrow_d \mathcal{N}\bigg(\frac{\bigg((\theta_2 - \theta_1)'E[\tilde\Delta_{ni}\tilde\Delta_{ni}'](\theta_2 - \theta_1)\bigg)^{1/2}}{2\sigma_{\omega_0}},1\bigg)\\
&=\mathcal{N}\bigg(\frac{\bigg(E[(\tilde\Delta_{2ni}-\tilde\Delta_{1ni})^2]\bigg)^{1/2}}{2\sigma_{\omega_0}},1\bigg)\\
&=\mathcal{N}\bigg(\frac{\sqrt{c}}{2\sigma_{\omega_0}},1\bigg).
\end{align} 
Therefore
$$(T^{RV})^2\rightarrow_d \chi^2_{1}\bigg(\frac{c}{4\sigma^2_{\omega_0}} \bigg).$$


\item[\textbf{(iv) - Cox}] To derive the asymptotic distribution of the Cox test statistic, recall that $\theta_0 = \theta_{-m}$.  
Since the numerator of the test statistic is 
\begin{align*}
    \frac{\hat \sigma^{Cox,m}}{\sqrt{n}} T^{Cox,m} &=Q_{-m} - Q_m -(g_{-m} - g_m)'\hat A_{zz}^{-1}(g_{-m} - g_m),
\end{align*}
so that the first two terms equal the numerator of the RV test statistic. We conjecture (and verify at the end) that in this environment the asymptotic variance of the Cox test statistic is equal to the one of the RV test statistic, so that we can write
\begin{align*}
    T^{Cox,m} - T^{RV}=  - \frac{\sqrt{n}}{\hat \sigma^{RV}}(g_{-m} - g_m)'\hat A_{zz}^{-1}(g_{-m} - g_m),
\end{align*}
and for this term notice
\begin{align*}
- \frac{\sqrt{n}}{\hat \sigma^{RV}}(g_{-m} - g_m)'\hat A_{zz}^{-1}(g_{-m} - g_m)    &=-\frac{\sqrt{n}}{\hat \sigma^{RV}}(\theta_m - \theta_{-m})'\hat A_{z\Delta}' \hat A_{zz}^{-1} \hat A_{z\Delta}(\theta_m - \theta_{-m})\\
&= -\frac{1}{2 \hat \sigma_{\omega_0}}\bigg((\theta_m - \theta_{-m})'\sqrt{n}\hat A_{z\Delta}' \hat A_{zz}^{-1} \sqrt{n}\hat A_{z\Delta}(\theta_m - \theta_{-m})\bigg)^{1/2}\\
&\rightarrow_p -\frac{1}{2 \hat \sigma_{\omega_0}}\bigg((\theta_m - \theta_{-m})'E[\tilde\Delta_{ni}\tilde\Delta_{ni}'](\theta_m - \theta_{-m})\bigg)^{1/2}\\
&= -\frac{c^{1/2}}{2 \hat \sigma_{\omega_0}}
\end{align*}
So that, since this term converges in probability to a constant, the asymptotic variance for the Cox statistic that we conjecture is correct. In fact:
\begin{align}
    T^{Cox,m}\rightarrow_d N\bigg(\frac{c^{1/2}}{\hat \sigma_{\omega_0}},1\bigg)
\end{align}
\noindent Following the results above, we obtain 
\begin{align}
(T^{cox})^2 \rightarrow_d \chi^2_1\bigg(\frac{c}{\sigma^2_{\omega_0}}\bigg).
\end{align}

\end{proof}



==> Submission/ReStud/Proofs/Pf_ConvergProb_Misspecification.tex <==
\begin{proof}[Proof of Proposition \ref{prop:distrib_TE2}.]
For $(i)$, we use Equations \eqref{eq:line2} and \eqref{eq:line5} in addition to the definition of the local alternative in Equation \eqref{eq:local selection} to write
\begin{align}
\sqrt{n}\left( Q_1 -Q_2 \right) &= \sqrt{n}\left( (\Gamma_0-\Gamma_1) - (\Gamma_0-\Gamma_2) \right)\!' E[z_iz_i']\!\left( (\Gamma_0-\Gamma_1) + (\Gamma_0-\Gamma_2) \right)\! \\
&= q'E[z_iz_i']\!\left( (\Gamma_0-\Gamma_1) + (\Gamma_0-\Gamma_2) \right)\!.
\end{align}
%From Lemma 1 in \cite{rv02} or the proof of Proposition \ref{prop:degen}, we have that Assumption \ref{as:nodegen} implies that $\sqrt{n}\left( Q_1 -Q_2 \right)$ is bounded away from zero.
%From Proposition \ref{prop:degen} and its proof, we have that Assumption \ref{as:nodegen} and the local alternative in \eqref{eq:local selection} implies that $(\Gamma_0-\Gamma_1) + (\Gamma_0-\Gamma_2)$ is bounded away from zero. Furthermore, 
Assumption \ref{as:regcond}, part (iii), implies that $(\Gamma_0-\Gamma_1) + (\Gamma_0-\Gamma_2) $ is bounded. We therefore assume essentially without loss of generality that $\sqrt{n}\left( Q_1 -Q_2 \right)$ is a constant, say $c$.\footnote{This assumption is essentially without loss of generality since the boundedness of $(\Gamma_0-\Gamma_1) + (\Gamma_0-\Gamma_2)$, and therefore of $\sqrt{n}\left( Q_1 -Q_2 \right)$, allows us to otherwise argue along subsequences where $\sqrt{n}\left( Q_1 -Q_2 \right)$ converges to a constant.} From Equations \eqref{eq:line1} and \eqref{eq:line5}, we can also write 
\begin{align}
    c &= \sqrt{n} \!\left( E\!\left[(\Delta_{0i}^{z}-\Delta_{1i}^z)^2\right] - E\!\left[(\Delta_{0i}^{z}-\Delta_{2i}^z)^2\right] \right) \\
    &= E\!\big[(\Delta_{0i}^{\text{RV},z}-\Delta_{1i}^{\text{RV},z})^2\big] - E\!\big[(\Delta_{0i}^{\text{RV},z}-\Delta_{2i}^{\text{RV},z})^2\big].
\end{align}

As in Remark \ref{rem:validity}, a first order Taylor expansion, Lemma \ref{lem:asymp norm}, parts $(i)$ and $(ii)$, together with consistency of $\hat \sigma^2_\text{RV}$ now leads to
\begin{align}
    T^\text{RV} = \frac{c}{\sigma_\text{RV}} + \frac{g_1'W^{1/2} \hat W^{1/2}\hat g_1 - g_2'W^{1/2} \hat W^{1/2}\hat g_2}{\sigma_\text{RV}} + o_p(1) \xrightarrow{d} N(c,1).
\end{align}

For $(ii)$, we first note that Assumption \ref{as:homsked} implies that
\begin{align}
    V^\text{AR}_{mm} = E[z_iz_i']\inverse E[e_{mi}^2 z_iz_i'] E[z_iz_i']\inverse = \sigma_m^2 E[z_iz_i'].
\end{align}
Thus we have from Equations \eqref{eq:line2} and \eqref{eq:line5} that 
\begin{align}
    \sigma_m^2 n\pi_m'\big( V^\text{AR}_{mm}\big)\inverse\pi_m = n(\Gamma_0-\Gamma_m)'E[z_i z_i'](\Gamma_0-\Gamma_m) = q_m'E[z_i z_i']q_m
\end{align}
which in turn yields that $n\pi_m'\big( V^\text{AR}_{mm}\big)\inverse\pi_m = E\big[(\Delta^{\text{AR},z}_{0i}-\Delta^{\text{AR},z}_{mi}) ^2\big]/\sigma_m^2$ is a constant, say $c_m$. From Lemma \ref{lem:asymp norm}, parts $(iii)$ and $(iv)$, and continuous mapping we then have
\begin{align}
    T_m^\text{AR} &= n \hat \pi_m'\big( \hat V^\text{AR}_{mm}\big)\inverse \hat \pi_m = n \hat \pi_m'\big( V^\text{AR}_{mm}\big)\inverse \hat \pi_m + o_p(1) \xrightarrow{d} \chi^2_{d_z}(c_m). \qedhere
\end{align}
%
\begin{comment}
It is useful to note the following identities for each model $m$:
\begin{align}
\omega_m &= p-\Delta\theta_m\\
\omega_m &= \Delta^{*}\theta_0-\Delta\theta_m + \omega_0\\
\omega_m &= \Delta^{*}_0-\Delta_m + \omega_0.
\end{align}
Since in this environment true markups $\Delta^*$ differ from observed markups $\Delta$, we need the following definitions:
\begin{align}
A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta^*} &=  E[\tilde\Delta_{i} \tilde\Delta^{*\prime}_{i}], 
\end{align}
and
\begin{align}
    \lambda = E[\tilde\Delta_{i} \tilde\Delta_{i}']^{-1}E[\tilde\Delta_{i} \tilde\Delta^{*\prime}_{i}].
\end{align}

\begin{enumerate}
\item[\textbf{(i) - EB}] For EB, we first consider the object $\hat\theta$
\begin{align*}
\hat\theta  &= (\Delta'P_z\Delta)^{-1}\Delta'P_zp\\
&=  (\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}\hat A_{\Delta z} \hat A_{z z}^{-1}\hat A_{z\Delta^*}\theta_0+  (\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}\hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{n}\\
&\rightarrow_p (A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1} A_{\Delta z}  A_{z z}^{-1}A_{z\Delta^*}\theta_0+ (A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1} A_{\Delta z}  A_{z z}^{-1} E[z_i \omega_{0i}']\\
&=\lambda\theta_0
\end{align*}
So we have, approximating the asymptotic variance with the expression (\ref{eq:avarapprox})\footnote{Since the proposition concerns the plim of the test statistic, adopting this approximation does not alter the result.}:
\begin{align}
{n}(\hat\theta - \theta_m)'\hat V_{\theta}^{-1} (\hat\theta - \theta_m)
&\rightarrow_p \lim_{n\rightarrow\infty} {n}( (\lambda\theta_0- \theta_m)' V_{\theta}^{-1}( \lambda\theta_0- \theta_m))\\
&\approx \lim_{n\rightarrow\infty} {n}\frac{( \lambda\theta_0- \theta_m)'  E[\tilde\Delta_{i}\tilde\Delta_{i}']( \lambda\theta_0- \theta_m)}{\sigma^2_{\omega_0}}\\
&= \lim_{n\rightarrow\infty} {n}\frac{E[(\theta_0'\lambda\tilde\Delta_{i}-\tilde\Delta_{mi})^2]}{\sigma^2_{\omega_0}}\\
&=\lim_{n\rightarrow\infty} {n}\frac{ E\bigg[\bigg((\tilde{\tilde{\Delta}}^{*}_{0i}-\tilde\Delta_{0i})+(\tilde\Delta_{0i}-\tilde\Delta_{mi})\bigg)^2\bigg] }{\sigma^2_{\omega_{0}}}.
\end{align}
Note that, by Proposition \ref{prop:absfit}, $\tilde{\tilde{\Delta}}^*_{0i} = \tilde\Delta^*_{0i}$
\item[\textbf{(ii) - AR}] To derive the plim of the AR test statistic, we first consider the object $\hat\pi_m$
\begin{align*}
\hat\pi_m &= (z'z)^{-1}z'(\Delta^*\theta_0 + \omega_0 - \Delta\theta_m)\\
&= \hat A_{zz}^{-1}(\hat A_{z\Delta^*}\theta_0-\hat A_{z\Delta}\theta_m) + \hat A_{zz}^{-1}\frac{z'\omega_0}{n} \\
&\rightarrow_p A_{zz}^{-1} (A_{z\Delta^*}\theta_0-A_{z\Delta}\theta_m) + A_{zz}^{-1}E[z_i\omega_{0i}']\\
&=  \Gamma^*\theta_0-\Gamma\theta_m 
\end{align*}
So we have, under the approximation of the asymptotic variance given in (\ref{eq:avarapprox}):
\begin{align*}
T^{AR,m}&\rightarrow_p \lim_{n\rightarrow\infty} {n}(\Gamma^*\theta_0-\Gamma\theta_m)' V_{\pi_m}^{-1} (\Gamma^*\theta_0-\Gamma\theta_m)  \\
&\approx\lim_{n\rightarrow\infty} {n}\frac{(\Gamma^*\theta_0-\Gamma\theta_m)' A_{zz} (\Gamma^*\theta_0-\Gamma\theta_m)}{\sigma^2_{\omega_{0}}}  \\
&=\lim_{n\rightarrow\infty} {n}\frac{ E[(\tilde\Delta^*_{0i}-\tilde\Delta_{mi})^2] }{\sigma^2_{\omega_{0}}}  \\
&=\lim_{n\rightarrow\infty} {n}\frac{ E\bigg[\bigg((\tilde\Delta^*_{0i}-\tilde\Delta_{0i})+(\tilde\Delta_{0i}-\tilde\Delta_{mi})\bigg)^2\bigg] }{\sigma^2_{\omega_{0}}}  \\
\end{align*}

\item[\textbf{(iii) - RV}] To derive the plim of the RV test statistic we start from the object:

\begin{align*}
Q_1 - Q_2 
&= g_1'Wg_1 - g_2'Wg_2\\
&= \frac{1}{n}(\Delta^*\theta_0 - \Delta\theta_1+ \omega_0)' P_z(\Delta^*\theta_0 - \Delta\theta_1+ \omega_0)- \frac{1}{n}(\Delta^*\theta_0 - \Delta\theta_2+ \omega_0)'  P_z(\Delta^*\theta_0 - \Delta\theta_2+ \omega_0)\\
&= (\theta_0\hat A_{\Delta^*z} -\theta_1\hat A_{\Delta z})' \hat A_{zz}^{-1}(\hat A_{\Delta^*z}\theta_0 - \hat A_{\Delta z}\theta_1) - (\theta_0\hat A_{\Delta^*z} -\theta_2\hat A_{\Delta z})' \hat A_{zz}^{-1}(\hat A_{\Delta^*z}\theta_0 - \hat A_{\Delta z}\theta_2) \\
&\qquad+ 2(\theta_2-\theta_1)\hat A_{\Delta z} A_{zz}^{-1} \frac{\omega_0'z}{n}\\
& \rightarrow_p   (\theta_0 A_{\Delta^*z} -\theta_1 A_{\Delta z})'  A_{zz}^{-1}A_{zz}A_{zz}^{-1}( A_{\Delta^*z}\theta_0 - A_{\Delta z}\theta_1) \\
&\qquad- (\theta_0 A_{\Delta^*z} -\theta_2 A_{\Delta z})' A_{zz}^{-1}A_{zz}A_{zz}^{-1}( A_{\Delta^*z}\theta_0 -  A_{\Delta z}\theta_2)\\
& =  E[(\theta_0 \tilde\Delta^*_{i} -\theta_1 \tilde\Delta_i)^2] - E[(\theta_0 \tilde\Delta^*_{i} -\theta_2 \tilde\Delta_i)^2]
\end{align*}



\item[\textbf{(iv) - Cox}] For Cox, the numerator of the test statistic when using the formulation in Smith (1992) is:
 \begin{align*}
&  g_{-m}'A_{zz}^{-1}  g_{-m} - g_{m}'A_{zz}^{-1} g_m -(g_{-m} - g_m)'A_{zz}^{-1}(g_{-m} - g_m)\\
&= Q_{-m} - Q_m - (\theta_m'\hat A_{z\Delta*}' - \theta_{-m}'\hat A_{z\Delta}')\hat A_{z'z}^{-1}(\hat A_{z\Delta*}\theta_m - \hat A_{z\Delta}\theta_{-m}))\\
&\rightarrow_p  E[(\tilde\Delta^*_{0i}-\tilde\Delta_{-mi})^2] -E[(\tilde\Delta^*_{0i}-\tilde\Delta_{mi})^2]  - E[(\tilde\Delta^*_{mi}-\tilde\Delta_{-mi})^2] 
\end{align*}
So we have, under the approximation of the asymptotic variance given in (\ref{eq:avarapprox}):
\begin{align}
T^{cox,m}
&\rightarrow_p  2\lim_{n\rightarrow\infty} \sqrt{n}\frac{  E[(\tilde\Delta^*_{0i}-\tilde\Delta_{-mi})^2] -E[(\tilde\Delta^*_{0i}-\tilde\Delta_{mi})^2]  - E[(\tilde\Delta^*_{mi}-\tilde\Delta_{-mi})^2]  }{\sigma_{cox}} \\
&\approx 2\lim_{n\rightarrow\infty} \sqrt{n}\frac{  E[(\tilde\Delta^*_{0i}-\tilde\Delta_{-mi})^2] -E[(\tilde\Delta^*_{0i}-\tilde\Delta_{mi})^2]  - E[(\tilde\Delta^*_{mi}-\tilde\Delta_{-mi})^2]  }{2\sigma_{\omega_0} \sqrt{E[(\tilde\Delta_{1i}-\tilde\Delta_{2i})^2]}}.
\end{align} 
\end{enumerate}
\end{comment}
\end{proof}

==> Submission/ReStud/Proofs/Pf_ConvergProb_NoMisspecification.tex <==
\begin{proof}
\noindent We start by proving the first part of the proposition in which we show that the modified test statistics converge in probability to constants that depend on $E[(\tilde\Delta_{0i}-\tilde\Delta_{mi})^2]$.
\begin{enumerate}
\item[\textbf{(i) - EB}] 
Consider the test statistic $T^{EB,m}$ under the assumptions of weight matrix $W=A_{zz}^{-1}$ and homoskedasticity. We first consider the object $\hat\theta$:
\begin{align*}
\hat\theta  &= \theta_0 + (\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}\hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{n}
\end{align*}
and
\begin{align}
\hat V_{\hat \theta}  &= \frac{\hat \sigma^2_{\omega_{0}}}{n}(\hat A_{\Delta z}  \hat A_{z z}^{-1}  \hat A_{z\Delta})^{-1}\\
&= \hat \sigma^2_{\omega_{0}}(\Delta' z (z' z)^{-1}  z'\Delta)^{-1}
\end{align}
so that:
\begin{align}
    T^{EB,m} =& (\theta_0 - \theta_m)'\hat V_{\hat \theta}^{-1} (\theta_0 - \theta_m) \\
    &+\frac{\frac{z'\omega_0}{\sqrt{n}} \hat A_{z z}^{-1}\hat A_{z \Delta }(\hat A_{\Delta z}  \hat A_{z z}^{-1}  \hat A_{z\Delta})^{-1}\hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{\sqrt{n}}} {\hat \sigma^2_{\omega_{0}}} \\
    &+2n\frac{(\theta_0 - \theta_m)'\hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{n}}{\hat\sigma^2_{\omega_{0}}}\\
= & \frac{(\tilde \Delta_0 - \tilde \Delta_m)'(\tilde \Delta_0 - \tilde \Delta_m)}{\hat \sigma^2_{\omega_0}} + \zeta_{EB}'\zeta_{EB} + \frac{2n}{\hat\sigma^2_{\omega_{0}}}\frac{(\tilde \Delta_0 - \tilde \Delta_m)'\omega_0}{n}
\end{align}

To derive the plim of the test statistic $T^{EB,m}$, we first consider the object $\hat\theta$:
\begin{align*}
\hat\theta  &= (\Delta'P_z\Delta)^{-1}\Delta'P_z(\Delta\theta_0 + \omega_0)\\
&= \theta_0 + (\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}\hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{n}\\
&\rightarrow_p \theta_0. 
\end{align*}

Now, from standard GMM theory the asymptotic variance of $\hat \theta$ under homoskedasticity of the error term is 
\begin{align}
V_{\theta}  &= \sigma^2_{\omega_{0}}(A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1} \\
    &= \sigma^2_{\omega_{0}}E[\tilde\Delta_{i}\tilde\Delta_{i}']^{-1}.
\end{align}

Since $\hat V_{\theta}$ is a consistent estimator of $V_{\theta}$ we have:
\begin{align}
\frac{T^{EB,m}}{n}&\rightarrow_p \frac{(\theta_0 - \theta_m)' E[\tilde\Delta_{i}\tilde\Delta_{i}'](\theta_0 - \theta_m)}{\sigma^2_{\omega_{0}}}\\
&= \frac{ E[(\tilde\Delta_{0i} - \tilde\Delta_{mi})^2]}{\sigma^2_{\omega_{0}}}
\end{align}



\item[\textbf{(ii) - AR}] 
To derive the plim of the test statistic $T^{AR,m}$, we first consider the object $\hat\pi_m$
\begin{align*}
\hat\pi_m  &= (z'z)^{-1}z'(\Delta\theta_0 + \omega_0 - \Delta\theta_m)\\
&= \hat A_{zz}^{-1}\hat A_{z'\Delta}(\theta_0-\theta_m) + \hat A_{zz}^{-1}\frac{z'\omega_0}{n} \\
&\rightarrow_p A_{zz}^{-1} A_{z'\Delta}(\theta_0-\theta_m) .
\end{align*}
Under the assumption of homoskedasticity, $V_{\pi_m}$  has the usual OLS form of:
\begin{align}
V_{\pi_m} &= \sigma^2_{\eta_{m}}A_{z z}^{-1}   
\end{align}
Since $\hat V_{\pi_m}$ is constructed to be a consistent estimator of $V_{\pi_m}$ we have
\begin{align}
\frac{T^{AR,m}}{n}&\rightarrow_p  (\theta_0-\theta_m)'  A_{\Delta'z}A_{zz}^{-1}V^{-1}_{\pi_m}A_{zz}^{-1} A_{z'\Delta}(\theta_0-\theta_m) \\
&=  \frac{(\theta_0-\theta_m)' \Gamma'E[z_iz_i']\Gamma(\theta_0-\theta_m) }{\sigma^2_{\eta_{m}}}\\
&=  \frac{E[(\tilde\Delta_{0i}-\tilde\Delta_{mi})^2] }{\sigma^2_{\eta_{m}}}.
\end{align}

\item[\textbf{(iii) - RV}] To derive the plim for $T^{RV}$, first consider the object $Q_1 - Q_2$:
\begin{align*}
Q_1 - Q_2 
&= g_1'Wg_1 - g_2'Wg_2\\
&= \frac{1}{n}(\Delta(\theta_0 - \theta_1)+ \omega_0)' P_z(\Delta(\theta_0 - \theta_1)+ \omega_0)- \frac{1}{n}(\Delta(\theta_0 -\theta_2)+ \omega_0)'  P_z(\Delta(\theta_0 - \theta_2)+ \omega_0)\\
& \rightarrow_p  E[(\tilde\Delta_{0i}-\tilde\Delta_{1i})^2]-E[(\tilde\Delta_{0i}-\tilde\Delta_{2i})^2]
\end{align*}
So that, assuming $\hat\sigma_{RV} \rightarrow_p \sigma_{RV}$, we have
\begin{align}
\frac{T^{RV}}{\sqrt{n}}&= \frac{Q_1 - Q_2}{\hat\sigma_{RV}} \\
&\rightarrow_p \frac{E[(\tilde\Delta_{0i}-\tilde\Delta_{1i})^2]-E[(\tilde\Delta_{0i}-\tilde\Delta_{2i})^2]}{\sigma_{RV}}
\end{align} 
which is consistent with Theorem 1 (ii) in \cite{rv02}.

\item[\textbf{(iv) - Cox}] For the Cox procedure, notice that the numerator of the test statistic is 
\begin{align*}
    Q_{-m} - Q_m -(g_{-m} - g_m)'A_{zz}^{-1}(g_{-m} - g_m), 
\end{align*}
for which we obtain
 \begin{align*}
&g_{-m}'A_{zz}^{-1}  g_{-m} -g_{m}'A_{zz}^{-1} g_m -(g_{-m} - g_m)'A_{zz}^{-1}(g_{-m} - g_m)\\
&\rightarrow_p (\theta_0 - \theta_{-m})'A_{z\Delta}'A_{zz}^{-1}A_{z\Delta}(\theta_0 - \theta_{-m}) - (\theta_0 - \theta_m)'A_{z\Delta}'A_{zz}^{-1}A_{z\Delta}(\theta_0 - \theta_m)\\
&\qquad-(\theta_m - \theta_{-m})'A_{z\Delta}'A_{zz}^{-1}A_{z\Delta}(\theta_m - \theta_{-m})\\
 &= E[(\tilde\Delta_{0i}-\tilde\Delta_{-mi})^2] -E[(\tilde\Delta_{0i}-\tilde\Delta_{mi})^2]  - E[(\tilde\Delta_{mi}-\tilde\Delta_{-mi})^2] \\
                          &= 2E[(\tilde\Delta_{0i}- \tilde\Delta_{mi})(\tilde\Delta_{-mi}-\tilde\Delta_{mi})]   
\end{align*}
So that, assuming $\hat\sigma_{Cox} \rightarrow_p \sigma_{Cox}$, we have
\begin{align}
\frac{T^{Cox,m}}{\sqrt{n}}&\rightarrow_p  \frac{ 2E[(\tilde\Delta_{0i}- \tilde\Delta_{mi})(\tilde\Delta_{-mi}-\tilde\Delta_{mi})] }{\sigma_{Cox}}.
\end{align} 

\end{enumerate}
To prove the second part of the proposition, that the tests are consistent, notice that for each test $y$, there exists an increasing function of n, $a_n$ such that
$\frac{T^{y,m}}{a_n} \rightarrow_p \zeta.$ The quantity $\zeta$ is positive and finite when $\theta_m\neq\theta_0$ and $E(\tilde\Delta_{0i}) \neq E(\tilde\Delta_{mi}).$ Hence, $T^{y,m}\rightarrow_p \infty,$ so that each test has power of one against fixed alternatives.
\end{proof}


==> Submission/ReStud/Proofs/Pf_Degeneracy.tex <==
\begin{proof}[Proof of Proposition \ref{prop:degen} and Corollary \ref{cor:degen}]

From Equations \eqref{eq:line1} and \eqref{eq:line2}, we have equivalence between $E[(\Delta^z_{0i}-\Delta^z_{mi})^2] = 0$ and $\Gamma_0-\Gamma_m=0$. Furthermore, we recall that $\pi_m=\Gamma_0-\Gamma_m$. Thus, we only need to show that $\sigma^2_\text{RV}=0$ if and only if $\pi_m=0$ for all $m\in\{1,2\}$. Rewriting Equation \eqref{eq:sig2rv} in matrix notation, we have
\begin{align}
    \sigma^2_\text{RV} = 4 
    \begin{pmatrix} W^{-1/2}\pi_1 \\ W^{-1/2}\pi_2 \end{pmatrix}'
    \begin{bmatrix}    V^\text{RV}_{11} & - V^\text{RV}_{12} \\ - V^\text{RV}_{12} & V^\text{RV}_{22}\end{bmatrix}
    \begin{pmatrix} W^{-1/2}\pi_1 \\ W^{-1/2}\pi_2 \end{pmatrix}.
\end{align}
Therefore, the claims to be proven follow from positive definiteness of the variance matrix $V^\text{RV} = E[(\psi_{1i}',\psi_{2i}')'(\psi_{1i}',\psi_{2i}')]$, which is the matrix with $V^\text{RV}_{11}$, $V^\text{RV}_{12}$, and $V^\text{RV}_{22}$ as its entries.

To show that $V^\text{RV}$ is positive definite, we take an arbitrary non-zero, non-random vector $v=(v_1',v_2')' \in \mathbb{R}^{2d_z}$. $V^\text{RV}$ is positive definite if $E(v_1'\psi_{1i}+v_2'\psi_{2i})^2 > 0$ for any such $v$. For certain implied non-random $u = (u_1',u_2')'$ and $t=(t_1',t_2')'$ where $t$ is non-zero, we have $E(v_1'\psi_{1i}+v_2'\psi_{2i})^2 = E(u_1'z_i \cdot u_2'z_i + t_1'z_i \cdot e_{1i} + t_2'z_i \cdot e_{2i} )^2$. Because $\sigma_{12}^2 < \sigma_1^2\sigma_2^2$ (Assumption \ref{as:homsked}), we have that $E(t_1'z_i \cdot e_{1i} + t_2'z_i \cdot e_{2i} )^2 > 0$. Therefore, we can only have $E(v_1'\psi_{1i}+v_2'\psi_{2i})^2 = 0$ if $e_{1i}$ or $e_{2i}$ is a linear function of $z_i$ almost surely. However, because $E[z_ie_{mi}]=0$, such dependence is ruled out by $\sigma_m^2>0$ (Assumption \ref{as:homsked}).
%
%
%
%
% We begin by noting that Lemma 1 in \citeA{rv02} shows that $\sigma^2_{RV}=0$ if and only if $   \sqrt{n}(Q_1-Q_2)=o_p(1)$.
% Thus, for Proposition \ref{prop:weakinstr}, we need to show the equivalence
% $$\sqrt{n}(\hat Q_1-\hat Q_2) = o_p(1) \qquad \Leftrightarrow  \qquad E[(\Delta^z_{0i}-\Delta^z_{mi})^2] = 0 \qquad\text{for both $m=1,2$}$$
% From \eqref{eq:line1}, \eqref{eq:line4}, and the positive definiteness of $E[z_iz_i']$, $E[(\Delta^z_{0i}-\Delta^z{m_i})^2] = 0$ iff $g_m = 0$. By \eqref{eq:sig2rv}, if $g_1$ and $g_2$ = 0, then $\sigma^2_{RV} = 0$.  Furthermore, if $\sigma^2_{RV} = 0$ 
%
%
% Consider $Q_1-Q_2$:
% \begin{align*}
% Q_1-Q_2 &=
% %\frac{1}{n} \omega_1'z(z'z)^{-1}z'\omega_1  -  \frac{1}{n}\omega_2'z(z'z)^{-1}z'\omega_2 \\ &=
% \frac{1}{n} \bigg(\omega_1-\omega_2\bigg)'z(z'z)^{-1}z'\bigg(\omega_1+\omega_2\bigg) \\
% % &= \frac{1}{n}\bigg(p-\Delta_1-p+\Delta_2\bigg)'z(z'z)^{-1}z'\bigg(p-\Delta_1+p-\Delta_2\bigg) \\
%   &= \frac{1}{n}\bigg(p-\Delta_1-p+\Delta_2\bigg)'z(z'z)^{-1}z'\bigg(2p-\Delta_1-\Delta_2\bigg) \\
%   &= \frac{1}{n}\bigg(p-\Delta_1-p+\Delta_2\bigg)'z(z'z)^{-1}z'\bigg(2\Delta^*_0 +2\omega_0-\Delta_1-\Delta_2\bigg) \\
% %    &= \frac{1}{n}\bigg(\Delta_2-\Delta_1\bigg)'z(z'z)^{-1}z'\bigg(\Delta_1 +2\omega_0-\Delta_2\bigg) \\
%       &= \frac{1}{n}\bigg(\Delta_2-\Delta_1\bigg)'z(z'z)^{-1}z'\bigg(\Delta^*_0 - \Delta_1 + \Delta^*_0 -\Delta_2\bigg) +2\frac{1}{n}\bigg(\Delta_2-\Delta_1\bigg)'z(z'z)^{-1}z'\omega_0 \\
% %  &= \frac{1}{n}\bigg(\Delta_2-\Delta_1\bigg)'z(z'z)^{-1}z'z(z'z)^{-1}z'\bigg(\Delta_1-\Delta_2\bigg) +2\frac{1}{n}\bigg(\Delta_2-\Delta_1\bigg)'z(z'z)^{-1}z'\omega_0 \\
%   &= \frac{1}{n}\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'z'z\bigg(\hat\Gamma_0 - \hat\Gamma_1 + \hat\Gamma_0 -\hat\Gamma_2\bigg) +2\frac{1}{n}\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'z'\omega_0 
%   \end{align*}
% %  So we have:
% %  \begin{align*}
% %    \sqrt{n}(Q_1-Q_2) &= \frac{1}{\sqrt{n}}\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'z'z\bigg(\hat\Gamma_0 - \hat\Gamma_1 + \hat\Gamma_0 -\hat\Gamma_2\bigg) +2\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'\frac{z'\omega_0}{\sqrt{n}}
% %  \end{align*}
%
% %If $\hat \gamma = \hat \Gamma_1-\hat \Gamma_2 = o_p(1)$, $\hat \Gamma_0-\frac{\hat \Gamma_1 + \hat\Gamma_2}{2} = \frac{O_p(1)}{\sqrt{n}} =  o_p(1)$, and $\frac{z'\omega_0}{\sqrt{n}} = O_p(1)$, then we have:
% %  \begin{align*}
% %      \sqrt{n}(Q_1-Q_2) &=\sqrt{n}\bigg(\hat\Gamma_0 - \hat\Gamma_1 + \hat\Gamma_0 -\hat\Gamma_2\bigg)'\frac{z'z}{n}\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg) +2\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'\frac{z'\omega_0}{\sqrt{n}}
% %  \end{align*}
% %    \begin{align*}
%  %     \sqrt{n}(Q_1-Q_2) &=\underbrace{\sqrt{n}\bigg(\hat\Gamma_1 - \hat\Gamma_0 + \hat\Gamma_2 -\hat\Gamma_0\bigg)'}_{= O_p(1)}\underbrace{\frac{z'z}{n}}_{\rightarrow A_{zz}}\underbrace{\bigg(\hat\Gamma_1-\hat\Gamma_2\bigg)}_{=o_p(1)} +\underbrace{2\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'}_{=o_p(1)}\underbrace{\frac{z'\omega_0}{\sqrt{n}}}_{= O_p(1)}
%  % \end{align*}
%  % so that $ \sqrt{n}(Q_1-Q_2) = o_p(1)$ if and only if $\hat \gamma = o_p(1)$.
% 
%  For $m = 0,1,2$, given that $\hat\Gamma_m$ is a OLS regression coefficient and given the regularity conditions in Assumptions \ref{as:regcond}, $\hat\Gamma_m \rightarrow_p \Gamma_m$ so that $\hat\Gamma_m - \Gamma_m = o_p(1)$ and $\sqrt{n}(\hat\Gamma_m-\Gamma_m) = O_p(1)$.  Let $\hat\psi_m = (\hat\Gamma_m-\Gamma_m)$.
%       \begin{align*}
%       \sqrt{n}(Q_1-Q_2) &=\sqrt{n}\bigg(\hat\Gamma_1 - \hat\Gamma_0 + \hat\Gamma_2 -\hat\Gamma_0\bigg)'\frac{z'z}{n}\bigg(\hat\Gamma_1-\hat\Gamma_2\bigg) + 2\bigg(\hat\Gamma_2-\hat\Gamma_1\bigg)'\frac{z'\omega_0}{\sqrt{n}}\\
%       &= \bigg(\sqrt{n}\bigg(\hat\psi_1-2\hat\psi_0 +  \hat\psi_2 \bigg) +\sqrt{n}(\Gamma_1 + \Gamma_2 - 2\Gamma_0)\bigg)'\frac{z'z}{n}\bigg(\hat\psi_1 -\hat\psi_2+\Gamma_1 - \Gamma_2\bigg)+\\&\qquad 2\bigg(\hat\psi_2-\hat\psi_1 +\Gamma_2-\Gamma_1\bigg)'\frac{z'\omega_0}{\sqrt{n}}
%   \end{align*}
%   Notice that, by Assumptions \ref{as:momcond} and \ref{as:regcond}, $\frac{z'\omega_0}{\sqrt{n}} = O_p(1)$ and $\frac{z'z}{n} = O_p(1)$.  Using the following facts\footnote{See page 12 of van der Vaart's \textit{Asymptotic Statistics}} $O_p(1)o_p(1) = o_p(1)$, $o_p(1) + o_p(1) = o_p(1)$, we can show that $\sqrt{n}(Q_1-Q_2) = o_p(1)$ if and only if the following two conditions hold: (i) $\Gamma_2 = \Gamma_1$ and (ii) $\Gamma_0 = \frac{\Gamma_1+\Gamma_2}{2}$.  To show the if part of the statement, if both (i) and (ii) hold, then:
%   \begin{align*}
%       \sqrt{n}(Q_1-Q_2) &=\bigg(\sqrt{n}\bigg(\hat\psi_1-2\hat\psi_0 +  \hat\psi_2 \bigg)\bigg)'\frac{z'z}{n}\bigg(\hat\psi_1 -\hat\psi_2\bigg)+ 2\bigg(\hat\psi_2-\hat\psi_1 \bigg)'\frac{z'\omega_0}{\sqrt{n}}\\
%       &= O_p(1)(O_p(1)o_p)) + o_p(1)O_p(1)\\
%       &= o_p(1) + o_p(1)\\
%       & = o_p(1)
%   \end{align*}
% Now to show the only if part of the statement, first suppose (i) holds but (ii) does not.  Then we have
%   \begin{align*}
%       \sqrt{n}(Q_1-Q_2) &=
%       \bigg(O_p(1) +\sqrt{n}(\Gamma_1 + \Gamma_2 - 2\Gamma_0)\bigg)'o_p(1)+ o_p(1) \\
%       &=
%       o_p(1) +\sqrt{n}(\Gamma_1 + \Gamma_2 - 2\Gamma_0)o_p(1)\\
%     &= o_p(1) + o_p(\sqrt{n}(\Gamma_1 + \Gamma_2 - 2\Gamma_0)\\
%     &\neq o_p(1)
%     \end{align*}
%   Now suppose (ii) holds but (i) does not. 
%   \begin{align*}
%       \sqrt{n}(Q_1-Q_2) &= O_p(1)(o_p(1) + \Gamma_1-\Gamma_2) + o_p + (\Gamma_1-\Gamma_2)O_p(1)\\
% &= o_p(1) + O_p(1)(\Gamma_1-\Gamma_2)\\
% &\neq o_p(1)
%       \end{align*}
%
% Thus, we have established $\sqrt{n}(Q_1-Q_2) = o_p(1)$ iff $\Gamma_1 = \Gamma_2$ and $\Gamma_0 = \frac{\Gamma_1 + \Gamma_2}{2}$.  Notice, that, if we combine conditions (i) and (ii), $\sqrt{n}(Q_1-Q_2) = o_p(1)$ iff $\Gamma_1 = \Gamma_2 = \Gamma_0$.  Thus, we can express this in terms of weak instruments.  Specifically,  $\sqrt{n}(Q_1-Q_2) = o_p(1)$ iff $\hat\Gamma_0 - \hat\Gamma_m = o_p(1)$ for $m = 1,2$.  We can also express degeneracy in terms of predicted markups.  $E[(\tilde\Delta^*_{0i}-\tilde\Delta_{mi})^2] = E[(\Gamma_0-\Gamma_m)z_iz_i'(\Gamma_0-\Gamma_m)] = (\Gamma_0-\Gamma_m)E[z_iz_i'](\Gamma_0-\Gamma_m)] = 0$  So under Assumption \ref{as:regcond}, $\sqrt{n}(Q_1-Q_2) = o_p(1)$ iff $E[(\tilde\Delta^*_{0i} - \tilde\Delta_{mi})^2] = 0$ for $m =1,2$.  We could also write $E[(\tilde\Delta_{0i}-\tilde\Delta_{mi}] = E[((\Gamma_0-\Gamma_m)z_i] = (\Gamma_0-\Gamma_m)E[z_i] $ but this is always 0 due to the orthogonalization
\end{proof}


==> Submission/ReStud/Proofs/Pf_DemandSimSeq.tex <==
\begin{proof}
By definition of $\theta_m^{Dsim}$ and because $\theta^{Dseq}$ is the minimizer of $\mathcal{Q}^{dem}$, it must be that $\mathcal{Q}^{sim}_m(\theta_m^{Dsim}) < \mathcal{Q}^{sim}_m(\theta^{Dseq})$. In turn, this implies that $\mathcal{Q}_m(\theta_m^{Dsim}) < \mathcal{Q}_m(\theta^{Dseq})$ - if this inequality did not hold, we would need to have $\mathcal{Q}^{dem}(\theta^{Dseq})> \mathcal{Q}^{dem}(\theta^{Dsim})$. Since each objective function is assumed to have a unique minimizer, this last inequality is a contradiction. Moreover, in case 1. where cost shifters are correctly specified, we have  $\mathcal{Q}_{m}\left(\Delta(\theta^D)\right) = E[(\tilde \Delta^*_0 - \tilde \Delta_m(\theta^D))^2]$. Therefore, 
    \begin{align*}
        E[(\tilde \Delta^*_0 - \tilde \Delta_m(\theta_m^{Dsim}))^2] <         E[(\tilde \Delta^*_0 - \tilde \Delta_m(\theta^{Dseq}))^2].
    \end{align*}
In case 2. where cost shifters are misspecified, we have instead $\mathcal{Q}_{m}\left(\Delta(\theta^D)\right) = E[(\tilde \Delta^C_0 - \tilde \Delta_m(\theta^D))^2]$. Therefore, 
    \begin{align*}
        E[(\tilde \Delta^C_0 - \tilde \Delta_m(\theta_m^{Dsim}))^2] <         E[(\tilde \Delta^C_0 - \tilde \Delta_m(\theta^{Dseq}))^2].
    \end{align*}     
\end{proof}

==> Submission/ReStud/Proofs/Pf_Fstats.tex <==
Specifically, we can compute F-statistics for two regressions (i) $2p-\Delta_1-\Delta_2$  on instruments and (ii) $\Delta_1-\Delta_2$ on instruments as follows, letting the residuals from these regressions be $\hat\zeta_1$ and $\hat\zeta_2$ respectively. 
\begin{align*}
    F_1 &= \frac{((z'z)^{-1}z'(2\Delta_0+2\omega_0-\Delta_1-\Delta_2))'z'z((z'z)^{-1}z'(z(2\Delta_0+2\omega_0-\Delta_1-\Delta_2))}{d_z\hat\sigma^2_{\zeta_1}},\\
&=    \frac{((z'z)^{-1}z'(z\frac{q_1+q_2}{\sqrt{n}}+\zeta_1))'z'z((z'z)^{-1}z'(z\frac{q_1+q_2}{\sqrt{n}}+\zeta_1))}{d_z\hat\sigma^2_{\zeta_1}},\\
&= \frac{ ( \hat A_{zz}^{1/2}(q_1+q_2)\hat A_{zz}^{-1/2}\frac{z'\zeta_1}{\sqrt{n}})'( \hat A_{zz}^{1/2}(q_1+q_2)+\hat A_{zz}^{-1/2}\frac{z'\zeta_1}{\sqrt{n}})}{d_z\hat\sigma^2_{\zeta_1}},\\
&= \frac{( \hat A_{zz}^{1/2}(q_1+q_2)+\hat A_{zz}^{-1/2}\frac{z'\zeta_1}{\sqrt{n}})'}{\sqrt{d_z}\hat\sigma_{\zeta_1}}\frac{( \hat A_{zz}^{1/2}(q_1+q_2)+\hat A_{zz}^{-1/2}\frac{z'\zeta_1}{\sqrt{n}})}{\sqrt{d_z}\hat\sigma_{\zeta_1}},\\
 d_z F_1&\rightarrow_d \chi^2_{d_z}(\pi_{01}'\pi_{01})
\end{align*}
where $\zeta_1=2\omega_0 + e_1 + e_2$ and $\sigma^2_{\zeta_1} = 4\sigma^2_{\omega_0} + \sigma^2_{e_1} + \sigma^2_{e_2} + 4\sigma_{\omega_0 e_1} + 4\sigma_{\omega_0 e_2} + 2\sigma_{e_1 e_2}=\Omega_{11}$.

Also, 
\begin{align*}
    F_2 &= \frac{(\hat\Gamma_1-\hat\Gamma_2)'z'z(\hat\Gamma_1-\hat\Gamma_2)}{d_z\hat\sigma^2_{\zeta_2}},\\
&=    \frac{((z'z)^{-1}z'(\Delta_1-\Delta_2))'z'z((z'z)^{-1}z'(\Delta_1-\Delta_2)}{d_z\hat\sigma^2_{\zeta_2}},\\
&=    \frac{((z'z)^{-1}z'(z\frac{q_1-q_2}{\sqrt{n}}+\zeta_2))'z'z((z'z)^{-1}z'(z\frac{q_1-q_2}{\sqrt{n}}+\zeta_2))}{d_z\hat\sigma^2_{\zeta_2}},\\
&= \frac{ ( \hat A_{zz}^{1/2}(q_1-q_2)+\hat A_{zz}^{-1/2}\frac{z'\zeta_2}{\sqrt{n}})'( \hat A_{zz}^{1/2}(q_1-q_2)+\hat A_{zz}^{-1/2}\frac{z'\zeta_2}{\sqrt{n}})}{d_z\hat\sigma^2_{\zeta_2}},\\
&= \frac{( \hat A_{zz}^{1/2}(q_1-q_2)+\hat A_{zz}^{-1/2}\frac{z'\zeta_2}{\sqrt{n}})'}{\sqrt{d_z}\hat\sigma_{\zeta_2}}\frac{( \hat A_{zz}^{1/2}(q_1-q_2)+\hat A_{zz}^{-1/2}\frac{z'\zeta_2}{\sqrt{n}})}{\sqrt{d_z}\hat\sigma_{\zeta_2}},\\
 d_z F_2&\rightarrow_d \chi^2_{d_z}(\pi_{02}'\pi_{02})
\end{align*}


==> Submission/ReStud/Proofs/Pf_ManyInstr.tex <==


As a preliminary step, we define the first stage models as:
\begin{align*}
    \Delta &= z\Gamma + e\\
    \Delta^* &= z\Gamma^* + e^*.
\end{align*}
Further, we define $ \Sigma_{ee} = E[e_ie_i']$, $\Sigma_{ee^*} = E[e_ie^{*\prime}_i] $, and $\Sigma_{e\omega_0} = E[e_i\omega_{0i}']$.


\begin{proof}
We proceed in several steps:

\noindent \textbf{Step 1:} We first establish the following convergence in probability result:
\begin{align*}
    \hat A_{\Delta z}\hat A_{zz}^{-1}\hat A_{z\Delta} 
    %&= \frac{\Gamma'z'z\Gamma}{n} + \frac{\Gamma'z'e}{n} + \frac{e'z\Gamma}{n} + \frac{e'z(z'z)^{-1}z'e}{n}\\
    &\rightarrow_p H + \delta_z\Sigma_{ee}
\end{align*}
Note that, by plugging in the first stage equation for $\Delta$, we obtain:
\begin{align}
    \hat A_{\Delta z}\hat A_{zz}^{-1}\hat A_{z\Delta} 
    &= \underbrace{\frac{\Gamma'z'z\Gamma}{n}}_{I} + \underbrace{\frac{\Gamma'z'e}{n}}_{II} + \underbrace{\frac{e'z\Gamma}{n}}_{III} + \underbrace{\frac{e'z(z'z)^{-1}z'e}{n}}_{IV}
\end{align}
By Assumption \ref{as:manyinstr}, $I\rightarrow_p H$.  Now, consider $II$.  Following Hansen (2021, page 391), if we vectorize $II$, $Var(vec(II))\rightarrow_p 0$ which implies that $II \rightarrow_p0$.  By the same argument, $III\rightarrow_p 0$.  Finally, note that, by Equation 12.28 in Hansen 2021, for the $(j,k)^\text{th}$ element of IV, $E[IV_{jk} \mid z] \rightarrow_p \delta_{z} \Sigma_{ee}(j,k)$.  Further $Var[IV_{jk} \mid z] \rightarrow_p 0$.  Thus, by considering all elements and applying Markov's inequality,  in Equation 12.83, $IV\rightarrow_p \delta_z \Sigma$. \\ 

\noindent \textbf{Step 2:} We derive the plim of the RV numerator with a many instrument asymptotic:
\begin{align*}
Q_1 - Q_2 
&= (g_1-g_2)'W(g_1+g_2)\\
%&= \frac{1}{n}(\Delta(\theta_0 - \theta_1)+ \omega_0)' P_z(\Delta(\theta_0 - \theta_1)+ \omega_0)- \frac{1}{n}(\Delta(\theta_0 -\theta_2)+ \omega_0)'  P_z(\Delta(\theta_0 - \theta_2)+ \omega_0)\\
&= \frac{1}{n}\bigg(\theta_1-\theta_2\bigg)'\Delta'z(z'z)^{-1}z'\bigg(-2p + \Delta(\theta_1+\theta_2)\bigg)\\
    %&= \frac{1}{n}\bigg(\theta_1-\theta_2\bigg)'\Delta'z(z'z)^{-1}z'\Delta\bigg(\theta_1+\theta_2\bigg) -2 \frac{1}{n}\bigg(\theta_1-\theta_2\bigg)'\Delta'z(z'z)^{-1}z'p\\
   % &= \frac{1}{n}\bigg(\Delta_1-\Delta_2\bigg)'z(z'z)^{-1}z'\bigg(\Delta_1+\Delta_2\bigg) -2 \frac{1}{n}\bigg(\theta_1-\theta_2\bigg)'\Delta'z(z'z)^{-1}z'\Delta\hat\theta_{2SLS}\\
 %       &= \frac{1}{n}\bigg(\Gamma_1-\Gamma_2\bigg)(z'z)\bigg(\Gamma_1+\Gamma_2\bigg) -2 \frac{1}{n}\bigg(\theta_1-\theta_2\bigg)'\Gamma(z'z)\Gamma\hat\theta_{2SLS}\\
        &= \frac{1}{n}\bigg(\theta_1-\theta_2\bigg)'(\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})\bigg(\theta_1+\theta_2\bigg) -2 \frac{1}{n}\bigg(\theta_1-\theta_2\bigg)'(\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta}) \hat\theta_{2SLS}\\
        & \rightarrow_p  \bigg(\theta_1-\theta_2\bigg)(H+\delta_z \Sigma_{ee})\bigg(\theta_1+\theta_2\bigg) -2 \bigg(\theta_1-\theta_2\bigg)'(H+\delta_z \Sigma_{ee})\theta_{2SLS}, 
\end{align*}

\noindent Under the same many instrument asymptotics we derive $\theta_{2SLS}$, the plim of the 2SLS estimator:
\begin{align*}
\hat\theta_{2SLS}  &= (\Delta'P_z\Delta)^{-1}\Delta'P_zp\\
&=  (\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}\hat A_{\Delta z} \hat A_{z z}^{-1}\hat A_{z\Delta^*}\theta_0 +  (\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}\hat A_{\Delta z} \hat A_{z z}^{-1} \frac{z'\omega_0}{n}\\
&=  \underbrace{(\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}}_{I}\underbrace{\hat A_{\Delta z} \hat A_{z z}^{-1}\hat A_{z\Delta^*}\theta_0}_{II} +  \underbrace{(\hat A_{\Delta z} \hat A_{z z}^{-1} \hat A_{z\Delta})^{-1}}_{I} \bigg(\underbrace{\frac{\Gamma'z'\omega_0}{n}}_{III} + \underbrace{\frac{e'z'(z'z)^{-1}z'\omega_0}{n}}_{IV}\bigg)
\end{align*}
By the results established in Step 1, $I\rightarrow_p H+\delta_z\Sigma_{ee}$.  By the same argument, $I\rightarrow_p H+\delta_z\Sigma_{ee^*}$.  Fianlly, we can show that $III\rightarrow_p \delta_z\Sigma_{e\omega_0}$.  Following the argument in Hansen (2021), $Var(vec(III))\rightarrow_p0$ so that $III\rightarrow_p 0$.  Finally, note that, by Equation 12.28 in Hansen 2021, for the $(j,k)^\text{th}$ element of IV, $E[IV_{jk} \mid z] \rightarrow_p \delta_{z} \Sigma_{e\omega_0}(j,k)$.  Further $Var[IV_{jk} \mid z] \rightarrow_p 0$.  Thus, by considering all elements and applying Markov's inequality,  in Equation 12.83, $IV\rightarrow_p \delta_z \Sigma_{e\omega_0}$.  Thus, $\theta_{2SLS}$ is given as
\begin{align*}
\theta_{2SLS} =  (H+\delta_z \Sigma_{ee})^{-1}(H^*+\delta_z \Sigma_{ee^*})\theta_0+(H+\delta_z \Sigma_{ee})^{-1}\delta_z \Sigma_{e \omega_0}
\end{align*}
So that:
\begin{align*}
    Q_1 - Q_2 %&\rightarrow_p \bigg(\theta_1-\theta_2\bigg)(H+\delta_z \Sigma_{ee})\bigg(\theta_1+\theta_2\bigg) -2 \bigg(\theta_1-\theta_2\bigg)'[(H^*+\delta_z \Sigma_{ee^*})\theta_0+\delta_z \Sigma_{e \omega_0}]\\
    &\rightarrow_p (\theta_1-\theta_2)\bigg(H(\theta_1+\theta_2)  -2 H^*\theta_0\bigg)  + \delta_z(\theta_1-\theta_2)'\bigg( \Sigma_{ee}(\theta_1+\theta_2)
    -2 \Sigma_{ee^*}\theta_0+ \Sigma_{e \omega_0}\bigg)
    %&= E[(\tilde\Delta_{1i}-\tilde\Delta^*_{0i})^2] - E[(\tilde\Delta_{2i}-\tilde\Delta^*_{0i})^2] + \delta_z\bigg( \sigma^2_{e_1}-\sigma^2_{e_2}
    %-2 \sigma_{e_0e^*_0}+2\sigma_{e_{-0}e^*_{0}}+ \sigma_{e_1 \omega_0}-\sigma_{e_2 \omega_0}\bigg)
\end{align*}

\noindent \textbf{Step 3:}  We show that when $\delta_z = 1$, $plim(Q_1-Q_2) = plim(Q^{RSS}_1-Q^{RSS}_2)$. Recall that, by Lemma \ref{lemma2}, $Q^{OLS}_1-Q^{OLS} = Q^{RSS}_1-Q^{RSS}$.  So, consider the numerator of the RSS statistic:
\begin{align*}
Q_1^{OLS} - Q_2^{OLS}
&= (g_1-g_2)'W(g_1+g_2)\\
%&= \frac{1}{n}(\omega_1'\Delta-\omega_2'\Delta)(\Delta'\Delta)^{-1}(\Delta'\omega_1+\Delta'\omega_2)\\
%&= ((p-\Delta_1)'-(p-\Delta_2)')\Delta(\Delta'\Delta)^{-1}\Delta'((p-\Delta_1)+(p-\Delta_2))\\
&= \frac{1}{n}(\Delta_2-\Delta_1)'\Delta(\Delta'\Delta)^{-1}\Delta'(2p-\Delta_1-\Delta_2)\\
%&= (\Delta_2-\Delta_1)'\Delta(\Delta'\Delta)^{-1}\Delta'(2\Delta^*_0-\Delta_1-\Delta_2) + (\Delta_2-\Delta_1)'\Delta(\Delta'\Delta)^{-1}\Delta'\omega_0 \\
&= \frac{1}{n}(\Delta_1-\Delta_2)'\Delta(\Delta'\Delta)^{-1}\Delta'(\Delta_1+\Delta_2) - 2\frac{1}{n}(\Delta_1-\Delta_2)'\Delta(\Delta'\Delta)^{-1}\Delta'p\\
%&= (\theta_1-\theta_2)'\Delta'\Delta(\Delta'\Delta)^{-1}\Delta'\Delta(\theta_1+\theta_2) - 2(\theta_1-\theta_2)'\Delta'\Delta\hat\theta_{OLS}\\
%&= (\theta_1-\theta_2)'\Delta'\Delta(\theta_1+\theta_2) - 2(\theta_1-\theta_2)'\Delta'\Delta\hat\theta_{OLS}\\
%&= \frac{1}{n}(\theta_1-\theta_2)'(z\Gamma+e)'(z\Gamma+e)(\theta_1+\theta_2) - 2\frac{1}{n}(\theta_1-\theta_2)'(z\Gamma+e)'(z\Gamma+e)\hat\theta_{OLS}\\
&= (\theta_1-\theta_2)'\bigg(\frac{\Gamma'z'z\Gamma}{n}+ \frac{\Gamma'z'e}{n} + \frac{e'z\Gamma}{n} + \frac{e'e}{n}\bigg) (\theta_1+\theta_2)  \\
&\qquad- 2(\theta_1-\theta_2)'\bigg(\frac{\Gamma'z'z\Gamma}{n}+ \frac{\Gamma'z'e}{n} + \frac{e'z\Gamma}{n} + \frac{e'e}{n}\bigg)\hat\theta_{OLS}\\
&\rightarrow_p (\theta_1-\theta_2)'(H + \Sigma_{ee}) (\theta_1+\theta_2)  
- 2(\theta_1-\theta_2)'(H + \Sigma_{ee})\theta_{OLS}
\end{align*}
It is easy to show that, when $\delta_z = 1$, $\theta_{2SLS} = \theta_{OLS}$.  Thus, when $\delta_z = 1$, $plim(Q_1-Q_2) = plim(Q^{OLS}_1-Q^{OLS}_2)$. We establish in Proposition \ref{prop:RSS} that $plim(Q^{OLS}_1-Q^{OLS}_2) = E[(\Delta_{1i}-\Delta_{OLSi})^2] - E[(\Delta_{2i}-\Delta_{OLSi})^2]$. \\

\noindent \textbf{Step 4:}  We show that $Q_1-Q_2$ can be expressed as a linear combination of numerators of the fixed instrument RV test statistic and the RSS test statistic.  Note that when $\delta_z = 0$, we are in a fixed instruments setup, so that the usual asymptotics obtains.  This means that, by Proposition \ref{prop:plims_TE2}: \begin{align}
    (\theta_1-\theta_2)\bigg(H(\theta_1+\theta_2)  -2 H^*\theta_0\bigg) =
E[(\tilde\Delta_{1i}-\tilde\Delta^*_{0i})^2] - E[(\tilde\Delta_{2i}-\tilde\Delta^*_{0i})^2] 
\end{align}
%and we can rewrite
%\begin{align*}
%    Q_1 - Q_2 &\rightarrow_p E[(\tilde\Delta_{1i}-\tilde\Delta^*_{0i})^2] - E[(\tilde\Delta_{2i}-\tilde\Delta^*_{0i})^2]  + \delta_z(\theta_1-\theta_2)'\bigg( \Sigma_{ee}(\theta_1+\theta_2)
 %   -2 \Sigma_{ee^*}\theta_0+ \Sigma_{e \omega_0}\bigg)
  %  \end{align*}

Therefore, by the results established in the previous steps,
% $$\delta_z(\theta_1-\theta_2)'\bigg( \Sigma_{ee}(\theta_1+\theta_2)
 %   -2 \Sigma_{ee^*}\theta_0+ \Sigma_{e \omega_0}\bigg) = E[(\Delta_{1i}-\Delta_{OLSi})^2] - E[(\Delta_{2i}-\Delta_{OLSi})^2]-E[(\tilde\Delta_{1i}-\tilde\Delta^*_{0i})^2] + E[(\tilde\Delta_{2i}-\tilde\Delta^*_{0i})^2]   $$
 %   so that
\begin{align*}
    Q_1-Q_2\rightarrow_p (1-\delta_z)\bigg(E[(\tilde\Delta_{1i}-\tilde\Delta^*_{0i})^2] - E[(\tilde\Delta_{2i}-\tilde\Delta^*_{0i})^2]\bigg) + \delta_z\bigg(E[(\Delta_{1i}-\Delta_{OLSi})^2] - E[(\Delta_{2i}-\Delta_{OLSi})^2]\bigg) 
\end{align*} 

\end{proof}


==> Submission/ReStud/Proofs/Pf_Nulls.tex <==
\begin{proof}[Proof of Proposition \ref{prop:nulls}]
For $(i)$, we need to show the equivalence
\begin{align}\label{eq:equiv_prop1_ar}
\pi_m = 0 \qquad \Leftrightarrow \qquad   E[(\Delta^z_{0i}-\Delta^z_{mi})^2] = 0  
\end{align}
This equivalence is a consequence of Equations \eqref{eq:line1} and \eqref{eq:line5} in addition to $E[z_i z_i']$ being positive definite.
For $(ii)$, we we need to show the equivalence
\begin{align}
    {Q}_1-{Q}_2 =0  \qquad \Leftrightarrow \qquad  E[(\Delta^z_{0i}-\Delta^z_{1i})^2]-E[(\Delta^z_{0i}-\Delta^z_{2i})^2]=0. 
\end{align}
This equivalence is a consequence of Equations \eqref{eq:line1} and \eqref{eq:line5}.
%
\begin{comment}
\begin{align}\label{eq:equiv_prop1_ar}
\pi_m = 0 \qquad \Leftrightarrow \qquad   E[(\Delta^z_{0i}-\Delta^z_{mi})^2] = 0  
\end{align}
By definition of the OLS estimator, $\pi_m$ is:
\begin{align}
    \pi_m &= E[z_iz_i']^{-1}E[z_i(p_i-\Delta_{mi})] \\
        %&=E[z_iz_i']^{-1}E[z_i(\Delta_{0i}-\Delta_{mi})]\\
        &=(\Gamma_{0}-\Gamma_{m})
    \end{align}
where the second equality follows from Assumption \ref{as:momcond}, $E[z_i w_{0i}]=0$, and $\Delta_{0i} = p_i - \omega_{0i}$.  From the Proof of Lemma 1, it follows that $E[(\Delta^z_{0i}-\Delta^z_{mi})^2]=\pi_m'E[z_i'z_i]\pi_m$. 
The equivalence in \eqref{eq:equiv_prop1_ar} now follows from $E[z_i z_i']$ being positive definite.\\
For (ii), we can directly show the equivalence ${Q}_m = E[(\Delta^z_{0i}-\Delta^z_{mi})^2] $.
\begin{align*}
{Q}_m &= E[\omega_{mi}z_i]'E[z_i z_i']^{-1}E[\omega_{mi}z_i]\\
&=E[(\Delta_{0i}-\Delta_{mi})z_i]'E[z_i z_i']^{-1}E[(\Delta_{0i}-\Delta_{mi})z_i]\\
%&=E[(\Delta_{0i}-\Delta_{mi})z_i]'E[z_i z_i']^{-1}E[z_i z_i']E[z_i z_i']^{-1}E[(\Delta_{0i}-\Delta_{mi})z_i]\\
&=(\Gamma_0-\Gamma_m)'E[z_i z_i'](\Gamma_0-\Gamma_m)\\
&=E[(\Delta^z_{0i}-\Delta^z_{mi})^2]
\end{align*}     
where the second equality follows from  Assumption \ref{as:momcond}, $E[z_i w_{0i}]=0$, $\Delta_{mi} = p_i-\omega_{mi}$, and  $\Delta_{0i} = p_i - \omega_{0i}$. The last equality is proven in the Proof of Lemma 1.  Thus, ${Q}_1-{Q}_2 = E[(\Delta^z_{0i}-\Delta^z_{1i})^2]-E[(\Delta^z_{0i}-\Delta^z_{2i})^2] $
\end{comment}
%
\begin{comment}
\begin{enumerate}
    \item Note that for AR, the OLS estimator is given as:
    \begin{align}
    \pi_m &= E[z_iz_i']^{-1}E[z_i(p_i-\Delta_{mi})] \\
    &=E[z_iz_i']^{-1}E[z_i(\Delta_{0i}-\Delta_{mi})] + E[z_iz_i']^{-1}E[z_i\omega_{0i})]\\
        &=E[z_iz_i']^{-1}E[z_i(\Delta_{0i}-\Delta_{mi})]\\
        &=(\Gamma_{0i}-\Gamma_{mi})
    \end{align}
    We can rewrite the moment in Lemma \ref{lemma1} as:
    \begin{align}
        E[(\Delta^z_{0i}-\Delta^z_{mi})^2] &=E[(z_iE[z_iz_i']^{-1}E[z_i(\Delta_{0i}-\Delta_{mi})])^2]\\
        &=E[(z_i\pi_m)^2]\\
         &=E[z_i\pi_m \pi_m'z_i']\\
         &=E[\pi_m'z_i'z_i\pi_m ]\\
                  &=\pi_m'E[z_i'z_i]\pi_m 
    \end{align}
    Since $E[z_i'z_i]$ is positive definite, then it immediately follows from the definition of positive definite that $E[(\Delta^z_{0i}-\Delta^z_{mi})^2] = 0$ iff $\pi_m = 0$.
\item 
\begin{align*}
\mathcal{Q}_m &= E[\omega_{mi}z_i]'E[z_i z_i']^{-1}E[\omega_{mi}z_i]\\
&= E[(\Delta_{0i}-\Delta_{mi}+\omega_{0i})z_i]'E[z_i z_i']^{-1}E[(\Delta_{0i}-\Delta_{mi}+\omega_{0i})z_i]\\
&=E[(\Delta_{0i}-\Delta_{mi})z_i]'E[z_i z_i']^{-1}E[(\Delta_{0i}-\Delta_{mi})z_i]\\
&=E[(\Delta_{0i}-\Delta_{mi})z_i]'E[z_i z_i']^{-1}E[z_i z_i']E[z_i z_i']^{-1}E[(\Delta_{0i}-\Delta_{mi})z_i]\\
&=(\Gamma_0-\Gamma_m)'E[z_i z_i'](\Gamma_0-\Gamma_m)\\
&=E[(\Gamma_0-\Gamma_m)'z_i z_i'(\Gamma_0-\Gamma_m)]\\
&=E[(\Delta^z_{0i}-\Delta^z_{mi})'(\Delta^z_{0i}-\Delta^z_{mi})]\\
&=E[(\Delta^z_{0i}-\Delta^z_{mi})^2]
\end{align*}     
Since $\mathcal{Q}_m = E[(\Delta^z_{0i}-\Delta^z_{mi})^2] $, $\mathcal{Q}_1-\mathcal{Q}_2 = E[(\Delta^z_{0i}-\Delta^z_{1i})^2]-E[(\Delta^z_{0i}-\Delta^z_{2i})^2] $
\end{enumerate}
\end{comment}
\end{proof}

==> Submission/ReStud/Proofs/Pf_Plims.tex <==
\begin{proof}[Proof of Lemma \ref{cor:modelmisc}.] For $(i)$, suppose for concreteness that $E[(\Delta^z_{0i}-\Delta^z_{1i})^2]<E[(\Delta^z_{0i}-\Delta^z_{2i})^2]$. We need to show that $\Pr\big( T^\text{RV} < -q_{1-\alpha/2}(N) \big) \rightarrow 1$ where $q_{1-\alpha/2}(N)$ is the $(1-\alpha/2)$-th quantile of a standard normal distribution. From Proposition \ref{prop:nulls}, part $(ii)$, we have $Q_1 < Q_2$. Lemma \ref{lem:asymp norm}, parts $(i)$ and $(ii)$, together with Remark \ref{rem:validity} yields $T^\text{RV}/\sqrt{n} = \frac{ \hat Q_1-\hat Q_2}{\hat \sigma_\text{RV}} \xrightarrow{p}  \frac{Q_1-Q_2}{\sigma_\text{RV}} < 0$. Therefore, $\Pr\big( T^\text{RV}/\sqrt{n} < -q_{1-\alpha/2}(N_{0,1})/\sqrt{n} \big) \rightarrow 1$.

For $(ii)$, suppose that $E[(\Delta^z_{0i}-\Delta^z_{mi})^2]\neq 0$ for some $m \in \{1,2\}$.  We need to show that $\Pr\big( \text{reject } H^\text{AR}_{0,m} \big) \rightarrow 1$. From Proposition \ref{prop:nulls}, part $(i)$, it follows that $\pi_m \neq 0$ and since $V^\text{AR}_{mm}$ is positive definite we have $\pi_m'V^\text{AR}_{mm}\inverse \pi_m > 0$. Using Lemma \ref{lem:asymp norm}, parts $(iii)$ and $(iv)$, we have $(\hat \pi_m,\hat V^\text{AR}_{mm}) \xrightarrow{p} (\pi_m,V^\text{AR}_{mm})$ so that $T^\text{AR}_m/n = \hat\pi_m'\big(\hat V^\text{AR}_{mm}\big)\inverse \hat\pi_m \xrightarrow{p} \pi_m'\big( V^\text{AR}_{mm}\big)\inverse \pi_m > 0$. Therefore, $\Pr\big( \text{reject } H^\text{AR}_{0,m} \big) = \Pr\big( T^\text{AR}_m/n > q_{1-\alpha}(\chi^2_{d_z})/n \big) \rightarrow 1$ where $q_{1-\alpha}(\chi^2_{d_z})/n ) \rightarrow 1$ where $q_{d_z}(1-\alpha)$ denotes the $(1-\alpha)$-th quantile of a $\chi^2_{d_z}$ distribution.
\begin{comment}
\begin{itemize}

\item[(i)]  Consider anly model $m$ such that $E[(\Delta^z_{0i}-\Delta^z_{mi})^2]\neq 0$.  By \eqref{eq:line1}, \eqref{eq:line5} and the positive definiteness of $E[z_iz_i']$, $\pi_m\neq 0$, representing a fixed alternative of the AR test under $H^{AR}_{A,m}$.  From Lemma A.1 (iii) $\hat\pi_m\rightarrow\pi_m$, and from  (iv) $\hat V_m\rightarrow V_m$. Thus, $\hat\pi_m'\hat V_m\hat\pi_m\rightarrow_p \pi_m' V_m\pi_m >0$, where the inequality hold because  $V_m$ is positive definite. It immediately follows that $T^{AR} \rightarrow \infty$ and $\Pr(\text{reject } H^{AR}_{0,m}) \rightarrow 1$.  

    \item[(ii)]  By Lemma A.1 (i), $\hat Q_m \rightarrow_p Q_m$ for $m=1,2$ and  by (ii), $\hat\sigma^2_{RV} \rightarrow_p \sigma^2_{RV} \neq 0$ under Assumption \ref{as:nodegen}. Thus, $T^{RV} = \frac{\sqrt{n} (\hat Q_1-Q_2)}{\hat \sigma_{RV}} \rightarrow_p \lim_{n\rightarrow\infty }  \frac{\sqrt{n}(Q_1-Q_2)}{\sigma_{RV}}$. For any pair of models $1,2$ by which     $E[(\Delta^z_{0i}-\Delta^z_{1i})^2]<E[(\Delta^z_{0i}-\Delta^z_{2i})^2]$, $Q_1<Q_2$  from \eqref{eq:line1} and \eqref{eq:line5}.  Thus, the models represent a fixed alternative satisfying $H^{RV}_{1}$
 In this case  $T^{RV}\rightarrow_p -\infty$ so that $\Pr(\text{reject } H^{RV}_0 \text{ for } m=1) \rightarrow 1$ as $n\rightarrow\infty$. Likewise for fixed alternatives satisfying $H^{RV}_{2}$,  $Q_1>Q_2$ and, from \eqref{eq:line1} and \eqref{eq:line5}, $E[(\Delta^z_{0i}-\Delta^z_{1i})^2]>E[(\Delta^z_{0i}-\Delta^z_{1i})^2]$ .  In this case  $T^{RV}\rightarrow_p \infty$ so that $\Pr(\text{reject } H^{RV}_0 \text{ for } m=2) \rightarrow 1$ as $n\rightarrow\infty$.
\end{itemize}
\end{comment} 
\end{proof}

==> Submission/ReStud/Proofs/Pf_RSS.tex <==
\subsection{The Problem with Testing without Instruments}\label{sec:RSS}

The RV test statistic depends on measures of fit formed with excluded instruments $z$.  However, implementations of the RV test based on residual sum of squares (RSS) have been popular in the applied IO literature.\footnote{For example, \cite{b87}, \cite{glv92}, \cite{bd10} and \cite{bdvk13} use RSS-based procedures to test hypotheses on conduct.}  These RSS-based tests are inconsistent.  To illustrate why, we briefly summarize how  one could implement an RSS based test.  First, one would impose model $m$ and rearrange the first order conditions of the firm as follows:
\begin{align}\label{OLSreg}
\mathbf{p} - \mathbf{\Delta}_m = \mathbf{w} \tau + \boldsymbol{\omega}_m.
\end{align}
Under the imposed model, $\mathbf{p} - \mathbf{\Delta}_m $ is observed and one can obtain an OLS residual $\hat{\boldsymbol{\omega}}_m$ from the regression (\ref{OLSreg}). Given that the OLS regression imposes that $\textbf{w}$ is orthogonal to $\boldsymbol \omega_m$, one can equivalently set $\hat{\boldsymbol{\omega}}_m = p - \Delta_m  = \hat{\omega}_m.$ One then constructs for model $m$ a measure of fit $Q_m^{RSS} = \frac{1}{n} \sum_i (\hat\omega_{mi})'(\hat\omega_{mi})$, and computes a test statistic as in  (\ref{RVt}):
\begin{align}
T^{RSS} = \frac{\sqrt{n}}{\hat  \sigma_{RSS}} (Q_1^{RSS} - Q_2^{RSS}), 
\end{align}
where $\hat  \sigma_{RSS}$ is a consistent estimator of the standard deviation of the difference in the RSS measures of fit. The formulation of the hypotheses is identical to what we have described for RV in Section \ref{sec:thetests}, except for the different measure of fit. 

Consider alternative moments
$g^{OLS}_m = \frac{\Delta'\hat\omega_m}{n}$,
which are the moments one would use to estimate Equation (\ref{eq:test}) by OLS. We define a measure of fit using these moments as $Q_m^{OLS} = g^{OLS\prime}_m(\frac{\Delta'\Delta}{n})^{-1} g^{OLS}_m$. Now we can prove the following lemma: 

\begin{lemma}\label{lemma2}

For any pair of models $m=1,2$,  
$T^{RSS} = \frac{\sqrt{n}}{\hat  \sigma_{RSS}} (Q_1^{OLS} - Q_2^{OLS}).$
\end{lemma}

\noindent The lemma establishes the equivalence between the RSS-based test and testing with OLS moments. As markups are endogenous,  tests based on $T^{RSS}$  have the wrong size and possibly no power against some fixed alternatives. Suppose that $\Delta_0=\Delta_1$ and consider testing two models:  the true model  and the OLS model with markups $\Delta^{OLS} = \Delta\theta^{OLS}$ where $\theta^{OLS}= E[\Delta_{i} \Delta_{i}']^{-1} E[\Delta_{i} p_i]$. As $Q_m^{OLS}$ is minimized at $\hat\theta^{OLS}$, $T^{RSS}$ asymptotically rejects for the wrong model. We formalize this in a proposition:\looseness=-1 
\begin{proposition}\label{prop:RSS} Assume that Assumptions \ref{as:momcond}, \ref{as:regcond} and \ref{as:homsked} are satisfied. Then:
\begin{align}
\frac{T^{RSS}}{\sqrt{n}} &\rightarrow_p  \frac{E[(\Delta^{OLS}_i -\Delta_{1i})^2 - (\Delta^{OLS}_i -\Delta_{2i})^2]	}{\sigma_{RSS}}
\end{align} 
\end{proposition}

When a researcher observes true markups, a valid way to perform model selection is to compare the implied markups for each model to the true markups.  This proposition shows that RSS-based tests asymptotically reject in favor of the model for which the implied markups are closer to the OLS markups. Thus, the RSS procedure implicitly uses the observed $\Delta^{OLS}$ in place of $\Delta_0$.  Since $\Delta$ is generally correlated with $\omega$, $\Delta^{OLS}$ may be very far from $\Delta_0$, making the RSS procedure inconsistent.\footnote{Our discussion thus far in this section is based on an RV-like test statistic because this has been used in the applied literature. In fact, other testing procedures (most notably, Cox and EB) could be performed using the moments $h$ based on OLS fit, thus incurring in the same problems.} An obvious solution is to test based on the moments formed with excluded instruments as in the procedures described in Section \ref{sec:thetests}. 




Useful objects for the proof: 
\begin{align*}
        \hat A_{\Delta \Delta} = \frac{\Delta'\Delta}{n}\\
        \hat A_{\Delta p} = \frac{\Delta'p}{n}
\end{align*}
and the facts:
\begin{align*}
    \hat A_{\Delta \Delta} &= A_{\Delta \Delta} + o_p(1)\\
    \hat A_{\Delta p} &= A_{\Delta p} + o_p(1).
\end{align*}
Notice moreover that:
\begin{align*}
    E[\hat\theta_{OLS}] = A_{\Delta \Delta}^{-1} A_{\Delta p} = \theta_{OLS} \neq \theta_0.
\end{align*}
where the inequality comes from our assumption on the endogeneity of the markup term. We first prove a useful lemma:

\begin{lemma}

Define the RSS measure of fit as 

\begin{align}
Q^{RSS}(\theta) = \frac{1}{n} \sum \hat \omega_{jt}(\theta)^2.
\end{align}
Also define a GMM measure of fit constructed with the OLS moments as 
\begin{align}\label{eq:QnOLS}
Q^{OLS}(\theta) = h(\theta)'W h(\theta)
\end{align}
 for
\begin{align}\label{eq:gn_OLS}
h(\theta) = \frac{1}{n} \Delta'\hat\omega(\theta),
\end{align}
and $W$ equals to $(\Delta'\Delta)^{-1}$.
Then, the two functions $Q^{RSS}(\theta)$ and $Q^{OLS}(\theta)$ are equal up to a constant, and have the same minimizers. It follows that:
\begin{align*}
T^{RSS} &= \sqrt{n} \frac{Q_1^{OLS} - Q_2^{OLS}}{\hat\sigma_{RSS}}    
\end{align*}

\end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma2}]

We can rewrite (\ref{eq:QnOLS}) in matrix notation as:
\begin{align}
n\cdot Q^{OLS}(\theta) &= \hat \omega(\theta)' \Delta (\Delta'\Delta)^{-1} \Delta'\hat \omega(\theta)\\
&= p'\Delta (\Delta'\Delta)^{-1} \Delta'p + (\theta'\Delta' \Delta \theta) - 2p'\Delta \theta \\
&= p'p-p'p+p'\Delta (\Delta'\Delta)^{-1} \Delta'p + (\theta'\Delta' \Delta \theta) - 2p'\Delta \theta \\
&= n\cdot Q^{RSS}(\theta) -(p'p-p'\Delta (\Delta'\Delta)^{-1} \Delta'p)\\
&= n\cdot Q^{RSS}(\theta) + c_n.
\end{align}
Since the functions $Q^{OLS}$ and $Q^{RSS}$ are equal up to the constant  $\frac{c_n}{n}$,  they also have the same minimizer $( \hat \theta_{OLS})$. Moreover, 
\begin{align}
   Q^{RSS}(\theta_1) - Q^{RSS}(\theta_2) &= Q_1^{RSS} - Q_2^{RSS}\\          
   &=Q_1^{OLS} - Q_2^{OLS}. 
\end{align}
\end{proof}

\begin{proof}[Proof of Proposition 3:]

By Lemma 1, the RSS test statistic is:
\begin{align}
T^{RSS} &= \sqrt{n} \frac{Q_1^{OLS} - Q_2^{OLS}}{\hat\sigma_{RSS}}
\end{align}
where $\hat\sigma^{RSS}_{I,II} \rightarrow_p \sqrt{\sigma^{2,RSS}_{I,II}}$ and $\sigma^{2 RSS}_{I,II}$ is the asymptotic variance of $\sqrt{n}(Q_1^{OLS} - Q_2^{OLS})$. To
derive the plim of the test statistic, first consider the object:
\begin{align*}
Q_1^{OLS} - Q_2^{OLS}
&= g_1'Wg_1 - ng_2'Wg_2\\
&= -(\theta_1-\theta_2)'\hat A_{\Delta\Delta}(\theta_1-\theta_2)-2(\theta_1-\theta_2)'\frac{\Delta'\omega_0}{n}\\
& \rightarrow_p  -(\theta_1-\theta_2)'A_{\Delta\Delta}(\theta_1-\theta_2) -2(\theta_1-\theta_2)'E[\Delta'\omega_0]\\
&= -E[(\Delta_{1i} -\Delta_{2i} )^2] - 2(\theta_1-\theta_2)' E[\Delta_i\Delta_i'](\theta_{OLS} -\theta_0)\\
&= -E[(\Delta_{1i} -\Delta_{2i} )^2] -  2E[(\Delta_{1i}-\Delta_{2i})'(\Delta_{OLS,i} -\Delta_{1i})]\\
&=E[(\Delta_{OLS,i} -\Delta_{1i}))^2 - (\Delta_{OLS,i} -\Delta_{2i}))^2],	
\end{align*}
so that we have
\begin{align}
\frac{T^{RSS}}{\sqrt{n}} &\rightarrow_p  \frac{E[(\Delta_{OLS,i} -\Delta_{1i}))^2 - (\Delta_{OLS,i} -\Delta_{2i}))^2]	}{\sigma^{RSS}_{I,II}}.
\end{align} 
\end{proof}

==> Submission/ReStud/Proofs/Pf_RVDistribWeakInstr.tex <==
We start by recapping our setup of weak instruments for testing. Recall our model:
\begin{align*}
    p = \Delta_0 + \omega_0,
\end{align*}
and for model $m$ we define a modified first stage regression:
\begin{align*}
    \Delta_0 - \Delta_m = z(\Gamma^*_0 - \Gamma_m) + e_m.
\end{align*}
Then, we adopt a weak instrument asymptotics similar to \cite{ss97}: $(\hat\Gamma^{*}_0-\hat\Gamma_m) = \frac{q_m}{\sqrt{n}} + o_p(n^{-1/2})$ for a finite vector $q_m$. This is a special case of weak instruments for testing as defined in Proposition \ref{prop:degen}. Under this weak instruments for testing asymptotics, we have:
\begin{align}
\frac{z'\omega_0}{\sqrt{n}} &\rightarrow_d \xi_{\omega_0}\\
\frac{z'e_m}{\sqrt{n}} &\rightarrow_d \xi_{e_m}\\ 
%\frac{z'p}{\sqrt{n}}&=\frac{z'\Delta_0^* +z'e_0^* + z'\omega_0 }{\sqrt{n}}\\ &\rightarrow_d A_{zz}'c^*_0 + \xi_{e^*_0} + \xi_{\omega_0}\\
\frac{z'(\Delta_0 - \Delta_m)}{\sqrt{n}} &\rightarrow_d A_{zz}q_m + \xi_{e_m}\\
\frac{z'(p-\Delta_m)}{\sqrt{n}} &\rightarrow_d A_{zz}q_m + \xi_{e_m}+ \xi_{\omega_0}\\
\hat A_{zz}^{-1/2}\frac{z'(p-\Delta_m)}{\sqrt{n}} &\rightarrow_d A_{zz}^{1/2} q_m + A_{zz}^{-1/2}\bigg(\xi_{e_m}+ \xi_{\omega_0}\bigg)\\
&= D_m
%\Delta'z(z'z)^{-1}z'\Delta &\rightarrow_d ((A_{zz} C + \xi_e)' A^{-1}_{zz}(A_{zz} C + \xi_e))\\
%\hat\theta_{2SLS} &\rightarrow_d ((A_{zz} C + \xi_e)' A^{-1}_{zz}(A_{zz} C + \xi_e))^{-1}((A_{zz} C + \xi_e)' A^{-1}_{zz}(A_{zz} c^*_0 + \xi_{e^*_0}))\\
%&\qquad + ((A_{zz} C + \xi_e)' A^{-1}_{zz}(A_{zz} C + \xi_e))^{-1}((A_{zz} C + \xi_e)' A^{-1}_{zz}\xi_{\omega_0})
\end{align}
where, if we denote $\xi = (\xi_{\omega_0},\xi_{e_1},\xi_{e_2})$ and $u = (\omega_0, e_1, e_2)$ then $vec(\xi) \sim N(0,E[u_i u_i' \otimes z_i z_i'])$. We also define $$E[u_iu_i'] = \begin{bmatrix} \sigma^2_{\omega_0} & 
\sigma_{\omega_0e_1} &
\sigma_{\omega_0e_2} \\  
\sigma_{\omega_0e_1} &  
\sigma^2_{e_1} &
\sigma_{e_1e_2}\\
\sigma_{\omega_0e_2} & 
\sigma_{e_1e_2} &
\sigma^2_{e_2}
\end{bmatrix}.
$$

Thus, letting $D = (D_1,D_2)'$, the joint distribution of $D$ is given as $D \sim N( D_0 , V)$
where $D_0 = (A_{zz}^{1/2} q_1,A_{zz}^{1/2} q_2)'$ and $$V = \begin{bmatrix}
\sigma^2_{\omega_0} + \sigma^2_{e_1} + 2 \sigma_{\omega_0 e_1} &\sigma^2_{\omega_0} + \sigma_{\omega_0 e_1}+ \sigma_{\omega_0 e_2} + \sigma_{e_1 e_2} \\
\sigma^2_{\omega_0} + \sigma_{\omega_0 e_1}+ \sigma_{\omega_0 e_2} + \sigma_{e_1 e_2} & \sigma^2_{\omega_0} + \sigma^2_{e_2} + 2 \sigma_{\omega_0 e_2}
\end{bmatrix}\otimes I_{d_z}$$.

With the preliminaries defined, we now use them to derive the distribution of the RV test statistic under a weak instruments for testing asymptotic.  We first consider the numerator of $T^{RV}$.  First note the following:
\begin{align*}
   Q_1 - Q_2 
&= (g_1-g_2)'W(g_1+g_2)\\
&= \frac{1}{n}\bigg((p-\Delta_1)-(p-\Delta_2)\bigg)'z(z'z)^{-1}z'\bigg(p - \Delta_1 +(p-\Delta_2)\bigg)\\
&= \bigg(\frac{(p-\Delta_1)'z}{n}\hat A_{zz}^{-1/2}-\frac{(p-\Delta_2)'z}{n}\hat A_{zz}^{-1/2}\bigg)\bigg( \hat A_{zz}^{-1/2}\frac{z'(p - \Delta_1)}{n} + \hat A_{zz}^{-1/2}\frac{z'(p-\Delta_2)}{n}\bigg)
\end{align*}

so that:
\begin{align*}
     n(Q_1 - Q_2) & = \bigg(\frac{(p-\Delta_1)'z}{\sqrt{n}}\hat A_{zz}^{-1/2}-\frac{(p-\Delta_2)'z}{\sqrt{n}}\hat A_{zz}^{-1/2}\bigg)\bigg( \hat A_{zz}^{-1/2}\frac{z'(p - \Delta_1)}{\sqrt{n}} + \hat A_{zz}^{-1/2}\frac{z'(p-\Delta_2)}{\sqrt{n}}\bigg)\\ &\rightarrow_d  (D_1-D_2)'(D_1+D_2)
     %\bigg( A_{zz}c_2 + \xi_{e_2}- A_{zz}c_1 - \xi_{e_1}\bigg)'A_{zz}^{-1}\bigg(2A_{zz}c^*_0 + 2\xi_{e^*_0} + 2\xi_{\omega_0} - A_{zz}c_1 - \xi_{e_1}- A_{zz}c_2 - \xi_{e_2}\bigg)\\
     %&= \bigg( A_{zz}^{1/2}c_2 + A_{zz}^{-1/2}\xi_{e_2}- A_{zz}^{1/2}c_1 - A_{zz}^{-1/2}\xi_{e_1}\bigg)'\\
     %&\qquad \times \bigg(2A_{zz}^{1/2}c^*_0 + 2A_{zz}^{-1/2}\xi_{e^*_0} + 2A_{zz}^{-1/2}\xi_{\omega_0} - A_{zz}^{1/2}c_1 - A_{zz}^{-1/2}\xi_{e_1}- A_{zz}^{1/2}c_2 - A_{zz}^{-1/2}\xi_{e_2}\bigg)\\
     %&= \bigg( \iota_1 - \iota_2 + A_{zz}^{-1/2}\xi_{e_2} -A_{zz}^{-1/2}\xi_{e^*_0} - A_{zz}^{-1/2}\xi_{e_1}+A_{zz}^{-1/2}\xi_{e^*_0}
     %+A_{zz}^{-1/2}\xi_{\omega_0}-A_{zz}^{-1/2}\xi_{\omega_0}\bigg)'\\
     %&\qquad \times \bigg(\iota_1 + \iota_2 + 2A_{zz}^{-1/2}\xi_{e^*_0} + 2A_{zz}^{-1/2}\xi_{\omega_0} - A_{zz}^{-1/2}\xi_{e_1} - A_{zz}^{-1/2}\xi_{e_2}\bigg)\\
\end{align*}



Now we consider the denominator of the test statistic.  In particular, we define an estimator of the asymptotic variance, denoted $\hat \sigma^2_{RV}$, as:\footnote{See \cite{hp11} for the exact asymptotic variance of the RV test statistic without weak instruments.} 
\begin{align}
    \hat\sigma_{RV}^2 
&= 4g_1'\hat A_{zz}^{-1}\Sigma_1 \hat A_{zz}^{-1}g_1 +4g_2'\hat A_{zz}^{-1}\Sigma_2 \hat A_{zz}^{-1} g_2 - 8g_1'\hat A_{zz}^{-1}\Sigma_{1,2} \hat A_{zz}^{-1} g_2.
\end{align}
where
\begin{align}
&\Sigma_m = \frac{1}{n}\sum_{i=1}^n \bigg( z_i\hat \omega_{mi} \bigg) \bigg(z_i \hat\omega_{mi} \bigg)'\label{eq:Sigma_m}\\
%
&\Sigma_{1,2} = \frac{1}{n}\sum_{i=1}^n \bigg( z_i \hat \omega_{1i} \bigg) \bigg( z_i \hat \omega_{2i} \bigg) '
\end{align}

We first examine the convergence of $g_1$ and $g_2$:
\begin{align*}
    \sqrt{n} g_m &= \hat A_{zz}^{1/2} \hat A_{zz}^{-1/2}\frac{z'\Delta^*_0-z'\Delta_m + z'\omega_0}{\sqrt{n}}\\
    &\rightarrow_d A_{zz}^{1/2} \bigg(A_{zz}^{1/2}c^*_0 + A_{zz}^{-1/2}\xi_{e^*_0} + A_{zz}^{-1/2}\xi_{\omega_0} - A_{zz}^{1/2}c_m - A_{zz}^{-1/2}\xi_{e_m}\bigg)\\
        &= A_{zz}^{1/2} D_m
\end{align*}

Now, we examine the convergence of $\Sigma_m$.  In doing so, it is convenient to define $u_{mi} = \omega_{0i}+e_{mi}$:
\begin{align}
       \Sigma_m &= \frac{1}{n}\sum_{i=1}^n ( z_i \hat \omega_m) ( z_i \hat \omega_m)'\\
       %&=\frac{1}{n}\sum_{i=1}^n \bigg( z_i( p_i-\Delta_{mi}) \bigg) \bigg( z_i( p_i-\Delta_{mi}) \bigg)'\\
       &=\frac{1}{n}\sum_{i=1}^n \bigg( z_i( \Delta^*_{0i}+\omega_{0i}-\Delta_{mi}) \bigg) \bigg( z_i(\Delta^*_{0i}+\omega_{0i}-\Delta_{mi}) \bigg)'\\
       &=\frac{1}{n}\sum_{i=1}^n \bigg(  z_iz_{i}'\frac{q_m}{\sqrt{n}}+z_i(e_{mi}+\omega_{0i}) \bigg) \bigg( z_iz_{i}'\frac{q_m}{\sqrt{n}}+z_i(e_{mi}+\omega_{0i}) \bigg)'\\
     %&=\frac{1}{n}\sum_{i=1}^n \bigg(  z_iz_{i}'\frac{q_m}{\sqrt{n}}+z_iu_{mi} \bigg) \bigg( z_iz_{i}'\frac{q_m}{\sqrt{n}}+z_iu_{mi} \bigg)'\\
       &=\frac{1}{n}\sum_{i=1}^n  z_iz_{i}'\frac{q_m}{\sqrt{n}}\frac{q_m'}{\sqrt{n}}z_iz_{i}'+ \frac{1}{n}\sum_{i=1}^n  z_iz_{i}'\frac{q_m}{\sqrt{n}}'u_{mi}z_i'
 +\frac{1}{n}\sum_{i=1}^n z_iu_{mi}'\frac{q_m'}{\sqrt{n}}z_iz_{i}' +\frac{1}{n}\sum_{i=1}^n z_iu_{mi}'u_{mi} z_i'\\
 &\rightarrow_p (\sigma^2_{\omega_0} + \sigma^2_{e_m}  +2\sigma_{\omega_0e_m}) A_{zz}
\end{align}
By similar steps,  $\Sigma_{12}\rightarrow_p (\sigma^2_{\omega_0} + \sigma_{\omega_0e_1} +\sigma_{\omega_0e_2} + \sigma_{e_1e_2}) A_{zz}$.

Thus, the denominator of the RV test converges in distribution as follows:
\begin{align*}
    \hat\sigma^2&=4g_1'\hat A_{zz}^{-1}\Sigma_1 \hat A_{zz}^{-1}g_1 +4g_2'\hat A_{zz}^{-1}\Sigma_2 \hat A_{zz}^{-1} g_2 - 8g_1'\hat A_{zz}^{-1}\Sigma_{1,2} \hat A_{zz}^{-1} g_2\\
    &\rightarrow_d %4\sigma^2_{u_1}D_1'A_{zz}^{1/2} A_{zz}^{-1}A_{zz}A_{zz}^{-1}A_{zz}^{1/2} D_1 + 4\sigma^2_{u_2}D_2'A_{zz}^{1/2} A_{zz}^{-1}A_{zz}A_{zz}^{-1}A_{zz}^{1/2} D_2 - 8\sigma^2_{u_{12}}D_1'A_{zz}^{1/2} A_{zz}^{-1}A_{zz}A_{zz}^{-1}A_{zz}^{1/2} D_2\\
    4\sigma^2_{u_1}D_1'D_1 + 4\sigma^2_{u_2}D_2'D_2 - 8\sigma^2_{u_{12}}D_1'D_2\\
    &= 4 \bigg(D'\begin{bmatrix}I_{d_z} & 0 \\0 &-I_{d_z} \end{bmatrix}V\begin{bmatrix}I_{d_z} &0 \\0 &-I_{d_z} \end{bmatrix}D\bigg)
\end{align*}



Using the convergence results for the numerator and denominator, we can thus construct an asymptotic distribution for the test statistic $T^{RV}$. 
\begin{align}
    T^{RV} &\rightarrow_d\frac{D_1'D_1 - D_2'D_2}{2\sqrt{D'\begin{bmatrix}I_{d_z} & 0 \\0 &-I_{d_z} \end{bmatrix}V\begin{bmatrix}I_{d_z} &0 \\0 &-I_{d_z} \end{bmatrix}D}}
\end{align}
It is useful to consider an equivalent representation of the asymptotic distribution of $T^{RV}$. This representation is based on the rotation proposed in Magnolfi, Soelvsten, and Sullivan (2021). Consider $\pi = (\pi_1,\pi_2)' = (D_1+D_2,D_1-D_2)' = RD$ where $R = \begin{bmatrix} 1 & 1 \\ 1 & -1\end{bmatrix}$.  Thus, the distribution of $\pi$ is given as: $\pi \sim N(R D_0, \Omega)$ where $\Omega = R V R$.  Then we can write $T^{RV}$ as a function of $\pi$.

\begin{align}
    T^{RV} 
  &\rightarrow_d \frac{(D_1+D_2)'(D_1-D_2)}{2\sqrt{D'\begin{bmatrix}I_{d_z} & 0 \\0 &-I_{d_z} \end{bmatrix}V\begin{bmatrix}I_{d_z} &0 \\0 &-I_{d_z} \end{bmatrix}D}} \\ 
      %&= \frac{(D_1'+D_2)'(D_1-D_2)}{2\sqrt{D'\begin{bmatrix}I_{d_z} & I_{d_z}  \\I_{d_z}  &-I_{d_z} \end{bmatrix}\begin{bmatrix}0& I_{d_z}  \\I_{d_z}  &0 \end{bmatrix}\begin{bmatrix}.5I_{dz} &.5I_{dz} \\.5I_{dz} &-.5I_{dz} \end{bmatrix}V\begin{bmatrix}.5I_{dz} &.5I_{dz} \\.5I_{dz} &-.5I_{dz} \end{bmatrix}\begin{bmatrix}0& I_{d_z}  \\I_{d_z}  &0 \end{bmatrix}\begin{bmatrix}I_{d_z} & I_{d_z}  \\I_{d_z}  &-I_{d_z} \end{bmatrix}D}} \\ 
       &= \frac{(D_1+D_2)'(D_1-D_2)}{\sqrt{D'\begin{bmatrix}I_{d_z} & I_{d_z}  \\I_{d_z}  &-I_{d_z} \end{bmatrix}\begin{bmatrix}0& I_{d_z}  \\I_{d_z}  &0 \end{bmatrix}\begin{bmatrix}I_{dz} &I_{dz} \\I_{dz} &-I_{dz} \end{bmatrix}V\begin{bmatrix}I_{dz} &I_{dz} \\I_{dz} &-I_{dz} \end{bmatrix}\begin{bmatrix}0& I_{d_z}  \\I_{d_z}  &0 \end{bmatrix}\begin{bmatrix}I_{d_z} & I_{d_z}  \\I_{d_z}  &-I_{d_z} \end{bmatrix}D}} \\ 
       &= \frac{(D_1+D_2)'(D_1-D_2)}{\sqrt{D'R S_p R V R S_p R D}} \\ 
        &= \frac{\pi_1'\pi_2}{\sqrt{\pi' S_p\Omega S_p \pi}} 
\end{align}
where $S_p = \begin{bmatrix} 0 & I_{d_z} \\ I_{d_z} & 0 \end{bmatrix}$.

It is further useful to standardize $\pi$.  We partition $\Omega$ into four $d_z \times d_z$ block matrices.  Let $\pi^{std} = (\Omega_{11}^{-1/2} \pi_1,\Omega_{22}^{-1/2} \pi_2)\sim N(\pi_0^{std}, \Omega^{std}\otimes I_{d_z} )$, where $\pi^{std}_{01} =  \Omega_{11}^{-1/2} A^{1/2}_{zz} (q_1 + q_2) $ and $\pi^{std}_{02} =  \Omega_{22}^{-1/2} A^{1/2}_{zz} (q_1 - q_2)$ and  $\Omega^{std} = \begin{bmatrix} 1 & \rho \\ \rho & 1 \end{bmatrix}$, and  $\rho$ is the correlation between $\pi_1^{std}$ and $\pi_2^{std}$. Then we can write the asymptotic distribution of the RV test statistic as a function of $\pi^{std}$.

%\begin{align}
%    V^{std} &= \begin{bmatrix}1 & \rho\\ \rho & 1\end{bmatrix}\\
%    &= \begin{bmatrix}V_{11}^{-1/2} & 0 \\ 0 & V_{22}^{-1/2}\end{bmatrix} \begin{bmatrix}V_{11} & V_{12}\\ V_{12} & V_{22}\end{bmatrix} \begin{bmatrix}V_{11}^{-1/2} & 0 \\ 0 & V_{22}^{-1/2}\end{bmatrix}\\
%    &= S_VVS_V
%\end{align}
%so that 
%\begin{align}V &= \begin{bmatrix}V_{11}^{1/2} & 0 \\ 0 & V_{22}^{1/2}\end{bmatrix} \begin{bmatrix} 1& \rho \\ \rho & 1\end{bmatrix} \begin{bmatrix}V_{11}^{1/2} & 0 \\ 0 & V_{22}^{1/2}\end{bmatrix}\\
%&=S_V^{-1} V^{std} S_V^{-1}\end{align}

\begin{align}
     \frac{\pi_1'\pi_2}{\sqrt{\pi' S_p\Omega S_p \pi}} 
    &= \frac{\pi_1'\pi_2}{\sqrt{\pi' S_p\begin{bmatrix}\Omega_{11}^{1/2} I_{dz} & 0 \\ 0 & \Omega_{22}^{1/2} I_{dz}\end{bmatrix}\Omega^{std} \begin{bmatrix}\Omega_{11}^{1/2} I_{dz} & 0 \\ 0 & \Omega_{22}^{1/2} I_{dz}\end{bmatrix}S_p \pi}} \\
    %&= \frac{\pi_1'\pi_2}{\sqrt{\pi' S_p S^{-1}_\Omega\Omega^{std} S^{-1}_\Omega S_p \pi}} \\
    &= \frac{\pi_1'\pi_2}{\sqrt{\begin{bmatrix}\Omega_{11}^{1/2} \pi_2'  &  \Omega_{22}^{1/2} \pi_1'  \end{bmatrix}\Omega^{std} \begin{bmatrix}  \Omega_{11}^{1/2} \pi_2\\ \Omega_{22}^{1/2} \pi_1  \end{bmatrix}}} \\
        &=\frac{\Omega_{11}^{-1/2}\Omega_{22}^{-1/2}}{\Omega_{11}^{-1/2}\Omega_{22}^{-1/2}} \frac{\pi_1'\pi_2}{\sqrt{\begin{bmatrix}\Omega_{11}^{1/2} \pi_2'  &  \Omega_{22}^{1/2} \pi_1'  \end{bmatrix}\Omega^{std} \begin{bmatrix}  \Omega_{11}^{1/2} \pi_2\\ \Omega_{22}^{1/2} \pi_1  \end{bmatrix}}} \\
                %&=\frac{\pi_1^{std}'\pi_2^{std}}{\sqrt{\begin{bmatrix}\Omega_{22}^{-1/2} \pi_2'  &  \Omega_{11}^{-1/2} \pi_1'  \end{bmatrix}\Omega^{std} \begin{bmatrix}  \Omega_{22}^{-1/2} \pi_2\\ \Omega_{11}^{-1/2} \pi_1  \end{bmatrix}}} \\
                &=\frac{\pi_1^{std\prime}\pi_2^{std}}{\sqrt{\begin{bmatrix}\Omega_{11}^{-1/2} \pi_1 \\\Omega_{22}^{-1/2} \pi_2    \end{bmatrix}'S_p\Omega^{std} S_p\begin{bmatrix}  \Omega_{11}^{-1/2} \pi_1 \\\Omega_{22}^{-1/2} \pi_2 \end{bmatrix}}}\\          %&=\frac{\pi_1^{std}'\pi_2^{std}}{\sqrt{(S_\Omega\pi)'S_p\Omega^{std} S_\Omega\pi}}\\
     &=\frac{\pi_1^{std\prime}\pi_2^{std}}{\sqrt{\pi^{std\prime}S_p\Omega^{std} S_p\pi^{std}}}
\end{align}
Finally,
\begin{align}
    T^{RV} \rightarrow_d \frac{\pi_1^{std}'\pi_2^{std}}{\sqrt{\pi^{std}'S_p\Omega^{std} S_p\pi^{std}}}
\end{align}

%$V = \begin{bmatrix}
%\sigma^2_{\omega_0} + \sigma^2_{e_1} + 2 \sigma_{\omega_0 e_1} &\sigma^2_{\omega_0} + \sigma_{\omega_0 e_1}+ \sigma_{\omega_0 e_2} + \sigma_{e_1 e_2} \\
%\sigma^2_{\omega_0} + \sigma_{\omega_0 e_1}+ \sigma_{\omega_0 e_2} + \sigma_{e_1 e_2} & \sigma^2_{\omega_0} + \sigma^2_{e_2} + 2 \sigma_{\omega_0 e_2}
%\end{bmatrix}\otimes I_{d_z}$
%\begin{align}
%    \Omega &= RVR\\
 %   &= R \begin{bmatrix}
%\sigma^2_{\omega_0} + \sigma^2_{e_1} + 2 \sigma_{\omega_0 e_1} &\sigma^2_{\omega_0} + \sigma_{\omega_0 e_1}+ \sigma_{\omega_0 e_2} + \sigma_{e_1 e_2} \\
%\sigma^2_{\omega_0} + \sigma_{\omega_0 e_1}+ \sigma_{\omega_0 e_2} + \sigma_{e_1 e_2} & \sigma^2_{\omega_0} + \sigma^2_{e_2} + 2 \sigma_{\omega_0 e_2}
%\end{bmatrix}\otimes I_{d_z} R\\
%&=  \begin{bmatrix}
%2\sigma^2_{\omega_0} + \sigma^2_{e_1} + 3  \sigma_{\omega_0 e_1} + \sigma_{\omega_0 e_2} + \sigma_{e_1 e_2} &2\sigma^2_{\omega_0} + \sigma^2_{e_2} + \sigma_{\omega_0 e_1}+ 3\sigma_{\omega_0 e_2} + \sigma_{e_1 e_2} \\
%\sigma^2_{e_1}+ \sigma_{\omega_0 e_1}- \sigma_{\omega_0 e_2} - \sigma_{e_1 e_2} & -\sigma^2_{e_2} -  \sigma_{\omega_0 e_2} + \sigma_{\omega_0 e_1} + \sigma_{e_1e_2}
%\end{bmatrix}\otimes I_{d_z}R\\
%&=  \begin{bmatrix}
%4\sigma^2_{\omega_0} + \sigma^2_{e_1} + \sigma^2_{e_2} + 4  \sigma_{\omega_0 e_1} + 4 \sigma_{\omega_0 e_2} + 2\sigma_{e_1 e_2} &\sigma^2_{e_1} - \sigma^2_{e_2} + 2\sigma_{\omega_0 e_1}-2\sigma_{\omega_0 e_2}  \\
%\sigma^2_{e_1} - \sigma^2_{e_2} + 2\sigma_{\omega_0 e_1}-2\sigma_{\omega_0 e_2}& \sigma^2_{e_1} +  \sigma^2_{e_2} - 2 \sigma_{e_1e_2}
%\end{bmatrix}\otimes I_{d_z}
%\end{align}
Notice that the asymptotic distribution of the  RV test statistic depends on three paramaters, $\pi_{01}, \pi_{02}$, and $\rho$. The null space in this parameterization is characterized by $\pi_{01}'\pi_{02} = 0$.  In the null space, but far from the origin, instruments are relatively strong and the RV test statistic converges to a standard normal.  However, close to the origin, the RV test suffers from a size distortion due to degeneracy.   


==> Submission/ReStud/Proofs/Pf_Testability.tex <==
\begin{proof}[Proof of Lemma \ref{as:falsify}.]

% \noindent Let model 1 be the true model. We want to show that if and only if the condition     \begin{align}\label{eq:testability3}
%     E[(\tilde\Delta_{1i} - \tilde\Delta_{2i})^2] \neq 0
%     \end{align}
% a candidate model $m=2$ is falsified, in the sense of Definition 1:
% \begin{align}\label{eq:testability2}
% E[z_i(p_i-\Delta_{2i})]\neq0. 
% \end{align}
% As a useful preliminary, recall that the first stage is:
% \begin{align*}
% \Delta_i &= z_i\Gamma + \eta_i\\
%         &= \tilde \Delta_i + \eta_i,
% \end{align*}
% where $\eta$   is projection error orthogonal to $z$ by construction, so that $E[z_i\eta_i] = 0$.

% We first prove that (\ref{eq:testability3}) implies (\ref{eq:testability2}). Notice that a necessary and sufficient for (\ref{eq:testability3}) to be true is that there exists some nonzero measure subset $Z$ of the support of $z_i$ such that for $z_i\in Z$ we have $\tilde \Delta_{1i}\neq\tilde \Delta_{2i}.$ In turn, because of the definition of projection, it must be that for $z_i\in Z$ we have $z_i \Gamma_1 \neq z_i \Gamma_2.$ Then, we know that $\Gamma_1 \neq  \Gamma_2$ which in turn implies $E[z_i\Delta_{1i}] \neq E[z_i\Delta_{2i}]$ since $\Gamma = E[z_iz_i']^{-1}E[z_i\Delta_i] $. Condition (\ref{eq:testability2}) follows immediately from the fact that model $m=1$ is the true model.

% Now we prove that (\ref{eq:testability2}) implies (\ref{eq:testability3}). To do so, we proceed by contradiction: suppose that (\ref{eq:testability2}) holds, but $ E[(\tilde\Delta_{1i} - \tilde\Delta_{2i})^2]=0.$ Then, almost surely $\tilde \Delta_{1i}=\tilde \Delta_{2i}$. Hence we can write:
% \begin{align*}
%     E[z_i(p_i - \tilde \Delta_{1i})] = E[z_i(p_i - \tilde \Delta_{2i})],
% \end{align*}
% and since $E[z_i\eta_i] = 0$ we have:
% \begin{align*}
%     E[z_i(p_i - \tilde \Delta_{1i} - \eta_{1i})] = E[z_i(p_i - \tilde \Delta_{2i} - \eta_{2i})],
% \end{align*}
% which leads to a contradiction of (\ref{eq:testability2}). Hence, when (\ref{eq:testability2}) holds, (\ref{eq:testability3}) must hold as well.

%This is now the proof that our definition corresponds to that in BH14 under parametric restrictions.\\

In our parametric framework, the falsifiable condition in Equation (28) of \cite{bh14} is\footnote{See Section 6, Case 2 in \cite{bh14} for a discussion of their non-parametric environment.}
\begin{align}\label{eq:BH14}
    E[ \boldsymbol{p}_i-\boldsymbol{\Delta}_{mi} \mid z_i,\textbf{w}_i ] = \textbf{w}_i \tau + E[ \omega_{0i} \mid z_i,\textbf{w}_i ] \quad \text{a.s.}
\end{align}
This equation, together with residualization against $\textbf{w}_i$ and integration over the distribution of  $\textbf{w}_i$, then implies that
\begin{align}\label{eq:BH14}
    E[ {p}_i-{\Delta}_{mi} \mid z_i ] = E[ \omega_{0i} \mid z_i] \quad \text{a.s.}
\end{align}
Integrating the above against $z_i$, using the assumption $E[z_i\omega_{0i} ]=0$, and relying on the law of iterated expectations, then yields
\begin{align}
    E[z_i(p_i-\Delta_{mi})] = 0
\end{align}
Finally, we note the equivalence
\begin{align}\label{eq:equivalence}
    E[(\Delta_{0i}^{z}-\Delta_{mi}^z)^2] = 0 \quad  &\Leftrightarrow \quad E[z_i(p_i-\Delta_{mi})] = 0 
\end{align}
which follows from \eqref{eq:line1}, \eqref{eq:line4}, and $E[z_i z_i']$ being positive definite. Thus we have shown that Equation (28) of \cite{bh14} implies \eqref{eq:testability}.
%
%
%{The falsifiable condition in Equation (28) of \cite{bh14} is the right most expression in \eqref{eq:equivalence}, as our environment is nested in their nonparametric testing setup. See Section 6, Case 2 in \cite{bh14} for a discussion of their environment.  After conditioning on $\textbf{w}$, the marginal revenue function for model $m$ is $p_i - \Delta_{mi}$.  So, under constant marginal costs, condition (28) in \cite{bh14} for a model to be testable becomes the one above:$ E[p_i - \Delta_{mi} \!\mid\! z_i,\textbf{w}_i]=0$ with probability one.}
%
% Part (ii) of Assumption \ref{as:regcond} implies that $E[z'z]$ and $E[z_i z_i']$ are positive definite so that $\Gamma_m = E[z'z]^{-1} E[z'\Delta_m] = E[z_iz_i']^{-1} E[z_i\Delta_{mi}]$ and $\Delta_{mi}^z = z_i'\Gamma_m$ are well-defined. We can then note that
% \begin{align}
%     E[(\Delta_{0i}^{z}-\Delta_{mi}^z)^2] &= E[(z_i'(\Gamma_0-\Gamma_m))^2] \\
%     &= (\Gamma_0-\Gamma_m)'E[z_i z_i'](\Gamma_0-\Gamma_m) \\
%     &= E[z_i(\Delta_{0i}-\Delta_{mi})]'E[z_i z_i']^{-1}E[z_i(\Delta_{0i}-\Delta_{mi})]\\
%     &= E[z_i(p_i-\Delta_{mi})]'E[z_i z_i']^{-1}E[z_i(p_i-\Delta_{mi})]
% \end{align}
% where the last equality follows from Assumption \ref{as:momcond}, $E[z_i w_{0i}]=0$, and $\Delta_{0i} = p_i - \omega_{0i}$. The equivalence in \eqref{eq:equivalence} now follows from $E[z_i z_i']$ being positive definite.
\end{proof}

==> Submission/ReStud/Proofs/Pf_WkInstrAsymptotic_Trv_F.tex <==
\begin{proof}[Proof of Proposition \ref{prop:wkinstrF}.]
The proof proceeds in three steps. Step (1) provides a function of the data $(\tilde \Psi_-',\tilde \Psi_+')'$ and two constants $\mu_-$, $\mu_+$ such that $(\tilde \Psi_-',\tilde \Psi_+')' \xrightarrow{d} (\Psi_-',  \Psi_+')'$. All of $(\tilde \Psi_-',\tilde \Psi_+')'$, $\mu_-$, and $\mu_+$ are also functions of the DGP. Step (2) establishes parts $(ii)$--$(iv)$. Step (3) shows that $\abs{T^\text{RV}} = \abs{\tilde \Psi_-'\tilde \Psi_+}/\big(\norm{\tilde \Psi_-}^2 + \norm{\tilde \Psi_+}^2 + 2 \rho \tilde \Psi_-'\tilde \Psi_+ + o_p(1) \big)^{1/2}$ and $F=\big( \norm{\tilde \Psi_-}^2 + \norm{\tilde \Psi_+}^2 - 2\rho \tilde \Psi_-'\tilde \Psi_+ \big)/\big(2d_z \big) + o_p(1)$. Part $(i)$ follows from continuous mapping, step (1), and step (3).
	
	
\noindent \textbf{Step (1)} We first provide definitions of $\mu_-$ and $\mu_+$. Let $\tau_+ = 2(\sigma_1^2 + \sigma_2^2 + 2\sigma_{12})^{1/2}$ and $\tau_- = 2(\sigma_1^2 + \sigma_2^2 - 2\sigma_{12})^{1/2}$ and use these two positive constants to define% the vectors
\begin{align}
		\begin{pmatrix}
			 \mu_1 \\  \mu_2
		\end{pmatrix}  =
		\left(\frac{1}{{\tau_-}} + \frac{1}{{\tau_+}}\right)\! \begin{pmatrix} \sqrt{n} W^{1/2} g_1    \\	 	-\sqrt{n} W^{1/2}  g_2		\end{pmatrix}
		+
		\left(\frac{1}{{\tau_-}} - \frac{1}{{\tau_+}}\right)\!\begin{pmatrix}	-\sqrt{n} W^{1/2}  g_2  \\ 		\sqrt{n} W^{1/2}  g_1 		\end{pmatrix}\!.
\end{align}
Defining $\kappa = 1 + \mathbf{1}\{ \norm{\mu_1} \le \norm{\mu_2}  \}$, we then let $\mu_- = \norm{\mu_\kappa} - \norm{\mu_{3-\kappa}}$ and $\mu_+ = \norm{\mu_1} + \norm{\mu_2}$. Since the instruments are weak for testing, we have that $\sqrt{n} W^{1/2} g_m = E[z_i z_i']^{1/2} q_m$ so $\mu_-$ and $\mu_+$ do not depend on $n$. 
	
	
To introduce $\tilde \Psi_-$ and $\tilde \Psi_+$, we let ${\cal Q}_m \in \R^{d_z \times d_z}$ be a non-random orthogonal matrix $({\cal Q}_m{\cal Q}_m'={\cal Q}_m'{\cal Q}_m=I_{d_z})$ such that ${\cal Q}_m \mu_m = \norm{\mu_m} \boldsymbol e_1$. With these matrices in hand, we define $\tilde \Psi_- = \tilde \mu_\kappa - \tilde \mu_{3-\kappa}$ and $\tilde \Psi_+ = \tilde \mu_1 + \tilde \mu_2$ where
\begin{align}
		\begin{pmatrix}
			\tilde \mu_1 \\ \tilde \mu_2
		\end{pmatrix} = 
		\left(\frac{1}{{\tau_-}} + \frac{1}{{\tau_+}}\right)\! \begin{pmatrix} \sqrt{n} {\cal Q}_1\hat W^{1/2} \hat g_1    \\	 	-\sqrt{n} {\cal Q}_2\hat W^{1/2}  \hat g_2		\end{pmatrix}
		+
		\left(\frac{1}{{\tau_-}} - \frac{1}{{\tau_+}}\right)\!\begin{pmatrix}	-\sqrt{n} {\cal Q}_1\hat W^{1/2}  \hat g_2  \\ 		\sqrt{n} {\cal Q}_2\hat W^{1/2}  \hat g_1 		\end{pmatrix}\!.
\end{align}
	
	
The preceding definitions imply that $(\tilde \Psi_-',\tilde \Psi_+')' = \sqrt{n} A (\hat g_1'\hat W^{1/2},\hat g_2'\hat W^{1/2} )'$ for a particular non-random matrix $A \in \mathbb{R}^{2d_z \times 2d_z}$ with $\sqrt{n} A ( g_1' W^{1/2}, g_2' W^{1/2} )' = (\mu_-\boldsymbol e_1',\mu_+\boldsymbol e_1')'$. Since $\mu_-$ and $\mu_+$ do not depend on $n$, it therefore follows from Lemma \ref{lem:asymp norm}, part $(i)$, that $(\tilde \Psi_-',\tilde \Psi_+')' \xrightarrow{d} (\Psi_-',  \Psi_+')'$ provided that $AV^\text{RV}A' = {\tiny \begin{bmatrix} 1 & \rho \\ \rho & 1 \end{bmatrix} }\otimes I_{d_z}$ where $\rho$ is the correlation between $e_{\kappa i}-e_{3-\kappa, i}$ and $e_{1i}+e_{2i}$. To see why this convergence occurs, note first that weak instruments for testing (Assumption \ref{as:wkinstr}) implies that $g_m = O(n^{-1/2})$ for $m=1,2$, which in turn yields that the second part of $\psi_{mi}$ is $O_p(n^{-1/2})$. From Assumption \ref{as:homsked}, we then have
\begin{align}\label{eq:varconv}
		V^\text{RV}_{\ell k} = W^{1/2} E[ e_{\ell i} e_{k i} z_iz_i'] W^{1/2} + O(n^{-1/2}) = \sigma_{\ell k} I_{d_z} + O(n^{-1/2})
\end{align}
where we write $\sigma_{mm}$ for $\sigma_m^2$. Thus, we have that $V^\text{RV} = {\tiny \begin{bmatrix} \sigma_1^2 & \sigma_{12} \\ \sigma_{12} & \sigma_{2}^2 \end{bmatrix} }\otimes I_{d_z} .$ Furthermore, we note that $A$ takes the form
\begin{align}
			A = 
			\begin{bmatrix}	(-1)^{3-\kappa}I & (-1)^\kappa I \\ I & I	\end{bmatrix}
			\begin{bmatrix}	{\cal Q}_1 & 0 \\ 0 & {\cal Q}_2	\end{bmatrix}
			\begin{bmatrix}	I & I \\ I & -I	\end{bmatrix}
			\begin{bmatrix}	I\tau_-^{-1} & 0 \\ 0 & I\tau_+^{-1}	\end{bmatrix}
			\begin{bmatrix}	I & -I \\ I & I	\end{bmatrix}
\end{align}
and leave the verification of $A\big( {\tiny \begin{bmatrix} \sigma_1^2 & \sigma_{12} \\ \sigma_{12} & \sigma_{2}^2 \end{bmatrix} }\otimes I_{d_z} \big)A' = {\tiny \begin{bmatrix} 1 & \rho \\ \rho & 1 \end{bmatrix} }\otimes I_{d_z}$ to the reader.
	
	
\noindent \textbf{Step (2)} Part $(iv)$ is an immediate implication of the triangle inequality and the definitions $\mu_- = \norm{\mu_\kappa} - \norm{\mu_{3-\kappa}}$ and $\mu_+ = \norm{\mu_1} + \norm{\mu_2}$. For part $(ii)$, we have that $\mu_-=0$ if and only if $\norm{\mu_1}^2 - \norm{\mu_2}^2 =0$. In turn, we have that
\begin{align}
		\norm{\mu_1}^2 - \norm{\mu_2}^2 &= n\!\left( \!\left(\tau_-^{-1} + \tau_+^{-1} \right)^2  - \!\left(\tau_-^{-1} - \tau_+^{-1} \right)^2 \right)\! \left( Q_1 - Q_2\right) \\
		&=4n (\tau_+ \tau_-)^{-1} \left( Q_1 - Q_2\right),
\end{align}
from which part $(ii)$ is immediate. For part $(iii)$, we have that $\mu_+=0$ if and only if $\norm{\mu_1}^2 + \norm{\mu_2}^2 =0$. We now have,
\begin{align}
			\norm{\mu_1}^2 \!+\! \norm{\mu_2}^2
			&\!=\! n\!\begin{pmatrix} W^{1/2}g_1  \\ W^{1/2}g_2	\end{pmatrix}'\!
			A'A 
			\!\begin{pmatrix} W^{1/2}g_1  \\ W^{1/2}g_2	\end{pmatrix} \!
			=\! n\!\begin{pmatrix} W^{-1/2}\pi_1  \\ W^{-1/2}\pi_2	\end{pmatrix}'\!
			A'A 
			\!\begin{pmatrix} W^{-1/2}\pi_1  \\ W^{-1/2}\pi_2	\end{pmatrix} \!
\end{align}
so part $(iii)$ follows from the positive definiteness of both $W$ and the matrix $A'A = 4 \!{\tiny \begin{bmatrix} \tau_+^{-2} + \tau_-^{-2} & \tau_+^{-2} - \tau_-^{-2} \\ \tau_+^{-2} - \tau_-^{-2} & \tau_+^{-2} + \tau_-^{-2} \end{bmatrix} }\!\otimes I_{d_z}$.

		
\noindent \textbf{Step (3)} For $T^\text{RV}$ we first consider the numerator. Here, we observe that
\begin{align}
		\tilde \Psi_-' \tilde\Psi_+ = \tilde \mu_\kappa'\tilde \mu_\kappa - \tilde \mu_{3-\kappa}'\tilde \mu_{3-\kappa} = 4n (\tau_+ \tau_-)^{-1} \!\left( \hat Q_\kappa - \hat Q_{3-\kappa}\right)
\end{align}
so that $\sqrt{n}\abs{\hat Q_1-\hat Q_2} = (\tau_+\tau_-/4)\abs{\tilde\Psi_-' \tilde\Psi_+}/\sqrt{n}$. For the denominator, we initially note that Lemma \ref{lem:asymp norm}, part $(ii)$, and Equation \eqref{eq:varconv} yields that
\begin{align}
		(\tau_+ \tau_-/4)^{-2} n \hat \sigma^2_\text{RV} = \tfrac{4^3n}{\tau_+^2\tau_-^2}\!\left[ \sigma_1^2 \hat Q_1 + \sigma_2^2 \hat Q_2 - 2\sigma_{12} \hat g_1' \hat W \hat g_2  \right] + o_p(1).
\end{align}	
Similarly, we can calculate that
\begin{align}
		\norm{\tilde \Psi_-}^2  &+ \norm{\tilde \Psi_+}^2  + 2\rho \tilde \Psi_-'\tilde \Psi_+ 
		= n \begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix}
		'A' \bigg( {\tiny \begin{bmatrix} 1 & \rho \\ \rho & 1 \end{bmatrix} }\otimes  I_{d_z}  \bigg)A
		\begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix}\\
		&= {4^2n}{} \begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix}'
		\bigg( \! \tfrac{4}{\tau_+^2\tau_-^2}{\tiny \begin{bmatrix} \sigma_1^2 \! & \! -\sigma_{12} \\ -\sigma_{12} \! & \! \sigma_2^2 \end{bmatrix}} \!\otimes I_{d_z}  \bigg)
		\begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix} \\
		&= \tfrac{4^3n}{\tau_+^2\tau_-^2}\!\left[ \sigma_1^2 \hat Q_1 + \sigma_2^2 \hat Q_2 - 2\sigma_{12} \hat g_1' \hat W \hat g_2  \right]
\end{align}
where the second equality follows from the last sentences of steps (1) and (2) together with
\begin{align}
		{\tiny \begin{bmatrix} \tau_+^{-2} + \tau_-^{-2} & \tau_+^{-2} - \tau_-^{-2} \\ \tau_+^{-2} - \tau_-^{-2} & \tau_+^{-2} + \tau_-^{-2} \end{bmatrix} \begin{bmatrix} \sigma_1^2 & \sigma_{12} \\ \sigma_{12} & \sigma_{2}^2 \end{bmatrix}  \begin{bmatrix} \tau_+^{-2} + \tau_-^{-2} & \tau_+^{-2} - \tau_-^{-2} \\ \tau_+^{-2} - \tau_-^{-2} & \tau_+^{-2} + \tau_-^{-2} \end{bmatrix} = \begin{bmatrix} \sigma_1^2 & -\sigma_{12} \\ -\sigma_{12} & \sigma_2^2 \end{bmatrix} } \tfrac{4}{\tau_+^2\tau_-^2}.
\end{align}
Thus we have the desired conclusion
		\begin{align}
		\abs{T^\text{RV}} &= \sqrt{n}\frac{\abs{\hat Q_1 - \hat Q_2}}{\hat \sigma_\text{RV}} = \frac{4n (\tau_+ \tau_-)^{-1/2} \!\abs{ \hat Q_1 - \hat Q_2}}{\left( (\tau_+ \tau_-/4^2)\inverse n \hat \sigma^2_\text{RV}  \right)^{1/2}} \\
		&=
		 \abs{\tilde \Psi_-'\tilde \Psi_+}/\big(\norm{\tilde \Psi_-}^2 + \norm{\tilde \Psi_+}^2 + 2\kappa \tilde \Psi_-'\tilde \Psi_+  + o_p(1) \big)^{1/2}
\end{align}
	
	
For $F$, we first note that standard arguments lead to
\begin{align}
		2d_zF &=n(1-\hat \rho^2)\frac{\hat \sigma_2^2 \hat g_1' \hat W \hat g_1 + \hat \sigma_1^2 \hat g_2' \hat W \hat g_2 - 2\hat \sigma_{12} \hat g_1' \hat W \hat g_2}{\hat \sigma_1^2 \hat \sigma_2^2 - \hat \sigma_{12}^2 } \\
		&=n(1-\rho^2)\frac{\sigma_2^2 \hat Q_1 +  \sigma_1^2 \hat Q_2 - 2 \sigma_{12} \hat g_1' \hat W \hat g_2}{ \sigma_1^2  \sigma_2^2 -  \sigma_{12}^2 } + o_p(1).
\end{align}
Similarly, we can calculate that
\begin{align}
		\norm{\tilde \Psi_-}^2  &+ \norm{\tilde \Psi_+}^2  - 2\rho \tilde \Psi_-'\tilde \Psi_+ 
		= n \begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix}'
		A' \bigg( {\tiny \begin{bmatrix} 1 & -\rho \\ -\rho & 1 \end{bmatrix} }\otimes  I_{d_z}   \bigg)A
		\begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix} \\
		&= n(1-\rho^2) \begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix}'
		\bigg(  {\tiny \begin{bmatrix} \sigma_1^2  &  \sigma_{12} \\ \sigma_{12}  &  \sigma_2^2 \end{bmatrix}}\inverse \otimes I_{d_z}  \bigg)
		\begin{pmatrix}  \hat W^{1/2}\hat g_1 \\ \hat W^{1/2} \hat g_2		\end{pmatrix} \\
		&= n(1-\rho^2)\frac{\sigma_2^2 \hat Q_1 +  \sigma_1^2 \hat Q_2 - 2 \sigma_{12} \hat g_1' \hat W \hat g_2}{ \sigma_1^2  \sigma_2^2 -  \sigma_{12}^2 }
\end{align}
which follows from inverting the equality in the last sentence of step (1).
\end{proof}

==> Submission/ReStud/Proofs/Pf_absfit.tex <==
\begin{proposition}\label{prop:absfit}
Suppose that the markups $\Delta$ are unobserved and that Assumptions \ref{as:momcond} and \ref{as:regcond}  are satisfied.  Then $\hat{\tilde{\Delta}}^{2SLS} \rightarrow_p \Delta^z_{0}$
\end{proposition}


\begin{proof}
From the proof of Proposition \ref{prop:plims_TE2}, part 1, we have established that the 2SLS estimator of $\theta$ converges in probability to the following:
\begin{align*}
    \hat\theta \rightarrow _p (A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1} A_{\Delta z}  A_{z z}^{-1}A_{z\Delta^*}\theta_0
\end{align*}
Thus, for each observation $i$, the predicted markups implied by the 2SLS estimate of $\theta$ asymptotically converge to:
\begin{align*}
\hat{\tilde{\Delta}}_{2SLS,i} &\rightarrow_p  \tilde\Delta(A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1} A_{\Delta z}  A_{z z}^{-1}A_{z\Delta^*}\theta_0\\
 %&=  zA_{zz}^{-1}A_{z\Delta}(A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1} A_{\Delta z}  A_{z z}^{-1}A_{z\Delta^*}\theta_0\\
 &=  zA_{zz}^{-1}A_{z\Delta}(A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1} A_{\Delta z}  A_{z z}^{-1}A_{z\Delta^*_0}\\
 &=  ztr(A_{zz}^{-1}A_{z\Delta}(A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1} A_{\Delta z}  A_{z z}^{-1}A_{z\Delta^*_0}\\
&=  ztr(A_{z\Delta}'A_{zz}^{-1}A_{\Delta z}'(A_{\Delta z}  A_{z z}^{-1}  A_{z\Delta})^{-1}A_{z\Delta^*_0}'A_{z z}^{-1\prime})\\
 &=  ztr( A_{z\Delta^*_0}'A_{z z}^{-1\prime})\\
&=  ztr( A_{z z}^{-1}A_{z\Delta^*_0})\\
&=  z A_{z z}^{-1}A_{z\Delta^*_0}\\
&=\tilde{\Delta}^*_{0i}
\end{align*}
\end{proof}



==> Submission/ReStud/Proofs/Pf_plims_cost.tex <==
\begin{proof}[Proof of Lemma \ref{cor:cost_misc}.] 
Since $\textbf{w}_\textbf{a}$ is a subset of $\textbf{w}$, the proof follows immediately by replacing any variable $y$ residualized with respect to $\textbf{w}$ in the Proof of Lemma \ref{cor:modelmisc}, with $y^\textbf{a}$ which has been residualized with respect to $\textbf{w}_\textbf{a}$.
%
\begin{comment}
For $\textbf{w}_\textbf{a}\neq \textbf{w}$, by Equation \eqref{eq:cost_mispec2}, $p_i =  \Delta^\textbf{a}_{0i} + \omega_{0i}$, where $p_i = \boldsymbol{p}_m-\textbf{w}_{\textbf{a}}E[\textbf{w}_{\textbf{a}}'\textbf{w}_{\textbf{a}}]^{-1}E[\textbf{w}_{\textbf{a}}'\boldsymbol{p}_m]$ and $\Delta^a_m = \boldsymbol{\Delta}^{\textbf{a}}_m-\textbf{w}_{\textbf{a}}E[\textbf{w}_{\textbf{a}}'\textbf{w}_{\textbf{a}}]^{-1}E[\textbf{w}_{\textbf{a}}'\boldsymbol{\Delta}^{\textbf{a}}_m]$.  Define $\Delta^{\textbf{a}z}_{0i} = z_iE[z_iz_i']E[z_i\Delta^{\textbf{a}z}_{0i}]$.  Further, define $\Delta_m = \boldsymbol{\Delta}_m-\textbf{w}_{\textbf{a}}E[\textbf{w}_{\textbf{a}}'\textbf{w}_{\textbf{a}}]^{-1}E[\textbf{w}_{\textbf{a}}'\boldsymbol{\Delta}_m]$ and $\Delta^{z}_{mi} = z_iE[z_iz_i']E[z_i\Delta^{z}_{mi}]$.  Let $z = \boldsymbol{z}-\textbf{w}_{\textbf{a}}E[\textbf{w}_{\textbf{a}}'\textbf{w}_{\textbf{a}}]^{-1}E[\textbf{w}_{\textbf{a}}'\boldsymbol{z}]$. By Equation \eqref{eq:omega_costmisc} and under Assumption \ref{as:misspmc}, the right hand side of \eqref{eq:line4} can be rewritten as
$$E[z_i(\Delta^\textbf{a}_{0i}-\Delta_{mi})]'E[z_iz_i']^{-1}E[z_i(\Delta^\textbf{a}_{0i}-\Delta_{mi})].$$  Thus, replacing $\Delta^z_{0i}$ with $\Delta^{\textbf{a}z}_{0i}$ the equality between \eqref{eq:line1} and \eqref{eq:line4} holds as does the equality between \eqref{eq:line4} and \eqref{eq:line5}. 

\begin{itemize}
\item[(i)]  Under Assumption \ref{as:misspmc} and by the equality of \eqref{eq:line1}, \eqref{eq:line5}, and the positive definiteness of $E[z_iz_i']$, $\pi_m = 0$ iff $E[(\Delta^{\textbf{a}z}_{0i}-\Delta^{\textbf{a}z}_{mi})^2]=0$.  The proof then follows from the Proof of Lemma 2 (i). 
    \item[(ii)]  Under Assumption \ref{as:misspmc} and by the equality of \eqref{eq:line1}, \eqref{eq:line5}, and the positive definiteness of $E[z_iz_i']$, $Q_1=Q_2$ iff $E[(\Delta^{\textbf{a}z}_{0i}-\Delta^{z}_{1i})^2]=E[(\Delta^{\textbf{a}z}_{0i}-\Delta^{z}_{2i})^2]$ The proof then follows from the Proof of Lemma 2 (ii). 
\end{itemize}
\end{comment}
\end{proof}

==> Submission/ReStud/Tables/AR_results.tex <==
%\renewcommand{\arraystretch}{1.2}
\begin{widetable}{.98\columnwidth}{lccc}
\toprule
\textbf{BLP95 IVs} & 2 & 3 & 4  \\
\cmidrule(lr){2-4}
1. Zero wholesale margin&262.2$\,$,$\,$673.7&262.2$\,$,$\,$216.8&262.2$\,$,$\,$220.4\\
2. Zero retail margin &&673.7$\,$,$\,$216.8 & 673.7$\,$,$\,$220.4\\
3. Linear pricing&&&216.8$\,$,$\,$220.4\\
4. Hybrid model&&&\\
\bottomrule
\end{widetable}




==> Submission/ReStud/Tables/AR_results_slides.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}l r @{\hspace{0.1\tabcolsep}} r r @{\hspace{0.1\tabcolsep}} r}
\toprule
Model $j$ & \multicolumn{2}{c}{Full Sample}  & \multicolumn{2}{c}{20\% Sample}  \\\midrule
2.Zero retail margin & 	\only<2,5>{\cellcolor{yellow}}258.84,& \only<2,5>{\cellcolor{yellow}}654.31&	14.54,& 21.49\\
3.Linear pricing& 	\only<4-5>{\cellcolor{yellow}}258.84,& \only<4-5>{\cellcolor{yellow}}221.00&	\only<3-4>{\cellcolor{yellow}}14.54,& \only<3-4>{\cellcolor{yellow}}9.57\\
4.Hybrid model& 	\only<5>{\cellcolor{yellow}}258.84,& \only<5>{\cellcolor{yellow}}224.86&	14.54,& 9.76\\
5.Wholesale collusion& 	\only<5>{\cellcolor{yellow}}258.84,& \only<5>{\cellcolor{yellow}}218.66&	14.54,& 32.68\\
\bottomrule\end{tabular}
\end{footnotesize}



==> Submission/ReStud/Tables/ARstat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&3407.22, 5324.48&3407.22, 5825.49&3407.22, 5813.52&3407.22, 650.2\\
2.Zero retail margin&&5324.48, 5825.49&5324.48, 5813.52&5324.48, 650.2\\
3.Simple linear pricing&&&5825.49, 5813.52&5825.49, 650.2\\
4.Hybrid model&&&&5813.52, 650.2\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Submission/ReStud/Tables/ARstat2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&9.4, 18.11&9.4, 64.1&9.4, 65.74&9.4, 18.94\\
2.Zero retail margin&&18.11, 64.1&18.11, 65.74&18.11, 18.94\\
3.Simple linear pricing&&&64.1, 65.74&64.1, 18.94\\
4.Hybrid model&&&&65.74, 18.94\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Submission/ReStud/Tables/CombinedInstr.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{comment}
\begin{widetable}{.98\columnwidth}{lrrrc}
\toprule
\multicolumn{1}{l}{\textbf{Panel A: BLP95 + Diff + Cost + Demo} ($d_z=8$) } \\
& \multicolumn{3}{c}{$F_\rho$}& MCS $p$-values\\
\multicolumn{1}{l}{Models}&\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}&\\
\cmidrule(lr){2-5}
1. Zero wholesale margin&106.7&50.0&49.7&0.17 \\
2. Zero retail margin&&61.4&61.3&1.00 \\
3. Linear pricing&&&60.0&0.00 \\
4. Hybrid model&&&&0.00 \\
\midrule
\multicolumn{5}{l}{\textbf{Panel B: No PCA BLP95 + No PCA Diff + Cost + Demo } ($d_z=22$) }\\
& \multicolumn{3}{c}{$F_\rho$}& MCS $p$-values\\
\multicolumn{1}{l}{Models}&\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}&\\
\cmidrule(lr){2-5}
1. Zero wholesale margin&77.6&28.3&28.3&1.00 \\
2. Zero retail margin&&37.2&37.3&0.57 \\
3. Linear pricing&&&31.7&0.00 \\
4. Hybrid model&&&&0.00 \\
\bottomrule
\end{widetable}


\begin{widetable}{.98\columnwidth}{lrrrc}
\toprule
& \multicolumn{3}{c}{$F$-statistics} & MCS $p$-values \\
\cmidrule(lr){2-4}  \cmidrule(lr){5-5}
\multicolumn{1}{l}{Models} & 2 & 3 & 4 & \\
\midrule
\multicolumn{1}{l}{\textbf{Panel A: BLP95 + Demo + Cost + Diff} ($d_z=11$) } \\
1. Zero wholesale margin&106.7&50.0&49.7&0.17 \\
2. Zero retail margin&&61.4&61.3&1.00 \\
3. Linear pricing&&&60.0&0.00 \\
4. Hybrid model&&&&0.00 \\
\cmidrule(lr){1-5}
\multicolumn{5}{l}{\textbf{Panel B: No PCA BLP95 + Demo + Cost + No PCA Diff } ($d_z=22$) }\\
1. Zero wholesale margin&77.6&28.3&28.3&1.00 \\
2. Zero retail margin&&37.2&37.3&0.57 \\
3. Linear pricing&&&31.7&0.00 \\
4. Hybrid model&&&&0.00 \\
\bottomrule
\end{widetable}
\end{comment}

\begin{widetable}{.98\columnwidth}{lrrrrrrc}
\toprule
& \multicolumn{3}{c}{$T^\text{RV}$}& \multicolumn{3}{c}{$F$-statistics}&  MCS $p$-values\\
\cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-8}  
Models & 2 & 3 &  4 & 2 & 3 & 4 & \\ 
\midrule
\multicolumn{8}{l}{\textbf{Panel A: BLP95 + Demo + Cost + Diff} ($d_z=11$)}  \\ 
1. Zero wholesale margin&1.4&$-$11.1&$-$11.0&106.7&50.0&49.7&0.17 \\
2. Zero retail margin&&$-$5.8&$-$5.8&&61.4&61.3&1.00 \\
3. Linear pricing&&&0.0&&&60.0&0.00 \\
4. Hybrid model&&&&&&&0.00 \\
\cmidrule(lr){1-8}
\multicolumn{8}{l}{\textbf{Panel B: BLP95 + Demo + Cost + Diff} (no PCA, $d_z=22$)}  \\ 
%\multicolumn{8}{c}{\textbf{Panel B: No PCA BLP95 + Demo + Cost + No PCA Diff } ($d_z=22$)}\\
1. Zero wholesale margin&$-$0.6&$-$9.3&$-$9.3&77.6&28.3&28.3&1.00 \\
2. Zero retail margin&&$-$2.8&$-$2.8&&37.2&37.3&0.57 \\
3. Linear pricing&&&$-$1.8&&&31.7&0.00 \\
4. Hybrid model&&&&&&&0.00 \\
\bottomrule
\end{widetable}


==> Submission/ReStud/Tables/CostTable.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lccccccc}
\toprule
& Median& S.D.& Min& q10& q90& Max& \%$<0$ \\
\cline{2-8}Zero wholesale margin&0.4201&0.2312&-0.2602&2.1317&0.2309&0.7728&0.0400\\
Zero retail margin&0.5460&0.2605&0.0856&2.4372&0.3549&0.9569&0.0000\\
Simple linear pricing&0.3050&0.2150&-0.4023&1.9102&0.1241&0.6353&0.8600\\
Hybrid model&0.3102&0.2088&-0.2602&1.9102&0.1460&0.6361&0.5000\\
Wholesale collusion&0.1053&0.2546&-2.1383&1.5322&-0.1956&0.4335&31.6900\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Submission/ReStud/Tables/Coxstat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&-1.37, -2.74&1.32, -7.13&1.39, -7.02&2.54, -5.92\\
2.Zero retail margin&&-0.92, -3.31&-0.93, -3.31&-1.42, -5.38\\
3.Simple linear pricing&&&1.05, -1.09&2.38, -4.92\\
4.Hybrid model&&&&2.4, -4.92\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Submission/ReStud/Tables/Coxstat2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&-0.43, -1.51&0.8, -4.48&0.84, -4.39&0.88, -2.53\\
2.Zero retail margin&&-0.74, -1.2&-0.74, -1.2&-0.99, -2.28\\
3.Simple linear pricing&&&0.16, -0.18&0.82, -2.09\\
4.Hybrid model&&&&0.83, -2.09\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Submission/ReStud/Tables/Dem_robustness.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{widetable}{.98\columnwidth}{lrrrrc}
\toprule
\textbf{Panel A: Logit demand, BLP95 IVs} & \multicolumn{4}{c}{$F_\rho$}& MCS $p$-values\\
&\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&906.3&427.1&428.3&174.6&0.00\\
2. Zero retail margin&&422.6&422.6&348.5&1.00\\
3. Linear pricing&&&556.8&534.1&0.00\\
4. Hybrid model&&&&534.1&0.00\\
5. Wholesale collusion&&&&&0.00\\
\midrule
\textbf{Panel B: Nested logit demand, BLP95 IVs} & \multicolumn{4}{c}{$F_\rho$}& MCS $p$-values\\
&\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&&&&& \\
2. Zero retail margin&&&&& \\
3. Linear pricing&&&&& \\
4. Hybrid model&&&&& \\
5. Wholesale collusion&&&&& \\
\bottomrule
\end{widetable}


==> Submission/ReStud/Tables/EBstat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&386.32, 1516.42&378.29, 1819&374.15, 1772.99&89.12, 40.51\\
2.Zero retail margin&&707.84, 1960.33&712.64, 1940.86&1018.38, 3455.57\\
3.Simple linear pricing&&&2365.9, 2351.24&2284.54, 24725.95\\
4.Hybrid model&&&&2225.96, 24319.23\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Submission/ReStud/Tables/EBstat2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&8.68, 79.02&2.58, 12.77&2.53, 12.31&0.42, 0.06\\
2.Zero retail margin&&6.02, 29.45&6.12, 29.51&34.27, 152.76\\
3.Simple linear pricing&&&40.08, 39.14&20.17, 156.71\\
4.Hybrid model&&&&18.82, 156.14\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Submission/ReStud/Tables/FStats_supply_all.tex <==
%\renewcommand{\arraystretch}{1.2}
\begin{widetable}{.98\columnwidth}{lrrrr}
\toprule
\textbf{Panel A: BLP95 IVs} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5} \\
\cmidrule(lr){2-5}
1. Zero wholesale margin&66.3&26.3&26.2&90.7\\
2. Zero retail margin&&36.4&36.6&79.0\\
3. Simple linear pricing&&&50.8&27.2\\
4. Hybrid model&&&&26.9\\
5. Wholesale collusion&&&&\\
\midrule
\textbf{Panel B: GH20 IVs} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5} \\
\cmidrule(lr){2-5}
1. Zero wholesale margin&5.7&2.5&2.5&3.7\\
2. Zero retail margin&&2.2&2.2&4.3\\
3. Simple linear pricing&&&1.0&2.5\\
4. Hybrid model&&&&2.5\\
5. Wholesale collusion&&&&\\
\midrule
\textbf{Panel C: Rival Cost Shifters IVs} &\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5} \\
\cmidrule(lr){2-5}
1. Zero wholesale margin&68.6&1.1&1.3&131.6\\
2. Zero retail margin&&44.8&47.0&112.9\\
3. Linear pricing&&&5.2&33.7\\
4. Hybrid model&&&&34.6\\
5. Wholesale collusion&&&&\\
\bottomrule
\end{widetable}


==> Submission/ReStud/Tables/FStats_supply_all_new.tex <==
%\renewcommand{\arraystretch}{1.2}
\begin{widetable}{.98\columnwidth}{lrrrr}
\toprule
\textbf{Panel A: BLP95 IVs} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5} \\
\cmidrule(lr){2-5}
1. Zero wholesale margin&\tikzmark{top left 1}1269.2&499.5&498.0&1264.8\\
2. Zero retail margin&&468.4&467.2&1233.8\\
3. Simple linear pricing&&&639.1&1664.2\\
4. Hybrid model&&&&1659.1\tikzmark{bottom right 1}\\
5. Wholesale collusion&&&&\\
\midrule
\textbf{Panel B: GH20 IVs} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5} \\
\cmidrule(lr){2-5}
1. Zero wholesale margin&\tikzmark{top left 2}6.3&3.7&3.7&3.9\\
2. Zero retail margin&&3.3&3.3& 4.4\\
3. Simple linear pricing&&&1.9&3.1\\
4. Hybrid model&&&&3.1\tikzmark{bottom right 2}\\
5. Wholesale collusion&&&&\\
\midrule
\textbf{Panel C: Rival Cost Shifters IVs} &\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5} \\
\cmidrule(lr){2-5}
1. Zero wholesale margin&1249.7&\tikzmark{top left 5}15.4&16.6 \tikzmark{bottom right 5}&883.3\\
2. Zero retail margin&&65.8&69.4&985.0\\
3. Linear pricing&&&82.4&1084.0\\
4. Hybrid model&&&&1102.6\\
5. Wholesale collusion&&&&\\
\bottomrule
\end{widetable}

\only<1>{\DrawBox[ultra thick, red]{top left 2}{bottom right 2}}
\only<1>{\DrawBox[ultra thick, red]{top left 5}{bottom right 5}}
\only<1>{\DrawBox[ultra thick, mycolor]{top left 1}{bottom right 1}}



==> Submission/ReStud/Tables/FStats_supply_all_slides.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{.25pt}}lcccc}
\toprule
% \textbf{Panel A: BLP IVs}& 2& 3& 4& 5 \\
% 1.Zero wholesale margin&3962.3, 739.9&6309, 1042&6173.3, 1043.5&3064.5, 1622.4\\
% 2.Zero retail margin&&3038.3, 969.4&3070.9, 968.4&3302.8, 1346.3\\
% 3.Linear pricing&&&202, 1305.5&3188.3, 1776.6\\
% 4.Hybrid model&&&&3169.2, 1779.7\\
% 5.Wholesale collusion&&&&\\
% \toprule
% \textbf{Panel B: Differentiation IVs} 
% & 2& 3& 4& 5 \\
% 1.Zero wholesale margin&1.8, 6.7&12, 5.9&11.8, 5.9&1.8, 5.1\\
% 2.Zero retail margin&&3.2, 5.7&3.1, 5.7&1.8, 5.4\\
% 3.Linear pricing&&&1.5, 5&2, 4.5\\
% 4.Hybrid model&&&&2, 4.5\\
% 5.Wholesale collusion&&&&\\
% \toprule
\textbf{Panel A: BLP95 IVs} 
& 2& 3& 4& 5 \\
1.Zero wholesale margin&\only<2>{\cellcolor{yellow}}12506, 1710&26318, 3326&25683, 3329&8299, 5661\\
2.Zero retail margin&&7859, 2806&7963, 2800&9079, 4682\\
3.Simple linear pricing&&&660, 4569&9059, 6329\\
4.Hybrid model&&&&8985, 6339\\
5.Wholesale collusion&&&&\\
\toprule
\textbf{Panel B: GH20 IVs} 
& 2& 3& 4& 5 \\
1.Zero wholesale margin&2.6, 9.8&15.3, 8.8&15.1, 8.9&2.1, 7.8\\
2.Zero retail margin&&3.6, 8.4&3.5, 8.4&2.3, 8.2\\
3.Simple linear pricing&&&2, 7.4&2.8, 6.7\\
4.Hybrid model&&&&2.8, 6.7\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Submission/ReStud/Tables/F_critical_values.tex <==

%\newcolumntype{d}[1]{D{.}{.}{#1}}
%\renewcommand{\arraystretch}{1.05}
\begin{widetable}{.98\columnwidth}{r*{3}{>{\raggedleft\arraybackslash}p{3em}}c*{3}{>{\raggedleft\arraybackslash}p{3em}}}
\toprule
&  \multicolumn{3}{c}{\textbf{Panel A:} Maximal Size ${cv^s},\,\, r^s = $} &&  \multicolumn{3}{c}{\textbf{Panel B:} Maximal Power ${cv^p},\,\, r^p = $}\\ 
\cmidrule(lr){2-4}\cmidrule(lr){6-8} 
$d_z$  & 0.075 & 0.10 & 0.125 & & 0.95 & 0.75 & 0.50\\
\midrule
1&31.4&14.5&8.4&&31.1&22.6&18.0\\
2&0&0&0&&18.9&13.2&10.4\\
3&0&0&0&&14.6&10.2&8.0\\
4&0&0&0&&12.3&8.8&6.9\\
5&0&0&0&&10.8&7.8&6.2\\
6&0&0&0&&9.8&7.2&5.8\\
7&0&0&0&&9.0&6.7&5.4\\
8&0&0&0&&8.4&6.4&5.2\\
9&0.3&0&0&&8.0&6.1&5.0\\
10&1.7&0.4&0&&7.6&5.8&4.8\\
11&3.3&1.3&0.5&&7.2&5.6&4.6\\
12&5.0&2.1&1.1&&7.0&5.4&4.5\\
13&6.9&3.1&1.8&&6.7&5.3&4.4\\
14&8.8&4.0&2.4&&6.5&5.1&4.3\\
15&10.8&5.0&3.1&&6.3&5.0&4.2\\
20&21.1&10.2&6.6&&5.6&4.6&3.9\\
25&31.8&15.7&10.3&&5.1&4.2&3.7\\
30&42.8&21.2&14.1&&4.8&4.0&3.5\\
\bottomrule
\end{widetable}

==> Submission/ReStud/Tables/Fblp1stat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&3962.3, 739.9&6309, 1042&6173.3, 1043.5&3064.5, 1622.4\\
2.Zero retail margin&&3038.3, 969.4&3070.9, 968.4&3302.8, 1346.3\\
3.Simple linear pricing&&&202, 1305.5&3188.3, 1776.6\\
4.Hybrid model&&&&3169.2, 1779.7\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Submission/ReStud/Tables/Fdiff2stat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&3.8, 3.8&14.2, 3.3&13.4, 3.3&1.1, 2.5\\
2.Zero retail margin&&2, 4.1&2, 4&1.3, 3.1\\
3.Simple linear pricing&&&2.9, 3.5&1.3, 2.5\\
4.Hybrid model&&&&1.3, 2.5\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Submission/ReStud/Tables/Instr_robustness.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{widetable}{.98\columnwidth}{lrrrrc}
\toprule
\textbf{Panel A: BLP95 + GH20 + Rival Cost} & \multicolumn{4}{c}{$F_\rho$}& MCS $p$-values\\
\multicolumn{1}{l}{($d_z=8$)}&\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&65.7&21.5&21.5&91.7&0.71 \\
2. Zero retail margin&&30.1&30.2&80.1&1.00 \\
3. Linear pricing&&&36.3&33.1&0.09 \\
4. Hybrid model&&&&33.0&0.09 \\
5. Wholesale collusion&&&&&0.00 \\
\midrule
\textbf{Panel B: Difference in Cost Shifters IVs} & \multicolumn{4}{c}{$F_\rho$}& MCS $p$-values\\
\multicolumn{1}{l}{($d_z=1$)}&\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&12.1&3.8&3.8&4.8&0.72\\
2. Zero retail margin&&7.1&7.0&8.1&0.19\\
3. Linear pricing&&&1.8&2.8&0.72\\
4. Hybrid model&&&&2.8&0.70\\
5. Wholesale collusion&&&&&1.00\\
\midrule
\textbf{Panel C: BLP Constant IVs} & \multicolumn{4}{c}{$F_\rho$}& MCS $p$-values\\
\multicolumn{1}{l}{($d_z=2$)}&\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&63.6&28.0&28.0&91.3&0.61\\
2. Zero retail margin&&37.8&37.9&78.5&1.00\\
3. Linear pricing&&&50.1&29.3&0.02\\
4. Hybrid model&&&&29.1&0.02\\
5. Wholesale collusion&&&&&0.00\\
\bottomrule
\end{widetable}


==> Submission/ReStud/Tables/MarkupDescTable.tex <==
\begin{tabular}{lrr}
\hline
       &           IV1 &        Mixed 2 \\
\hline
 count & 205123        & 205123         \\
 mean  &      0.250668 &      0.222563  \\
 std   &      0.084924 &      0.0509135 \\
 min   &      0.057056 &      0.0939126 \\
 25\%   &      0.184493 &      0.184744  \\
 50\%   &      0.247817 &      0.217921  \\
 75\%   &      0.308962 &      0.255025  \\
 max   &      0.87463  &      0.621748  \\
\hline
\end{tabular}


==> Submission/ReStud/Tables/MixedFstat.tex <==
\begin{tabular}{llr}
\hline
                & Mixed 1   &   Mixed 2 \\
\hline
 prices         & 1295.4    &     656.3 \\
                & 175.3     &     249.6 \\
 income x price & 1849.8    &    1031.6 \\
                & 250.4     &     371.6 \\
 income x light &           &    6749   \\
                &           &   15784.5 \\
 age x light    &           &     967.6 \\
                &           &    2355.2 \\
 age x size     &           &     849.2 \\
                &           &    1303.1 \\
\hline
\end{tabular}


==> Submission/ReStud/Tables/MkupTable.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccccc}
\toprule
& Median& S.D.& Min& q10& q90& Max \\
\cline{2-7}Zero wholesale margin&37.6&10.7&13.6&27.4&53.3&169.9\\
Zero retail margin&19.7&4.3&8.3&14.7&25.7&53.9\\
Simple linear pricing&54.3&13.8&14.1&41.2&74.7&208.0\\
Hybrid model&52.7&13.0&14.1&40.1&71.9&178.2\\
Wholesale collusion&84.4&34.1&20.3&56.2&134.8&674.0\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Submission/ReStud/Tables/Model_assessment_all.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}ccccccc}
\toprule
&\multicolumn{3}{c}{Full sample}&\multicolumn{3}{c}{20\% sample}\\
\cline{2-4}\cline{5-7}
Model $j$ & EB &AR &Cox & EB &AR &Cox  \\
2& 113.63, 395.48&	258.84, 654.31&	-1.97, -1.24&	2.15, 5.31&	14.54, 21.49&	-0.67, -0.61\\
3& 357.24, 591.48&	258.84, 221&	1.4, -8.4&	10.52, 22.04&	14.54, 9.57&	0.86, -8.16\\
4& 369.55, 622.69&	258.84, 224.86&	1.45, -8.09&	11.22, 23.79&	14.54, 9.76&	0.88, -7.62\\
5& 6.2, 13.05&	258.84, 218.66&	3.39, -6.26&	0.05, 0.16&	14.54, 32.68&	1.29, -2.54\\
\bottomrule\end{tabular}
\end{footnotesize}


==> Submission/ReStud/Tables/PCM.tex <==
\begin{widetable}{.98\columnwidth}{lcccccc}
\toprule
& Mean& Median& S.D.& Min& Max & $\% >100$\\
\midrule
Zero wholesale margin&39.4&37.6&10.7&13.6&169.9&0.04\\
Zero retail margin&20.0&19.7&4.3&8.3&53.9&0\\
Linear pricing&56.6&54.3&13.8&14.1&208.0&0.86\\
Hybrid model&54.8&52.7&13.0&14.1&178.2&0.50\\
Wholesale collusion&91.3&84.4&34.1&20.3&674.0&31.69\\
\bottomrule
\end{widetable}



==> Submission/ReStud/Tables/RSS_IJIVE.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lccccc}
\toprule
\textbf{Panel A: RSS} \\
& 2& 3& 4& 5& MCS p-values \\
1.Zero wholesale margin&-0.57&1.19&1.19&-5.37&\\
2.Zero retail margin&&1.02&0.97&-4.39&\\
3.Simple linear pricing&&&-7.04&-3.08&\\
4.Hybrid model&&&&-3.08&\\
5.Wholesale collusion&&&&&\\
\toprule
\textbf{Panel B: RV-IJIVE with BLP instruments} \\
& 2& 3& 4& 5& MCS p-values \\
1.Zero wholesale margin&0.65&-3.45&-3.45&-5.36&0.51\\
2.Zero retail margin&&-3.18&-3.16&-4.24&1\\
3.Simple linear pricing&&&0.17&-4.47&0.04\\
4.Hybrid model&&&&-4.47&0.04\\
5.Wholesale collusion&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Submission/ReStud/Tables/RSSstat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&-0.57&1.19&1.19&-5.37\\
2.Zero retail margin&&1.02&0.97&-4.39\\
3.Simple linear pricing&&&-7.04&-3.08\\
4.Hybrid model&&&&-3.08\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Submission/ReStud/Tables/RV_Accumul.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{widetable}{.98\columnwidth}{lrrrrrrc}
\toprule
\textbf{Panel A: BLP95 IVs} $(d_z = 2)$ & \multicolumn{3}{c}{$T^{RV}$}& \multicolumn{3}{c}{$F$-statistics}&  MCS $p$-values\\ \cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-8}  
Models & 2 & 3 &  4 & 2 & 3 & 4 & \\ 
\cmidrule(lr){2-8}
1. Zero wholesale margin& 2.25&$-$12.56& $-$12.35&149.5&86.1&85.1&0.03\\
2. Zero retail margin&&$-$7.17&$-$7.14&&133.6&132.7&{1.00}\\
3. Linear pricing&&&0.12&&&101.9&0.00\\
4. Hybrid model&&&&&&&0.00\\
\midrule
\textbf{Panel B: DEMO IVs} $(d_z = 3)$ & \multicolumn{3}{c}{$T^{RV}$}& \multicolumn{3}{c}{$F$-statistics }&  MCS $p$-values\\ \cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-8}  
Models & 2 & 3 &  4 & 2 & 3 & 4 & \\ 
\cmidrule(lr){2-8}
1. Zero wholesale margin& 2.23&$-$6.81& $-$6.85&24.1&46.6&47.2&0.03\\
2. Zero retail margin&&$-$5.45&$-$5.51&&35.4&36.0&{1.00}\\
3. Linear pricing&&&0.35&&&41.1&0.00\\
4. Hybrid model&&&&&&&0.00\\
\midrule
\textbf{Panel C: COST IVs} $(d_z = 1)$ & \multicolumn{3}{c}{$T^{RV}$}& \multicolumn{3}{c}{$F$-statistics}&  MCS $p$-values\\ \cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-8}  
Models & 2 & 3 &  4 & 2 & 3 & 4 & \\ 
\cmidrule(lr){2-8}
1. Zero wholesale margin& $-$1.86&$-$0.94& $-$1.16&70.6&4.8$^\dagger$&5.2$^\dagger$&{1.00}\\
2. Zero retail margin&&1.78&1.73&&43.4&43.8&{0.13}\\
3. Linear pricing&&&$-$2.82&&&53.7&{0.35}\\
4. Hybrid model&&&&&&&0.01\\
\midrule
\textbf{Panel D: DIFF IVs} $(d_z = 5)$ & \multicolumn{3}{c}{$T^{RV}$}& \multicolumn{3}{c}{$F$-statistics}&  MCS $p$-values\\ \cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-8}  
Models & 2 & 3 &  4 & 2 & 3 & 4 & \\ 
\cmidrule(lr){2-8}
1. Zero wholesale margin& 0.81&0.34&0.33&6.1$^\dagger$&2.2$^\dagger$&2.2$^\dagger$&{0.67}\\
2. Zero retail margin&&0.24&0.23&&2.0$^\dagger$&2.0$^\dagger$&{0.81}\\
3. Linear pricing&&&$-$1.21&&&1.2$^\dagger$&{1.00}\\
4. Hybrid model&&&&&&&{0.54}\\
\midrule
\textbf{Aggregating Evidence:} &\multicolumn{7}{c}{ $\boldsymbol{M^* = \{2\}}$}\\
\multicolumn{8}{c}{Step 0: $M^*_A = \{2\}$,  $M^*_B = \{2\}$, $M^*_C = \{1,2,3\}$, $ M^*_D = \{1,2,3,4\}$ \hfill Step 1: No conflicting evidence}\\
\multicolumn{8}{l}{Step 2:  Smallest MCS is $M^*_A= \{2\}$, no additional models supported by strong instruments}\\
%&\multicolumn{7}{c}{No Conflicting Evidence$\qquad$ $M^* = \{2\}$}\\
%Conflicting Evidence: \multicolumn{7}{c}{No}\\
%$M^*$: \multicolumn{7}{c}{$\{2\}$}\\
\bottomrule
\end{widetable}


==> Submission/ReStud/Tables/RV_Accumul1.tex <==
\begin{widetable}{.98\columnwidth}{lrrrrrrc}
\toprule
& \multicolumn{3}{c}{$T^\text{RV}$}& \multicolumn{3}{c}{$F$-statistics}&  MCS $p$-values\\
\cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-8}  
Models & 2 & 3 &  4 & 2 & 3 & 4 & \\ 
\midrule
\textbf{Panel A: BLP95 IVs} $(d_z = 2)$ \\ 
1. Zero wholesale margin& 2.25&$-$12.56& $-$12.35&149.5&86.1&85.1&0.03\\
2. Zero retail margin&&$-$7.17&$-$7.14&&133.6&132.7&{1.00}\\
3. Linear pricing&&&0.12&&&101.9&0.00\\
4. Hybrid model&&&&&&&0.00\\
\cmidrule(lr){1-8}
\textbf{Panel B: Demo IVs} $(d_z = 3)$ \\
1. Zero wholesale margin& 2.23&$-$6.81& $-$6.85&24.1&46.6&47.2&0.03\\
2. Zero retail margin&&$-$5.45&$-$5.51&&35.4&36.0&{1.00}\\
3. Linear pricing&&&0.35&&&41.1&0.00\\
4. Hybrid model&&&&&&&0.00\\
\cmidrule(lr){1-8}
\textbf{Panel C: Cost IVs} $(d_z = 1)$\\
1. Zero wholesale margin& $-$1.86&$-$0.94& $-$1.16&70.6&4.8$^\dagger$&5.2$^\dagger$&{1.00}\\
2. Zero retail margin&&1.78&1.73&&43.4&43.8&{0.13}\\
3. Linear pricing&&&$-$2.82&&&53.7&{0.35}\\
4. Hybrid model&&&&&&&0.01\\
\cmidrule(lr){1-8}
\textbf{Panel D: Diff IVs} $(d_z = 5)$ \\
1. Zero wholesale margin& 0.81&0.34&0.33&6.1$^\dagger$&2.2$^\dagger$&2.2$^\dagger$&{0.67}\\
2. Zero retail margin&&0.24&0.23&&2.0$^\dagger$&2.0$^\dagger$&{0.81}\\
3. Linear pricing&&&$-$1.21&&&1.2$^\dagger$&{1.00}\\
4. Hybrid model&&&&&&&{0.54}\\
\midrule
\midrule
\textbf{Aggregating Evidence:} &\multicolumn{7}{c}{ $\boldsymbol{M^* = \{2\}}$}\\
\multicolumn{8}{c}{Step 0: $M^*_A = \{2\}$,  $M^*_B = \{2\}$, $M^*_C = \{1,2,3\}$, $ M^*_D = \{1,2,3,4\}$ \hfill Step 1: No conflicting evidence}\\
\multicolumn{8}{l}{Step 2:  Smallest MCS is $M^*_A= \{2\}$, no additional models supported by strong instruments}\\
%&\multicolumn{7}{c}{No Conflicting Evidence$\qquad$ $M^* = \{2\}$}\\
%Conflicting Evidence: \multicolumn{7}{c}{No}\\
%$M^*$: \multicolumn{7}{c}{$\{2\}$}\\
\bottomrule
\end{widetable}


==> Submission/ReStud/Tables/RV_application_full.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{widetable}{.98\columnwidth}{lrrrrc}
\toprule
\textbf{Panel A: BLP95 IVs} & \multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& MCS $p$-values \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&0.65&$-$3.45&$-$3.45&$-$5.37&0.52\\
2. Zero retail margin&&$-$3.18&$-$3.17&$-$4.25&1.00\\
3. Linear pricing&&&0.17&$-$4.47&0.04\\
4. Hybrid model&&&&$-$4.48&0.04\\
5. Wholesale collusion&&&&&0.00\\
\midrule
\textbf{Panel B: GH20 IVs} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& MCS $p$-values \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&0.77&0.40&0.39&$-$1.05&0.74 \\
2. Zero retail margin&&0.29&0.28&$-$1.02&0.78 \\
3. Linear pricing&&&$-$1.18&$-$0.81&1.00 \\
4. Hybrid model&&&&$-$0.80&0.78 \\
5. Wholesale collusion&&&&&0.55 \\
\midrule
\textbf{Panel C: Rival Cost Shifters IVs} & \multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}&MCS $p$-values \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&-0.76&-0.33&-0.46&-4.06&1.00\\
2. Zero retail margin&&0.82&0.80&-3.01&0.45\\
3. Linear pricing&&&-1.33&-3.94&0.75\\
4. Hybrid model&&&&-3.95&0.67\\
5. Wholesale collusion&&&&&0.00\\
\bottomrule
\end{widetable}


==> Submission/ReStud/Tables/RV_application_full_slides.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{2pt}}lccccc}
\toprule
\textbf{Panel A: BLP95 IVs} 
& 2& 3& 4& 5& MCS p-values \\
1.Zero wholesale margin& \only<2>{\cellcolor{yellow}}0.65&-3.45&-3.45&\only<4>{\cellcolor{yellow}}-5.37&\only<5-6>{\cellcolor{green}}0.52\\
2.Zero retail margin&&-3.18&-3.17&\only<4>{\cellcolor{yellow}}-4.25&\only<5-6>{\cellcolor{green}}1.00\\
3.Linear pricing&&&0.17&\only<4>{\cellcolor{yellow}}-4.47&\only<5-6>{\cellcolor{red}}0.04\\
4.Hybrid model&&&&\only<4>{\cellcolor{yellow}}-4.48&\only<5-6>{\cellcolor{red}}0.04\\
5.Wholesale collusion&&&&&\only<5-6>{\cellcolor{red}}0.00\\
\toprule
\textbf{Panel B: GH20 IVs}
& 2& 3& 4& 5& MCS p-values \\
1.Zero wholesale margin&\only<3>{\cellcolor{yellow}}0.77&\only<3>{\cellcolor{yellow}}0.40&\only<3>{\cellcolor{yellow}}0.39&\only<3-4>{\cellcolor{yellow}}-1.05&\only<6>{\cellcolor{green}}0.74\\
2.Zero retail margin&&\only<3>{\cellcolor{yellow}}0.29&\only<3>{\cellcolor{yellow}}0.28&\only<3-4>{\cellcolor{yellow}}-1.02&\only<6>{\cellcolor{green}}0.78\\
3.Linear pricing&&&\only<3>{\cellcolor{yellow}}-1.18&\only<3-4>{\cellcolor{yellow}}-0.81&\only<6>{\cellcolor{green}}1.00\\
4.Hybrid model&&&&\only<3-4>{\cellcolor{yellow}}-0.80&\only<6>{\cellcolor{green}}0.78\\
5.Wholesale collusion&&&&&\only<6>{\cellcolor{green}}0.55\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Submission/ReStud/Tables/RV_application_full_talk.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{widetable}{.98\columnwidth}{lrrrrc}
\toprule
\tikzmark{tl1}\textbf{Panel A: BLP95 IVs}\tikzmark{br1} & \multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& MCS p-values \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&\tikzmark{tl3}0.65&$-$3.45&$-$3.45&$-$5.37&\tikzmark{top left 1}0.52\\
2. Zero retail margin&&$-$3.18&$-$3.17&$-$4.25&1.00\tikzmark{bottom right 1}\\
3. Linear pricing&&&0.17&$-$4.47&\tikzmark{top left 2}0.04\\
4. Hybrid model&&&&$-$4.48\tikzmark{br3}&0.04\\
5. Wholesale collusion&&&&&0.00\tikzmark{bottom right 2}\\
\midrule
\tikzmark{tl2}\textbf{Panel B: GH20 IVs} \tikzmark{br2} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& MCS p-values \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&\tikzmark{tl4}0.77&0.40&0.39&$-$1.05&\tikzmark{top left 3}0.74 \\
2. Zero retail margin&&0.29&0.28&$-$1.02&0.78 \\
3. Linear pricing&&&$-$1.18&$-$0.81&1.00 \\
4. Hybrid model&&&&$-$0.80\tikzmark{br4}&0.78 \\
5. Wholesale collusion&&&&&0.55\tikzmark{bottom right 3} \\
\bottomrule
\end{widetable}

\only<1>{\DrawBox[ultra thick, mycolor]{tl1}{br1}}
\only<1>{\DrawBox[ultra thick, mycolor]{tl2}{br2}}
\only<2>{\DrawBox[ultra thick, mycolor]{tl3}{br3}}
\only<3>{\DrawBox[ultra thick, mycolor]{tl4}{br4}}
\only<4>{\DrawBox[ultra thick, red]{top left 2}{bottom right 2}}
\only<4>{\DrawBox[ultra thick, mycolor]{top left 1}{bottom right 1}}
\only<4>{\DrawBox[ultra thick, mycolor]{top left 3}{bottom right 3}}

==> Submission/ReStud/Tables/RV_application_full_talk_new.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{widetable}{.98\columnwidth}{lrrrrc}
\toprule
\tikzmark{tl1}\textbf{Panel A: BLP95 IVs}\tikzmark{br1} & \multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& MCS p-values \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&\tikzmark{tl6}\tikzmark{tl3}2.16\tikzmark{br6}&$-$5.88&$-$5.86&$-$23.85&\tikzmark{top left 8}0.03\tikzmark{bottom right 8}\\
2. Zero retail margin&&$-$23.63&$-$23.63&$-$31.83&\tikzmark{top left 1}1.00\tikzmark{bottom right 1}\\
3. Linear pricing&&&0.38&$-$29.87&\tikzmark{top left 2}0.00\\
4. Hybrid model&&&&$-$29.93\tikzmark{br3}&0.00\\
5. Wholesale collusion&&&&&0.00\tikzmark{bottom right 2}\\
\midrule
\tikzmark{tl2}\textbf{Panel B: GH20 IVs} \tikzmark{br2} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& MCS p-values \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&\tikzmark{tl4}0.84&0.64&0.63&$-$1.09&\tikzmark{top left 3}0.59 \\
2. Zero retail margin&&0.43&0.42&$-$1.07&0.66 \\
3. Linear pricing&&&$-$1.21&$-$1.26&1.00 \\
4. Hybrid model&&&&$-$1.25\tikzmark{br4}&0.66 \\
5. Wholesale collusion&&&&&0.35\tikzmark{bottom right 3} \\
\midrule
\tikzmark{tl5}\textbf{Panel C: Rival cost IVs} \tikzmark{br5} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& MCS p-values \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&-2.13&0.57&$-$0.76&$-$24.19&\tikzmark{top left 4}1.00\tikzmark{bottom right 4} \\
2. Zero retail margin&&2.55&2.48&$-$18.20&\tikzmark{top left 6}0.04\tikzmark{bottom right 6} \\
3. Linear pricing&&&$-$6.78&$-$24.04&\tikzmark{top left 7}0.58 \\
4. Hybrid model&&&&$-$24.08&0.45\tikzmark{bottom right 7} \\
5. Wholesale collusion&&&&& \tikzmark{top left 5}0.00\tikzmark{bottom right 5} \\
\bottomrule
\end{widetable}

\only<1>{\DrawBox[ultra thick, mycolor]{tl1}{br1}}
\only<1>{\DrawBox[ultra thick, mycolor]{tl2}{br2}}
\only<1>{\DrawBox[ultra thick, mycolor]{tl5}{br5}}
\only<2>{\DrawBox[ultra thick, mycolor]{tl6}{br6}}


\only<3>{\DrawBox[ultra thick, mycolor]{tl3}{br3}}
\only<4>{\DrawBox[ultra thick, mycolor]{tl4}{br4}}
\only<5>{\DrawBox[ultra thick, red]{top left 2}{bottom right 2}}
\only<5>{\DrawBox[ultra thick, red]{top left 5}{bottom right 5}}
\only<5>{\DrawBox[ultra thick, red]{top left 6}{bottom right 6}}
\only<5>{\DrawBox[ultra thick, red]{top left 8}{bottom right 8}}
\only<5>{\DrawBox[ultra thick, mycolor]{top left 1}{bottom right 1}}
\only<5>{\DrawBox[ultra thick, mycolor]{top left 3}{bottom right 3}}
\only<5>{\DrawBox[ultra thick, mycolor]{top left 4}{bottom right 4}}
\only<5>{\DrawBox[ultra thick, mycolor]{top left 7}{bottom right 7}}


==> Submission/ReStud/Tables/RV_stat_application.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lccccc}
\toprule
\textbf{Panel A: BLP instruments} \\
& 2& 3& 4& 5& MCS p-values \\
1.Zero wholesale margin&-0.25&-3.29&-3.33&-4.80& 1\\
2.Zero retail margin&&-1.22&-1.22&-3.66&0.81\\
3.Simple linear pricing&&&-1.07&-4.19&0.26\\
4.Hybrid model&&&&-4.19&0.26\\
5.Wholesale collusion&&&&&0.00\\
\toprule
\textbf{Panel B: differentiation instruments} \\
& 2& 3& 4& 5& MCS p-values \\
1.Zero wholesale margin&-1.70&0.10&0.10&-1.38&0.92\\
2.Zero retail margin&&0.56&0.57&-0.39&0.66\\
3.Simple linear pricing&&&0.33&-0.66&0.74\\
4.Hybrid model&&&&-0.67&1\\
5.Wholesale collusion&&&&&0.64\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Submission/ReStud/Tables/RV_tab_1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
\textbf{Panel A: No Instruments - RSS}\\
& 2& 3& 4& 5 \\
1.Zero wholesale margin&-0.57&1.19&1.19&-5.37\\
2.Zero retail margin&&1.02&0.97&-4.39\\
3.Simple linear pricing&&&-7.04&-3.08\\
4.Hybrid model&&&&-3.08\\
5.Wholesale collusion&&&&\\
\toprule
\textbf{Panel B: BLP Instruments}\\
& 2& 3& 4& 5 \\
1.Zero wholesale margin&-0.25&-3.29&-3.33&-4.80\\
2.Zero retail margin&&-1.22&-1.22&-3.66\\
3.Simple linear pricing&&&-1.07&-4.19\\
4.Hybrid model&&&&-4.19\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Submission/ReStud/Tables/RVstat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&-0.25&-3.29&-3.33&-4.80\\
2.Zero retail margin&&-1.22&-1.22&-3.66\\
3.Simple linear pricing&&&-1.07&-4.19\\
4.Hybrid model&&&&-4.19\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Submission/ReStud/Tables/demand_models.tex <==
\begin{widetable}{.98\columnwidth}{lrrrrrr}
\toprule
& \multicolumn{2}{c}{(1) Logit-OLS}  & \multicolumn{2}{c}{(2) Logit-2SLS}  & \multicolumn{2}{c}{(3) BLP}   \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
& coef. & \multicolumn{1}{c}{s.e.}
& coef. & \multicolumn{1}{c}{s.e.}
& coef. & \multicolumn{1}{c}{s.e.}    \\
\midrule
 Prices         &    $-1.750$ &   (0.019)    &    $-6.519$  &   (0.209)    &  $-12.001$  & (0.777)\\
 Size           &    0.037 &    (0.001)   &    0.018 &   (0.001)    &  $-0.060$  & (0.013) \\
 Light          &    0.259  &   (0.010)  &    0.413 &   (0.014)    &  $-0.270$  & (0.144) \\
 Plain   &    0.508 &   (0.007)   &    0.423  &   (0.009)   &  0.439 & (0.012) \\
 log(\#Flavors)   &    1.127  &   (0.004)  &    1.106 &   (0.005)    &  1.135    & (0.007) \\
 Income $\times$ price &      &       &        &      &  4.333   & (0.378)\\
 Income $\times$ light &     &        &        &      &  0.215  & (0.069)\\
Age $\times$ light    &      &       &      &        & $-0.565$  & (0.113)  \\
 Age $\times$ size     &    &         &   &           & $-0.067$& (0.008)  \\
\midrule 
Own elasticity-mean     &    \multicolumn{2}{c}{$-1.320$}    &    \multicolumn{2}{c}{$-4.917$}    & \multicolumn{2}{c}{$-6.306$}  \\
Own elasticity-median   &   \multicolumn{2}{c}{$-1.177$}    &    \multicolumn{2}{c}{$-4.384$ }   & \multicolumn{2}{c}{$-6.187$}  \\
 $J$-statistic         &   \multicolumn{2}{c}{2.0e-23}  &    \multicolumn{2}{c}{1.9e-21}    & \multicolumn{2}{c}{2.5e-01} \\
\bottomrule
\end{widetable}


==> Submission/ReStud/Tables/summary_stat.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Mar 12, 2021 - 03:58:35 PM
\begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Max} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Pctl(75)} \\ 
\hline \\[-1.8ex] 
price & 0.759 & 0.295 & 0.676 & 2.690 & 0.186 & 0.549 & 0.911 \\ 
sales & 1,461.252 & 3,199.272 & 503.000 & 104,492.000 & 2.000 & 213.333 & 1,301.000 \\ 
shares & 0.007 & 0.012 & 0.003 & 0.280 & 0.00001 & 0.001 & 0.007 \\ 
outside share & 0.710 & 0.111 & 0.708 & 0.995 & 0.318 & 0.631 & 0.788 \\ 
size & 17.815 & 10.574 & 16 & 32 & 6 & 6 & 32 \\ 
light & 0.925 & 0.263 & 1 & 1 & 0 & 1 & 1 \\ 
number flavors & 5.388 & 5.811 & 3 & 35 & 1 & 1 & 8 \\ 
private label & 0.088 & 0.283 & 0 & 1 & 0 & 0 & 0 \\ 
price reduction & 0.309 & 0.277 & 0.3 & 1 & 0 & 0 & 0.5 \\ 
distance to plant & 493.066 & 476.568 & 392.471 & 2,670.635 & 25.702 & 198.643 & 546.187 \\ 
freight cost & 211.932 & 242.070 & 164.3 & 1,466 & 0 & 51.9 & 270.8 \\ 
\hline \\[-1.8ex] 
\end{tabular} 


==> Submission/ReStud/Tables/summary_stat_count.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Mar 12, 2021 - 03:58:36 PM
\begin{tabular}{@{\extracolsep{5pt}} ccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & N & mean & sd & median & max & min \\ 
\hline \\[-1.8ex] 
Obs & $205,123$ & $$ & $$ & $$ & $$ & $$ \\ 
Stores & $1,309$ & $$ & $$ & $$ & $$ & $$ \\ 
Chains & $93$ & $$ & $$ & $$ & $$ & $$ \\ 
Cities & $48$ & $$ & $$ & $$ & $$ & $$ \\ 
Markets & $5,034$ & $$ & $$ & $$ & $$ & $$ \\ 
Firms & $105$ & $$ & $$ & $$ & $$ & $$ \\ 
Brands (per firm) & $171$ & $2$ & $3$ & $1$ & $20$ & $1$ \\ 
Products (per firm) & $530$ & $5$ & $5$ & $4$ & $52$ & $1$ \\ 
PUMs (per market) & $446,969$ & $9,312$ & $7,695$ & $7,224$ & $42,258$ & $1,747$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 


==> Tables/AR_results_slides.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}l r @{\hspace{0.1\tabcolsep}} r r @{\hspace{0.1\tabcolsep}} r}
\toprule
Model $j$ & \multicolumn{2}{c}{Full Sample}  & \multicolumn{2}{c}{20\% Sample}  \\\midrule
2.Zero retail margin & 	\only<2,5>{\cellcolor{yellow}}258.84,& \only<2,5>{\cellcolor{yellow}}654.31&	14.54,& 21.49\\
3.Linear pricing& 	\only<4-5>{\cellcolor{yellow}}258.84,& \only<4-5>{\cellcolor{yellow}}221.00&	\only<3-4>{\cellcolor{yellow}}14.54,& \only<3-4>{\cellcolor{yellow}}9.57\\
4.Hybrid model& 	\only<5>{\cellcolor{yellow}}258.84,& \only<5>{\cellcolor{yellow}}224.86&	14.54,& 9.76\\
5.Wholesale collusion& 	\only<5>{\cellcolor{yellow}}258.84,& \only<5>{\cellcolor{yellow}}218.66&	14.54,& 32.68\\
\bottomrule\end{tabular}
\end{footnotesize}



==> Tables/Accum_Evidence_slides.tex <==
\begin{widetable}{.98\columnwidth}{lrrrr}
\toprule
Models & BLP95 & Demo & Cost & Diff \\ 
\midrule
\textbf{Panel A: MCS $p$-values} &&&&\\ 
1. Zero wholesale margin& 0.03& 0.03& 1.00& 0.67\\
2. Zero retail margin&{1.00}&1.00&0.13&0.81\\
3. Linear pricing&0.00&0.00&0.35&1.00\\
4. Hybrid model&0.00&0.00&0.01&0.54\\
\midrule
\textbf{Panel B: Aggregating Evidence} &&&&\\
Step 0 & $\{2\}$ & $\{2\}$ & $\{1,2,3\}$ & $\{1,2,3,4\}$ \\
\multicolumn{5}{l}{Step 1: No conflicting evidence} \\
\multicolumn{1}{l}{Step 2: Smallest MCS is $\{2\}$; Min $F$:}&85.1&24.1&4.8&1.2\\
$M^* = \{2\}$\\%, no other models supported by strong instruments}\\
\bottomrule
\end{widetable}


==> Tables/FStats_supply_all.tex <==
%\renewcommand{\arraystretch}{1.2}
\begin{widetable}{.98\columnwidth}{lrrrr}
\toprule
\textbf{Panel A: BLP95 IVs} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5} \\
\cmidrule(lr){2-5}
1. Zero wholesale margin&66.3&26.3&26.2&90.7\\
2. Zero retail margin&&36.4&36.6&79.0\\
3. Simple linear pricing&&&50.8&27.2\\
4. Hybrid model&&&&26.9\\
5. Wholesale collusion&&&&\\
\midrule
\textbf{Panel B: GH20 IVs} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5} \\
\cmidrule(lr){2-5}
1. Zero wholesale margin&5.7&2.5&2.5&3.7\\
2. Zero retail margin&&2.2&2.2&4.3\\
3. Simple linear pricing&&&1.0&2.5\\
4. Hybrid model&&&&2.5\\
5. Wholesale collusion&&&&\\
\midrule
\textbf{Panel C: Rival Cost Shifters IVs} &\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5} \\
\cmidrule(lr){2-5}
1. Zero wholesale margin&68.6&1.1&1.3&131.6\\
2. Zero retail margin&&44.8&47.0&112.9\\
3. Linear pricing&&&5.2&33.7\\
4. Hybrid model&&&&34.6\\
5. Wholesale collusion&&&&\\
\bottomrule
\end{widetable}


==> Tables/FStats_supply_all_new.tex <==
%\renewcommand{\arraystretch}{1.2}
\begin{widetable}{.98\columnwidth}{lrrr}
\toprule
\textbf{Panel A: BLP95 IVs} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4} \\
\cmidrule(lr){2-4}
1. Zero wholesale margin&\tikzmark{top left 1}149.5&86.1&85.1\\
2. Zero retail margin&&133.6&132.7\\
3. Simple linear pricing&&&101.9\\
4. Hybrid model&&&\tikzmark{bottom right 1}\\
\midrule
\textbf{Panel B: Diff IVs} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}\\
\cmidrule(lr){2-4}
1. Zero wholesale margin&\tikzmark{top left 2}6.1&2.2&2.2\\
2. Zero retail margin&&2.0&2.0\\
3. Simple linear pricing&&&1.2\\
4. Hybrid model&&&\tikzmark{bottom right 2}\\
\bottomrule
\end{widetable}

\only<1>{\DrawBox[ultra thick, red]{top left 2}{bottom right 2}}
\only<1>{\DrawBox[ultra thick, mycolor]{top left 1}{bottom right 1}}



==> Tables/FStats_supply_all_slides.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{.25pt}}lcccc}
\toprule
% \textbf{Panel A: BLP IVs}& 2& 3& 4& 5 \\
% 1.Zero wholesale margin&3962.3, 739.9&6309, 1042&6173.3, 1043.5&3064.5, 1622.4\\
% 2.Zero retail margin&&3038.3, 969.4&3070.9, 968.4&3302.8, 1346.3\\
% 3.Linear pricing&&&202, 1305.5&3188.3, 1776.6\\
% 4.Hybrid model&&&&3169.2, 1779.7\\
% 5.Wholesale collusion&&&&\\
% \toprule
% \textbf{Panel B: Differentiation IVs} 
% & 2& 3& 4& 5 \\
% 1.Zero wholesale margin&1.8, 6.7&12, 5.9&11.8, 5.9&1.8, 5.1\\
% 2.Zero retail margin&&3.2, 5.7&3.1, 5.7&1.8, 5.4\\
% 3.Linear pricing&&&1.5, 5&2, 4.5\\
% 4.Hybrid model&&&&2, 4.5\\
% 5.Wholesale collusion&&&&\\
% \toprule
\textbf{Panel A: BLP95 IVs} 
& 2& 3& 4& 5 \\
1.Zero wholesale margin&\only<2>{\cellcolor{yellow}}12506, 1710&26318, 3326&25683, 3329&8299, 5661\\
2.Zero retail margin&&7859, 2806&7963, 2800&9079, 4682\\
3.Simple linear pricing&&&660, 4569&9059, 6329\\
4.Hybrid model&&&&8985, 6339\\
5.Wholesale collusion&&&&\\
\toprule
\textbf{Panel B: GH20 IVs} 
& 2& 3& 4& 5 \\
1.Zero wholesale margin&2.6, 9.8&15.3, 8.8&15.1, 8.9&2.1, 7.8\\
2.Zero retail margin&&3.6, 8.4&3.5, 8.4&2.3, 8.2\\
3.Simple linear pricing&&&2, 7.4&2.8, 6.7\\
4.Hybrid model&&&&2.8, 6.7\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Tables/F_critical_values_worstcase.tex <==

%\newcolumntype{d}[1]{D{.}{.}{#1}}
%\renewcommand{\arraystretch}{1.05}
\begin{widetable}{.98\columnwidth}{r*{3}{>{\raggedleft\arraybackslash}p{3em}}c*{3}{>{\raggedleft\arraybackslash}p{3em}}}
\toprule
&  \multicolumn{3}{c}{\textbf{Panel A:} Maximal Size ${cv^s},\,\, r^s = $} &&  \multicolumn{3}{c}{\textbf{Panel B:} Maximal Power ${cv^p},\,\, r^p = $}\\ 
\cmidrule(lr){2-4}\cmidrule(lr){6-8} 
$d_z$  & 0.075 & 0.10 & 0.125 & & 0.95 & 0.75 & 0.50\\
\midrule
1&31.4&14.5&8.4&&31.1&22.6&18.0\\
2&0&0&0&&18.9&13.2&10.4\\
3&0&0&0&&14.6&10.2&8.0\\
4&0&0&0&&12.3&8.8&6.9\\
5&0&0&0&&10.8&7.8&6.2\\
6&0&0&0&&9.8&7.2&5.8\\
7&0&0&0&&9.0&6.7&5.4\\
8&0&0&0&&8.4&6.4&5.2\\
9&0.3&0&0&&8.0&6.1&5.0\\
10&1.7&0.4&0&&7.6&5.8&4.8\\
11&3.3&1.3&0.5&&7.2&5.6&4.6\\
12&5.0&2.1&1.1&&7.0&5.4&4.5\\
13&6.9&3.1&1.8&&6.7&5.3&4.4\\
14&8.8&4.0&2.4&&6.5&5.1&4.3\\
15&10.8&5.0&3.1&&6.3&5.0&4.2\\
20&21.1&10.2&6.6&&5.6&4.6&3.9\\
25&31.8&15.7&10.3&&5.1&4.2&3.7\\
30&42.8&21.2&14.1&&4.8&4.0&3.5\\
\bottomrule
\end{widetable}

==> Tables/Instr_robustness.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{widetable}{.98\columnwidth}{lrrrrc}
\toprule
\textbf{Panel A: BLP95 + GH20 + Rival Cost} & \multicolumn{4}{c}{$F_\rho$}& MCS $p$-values\\
\multicolumn{1}{l}{($d_z=8$)}&\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&65.7&21.5&21.5&91.7&0.71 \\
2. Zero retail margin&&30.1&30.2&80.1&1.00 \\
3. Linear pricing&&&36.3&33.1&0.09 \\
4. Hybrid model&&&&33.0&0.09 \\
5. Wholesale collusion&&&&&0.00 \\
\midrule
\textbf{Panel B: Difference in Cost Shifters IVs} & \multicolumn{4}{c}{$F_\rho$}& MCS $p$-values\\
\multicolumn{1}{l}{($d_z=1$)}&\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&12.1&3.8&3.8&4.8&0.72\\
2. Zero retail margin&&7.1&7.0&8.1&0.19\\
3. Linear pricing&&&1.8&2.8&0.72\\
4. Hybrid model&&&&2.8&0.70\\
5. Wholesale collusion&&&&&1.00\\
\midrule
\textbf{Panel C: BLP Constant IVs} & \multicolumn{4}{c}{$F_\rho$}& MCS $p$-values\\
\multicolumn{1}{l}{($d_z=2$)}&\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&63.6&28.0&28.0&91.3&0.61\\
2. Zero retail margin&&37.8&37.9&78.5&1.00\\
3. Linear pricing&&&50.1&29.3&0.02\\
4. Hybrid model&&&&29.1&0.02\\
5. Wholesale collusion&&&&&0.00\\
\bottomrule
\end{widetable}


==> Tables/RV_Accumul.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{widetable}{.98\columnwidth}{lrrrrrrc}
\toprule
\textbf{Panel A: BLP95 IVs} $(d_z = 2)$ & \multicolumn{3}{c}{$T^{RV}$}& \multicolumn{3}{c}{$F$-statistics}&  MCS $p$-values\\ \cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-8}  
Models & 2 & 3 &  4 & 2 & 3 & 4 & \\ 
\cmidrule(lr){2-8}
1. Zero wholesale margin& 2.25&$-$12.56& $-$12.35&149.5&86.1&85.1&0.03\\
2. Zero retail margin&&$-$7.17&$-$7.14&&133.6&132.7&{1.00}\\
3. Linear pricing&&&0.12&&&101.9&0.00\\
4. Hybrid model&&&&&&&0.00\\
\midrule
\textbf{Panel B: DEMO IVs} $(d_z = 3)$ & \multicolumn{3}{c}{$T^{RV}$}& \multicolumn{3}{c}{$F$-statistics }&  MCS $p$-values\\ \cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-8}  
Models & 2 & 3 &  4 & 2 & 3 & 4 & \\ 
\cmidrule(lr){2-8}
1. Zero wholesale margin& 2.23&$-$6.81& $-$6.85&24.1&46.6&47.2&0.03\\
2. Zero retail margin&&$-$5.45&$-$5.51&&35.4&36.0&{1.00}\\
3. Linear pricing&&&0.35&&&41.1&0.00\\
4. Hybrid model&&&&&&&0.00\\
\midrule
\textbf{Panel C: COST IVs} $(d_z = 1)$ & \multicolumn{3}{c}{$T^{RV}$}& \multicolumn{3}{c}{$F$-statistics}&  MCS $p$-values\\ \cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-8}  
Models & 2 & 3 &  4 & 2 & 3 & 4 & \\ 
\cmidrule(lr){2-8}
1. Zero wholesale margin& $-$1.86&$-$0.94& $-$1.16&70.6&4.8$^\dagger$&5.2$^\dagger$&{1.00}\\
2. Zero retail margin&&1.78&1.73&&43.4&43.8&{0.13}\\
3. Linear pricing&&&$-$2.82&&&53.7&{0.35}\\
4. Hybrid model&&&&&&&0.01\\
\midrule
\textbf{Panel D: DIFF IVs} $(d_z = 5)$ & \multicolumn{3}{c}{$T^{RV}$}& \multicolumn{3}{c}{$F$-statistics}&  MCS $p$-values\\ \cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-8}  
Models & 2 & 3 &  4 & 2 & 3 & 4 & \\ 
\cmidrule(lr){2-8}
1. Zero wholesale margin& 0.81&0.34&0.33&6.1$^\dagger$&2.2$^\dagger$&2.2$^\dagger$&{0.67}\\
2. Zero retail margin&&0.24&0.23&&2.0$^\dagger$&2.0$^\dagger$&{0.81}\\
3. Linear pricing&&&$-$1.21&&&1.2$^\dagger$&{1.00}\\
4. Hybrid model&&&&&&&{0.54}\\
\midrule
\textbf{Aggregating Evidence:} &\multicolumn{7}{c}{ $\boldsymbol{M^* = \{2\}}$}\\
\multicolumn{8}{c}{Step 0: $M^*_A = \{2\}$,  $M^*_B = \{2\}$, $M^*_C = \{1,2,3\}$, $ M^*_D = \{1,2,3,4\}$ \hfill Step 1: No conflicting evidence}\\
\multicolumn{8}{l}{Step 2:  Smallest MCS is $M^*_A= \{2\}$, no additional models supported by strong instruments}\\
%&\multicolumn{7}{c}{No Conflicting Evidence$\qquad$ $M^* = \{2\}$}\\
%Conflicting Evidence: \multicolumn{7}{c}{No}\\
%$M^*$: \multicolumn{7}{c}{$\{2\}$}\\
\bottomrule
\end{widetable}


==> Tables/RV_application_full.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{widetable}{.98\columnwidth}{lrrrrc}
\toprule
\textbf{Panel A: BLP95 IVs} & \multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& MCS $p$-values \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&0.65&$-$3.45&$-$3.45&$-$5.37&0.52\\
2. Zero retail margin&&$-$3.18&$-$3.17&$-$4.25&1.00\\
3. Linear pricing&&&0.17&$-$4.47&0.04\\
4. Hybrid model&&&&$-$4.48&0.04\\
5. Wholesale collusion&&&&&0.00\\
\midrule
\textbf{Panel B: GH20 IVs} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& MCS $p$-values \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&0.77&0.40&0.39&$-$1.05&0.74 \\
2. Zero retail margin&&0.29&0.28&$-$1.02&0.78 \\
3. Linear pricing&&&$-$1.18&$-$0.81&1.00 \\
4. Hybrid model&&&&$-$0.80&0.78 \\
5. Wholesale collusion&&&&&0.55 \\
\midrule
\textbf{Panel C: Rival Cost Shifters IVs} & \multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}&MCS $p$-values \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&-0.76&-0.33&-0.46&-4.06&1.00\\
2. Zero retail margin&&0.82&0.80&-3.01&0.45\\
3. Linear pricing&&&-1.33&-3.94&0.75\\
4. Hybrid model&&&&-3.95&0.67\\
5. Wholesale collusion&&&&&0.00\\
\bottomrule
\end{widetable}


==> Tables/RV_application_full_slides.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{2pt}}lccccc}
\toprule
\textbf{Panel A: BLP95 IVs} 
& 2& 3& 4& 5& MCS p-values \\
1.Zero wholesale margin& \only<2>{\cellcolor{yellow}}0.65&-3.45&-3.45&\only<4>{\cellcolor{yellow}}-5.37&\only<5-6>{\cellcolor{green}}0.52\\
2.Zero retail margin&&-3.18&-3.17&\only<4>{\cellcolor{yellow}}-4.25&\only<5-6>{\cellcolor{green}}1.00\\
3.Linear pricing&&&0.17&\only<4>{\cellcolor{yellow}}-4.47&\only<5-6>{\cellcolor{red}}0.04\\
4.Hybrid model&&&&\only<4>{\cellcolor{yellow}}-4.48&\only<5-6>{\cellcolor{red}}0.04\\
5.Wholesale collusion&&&&&\only<5-6>{\cellcolor{red}}0.00\\
\toprule
\textbf{Panel B: GH20 IVs}
& 2& 3& 4& 5& MCS p-values \\
1.Zero wholesale margin&\only<3>{\cellcolor{yellow}}0.77&\only<3>{\cellcolor{yellow}}0.40&\only<3>{\cellcolor{yellow}}0.39&\only<3-4>{\cellcolor{yellow}}-1.05&\only<6>{\cellcolor{green}}0.74\\
2.Zero retail margin&&\only<3>{\cellcolor{yellow}}0.29&\only<3>{\cellcolor{yellow}}0.28&\only<3-4>{\cellcolor{yellow}}-1.02&\only<6>{\cellcolor{green}}0.78\\
3.Linear pricing&&&\only<3>{\cellcolor{yellow}}-1.18&\only<3-4>{\cellcolor{yellow}}-0.81&\only<6>{\cellcolor{green}}1.00\\
4.Hybrid model&&&&\only<3-4>{\cellcolor{yellow}}-0.80&\only<6>{\cellcolor{green}}0.78\\
5.Wholesale collusion&&&&&\only<6>{\cellcolor{green}}0.55\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Tables/RV_application_full_talk.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{widetable}{.98\columnwidth}{lrrrrc}
\toprule
\tikzmark{tl1}\textbf{Panel A: BLP95 IVs}\tikzmark{br1} & \multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& MCS p-values \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&\tikzmark{tl3}0.65&$-$3.45&$-$3.45&$-$5.37&\tikzmark{top left 1}0.52\\
2. Zero retail margin&&$-$3.18&$-$3.17&$-$4.25&1.00\tikzmark{bottom right 1}\\
3. Linear pricing&&&0.17&$-$4.47&\tikzmark{top left 2}0.04\\
4. Hybrid model&&&&$-$4.48\tikzmark{br3}&0.04\\
5. Wholesale collusion&&&&&0.00\tikzmark{bottom right 2}\\
\midrule
\tikzmark{tl2}\textbf{Panel B: GH20 IVs} \tikzmark{br2} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& MCS p-values \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&\tikzmark{tl4}0.77&0.40&0.39&$-$1.05&\tikzmark{top left 3}0.74 \\
2. Zero retail margin&&0.29&0.28&$-$1.02&0.78 \\
3. Linear pricing&&&$-$1.18&$-$0.81&1.00 \\
4. Hybrid model&&&&$-$0.80\tikzmark{br4}&0.78 \\
5. Wholesale collusion&&&&&0.55\tikzmark{bottom right 3} \\
\bottomrule
\end{widetable}

\only<1>{\DrawBox[ultra thick, mycolor]{tl1}{br1}}
\only<1>{\DrawBox[ultra thick, mycolor]{tl2}{br2}}
\only<2>{\DrawBox[ultra thick, mycolor]{tl3}{br3}}
\only<3>{\DrawBox[ultra thick, mycolor]{tl4}{br4}}
\only<4>{\DrawBox[ultra thick, red]{top left 2}{bottom right 2}}
\only<4>{\DrawBox[ultra thick, mycolor]{top left 1}{bottom right 1}}
\only<4>{\DrawBox[ultra thick, mycolor]{top left 3}{bottom right 3}}

==> Tables/RV_application_full_talk_new.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{widetable}{.98\columnwidth}{lrrrc}
\toprule
\tikzmark{tl1}\textbf{Panel A: BLP95 IVs}\tikzmark{br1} & \multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}&  MCS p-values \\
\cmidrule(lr){2-5}
1. Zero wholesale margin&\tikzmark{tl6}\tikzmark{tl3}2.25\tikzmark{br6}&$-$12.56&$-$12.35&\tikzmark{top left 8}0.03\tikzmark{bottom right 8}\\
2. Zero retail margin&&$-$7.17&$-$7.14&\tikzmark{top left 1}1.00\tikzmark{bottom right 1}\\
3. Linear pricing&&&0.12&\tikzmark{top left 2}0.00\\
4. Hybrid model&&&\tikzmark{br3}&0.00\tikzmark{bottom right 2}\\
\midrule
\tikzmark{tl2}\textbf{Panel B: Diff IVs} \tikzmark{br2} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& MCS p-values \\
\cmidrule(lr){2-5}
1. Zero wholesale margin&\tikzmark{tl4}0.81&0.34&0.33&\tikzmark{top left 3}0.67 \\
2. Zero retail margin&&0.24&0.23&0.81 \\
3. Linear pricing&&&$-$1.21&1.00 \\
4. Hybrid model&&&\tikzmark{br4}&0.54\tikzmark{bottom right 3} \\
\bottomrule
\end{widetable}

\only<1>{\DrawBox[ultra thick, mycolor]{tl1}{br1}}
\only<1>{\DrawBox[ultra thick, mycolor]{tl2}{br2}}
\only<2>{\DrawBox[ultra thick, mycolor]{tl6}{br6}}


\only<3>{\DrawBox[ultra thick, mycolor]{tl3}{br3}}
\only<4>{\DrawBox[ultra thick, mycolor]{tl4}{br4}}
\only<5>{\DrawBox[ultra thick, red]{top left 2}{bottom right 2}}

\only<5>{\DrawBox[ultra thick, red]{top left 8}{bottom right 8}}
\only<5>{\DrawBox[ultra thick, mycolor]{top left 1}{bottom right 1}}
\only<5>{\DrawBox[ultra thick, mycolor]{top left 3}{bottom right 3}}


==> Tables/RV_demand_log.tex <==
\begin{widetable}{.98\columnwidth}{lrrrrrrc}
\toprule
& \multicolumn{3}{c}{$T^\text{RV}$}& \multicolumn{3}{c}{$F$-statistics}&  MCS $p$-values\\
\cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-8}  
Models & 2 & 3 &  4 & 2 & 3 & 4 & \\ 
\midrule
\\ 
1. Zero wholesale margin&   6.88 & -13.10 & -13.10 &${190.5}$   &  ${252.4}$  &  ${252.6}$ &0.0  \\
2. Zero retail margin&    &   -12.43 &  -12.43   &    &    ${197.6}$ &   ${197.6}$  &     1.0 \\
3. Linear pricing&   &      &  5.28   &      &    &   ${308.8}$     &      0.0\\
4. Hybrid model&&&&&&&0.0\\
% \cmidrule(lr){1-8}
% \multicolumn{8}{l}{\textbf{Demand specification (4)}}  \\ 
% 1. Zero wholesale margin&1.74 & -1.45 &  -1.45& 10.0    &  7.1  &    7.3& 0.082\\
% 2. Zero retail margin&  & -1.853 & -1.862 & &     4.5  &    4.5& 1.0\\
% 3. Linear pricing&  &   &  1.035&   &   &    6.0& 0.123\\
% 4. Hybrid model& & & & & & & 0.126\\
\bottomrule
\end{widetable}

==> Tables/RV_demand_rob.tex <==
\begin{widetable}{.98\columnwidth}{lrrrrrrc}
\toprule
& \multicolumn{3}{c}{$T^\text{RV}$}& \multicolumn{3}{c}{$F$-statistics}&  MCS $p$-values\\
\cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-8}  
Models & 2 & 3 &  4 & 2 & 3 & 4 & \\ 
\midrule
\multicolumn{8}{l}{\textbf{Demand specification (1)}}  \\ 
1. Zero wholesale margin&   6.88 & -13.10 & -13.10 &${190.5}$   &  ${252.4}$  &  ${252.6}$ &0.0  \\
2. Zero retail margin&    &   -12.43 &  -12.43   &    &    ${197.6}$ &   ${197.6}$  &     1.0 \\
3. Linear pricing&   &      &  5.28   &      &    &   ${308.8}$     &      0.0\\
4. Hybrid model&&&&&&&0.0\\
\cmidrule(lr){1-8}
\multicolumn{8}{l}{\textbf{Demand specification (2)}}  \\ 
1. Zero wholesale margin&3.66 & -4.44 & -4.44 &${57.6}$  &   ${24.4}$     & ${24.4}$ & 0.0     \\
2. Zero retail margin&&-4.30 &  -4.30&&  ${19.7}$   &  ${19.8}$ & 1.0 \\
3. Linear pricing&&&1.60&& &  ${48.4}$ & 0.0 \\
4. Hybrid model&&&&& & &  0.0\\
\cmidrule(lr){1-8}
\multicolumn{8}{l}{\textbf{Demand specification (3)}}  \\ 
1. Zero wholesale margin&1.78 & -4.23 &  -4.28& $18.5^\dagger$  &    8.6$^\dagger$  &    8.9$^\dagger$ & 0.08\\
2. Zero retail margin&  & -4.09 & -4.13 & &    9.4$^\dagger$   &   9.9$^\dagger$ & 1.0 \\
3. Linear pricing&  &   &  -0.20&   &   &    15.4$^\dagger $ & 0.0\\
4. Hybrid model& & & & & & &0.0\\
% \cmidrule(lr){1-8}
% \multicolumn{8}{l}{\textbf{Demand specification (4)}}  \\ 
% 1. Zero wholesale margin&1.74 & -1.45 &  -1.45& 10.0    &  7.1  &    7.3& 0.082\\
% 2. Zero retail margin&  & -1.853 & -1.862 & &     4.5  &    4.5& 1.0\\
% 3. Linear pricing&  &   &  1.035&   &   &    6.0& 0.123\\
% 4. Hybrid model& & & & & & & 0.126\\
\bottomrule
\end{widetable}

==> Tables/demand_log.tex <==
\begin{widetable}{.85\columnwidth}{lrr}
\toprule
& \multicolumn{2}{c}{(1) Logit-2SLS}  \\
\cmidrule(lr){2-3} 
& coef. & \multicolumn{1}{c}{s.e.} \\
\midrule
 Prices              &    -6.519    &   (0.209)     \\
 Size                &    0.018     &   (0.001)     \\
 Light               &    0.413     &   (0.014)     \\
 Plain               &    0.423     &   (0.009)      \\
 log(\#Flavors)      &    1.106     &   (0.005)      \\
 \midrule 
Own price elasticity-mean       & \multicolumn{2}{c}{-4.917}  \\
Own price elasticity-median     & \multicolumn{2}{c}{-4.384}  \\
Diversion outside option-mean   &  \multicolumn{2}{c}{0.72}      \\
Diversion outside option-median &  \multicolumn{2}{c}{0.71}      \\
Observations                    & \multicolumn{2}{c}{205123}   \\
\bottomrule
\end{widetable}

==> Tables/demand_rob.tex <==
\begin{widetable}{.98\columnwidth}{lrrrrrrrr}
\toprule
& \multicolumn{2}{c}{(1) Logit-2SLS}  & \multicolumn{2}{c}{(2) BLP}  & \multicolumn{2}{c}{(3) BLP}   \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
& coef. & \multicolumn{1}{c}{s.e.}
& coef. & \multicolumn{1}{c}{s.e.}
& coef. & \multicolumn{1}{c}{s.e.} \\
\midrule
 Prices &    -6.519    &   (0.209)    &  -7.898   &  (0.632)  &  -11.917  &  (0.944)  \\
 Size  &    0.018     &   (0.001)    &  -0.109   &  (0.012)  &  -0.022   &  (0.008)  \\
 Light  &    0.413     &   (0.014)    &  -0.295   &  (0.133)  &   0.320   &  (0.673)  \\
 Plain &    0.423     &   (0.009)    &  -0.681   &  (0.01)   &   0.573   &  (0.059)  \\
 $\log$(\#flavors) &    1.106     &   (0.005)    &           &           &   1.115   &  (0.034)  \\
 Income$\times$price &              &              &   2.294   &  (0.319)  &   0.810   &  (0.664)  \\
 Income$\times$light &              &              &  -0.157   &  (0.106)  &  -0.316   &  (0.187)  \\
 Income$\times$size  &              &              &  -0.015   &  (0.012)  &  -0.006   &  (0.05)   \\
 Age$\times$light    &              &              &  -0.742   &  (0.089)  &  -0.313   &  (0.41)   \\
 Age$\times$size     &              &              &  -0.056   &  (0.007)  &   0.012   &  (0.056)  \\
\midrule 
Own price elasticity-mean       & \multicolumn{2}{c}{-4.917} & \multicolumn{2}{c}{-5.139} & \multicolumn{2}{c}{-8.885} \\
 Own price elasticity-median     & \multicolumn{2}{c}{-4.384} & \multicolumn{2}{c}{-4.967} & \multicolumn{2}{c}{-8.308}  \\
 Diversion outside option-mean   &  \multicolumn{2}{c}{0.72}  &  \multicolumn{2}{c}{0.47}  &  \multicolumn{2}{c}{0.74}    \\
 Diversion outside option-median &  \multicolumn{2}{c}{0.71}  &  \multicolumn{2}{c}{0.46}  &  \multicolumn{2}{c}{0.74}    \\
 Observations                    & \multicolumn{2}{c}{205123} & \multicolumn{2}{c}{205123} & \multicolumn{2}{c}{51628}   \\
\bottomrule
\end{widetable}

==> Tables/old/ARstat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&3407.22, 5324.48&3407.22, 5825.49&3407.22, 5813.52&3407.22, 650.2\\
2.Zero retail margin&&5324.48, 5825.49&5324.48, 5813.52&5324.48, 650.2\\
3.Simple linear pricing&&&5825.49, 5813.52&5825.49, 650.2\\
4.Hybrid model&&&&5813.52, 650.2\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Tables/old/ARstat2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&9.4, 18.11&9.4, 64.1&9.4, 65.74&9.4, 18.94\\
2.Zero retail margin&&18.11, 64.1&18.11, 65.74&18.11, 18.94\\
3.Simple linear pricing&&&64.1, 65.74&64.1, 18.94\\
4.Hybrid model&&&&65.74, 18.94\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Tables/old/CostTable.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lccccccc}
\toprule
& Median& S.D.& Min& q10& q90& Max& \%$<0$ \\
\cline{2-8}Zero wholesale margin&0.4201&0.2312&-0.2602&2.1317&0.2309&0.7728&0.0400\\
Zero retail margin&0.5460&0.2605&0.0856&2.4372&0.3549&0.9569&0.0000\\
Simple linear pricing&0.3050&0.2150&-0.4023&1.9102&0.1241&0.6353&0.8600\\
Hybrid model&0.3102&0.2088&-0.2602&1.9102&0.1460&0.6361&0.5000\\
Wholesale collusion&0.1053&0.2546&-2.1383&1.5322&-0.1956&0.4335&31.6900\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Tables/old/Coxstat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&-1.37, -2.74&1.32, -7.13&1.39, -7.02&2.54, -5.92\\
2.Zero retail margin&&-0.92, -3.31&-0.93, -3.31&-1.42, -5.38\\
3.Simple linear pricing&&&1.05, -1.09&2.38, -4.92\\
4.Hybrid model&&&&2.4, -4.92\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Tables/old/Coxstat2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&-0.43, -1.51&0.8, -4.48&0.84, -4.39&0.88, -2.53\\
2.Zero retail margin&&-0.74, -1.2&-0.74, -1.2&-0.99, -2.28\\
3.Simple linear pricing&&&0.16, -0.18&0.82, -2.09\\
4.Hybrid model&&&&0.83, -2.09\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Tables/old/Dem_robustness.tex <==
%\renewcommand{\arraystretch}{1.0}
\begin{widetable}{.98\columnwidth}{lrrrrc}
\toprule
\textbf{Panel A: Logit demand, BLP95 IVs} & \multicolumn{4}{c}{$F_\rho$}& MCS $p$-values\\
&\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&906.3&427.1&428.3&174.6&0.00\\
2. Zero retail margin&&422.6&422.6&348.5&1.00\\
3. Linear pricing&&&556.8&534.1&0.00\\
4. Hybrid model&&&&534.1&0.00\\
5. Wholesale collusion&&&&&0.00\\
\midrule
\textbf{Panel B: Nested logit demand, BLP95 IVs} & \multicolumn{4}{c}{$F_\rho$}& MCS $p$-values\\
&\multicolumn{1}{c}{2}& \multicolumn{1}{c}{3}& \multicolumn{1}{c}{4}& \multicolumn{1}{c}{5}& \\
\cmidrule(lr){2-6}
1. Zero wholesale margin&&&&& \\
2. Zero retail margin&&&&& \\
3. Linear pricing&&&&& \\
4. Hybrid model&&&&& \\
5. Wholesale collusion&&&&& \\
\bottomrule
\end{widetable}


==> Tables/old/EBstat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&386.32, 1516.42&378.29, 1819&374.15, 1772.99&89.12, 40.51\\
2.Zero retail margin&&707.84, 1960.33&712.64, 1940.86&1018.38, 3455.57\\
3.Simple linear pricing&&&2365.9, 2351.24&2284.54, 24725.95\\
4.Hybrid model&&&&2225.96, 24319.23\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Tables/old/EBstat2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&8.68, 79.02&2.58, 12.77&2.53, 12.31&0.42, 0.06\\
2.Zero retail margin&&6.02, 29.45&6.12, 29.51&34.27, 152.76\\
3.Simple linear pricing&&&40.08, 39.14&20.17, 156.71\\
4.Hybrid model&&&&18.82, 156.14\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Tables/old/Fblp1stat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&3962.3, 739.9&6309, 1042&6173.3, 1043.5&3064.5, 1622.4\\
2.Zero retail margin&&3038.3, 969.4&3070.9, 968.4&3302.8, 1346.3\\
3.Simple linear pricing&&&202, 1305.5&3188.3, 1776.6\\
4.Hybrid model&&&&3169.2, 1779.7\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Tables/old/Fdiff2stat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&3.8, 3.8&14.2, 3.3&13.4, 3.3&1.1, 2.5\\
2.Zero retail margin&&2, 4.1&2, 4&1.3, 3.1\\
3.Simple linear pricing&&&2.9, 3.5&1.3, 2.5\\
4.Hybrid model&&&&1.3, 2.5\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Tables/old/MarkupDescTable.tex <==
\begin{tabular}{lrr}
\hline
       &           IV1 &        Mixed 2 \\
\hline
 count & 205123        & 205123         \\
 mean  &      0.250668 &      0.222563  \\
 std   &      0.084924 &      0.0509135 \\
 min   &      0.057056 &      0.0939126 \\
 25\%   &      0.184493 &      0.184744  \\
 50\%   &      0.247817 &      0.217921  \\
 75\%   &      0.308962 &      0.255025  \\
 max   &      0.87463  &      0.621748  \\
\hline
\end{tabular}


==> Tables/old/MixedFstat.tex <==
\begin{tabular}{llr}
\hline
                & Mixed 1   &   Mixed 2 \\
\hline
 prices         & 1295.4    &     656.3 \\
                & 175.3     &     249.6 \\
 income x price & 1849.8    &    1031.6 \\
                & 250.4     &     371.6 \\
 income x light &           &    6749   \\
                &           &   15784.5 \\
 age x light    &           &     967.6 \\
                &           &    2355.2 \\
 age x size     &           &     849.2 \\
                &           &    1303.1 \\
\hline
\end{tabular}


==> Tables/old/MkupTable.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccccc}
\toprule
& Median& S.D.& Min& q10& q90& Max \\
\cline{2-7}Zero wholesale margin&37.6&10.7&13.6&27.4&53.3&169.9\\
Zero retail margin&19.7&4.3&8.3&14.7&25.7&53.9\\
Simple linear pricing&54.3&13.8&14.1&41.2&74.7&208.0\\
Hybrid model&52.7&13.0&14.1&40.1&71.9&178.2\\
Wholesale collusion&84.4&34.1&20.3&56.2&134.8&674.0\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Tables/old/Model_assessment_all.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}ccccccc}
\toprule
&\multicolumn{3}{c}{Full sample}&\multicolumn{3}{c}{20\% sample}\\
\cline{2-4}\cline{5-7}
Model $j$ & EB &AR &Cox & EB &AR &Cox  \\
2& 113.63, 395.48&	258.84, 654.31&	-1.97, -1.24&	2.15, 5.31&	14.54, 21.49&	-0.67, -0.61\\
3& 357.24, 591.48&	258.84, 221&	1.4, -8.4&	10.52, 22.04&	14.54, 9.57&	0.86, -8.16\\
4& 369.55, 622.69&	258.84, 224.86&	1.45, -8.09&	11.22, 23.79&	14.54, 9.76&	0.88, -7.62\\
5& 6.2, 13.05&	258.84, 218.66&	3.39, -6.26&	0.05, 0.16&	14.54, 32.68&	1.29, -2.54\\
\bottomrule\end{tabular}
\end{footnotesize}


==> Tables/old/PCM.tex <==
\begin{widetable}{.98\columnwidth}{lcccccc}
\toprule
& Mean& Median& S.D.& Min& Max & $\% >100$\\
\midrule
Zero wholesale margin&39.4&37.6&10.7&13.6&169.9&0.04\\
Zero retail margin&20.0&19.7&4.3&8.3&53.9&0\\
Linear pricing&56.6&54.3&13.8&14.1&208.0&0.86\\
Hybrid model&54.8&52.7&13.0&14.1&178.2&0.50\\
Wholesale collusion&91.3&84.4&34.1&20.3&674.0&31.69\\
\bottomrule
\end{widetable}



==> Tables/old/RSS_IJIVE.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lccccc}
\toprule
\textbf{Panel A: RSS} \\
& 2& 3& 4& 5& MCS p-values \\
1.Zero wholesale margin&-0.57&1.19&1.19&-5.37&\\
2.Zero retail margin&&1.02&0.97&-4.39&\\
3.Simple linear pricing&&&-7.04&-3.08&\\
4.Hybrid model&&&&-3.08&\\
5.Wholesale collusion&&&&&\\
\toprule
\textbf{Panel B: RV-IJIVE with BLP instruments} \\
& 2& 3& 4& 5& MCS p-values \\
1.Zero wholesale margin&0.65&-3.45&-3.45&-5.36&0.51\\
2.Zero retail margin&&-3.18&-3.16&-4.24&1\\
3.Simple linear pricing&&&0.17&-4.47&0.04\\
4.Hybrid model&&&&-4.47&0.04\\
5.Wholesale collusion&&&&&0.00\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Tables/old/RSSstat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&-0.57&1.19&1.19&-5.37\\
2.Zero retail margin&&1.02&0.97&-4.39\\
3.Simple linear pricing&&&-7.04&-3.08\\
4.Hybrid model&&&&-3.08\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Tables/old/RV_stat_application.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lccccc}
\toprule
\textbf{Panel A: BLP instruments} \\
& 2& 3& 4& 5& MCS p-values \\
1.Zero wholesale margin&-0.25&-3.29&-3.33&-4.80& 1\\
2.Zero retail margin&&-1.22&-1.22&-3.66&0.81\\
3.Simple linear pricing&&&-1.07&-4.19&0.26\\
4.Hybrid model&&&&-4.19&0.26\\
5.Wholesale collusion&&&&&0.00\\
\toprule
\textbf{Panel B: differentiation instruments} \\
& 2& 3& 4& 5& MCS p-values \\
1.Zero wholesale margin&-1.70&0.10&0.10&-1.38&0.92\\
2.Zero retail margin&&0.56&0.57&-0.39&0.66\\
3.Simple linear pricing&&&0.33&-0.66&0.74\\
4.Hybrid model&&&&-0.67&1\\
5.Wholesale collusion&&&&&0.64\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Tables/old/RV_tab_1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
\textbf{Panel A: No Instruments - RSS}\\
& 2& 3& 4& 5 \\
1.Zero wholesale margin&-0.57&1.19&1.19&-5.37\\
2.Zero retail margin&&1.02&0.97&-4.39\\
3.Simple linear pricing&&&-7.04&-3.08\\
4.Hybrid model&&&&-3.08\\
5.Wholesale collusion&&&&\\
\toprule
\textbf{Panel B: BLP Instruments}\\
& 2& 3& 4& 5 \\
1.Zero wholesale margin&-0.25&-3.29&-3.33&-4.80\\
2.Zero retail margin&&-1.22&-1.22&-3.66\\
3.Simple linear pricing&&&-1.07&-4.19\\
4.Hybrid model&&&&-4.19\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Tables/old/RVstat1.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}\begin{tabular}{@{\extracolsep{4pt}}lcccc}
\toprule
& 2& 3& 4& 5 \\
1.Zero wholesale margin&-0.25&-3.29&-3.33&-4.80\\
2.Zero retail margin&&-1.22&-1.22&-3.66\\
3.Simple linear pricing&&&-1.07&-4.19\\
4.Hybrid model&&&&-4.19\\
5.Wholesale collusion&&&&\\
\bottomrule\end{tabular}
\end{footnotesize}

==> Tables/old/summary_stat.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Mar 12, 2021 - 03:58:35 PM
\begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Max} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Pctl(75)} \\ 
\hline \\[-1.8ex] 
price & 0.759 & 0.295 & 0.676 & 2.690 & 0.186 & 0.549 & 0.911 \\ 
sales & 1,461.252 & 3,199.272 & 503.000 & 104,492.000 & 2.000 & 213.333 & 1,301.000 \\ 
shares & 0.007 & 0.012 & 0.003 & 0.280 & 0.00001 & 0.001 & 0.007 \\ 
outside share & 0.710 & 0.111 & 0.708 & 0.995 & 0.318 & 0.631 & 0.788 \\ 
size & 17.815 & 10.574 & 16 & 32 & 6 & 6 & 32 \\ 
light & 0.925 & 0.263 & 1 & 1 & 0 & 1 & 1 \\ 
number flavors & 5.388 & 5.811 & 3 & 35 & 1 & 1 & 8 \\ 
private label & 0.088 & 0.283 & 0 & 1 & 0 & 0 & 0 \\ 
price reduction & 0.309 & 0.277 & 0.3 & 1 & 0 & 0 & 0.5 \\ 
distance to plant & 493.066 & 476.568 & 392.471 & 2,670.635 & 25.702 & 198.643 & 546.187 \\ 
freight cost & 211.932 & 242.070 & 164.3 & 1,466 & 0 & 51.9 & 270.8 \\ 
\hline \\[-1.8ex] 
\end{tabular} 


==> Tables/old/summary_stat_count.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Mar 12, 2021 - 03:58:36 PM
\begin{tabular}{@{\extracolsep{5pt}} ccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & N & mean & sd & median & max & min \\ 
\hline \\[-1.8ex] 
Obs & $205,123$ & $$ & $$ & $$ & $$ & $$ \\ 
Stores & $1,309$ & $$ & $$ & $$ & $$ & $$ \\ 
Chains & $93$ & $$ & $$ & $$ & $$ & $$ \\ 
Cities & $48$ & $$ & $$ & $$ & $$ & $$ \\ 
Markets & $5,034$ & $$ & $$ & $$ & $$ & $$ \\ 
Firms & $105$ & $$ & $$ & $$ & $$ & $$ \\ 
Brands (per firm) & $171$ & $2$ & $3$ & $1$ & $20$ & $1$ \\ 
Products (per firm) & $530$ & $5$ & $5$ & $4$ & $52$ & $1$ \\ 
PUMs (per market) & $446,969$ & $9,312$ & $7,695$ & $7,224$ & $42,258$ & $1,747$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 


==> Todo_AER.tex <==
* Abstract must be down to 100 words
* Change the title? Testing Firm Conduct: Misspecification, Model Selection, and Weak Instruments
* In abstract, include an Andrews reference?
* Any other reference can be added to IA's work on structural models?
* "General Interest" effort in fist paragraph of intro
* Anything else to be done to intro?
* Appendices - finish putting in text
* Section 7 - clean up the text in case it doesn't match the new numbers 

* put in text references to the appendix tables
* comment on log(Flavors) in text



Testing Firm Conduct with Weak Instruments
Testing Firm Conduct: Weak Instruments and Misspecification
Testing Firm Conduct: Misspecification, Model Selection, and Weak Instruments
Testing Firm Conduct in the presence of Weak Instruments and Misspecification

==> old/Comments_IO_2.tex <==
*Multiple hypotheses (>2) issue

*Simultaneous vs Sequential (Compiani)

*Run RV test for bertrand vs collusion on entire Nielsen data (Dube)

*What if DGP is uniform pricing or perf comp so that in DGP, markups don't vary with instruments? (F Luco)

*Different cost structures, any bearing on instruments? (F. Luco)

*Rotemberg Saloner/Corts came up in talking with Luco, Miller, Weinberg

*Guidance on the instruments
(F. Luco - preempt in paper the weak instrument criticism by saying working on it in ongoing work)

*Guidance on low vs high bias -- can we illustrate in monte carlos how severe demand misspecification must be for the setting to become high bias

*Nate Miller: interesting point that you are saying instruments are model specific (ie think of Corts/RS repeated game, need cross sectional variation)

*Could you use both differentiation and BLP IVs (Matt Weinberg)

*Nate Miller: Practitioners are going to want to know everything they need to know or think about to do testing in our paper.

*F Luco: What if true world is collusion with fringe but you don't have data on the fringe.  What about all the retailer data if don't have all the retailers in the population? is it noise, is it bias, etc. (he wasn't super clear on this himself.  he seemed content with answer that demand and conduct are misspecified)

*Matt Backus: Agrees with the note we sent, thinks we proved prop 3 in chamberlain showing if flexible enough in z then can approximate optimal iv

*Matt Backus: testing many hypotheses somewhat trivial (see Backus and Peng 2019 for lit review of nested papers)

*Matt Backus: might want to look at empirical likilihood or at least if the full conditional moments offer more power in this seting

*Matt Backus: He had this thought when I was talking about my JMP and discussing RV testing in product stage.  Can you generalize things to come up with conditions which must hold for arbitrary game that makes testing non-nested models work 


==> old/Extensions.tex <==
* Nonparametric iv
* Nonparametric markups
* Sets of models (ie sign restrictions on parameters)
* Testing models of cost - sign restriction test likely 

==> old/Q_A.tex <==
* What about the assumption that we observe the plim of markups? Would results go through with estimated markups
A : plims would (standard 2 step GMM intuition of consistency applies); we have strong sense that distributional resutsl e.g. local alt power analysis would also go through, haven't proved it yet.

* You are assuming identification of conduct, as opposed to only testability in Berry and Haile? 
A: In assumption 3, we maintain that the two models of conduct we consider are testable in the sense of rejecting the wrong one - for that, only 1 instrument is necessary. However, 1 instrument is not enough for identification of theta. In assumption 4a we maintain that theta is identified (there are 2+ instruments) so we can run EB. 


*With local alternatives, how are you able to get wald statistic distributed chi2 - in the weak instrument literature, $\theta_{2sls}$ is non-normal
A: We are making a stronger assumption than the weak instruments literature, though one that also implies the instruments are weak.  This allows us to not only control the rate of the first stage parameter but also the rate of the cov of z and e.  Why do something stronger?  First, we arrive at the same distribution as would obtain with the weaker asymptotics if rho is large and number of instruments is fixed (Staiger and Stock (1997)).  Second, in the spirit of the literature on non-nested hypotheses, we need to perform local alternatives that allow the two models to become asymptotically close.  This can not be achieved via a local alternative on theta.  Thus, we need to put the local alternative on a moment of the data.  This is consistent with Marmer and Otsu, Smith, etc.  Even in the weak instruments literature, other asymptotics can be used which change the limiting distribution (see Xiaoxia's Weak Instruments Note, FN 1) 


*What about the menu approach?  How does it fit in?

A: Understand it as instead of identifying, posit different models and check if plausible - a testing approach consistent with us.  Differences, the rationale there has to do with lack of identification...
% 


==> old/Tables/LogitCoef.tex <==
\begin{tabular}{lcccc}
\hline
              &  Logit-OLS   &   Logit-2SLS    & ML1 & ML2  \\
              &(1) & (2) & (3) & (4)\\
\hline
 prices       &  -1.75  & -6.519   &  -11.119  &  -10.197  \\
              & (0.019) & (0.209)  &  (0.671)  &  (0.569)  \\
 size         &  0.037  &  0.018   &   0.013   &  -0.053   \\
              &  (0.0)  & (0.001)&  (0.001)  &  (0.013)  \\
 light        &  0.259  &  0.413    &   0.442   &  -0.275   \\
              & (0.01)  & (0.014)  &  (0.016)  &  (0.14)   \\
 flavor\_Plain &  0.508  &  0.423  &   0.41    &   0.452   \\
              & (0.007) & (0.009)  &  (0.011)  &  (0.011)  \\
 log\_nflavors &  1.127  &  1.106    &   1.115   &   1.137   \\
              & (0.004) & (0.005)  &  (0.006)  &  (0.007)  \\
  income x price &&&   3.885   &   3.525   \\
                &&&  (0.338)  &  (0.286)  \\
 income x light &&&           &   0.167   \\
                &&&          &  (0.061)  \\
 age x light    &&&           &  -0.562   \\
                &&&           &  (0.102)  \\
 age x size     &&&           &  -0.063   \\
                &&&           &  (0.008)  \\             
\hline              
 Elast mean   &  -1.32  & -4.917   &  -5.715   &   -5.62   \\
 Elast median & -1.177  & -4.384    &  -5.585   &  -5.527   \\
 J stat       & 2.0e-23 & 1.9e-21 &  3.9e+00  &  1.3e-01  \\
\hline
\end{tabular}



==> old/Tables/MarkupDescTable.tex <==
\begin{tabular}{lrr}
\hline
       &           IV1 &        Mixed 2 \\
\hline
 count & 205123        & 205123         \\
 mean  &      0.250668 &      0.222563  \\
 std   &      0.084924 &      0.0509135 \\
 min   &      0.057056 &      0.0939126 \\
 25\%   &      0.184493 &      0.184744  \\
 50\%   &      0.247817 &      0.217921  \\
 75\%   &      0.308962 &      0.255025  \\
 max   &      0.87463  &      0.621748  \\
\hline
\end{tabular}


==> old/Tables/MixedCoef.tex <==
\begin{tabular}{lcc}
\hline
                &  Mixed 1  &  Mixed 2  \\
\hline
 prices         &  -11.119  &  -10.197  \\
                &  (0.671)  &  (0.569)  \\
 size           &   0.013   &  -0.053   \\
                &  (0.001)  &  (0.013)  \\
 light          &   0.442   &  -0.275   \\
                &  (0.016)  &  (0.14)   \\
 flavor\_Plain   &   0.41    &   0.452   \\
                &  (0.011)  &  (0.011)  \\
 log\_nflavors   &   1.115   &   1.137   \\
                &  (0.006)  &  (0.007)  \\
 income x price &   3.885   &   3.525   \\
                &  (0.338)  &  (0.286)  \\
 income x light &           &   0.167   \\
                &           &  (0.061)  \\
 age x light    &           &  -0.562   \\
                &           &  (0.102)  \\
 age x size     &           &  -0.063   \\
                &           &  (0.008)  \\
 Elast mean     &  -5.715   &   -5.62   \\
 Elast median   &  -5.585   &  -5.527   \\
 J stat         &  3.9e+00  &  1.3e-01  \\
\hline
\end{tabular}


==> old/Tables/MixedFstat.tex <==
\begin{tabular}{llr}
\hline
                & Mixed 1   &   Mixed 2 \\
\hline
 prices         & 1295.4    &     656.3 \\
                & 175.3     &     249.6 \\
 income x price & 1849.8    &    1031.6 \\
                & 250.4     &     371.6 \\
 income x light &           &    6749   \\
                &           &   15784.5 \\
 age x light    &           &     967.6 \\
                &           &    2355.2 \\
 age x size     &           &     849.2 \\
                &           &    1303.1 \\
\hline
\end{tabular}


==> old/Tables/summary_stat.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Mar 12, 2021 - 03:58:35 PM
\begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Max} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Pctl(75)} \\ 
\hline \\[-1.8ex] 
price & 0.759 & 0.295 & 0.676 & 2.690 & 0.186 & 0.549 & 0.911 \\ 
sales & 1,461.252 & 3,199.272 & 503.000 & 104,492.000 & 2.000 & 213.333 & 1,301.000 \\ 
shares & 0.007 & 0.012 & 0.003 & 0.280 & 0.00001 & 0.001 & 0.007 \\ 
outside share & 0.710 & 0.111 & 0.708 & 0.995 & 0.318 & 0.631 & 0.788 \\ 
size & 17.815 & 10.574 & 16 & 32 & 6 & 6 & 32 \\ 
light & 0.925 & 0.263 & 1 & 1 & 0 & 1 & 1 \\ 
number flavors & 5.388 & 5.811 & 3 & 35 & 1 & 1 & 8 \\ 
%private label & 0.088 & 0.283 & 0 & 1 & 0 & 0 & 0 \\ 
%price reduction & 0.309 & 0.277 & 0.3 & 1 & 0 & 0 & 0.5 \\ 
distance to plant & 493.066 & 476.568 & 392.471 & 2,670.635 & 25.702 & 198.643 & 546.187 \\ 
freight cost & 211.932 & 242.070 & 164.3 & 1,466 & 0 & 51.9 & 270.8 \\ 
\hline \\[-1.8ex] 
\end{tabular} 


==> old/Tables/summary_stat_count.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Mar 12, 2021 - 03:58:36 PM
\begin{tabular}{@{\extracolsep{5pt}} ccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & N & mean & sd & median & max & min \\ 
\hline \\[-1.8ex] 
Obs & $205,123$ & $$ & $$ & $$ & $$ & $$ \\ 
Stores & $1,309$ & $$ & $$ & $$ & $$ & $$ \\ 
Chains & $93$ & $$ & $$ & $$ & $$ & $$ \\ 
Cities & $48$ & $$ & $$ & $$ & $$ & $$ \\ 
Markets & $5,034$ & $$ & $$ & $$ & $$ & $$ \\ 
Firms & $105$ & $$ & $$ & $$ & $$ & $$ \\ 
Brands (per firm) & $171$ & $2$ & $3$ & $1$ & $20$ & $1$ \\ 
Products (per firm) & $530$ & $5$ & $5$ & $4$ & $52$ & $1$ \\ 
PUMs (per market) & $446,969$ & $9,312$ & $7,695$ & $7,224$ & $42,258$ & $1,747$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 


==> old/TablesGraphs.tex <==

\subsection{The Rivers\&Vuong test in a Bertrand x Monopoly framework}

In this first set of results we show how the RV test using RSS as criterium can suffer from bias when testing for Bertrand vs Collusion conduct. Row (1) in table 1 show that the RV-RSS test can pin-down the correct data generating process in the baseline scenario . If we shut-down the random coefficients, and run a model with logit demand instead, then there is not enough variation in margins that allows the test to indentify conduct, as can be seen in row (2). Now, if we perform the test in a setting with only heterogeneity in taste for prices, as in row (3), then we can create a bias for the RV-RSS test towards the Collusion assumption. This bias can be amplified with both a larger $\sigma^2_\omega)$ and larger $\sigma_{\xi,\omega}$, as in row (4) and (5). We can see that the random coefficient in prices is key to create this bias, since $\sigma^2_\omega)$ and $\sigma_{\xi,\omega}$ alone does not break the test, row (6). Heterogeneity in taste for the characteristic does not have the same effect, row (7). Finally, if we increase the average taste parameter ($\beta_0$), then the margins generated by Bertrand and Collusion process set apart, and the test has no problem in identifying conduct, row (8). Note that the number of times the RV using the GMM criterium function indicate the wrong model is below the confidence level of the test, being evidence that it does not suffer from the same bias as the RV-RSS.

\begin{table}[b]\centering\caption{RV Test - Bertrand x Collusion - DGP Bertrand}
\input{Output/TabRV_BM_B.tex}
\end{table}

In table 2 we perform the same exercise as before but for a Collusion data generating process. In row (3),(4) and (5), the low number of samples where we can not reject the null using the RV-RSS test reinforce the bias result toward the monopoly case when heterogeneity in price is high.

\begin{table}[b]\centering\caption{RV Test - Bertrand x Collusion - DGP Collusion}
\input{Output/TabRV_BM_M.tex}
\end{table}

%\includegraphics[scale=0.5]{Output/histMarginsBM_1}
%\includegraphics[scale=0.5]{Output/histMarginsBM_2}

\begin{figure}[b]\centering\caption{}
\includegraphics[scale=0.8]{Output/figure1}
\end{figure}


\subsection{The Rivers\&Vuong test in a BertrandxCournot framework}

In a Bertrand vs Cournot exercise, table 3 and 4 shows that the bias can go both ways. For row (2) and (3), a logit demand setting, the bias is toward the Bertrand result. For row (4) and (5) the bias is toward Cournot. Although the RV-GMM test can not pin-down the correct model because of the similarity between margins, it does not suffer from the bias problem.

\begin{table}[b]\centering\caption{RV Test - Bertrand x Cournot - DGP Bertrand}
\input{Output/TabRV_BC_B.tex}
\end{table}

\begin{table}[b]\centering \caption{ RV Test - Bertrand x Cournot - DGP Cournot}
\input{Output/TabRV_BC_C.tex}
\end{table}

\subsection{Test Comparison}

Table 5 from the test comparison show how all the tests have a reasonably good performance in the baseline. Table 6 evaluate the instrument-based-tests in the same scenario where the RV-SSR test suffer from bias. It seems that none of them have the same bias problem.

\begin{figure}\caption{Comparing power - RV-GMM x RV-GMM adj}\centering
\includegraphics[scale=0.5]{Output/CompStat2.png}
\end{figure}


\begin{table}[b]\centering\caption{Test Comparison - Baseline}
\input{Output/Tab_Comp_1_CTLR.tex}
\end{table}

\begin{table}[b]\centering\caption{Test Comparison - $\sigma_p=0.17,\sigma_x=0,\sigma^2_\omega=0.3,\sigma_{\xi\omega}=0$}
\input{Output/Tab_Comp_2_CTLR.tex}
\end{table}

\subsubsection{Comparing tests while estimating demand}
For the next results we add noise to the conduct test from a demand estimation stage. We perform the demand estimation using the pyblp software.

\begin{itemize}
\item \textbf{Choice of instrument}: In table 7, 8 and 9 we compare the performance of BLP and Diff as instrument for both demand and conduct test. There is no significant difference between the instruments. Note that, for all the tests, the noise from the demand estimation made the number of wrong results to increase for the Collusion data generating process.

\begin{table}[b]\centering\caption{Choice of instrument - Demand Instr.:BLP,  Test Instr.: BLP}
\input{Output/Tab_Comp_3_CTLR.tex}
\end{table}
\begin{table}[b]\centering\caption{Choice of instrument - Demand Instr.:Diff,  Test Instr.: BLP}
\input{Output/Tab_Comp_4_CTLR.tex}
\end{table}
\begin{table}[b]\centering\caption{Choice of instrument - Demand Instr.:Diff,  Test Instr.: Diff}
\input{Output/Tab_Comp_5_CTLR.tex}
\end{table}

\item  \textbf{Weak instrument problem}: Using table 10, 11 and 12 we investigate how the tests perform under weak instrument. To do so, we generate and add noise to the original instruments based on a normal distribution with mean zero and variance that takes into account the variables level. Comparing table 8 and 10 we can see that a weak test instrument can have an effect on the power from all the tests. Comparing table 8 and 11, it seems that weak demand instruments does not impact power that much. 

\begin{table}[b]\centering\caption{Weak instrument - Demand Instr.:Diff,  Test Instr.: weakBLP}
\input{Output/Tab_Comp_6_CTLR.tex}
\end{table}
\begin{table}[b]\centering\caption{Weak instrument - Demand Instr.:weakDiff,  Test Instr.: BLP}
\input{Output/Tab_Comp_7_CTLR.tex}
\end{table}
\begin{table}[b]\centering\caption{Weak instrument - Demand Instr.:weakDiff,  Test Instr.: weakBLP}
\input{Output/Tab_Comp_8_CTLR.tex}
\end{table}

\item  \textbf{Demand misspecified} We evaluate the tests under misspecified demand. For table 13 we wrongly estimate demand assuming a logit setting. For table 14 and 15 we estimate demand with only one type of heterogeneity in taste, either price or characteristic. Comparing with table 8, we can see that misspeficied demand can have a significant impact in power and size. It is not clear which test is more affected by demand misspecification.

\begin{table}[b]\centering\caption{Demand misspecified - $\hat\sigma_p=0, \hat\sigma_x=0$ }
\input{Output/Tab_Comp_9_CTLR.tex}
\end{table}
\begin{table}[b]\centering\caption{Demand misspecified - $\hat\sigma_p=0$}
\input{Output/Tab_Comp_10_CTLR.tex}
\end{table}
\begin{table}[b]\centering\caption{Demand misspecified - $\hat\sigma_x=0$}
\input{Output/Tab_Comp_11_CTLR.tex}
\end{table}

\item \textbf{Supply misspecified} We perform a similar exercise for supply misspecification. Comparing table 16 and 17 to table 8, it seems that supply misspecifications do not have a significant impact on any test.

\begin{table}[b]\centering\caption{Supply misspecified - $\hat\psi_1=0$}
\input{Output/Tab_Comp_12_CTLR.tex}
\end{table}
\begin{table}[b]\centering\caption{Supply misspecified - $\hat\psi_2=0$}
\input{Output/Tab_Comp_13_CTLR.tex}
\end{table}

\end{itemize}

==> old/ToDoList_0523.tex <==
1. In Fig 4, does everything work with the average (instead of the median)? Average seems more natural finite sample equiv of the plim we have in the definition of B_EB
2. Two step correction for AR
3. 


*****************************************

* Simultaneous notes:
* Doing seq testing using misspecified demand and well specified (under one hypothesis) supply will do better than doing sequential
* Conversely we conjecture that doing simultaneous testing under well specified demand and misspecified supply could do worse than sequential
* These points can be made somewhat formally under the assumption of diagonal weights, will hold more generally unless weights/moments strongly undo the basic forces
* The strenght of the instruments determines relative importance of supply & demand moments in pinning down parameters; in turn, standard instruments (BLP, diff) may have stronger correlation with demand or with supply depending on how they correlate with cost shifters
* We need to find a way of misspecifying costs that make sense. Cost changing over time? Functional form is correct, params changing over time

==> old/TodoList_10_14.tex <==
* check TEs
* Quote from Hal White on misspecification? to be brought in either in intro or elsewhere
* What about approximations of variance under misspecification (Marco's comment?)
* And, are things well defined under misspecification?
* Change order of tests in proofs?
* Homoskedasticity: "convenient, makes our results look prettier, but main intuition still goes through"
* Figure 5 - can we do it with changing $\sigma_{\omega_0}?$
* Figure 5 - have panel labels
* What about considering the case of estimated markups in our proofs? [linked to two-step estimation literature in GMM/check Newey&McFadden chapter]
* Our TE2 is about Markup Misspecification or demand misspecification? Think also about simplicity of presenting.

* A few things on the structure of the paper:
1. Should the material in 4.0 be consolidate in an expanded Section 3, where we cover "foundations of testing", separate from testing procedures?
2. We now in Def 1 define how to falsify, and in Lemma 1 provide an alternative condition for a false model to be falsified. Should we instead have falsification as an assumption the the wrong model is falsified?

*The conditions in section 4.  Should everything including statements that statistics take on simple distributions under the null be more explicitely under TE1?  Should all falsifiability stuff be with $\Delta^*$'s?

* How to better discuss the practical steps/best practices? Some more formalities on what happens to $\theta_{2SLS}$ when there is misspecification?

* New: Should there be more emphasis on the point that the plim of the GMM objective function equals the expected squared difference in predicted markups? A Lemma before Proposition 1? A corollary?

==> old/TodoList_1_24.tex <==
Document for BCS

Things to do in the paper:
1. Expand on weight matrix, discuss how it can produce degeneracy in a larger area; gamma space graph
2. Replace bias and noise schematics
3. Take out Proposition 2
4. Fix Proposition 4 (almost done, do the proof for the modified assumption/hypothesis)
6. As running/leading example - Corts? for sure in discussion of invalidating the instruments!
5. Review exposition of: MCS/multiple hypotheses, degeneracy - put in graphs? 

==> old/mail_to_BCS.tex <==
Hi Matt,

Thanks so much for your email. We really like where you are going with the paper: it is shaping up to be a great article. We are also glad to see that you are using RV.  We had a couple of thoughts after reading your draft, especially on the issue of the formulation of the RV statistic. 


We tried to better understand the differences between the moments that you use and the reduced form moments that we consider. In the attached note, we try to highlight and show the following points:  

    1.  In our paper, we don't take a stand on the components of w - the observed cost shifters and z - the excluded instruments, although this is clearly an important issue in practice. Among other things, reading your paper made us appreciate even more the importance of choosing instruments, and possibly specifiying them in a flexible way. For example, one could define the matrices w and z in our paper to be consistent with sieve estimation of the first stage, or include lots of high-order terms and interactions to make the first stage very flexible in w and z. We believe it is an important contribution of your paper that you develop a procedure that generates instruments which (i) correspond nicely to the intuition underlying the testability of the two models, and (ii) have presumably good power. 

    2.  In fact, the criterion function you write down for each model can be written as a GMM objective function for the reduced form moments, and a specific choice of weight matrix, as long as the instruments are specified flexibly. Further, we think we can show that the Rivers and Vuong test statistic written with your criterion function is identical to the general form of the Rivers and Vuong test statistic we write down in the paper - if one would construct instruments as in your first stage. This makes sense to us, since ultimately we are all relying on the testability condition in Berry and Haile (2014).

It's entirely possible we are missing something here or made a mistake, so please let us know if you disagree with our note. 

We also amended how we cite you in our draft, and hope it better reflects the current status of your work. Please let us know if you feel we should change it in some way. 

We are thankful for your suggestions on your draft. You touch upon a number of important issues, where we hope to have something to say in future versions of our draft. 

